An Efficient Approach to Achieve Compositionality using Optimized Multi-Version Object Based Transactional Systems

In the modern era of multi-core systems, the main aim is to utilize the cores properly. This utilization can be done by concurrent programming. But developing a flawless and well-organized concurrent program is difficult. Software Transactional Memory Systems (STMs) are a convenient programming interface which assist the programmer to access the shared memory concurrently without worrying about consistency issues such as priority-inversion, deadlock, livelock, etc. Another important feature that STMs facilitate is compositionality of concurrent programs with great ease. It composes different concurrent operations in a single atomic unit by encapsulating them in a transaction. Many STMs available in the literature execute read/write primitive operations on memory buffers. We represent them as Read-Write STMs or RWSTMs. Whereas, there exist some STMs (transactional boosting and its variants) which work on higher level operations such as insert, delete, lookup, etc. on a hash-table. We refer these STMs as Object Based STMs or OSTMs. The literature of databases and RWSTMs say that maintaining multiple versions ensures greater concurrency. This motivates us to maintain multiple version at higher level with object semantics and achieves greater concurrency. So, this paper pro-poses the notion of Optimized Multi-version Object Based STMs or OPT-MVOSTMs which encapsulates the idea of multiple versions in OSTMs to harness the greater concurrency efficiently.

==> Submitted MVOSTM Journal-2019/citations <==
%%% ====================================================================
%%%  BibTeX-file{
%%%     author          = "Sathya Peri",
%%%     date            = "17 Spet 2009",
%%%     filename        = "citations.bib",
%%%     url             = ""
%%%     www-home        = "http://www.cs.mun.ca/~sathya/",
%%%     address         = "Department of Computer Science,
%%%                        MUN,
%%%                        St John's, CA A1B 3X5,
%%%                        Canada",
%%%     email           = "sathya at mun.ca",
%%%     dates           = {1950--},
%%%     keywords        = "",
%%%     supported       = "yes",
%%%     supported-by    = "Sathya Peri",
%%%     abstract        = "Bibliography for Sathya Peri"
%%%  }
%%% ====================================================================


@String{PROC = {Proceedings of the}}
@String{AMS = {American Mathematical Society}}
@String{AW = {Addison-Wesley}}
@String{TCS = {Theoretical Computer Science}}
@String{JPDC = {Journal of Parallel and Distributed Computing (JPDC)}}
@String{WDAG = {Workshop on Distributed Algorithms (WDAG)}}
@String{WPDD = {ACM/ONR Workshop on Parallel and Distributed Debugging}}
@String{DC = {Distributed Computing (DC)}}
@String{TrCS = {ACM Transactions on Computer Systems}}
@String{SPDP = {IEEE Symposium on Parallel and Distributed Processing (SPDP)}}
@String{ICPP = {International Conference on Parallel Processing}}
@String{Com = {IEEE Computer}}
@String{KAP = {Kluwer Academic Publishers}}
@String{WAD = {International Workshop on Automated Debugging (AADEBUG)}}
@String{CSS = {International Conference on System Sciences}}
@String{Fre = {W. H. Freeman and Company, New York}}
@String{TPDS = {IEEE Transactions on Parallel and Distributed Systems (TPDS)}}
@String{FTCS = {IEEE Fault-Tolerant Computing Symposium (FTCS)}}
@String{JCC = {Journal of Computer Communications}}
@String{WSCT = {International Workshop on Structures in Concurrency Theory (STRICT)}}
@String{MH = {McGraw-Hill}}
@String{CACM = {Communications of the ACM (CACM)}}
@String{ICDCS = {IEEE International Conference on Distributed Computing Systems (ICDCS)}}
@String{PODC = {ACM Symposium on Principles of Distributed Computing (PODC)}}
@String{JS = {Journal of Supercomputing}}
@String{CAV = {International Conference on Computer-Aided Verification (CAV)}}
@String{LNCS = {Lecture Notes in Computer Science (LNCS)}}
@String{WPDS = {Workshop on Parallel and Distributed Simulation}}
@String{DISC = {Symposium on Distributed Computing (DISC)}}
@String{CSE = {Computer Science and Education}}
@String{TMH = {Tata McGraw-Hill Publishing Company Limited}}
@String{ES = {Elsevier Science Publishers B. V. (North-Holland)}}
@String{PDS = {The Parallel and Distributed Systems Laboratory}}
@String{DECE = {Department of Electrical and Computer Engineering}}
@String{DCS = {Department of Computer Science}}
@String{PPL = {Parallel Programming Laboratory}}
@String{UIUC = {University of Illinois at Urbana-Champaign}}
@String{UTA = {The University of Texas at Austin}}
@String{OSU = {The Ohio State University}}
@String{UTD = {The University of Texas at Dallas}}
@String{TC = {IEEE Transactions on Computers}}
@String{IPL = {Information Processing Letters (IPL)}}
@String{AMCSJ = {Applied Mathematics and Computer Science Journal}}
@String{WLCPC = {Workshop on Language and Compilers for Parallel Computing}}
@String{IBMARC = {IBM Almaden Research Center}}
@String{IBMZ = {IBM Research Laboratory, Zurich}}
@String{ICDE = {International Conference on Data Engineering (ICDE)}}
@String{CUP = {Cambridge University Press}}
@String{MVPP = {International Meeting on Vector and Parallel Processing}}
@String{TOPLAS = {ACM Transactions on Programming Languages and Systems (TOPLAS)}}
@String{SPDT = {Symposium on Parallel and Distributed Tools}}
@String{CJ = {The Computer Journal}}
@String{PH = {Prentice Hall}}
@String{MK = {Morgan Kaufmann}}
@String{SIGMOD = {ACM SIGMOD International Conference on Managament of Data}}
@String{SIGACT = {ACM Special Interest Group on Algorithms and Computation Theory (SIGACT)}}
@String{USPATENT = {United States Patent Number}}
@String{INFORMIX = {Informix Software Incorporated}}
@String{SV = {Springer-Verlag}}
@String{PDCS = {ISCA International Conference on Parallel and Distributed Computing Systems (PDCS)}}
@String{MIT = {The MIT Press}}
@String{JHUP = {The Johns Hopkins University Press}}
@String{DAM = {Discrete Applied Mathematics}}
@String{DM = {Discrete Mathematics}}
@String{DS = {Distributed Systems}}
@String{ICSKE = {IEEE International Conference on Software and Knowledge Engineering}}
@String{FSTTCS = {Conference on the Foundations of Software Technology and Theoretical
                  Computer Science (FSTTCS)}}
@String{TSE = {IEEE Transactions on Software Engineering}}
@String{JSS = {The Journal of Systems and Software}}
@String{WGCS = {International Workshop on Graph-Theoretic Concepts in Computer Science (WG)}}
@String{JWS = {John Wiley and Sons Limited}}
@String{JWSUS = {John Wiley and Sons, Incorporated}}
@String{ORDAL = {International Conference on Orders, Algorithms and Applications (ORDAL)}}
@String{AJM = {American Journal of Mathematics}}
@String{SRKU = {Sci. Reports Kanazawa Univ.}}
@String{SIAMJDM = {SIAM Journal on Discrete Mathematics}}
@String{KRUSE = {International KRUSE Symposium: Knowledge Use, Retrieval and Storage for Efficiency}}
@String{SIAMJADM = {SIAM Journal on Algebraic and Discrete Methods}}
@String{SIAMJC = {SIAM Journal on Computing}}
@String{MCT = {Mathematical Center Tracts}}
@String{STOC = {Annual ACM Symposium on Theory of Computing (STOC)}}
@String{OOPSLA = {Conference on Object-Oriented Programming, Systems, Languages, and Applications (OOPSLA)}}
@String{JLMS = {Journal London Mathematics Society}}
@String{AM = {Annals of Mathematics}}
@String{TIT = {IEEE Transactions on Information Theory}}
@String{TR = {IEEE Transactions on Reliability}}
@String{WLP = {Workshop on Logics of Programs}}
@String{ISP = {International Symposium in Programming}}
@String{WSS = {Workshop on Self-Stabilizing Systems (WSS)}}
@String{ICALP = {International Colloquium on Automata, Languages and Systems (ICALP)}}
@String{JA = {Journal of Algorithms}}
@String{KDE = {IEEE Transactions on Knowledge and Data Engineering}}
@String{CS = {ACM Computing Surveys (CSUR)}}
@String{IPDPS = {International Parallel and Distributed Processing Symposium (IPDPS)}}
@String{PDC = {Parallel and Distributed Conference}}
@String{SP = {IEEE Symposium on Security and Privacy}}
@String{USS = {USENIX Security Symposium}}
@String{WNTS = {USENIX Windows NT Symposium}}
@String{UCS = {Computing Systems}}
@String{NCSC = {National Computer Security Conference}}
@String{RV = {Workshop on Runtime Verification (RV)}}
@String{ICPDCS = {IASTED International Conference on Parallel and Distributed Computing and Systems}}
@String{MCDS = {SCS MultiConference on Distributed Simulation}}
@String{SCS = {Society for Computer Simulation}}
@String{BCPC = {The Benjamin Cummings Publishing Company, Incorporated}}
@String{OPODIS = {International Conference on Principles of Distributed Systems (OPODIS)}}
@String{TWSIS = {Texas Workshop on Security of Information Systems (TWSIS)}}
@String{SCISS = {South Central Information Security Symposium (SCISS)}}
@String{CSS = {Computing Systems}}
@String{UCD = {University of California, Davis}}
@String{CSAC = {Annual Computer Security Applications Conference}}
@String{WETICE = {IEEE Workshop on Enabling Technologies: Infrastructure for Collaborative
                  Enterprises (WETICE)}}
@String{TOG = {ACM Transactions on Graphics}}
@String{SCCS = {School of Computer and Communication Sciences}}
@String{EPFL = {{\'E}cole Polytechnique F{\'e}d{\'e}rale de Laussane (EPFL)}}
@String{CORNELL = {Cornell University}}
@String{COMPSAC = {Annual Internation Computer Software and Applications Conference (COMPSAC)}}
@String{JPL = {Journal of Programming Languages}}
@String{PC = {Parallel Computing}}
@String{UWM = {University of Wisconsin, Madison}}
@String{UWTC = {USENIX Winter Technical Conference}}
@String{ICSSE = {Israeli Conference on Computer Systems and Software Engineering}}
@String{IPPS = {International Parallel and Processing Symposium (IPPS)}}
@String{HIS = {Journal of High Integrity Systems}}
@String{HPL = {Hewlett Packard Laboratories}}
@String{ACTA = {Acta Informatica}}
@String{FOCS = {Annual Symposium on Foundations of Computer Science (FOCS)}}
@String{CDS = {IEEE Proceedings---Computers and Digital Techniques}}
@String{JISE = {Journal of Information Science and Engineering}}
@String{ICPADS = {International Conference on Parallel and Distributed Systems (ICPADS)}}
@String{WPPS = {International Workshop on Peer-to-Peer Systems}}
@String{SAC = {IEEE Journal on Selected Areas in Communications}}
@String{TN = {IEEE/ACM Transactions on Networking}}
@String{SNA = {ACM-SIAM Symposium on Discrete Algorithms}}
@String{SIU = {Studia Informatica Universalis}}


@Unpublished{8LGM:1992,
  author =   {8LGM},
  title =    {{[8lgm]-Advisory-5.UNIX.mail.24-Jan-1992}},
  note =     {Available from \texttt{fileserv@bagpuss.demon.co.uk} (January 1992)}
}

@Article{AchBad:1992:IPL,
  author =   {A. Acharya and B. R. Badrinath},
  title =    {{Recording Distributed Snapshots Based on Causal
                   Order of Message Delivery}},
  journal =  IPL,
  volume =   {44},
  number =   {6},
  pages =    {317-321},
  year =     {1992},
  OPTurl =   {http://citeseer.nj.nec.com/acharya92recording.html}
}

@Misc{Adv:1990:SM,
  title =    {{Sendmail Vulnerability}},
  howpublished = {CERT Advisory CA-90:01 available from \textsf{cert.org} via anonymous ftp},
  month =    JAN,
  year =     {1990}
}

@Article{Adv:1992:Mail,
  author =   {8LGM},
  title =    {{[8lgm]-Advisory-5.UNIX.mail.24-Jan-1992}},
  note =     {Available from \texttt{fileserv@bagpuss.demon.co.uk}},
  month =    JAN,
  year =     1992
}

@Article{Adv:1994:Pwd,
  author =   {8LGM},
  title =    {{[8lgm]-Advisory-7.UNIX.passwd.11-May-1994}},
  note =     {Available from \texttt{fileserv@bagpuss.demon.co.uk}},
  month =    MAY,
  year =     1994
}

@Article{AfeBre:1998:TCS,
  author =   {Y. Afek and A. Bremler},
  title =    {{Self-Stabilizing Unidirectional Network Algorithms by Power Supply}},
  journal =      TCS,
  year =     1998,
  volume =   1998,
  number =   3,
  month =    DEC
}

@InProceedings{AfeKut+:1991:WDAG,
  author =       {Y. Afek and S. Kutten and M. Yung},
  title =        {{Memory-Efficient Self-Stabilizing Protocols for General Networks}},
  booktitle =    PROC # " 4th " # WDAG,
  year =         {1991},
  pages =        {15-28},
  address =      {Bari, Italy},
  publisher =    SV,
}

@Manual{AgaGoe+:1996:IBM,
  author =   {A. Agarwal and A. Goel and A. Sood},
  title =    {{Software Design Description for DLFS on Solaris,
                  HP-UX, and AIX}},
  year =     {1996}
}

@InProceedings{AgrBor+:1989:MD,
  author =   {R. Agrawal and A. Borgida and H. V. Jagadish},
  title =    {{Efficient Management of Transitive Relationships in
                  Large Data and Knowledge Bases}},
  booktitle =    PROC # " " # SIGMOD,
  pages =    {253-262},
  year =     1989,
  address =  {Portland, Oregon}
}

@Book{AhoHop:1974:AW,
  author =   {A. V. Aho and J. E. Hopcroft and J. D. Ullman},
  OPTeditor =    {~},
  title =    {{The Design and Analysis of Computer Algorithms}},
  publisher =    AW,
  year =     1974,
  OPTnote =  {pages 384-386}
}

@InProceedings{AlaVen:1993:WAD,
  author =   {S. Alagar and S. Venkatesan},
  title =    {{Hierarchy in Testing Distributed Programs}},
  booktitle =    PROC # " " # WAD,
  pages =    {101-116},
  year =     {1993}
}

@Article{AlaVen:1994:IPL,
  author =   {S. Alagar and S. Venkatesan},
  title =    {{An Optimal Algorithm for Recording Snapshots using Casual
                   Message Delivery}},
  journal =  IPL,
  year =     {1994},
  OPTkey =   {},
  volume =   {50},
  OPTnumber =    {},
  pages =    {311-316},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@InProceedings{AlaVen:1994:PDS,
  author =   {S. Alagar and S. Venkatesan},
  title =    {{Techniques to Tackle State Explosion in Global Predicate Detection}},
  booktitle =    PROC # " " # PDS,
  pages =    {412-417},
  month =    DEC,
  year =     {1994}
}

@Article{AlaVen:2001:TSE,
  author =   {S. Alagar and S. Venkatesan},
  title =    {{Techniques to Tackle State Explosion in Global Predicate Detection}},
  journal =  TSE,
  year =     2001,
  volume =   27,
  number =   8,
  pages =    {704-714},
  month =    AUG
}

@TechReport{AlaVid:1999:TR,
  author =   {K. Alagarsamy and K.Vidyasankar},
  title =    {{Elegant Solutions for Group Mutual Exclusion Problem}},
  institution =  {Department of Computer Science, Memorial University of Newfoundland,
                  St.John's, Newfoundland, Canada},
  year =     {1999},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{AlmBaq+:2002:ICDCS,
  author =   {P. S. Almeida and C. Baquero and V. Fonte},
  title =    {{Version Stamps---Decentralized Version Vectors}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 22nd " # ICDCS,
  pages =    {544-551},
  year =     {2002},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{AlvEln+:1999:FTCS,
  author =   {L. Alvisi and E. N. Elnozahy and S. Rao and
                  S. A. Hussain and A. D. Mel},
  title =    {{An Analysis of Communication-Induced Checkpointing}},
  booktitle =    PROC # " 29th " # FTCS,
  pages =    {242-249},
  year =     1999,
  address =  {Madison, Wisconsin},
  month =    JUN
}

@InProceedings{AlvMar:1995:ICDCS,
  author =   {L. Alvisi and K. Marzullo},
  title =    {{Message Logging: Pessimistic, Optimistic, and Causal}},
  booktitle =    PROC # " 15th " # ICDCS,
  pages =    {229-236},
  year =     1995,
  address =  {Vancouver, Canada},
  month =    JUN
}

@MastersThesis{Ang:2001:Thesis,
  author =   {R. Anguiano},
  title =    {{A Static Analysis Technique for the Detection of
                   TOCTTOU Vulnerabilities}},
  school =   {University of California, Davis},
  year =     {2001},
  OPTkey =   {},
  OPTtype =  {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@Article{AroGou:1994:TC,
  author =   {A. Arora and M. G. Gouda},
  title =    {{Distributed Reset}},
  journal =      TC,
  year =     1994,
  volume =   43,
  number =   9,
  pages =    {1026-1038}
}

@Article{AroSin:1995:HIS,
  author =   {A. Arora and A. Singhai},
  title =    {{Fault-Tolerant Reconfiguration of Trees and Rings in Distributed Systems}},
  journal =      HIS,
  year =     1995,
  volume =   1,
  number =   4,
  pages =    {375-384}
}

@InProceedings{AtrMit+:2003:OPODIS,
  author =   {R. Atreya and N. Mittal and V. K. Garg},
  title =    {{Detecting Locally Stable Predicates without
                   Modifying Application Messages}},
  booktitle =    PROC # " 7th " # OPODIS,
  year =     2003,
  pages =        {20-33},
  address =  {La Martinique, France},
  month =    DEC
}

@Article{BabFro+:1996:JSS,
  author =   {{\"O}. Babao{\v{g}}lu and E. Fromentin and
                  M. Raynal},
  title =    {{A Unified Framework for the Specification and Run-time Detection
                   of Dynamic Properties in Distributed Computations}},
  journal =  JSS,
  volume =   {33},
  number =   {3},
  month =    JUN,
  pages =    {287-298},
  year =     {1996},
  url =      {http://citeseer.nj.nec.com/10396.html}
}

@incollection{BabMar:1993:DS,
  author =   {{\"{O}}. Babao{\v g}lu and K. Marzullo},
  title =    {{Consistent Global States of Distributed Systems: Fundamental Concepts and
                   Mechanisms}},
  booktitle =    DS,
  publisher =    AW,
  editor =   {S. Mullender},
  pages =    {55-96},
  year =     {1993},
  url =
                  {http://citeseer.nj.nec.com/babaoglu93consistent.html}
}

@Article{BabRay:1995:JPDC,
  author =   {{\"{O}}. Babao{\v g}lu and M. Raynal},
  title =    {{Specification and Verification of Dynamic Properties in Distributed Computations}},
  journal =  JPDC,
  year =     1995,
  volume =   28,
  number =   2,
  pages =    {173-185}
}

@Book{Bac:1987:Book,
  author =   {M. J Bach},
  title =    {{The Design of the Unix Operating System}},
  publisher =    PH,
  year =     1987,
  isbn =     0132017997
}

@Book{Bac:1987:PH,
  author =   {M. J. Bach},
  title =    {{The Design of the Unix Operating System}},
  publisher =    PH,
  year =     1987
}

@Manual{BalKan:1999:INFORMIX,
  author =   {I. Balabine and R. Kandasamy},
  title =    {{File System Interface to a Database}},
  note =     USPATENT # " 5937406 granted to " # INFORMIX,
  year =     {1999},
  month =    AUG
}

@InProceedings{BarBra+:1996:ICSSE,
  author =   {A. Barak and A. Braverman and A. Gilderman and O. La'adan},
  title =    {{Performance of PVM with MOSIX Preemptive Process Migration}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 7th " # ICSSE,
  pages =    {38-45},
  year =     {1996},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Herzliya},
  month =    JUN,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{BeaCan+:2003:JISE,
  author =   {J. Beauquier and S. Cantarell and A. K. Datta and F. Petit},
  title =    {{Group Mutual Exclusion in Tree Networks}},
  journal =      JISE,
  year =     {2003},
  OPTkey =   {},
  volume =   {19},
  number =   {3},
  pages =    {415-432},
  month =    MAY,
  OPTnote =      {},
  OPTannote =    {}
}

@Manual{BegDon+:PVM2.0,
  title =    {{H}ence: {A} users' guide - version 2.0. {PVM}
                  {D}esign and {V}isualization},
  author =   {A. Beguelin and J. Dongarra and G. A. Geist and
                  R. Manchek and K. Moore and P. Newton and
                  V. Sunderam}
}

@InProceedings{Bel:1990:MCDS,
  author =   {S. Bellenot},
  title =    {{Global Virtual Time Algorithms}},
  booktitle =    PROC # " " # MCDS,
  pages =    {122-127},
  year =     1990,
  volume =   22,
  number =   1,
  month =    JAN,
  organization = SCS
}

@TechReport{Bis:1995:TR:8,
  author =   {M. Bishop},
  title =    {{Race Conditions, Files, and Security Flaws: or, The
                   Tortoise and the Hare \emph{Redux}}},
  institution =  DCS # ", " # UCD,
  year =     {1995},
  OPTkey =   {},
  OPTtype =  {},
  number =   {95-8},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@Article{BisDil:1996:CSS,
  author =   {M. Bishop and M. Dilger},
  title =    {{Checking for Race Conditions in File Accesses}},
  journal =  CSS,
  year =     2003,
  volume =   9,
  number =   2,
  pages =    {131-152}
}

@Article{BisDil:1996:UCS,
  author =   {M. Bishop and M. Dilger},
  title =    {{Checking for Race Conditions in File
                  Accesses}},
  journal =  UCS,
  year =     1996,
  volume =   9,
  number =   2,
  pages =    {131-152}
}

@Unpublished{BisHol:1978:PR:13,
  author =   {R. Bisbey and D. Hollingsworth},
  title =    {{Protection Analysis Project Final Report}},
  note =     {ISI/RR-78-13, DTIC AD A056816, USC/Information
                  Sciences Institute},
  OPTkey =   {},
  month =    MAY,
  year =     {1978},
  OPTannote =    {}
}

@Article{Bou:1987:TCS,
  author =   {L. Bouge},
  title =    {{Repeated Snapshots in Distributed Systems
                  with Synchronous Communication and their
                  Implementation in CSP}},
  journal =  TCS,
  year =     1987,
  volume =   49,
  pages =    {145-169}
}

@Article{Bre:1966:TIT,
  author =   {M. Breuer},
  title =    {{Coding Vertexes of a Graph}},
  journal =  TIT,
  year =     1966,
  volume =   12,
  pages =    {148-153}
}

@TechReport{BriLit+:1992:CONDOR,
  author =   {A. Bricker and M. Litzkow and M. Livny},
  title =    {{Condor Technical Summary, Version 4.1b}},
  institution =  "Computer Science Department, " # UWM,
  year =     {1992},
  OPTkey =   {},
  OPTtype =      {},
  number =   {CS-TR-92-1069},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{BrzHel+:1993:ICDCS,
  author =   {J. Brzezinski and J.-M. H{\'e}lary and M. Raynal},
  title =    {{Termination Detection in a Very General Distributed
                   Computing Model}},
  booktitle =    PROC # " " # ICDCS,
  pages =    {374-381},
  year =     1993
}

@article{BrzHel+:1995:JPDC,
  author =   {J. Brzezinski and J.-M. H{\'e}lary and M. Raynal and
                  M. Singhal},
  title =    {{Deadlock Models and a General Algorithm for
                   Distributed Deadlock Detection}},
  journal =  JPDC,
  volume =   {31},
  number =   {2},
  pages =    {112-125},
  year =     "1995"
}

@Misc{Bug:2002:RDR,
  title =    {{Recursive Directory Removal Race Condition}},
  howpublished = {http://mail.gnu.org/pipermail/bug-fileutils/2002-March/002433.html},
  month =    MAR,
  year =     2002
}

@Manual{CORBA:1997,
  author =   {Object Management Group},
  title =    {{The Common Object Request Broker: Architecture and Specification}}
}

@InProceedings{CanDat+:2001:ICDCS,
  author =   {S. Cantarell and A. K. Datta and F. Petit and V. Villain},
  title =    {{Token Based Group Mutual Exclusion for Asynchronous Rings}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICDCS,
  pages =    {691-694},
  year =     {2001},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{Cap:1994:ORDAL,
  author =   {C. Capelle},
  title =    {{Representation of an Order as Union of Interval Orders}},
  booktitle =    PROC # " " # ORDAL,
  pages =    {143-161},
  year =     1994,
  number =   831,
  series =   LNCS,
  address =  {Lyon, France},
  month =    JUL,
  publisher =    SV
}

@InProceedings{Cas:1993:OOPSLA,
  author =   {Y. Caseau},
  title =    {{Efficient Handling of Multiple Inheritance Hierarchies}},
  booktitle =    PROC # " " # OOPSLA,
  pages =    {271-287},
  year =     1993
}

@Article{Cas:1995:CSS,
  author =   {J. Casas and R. Konuru and S. W. Otto and R. M. Prouty and J. Walpole},
  title =    {{MPVM---A Migration Transparent Version of PVM}},
  journal =      CSS,
  year =     {1995},
  OPTkey =   {},
  volume =   {8},
  number =   {2},
  pages =    {171-216},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ChaDel+:1995:TOPLAS,
  author =   {B. Charron-Bost and C. Delporte-Gallet and
                  H. Fauconnier},
  title =    {{Local and Temporal Predicates in Distributed Systems}},
  journal =  TOPLAS,
  year =     1995,
  volume =   17,
  number =   1,
  pages =    {157-179}
}

@InProceedings{ChaGar:1995:WDAG,
  author =   {C. Chase and V. K. Garg},
  title =    {{On Techniques and their Limitations for the Global Predicate
                   Detection Problem}},
  booktitle =    PROC # " " # WDAG,
  year =     1995,
  address =  {France},
  month =    SEP,
  pages =    {303-317}
}

@Article{ChaGar:1998:DC,
  author =   {C. Chase and V. K. Garg},
  title =    {{Detection of Global Predicates: Techniques and their Limitations}},
  journal =  DC,
  year =     1998,
  volume =   11,
  number =   4,
  pages =    {191-201}
}

@Article{ChaLam:1985:TrCS,
  author =   {K. M. Chandy and L. Lamport},
  title =    {{Distributed Snapshots: Determining Global States of Distributed Systems}},
  journal =  TrCS,
  year =     1985,
  volume =   3,
  number =   1,
  pages =    {63-75},
  month =    FEB
}

@Article{ChaMis+:1983:TrCS,
  author =   {K. M. Chandy and J. Misra and L. M. Haas},
  title =    {{Distributed Deadlock Detection}},
  journal =      TrCS,
  year =     1983,
  volume =   1,
  number =   2,
  pages =    {144-156},
  month =    MAY
}

@Article{ChaMis:1984:TOPLAS,
  author =   {K. M. Chandy and J. Misra},
  title =    {{The Drinking Philosophers Problem}},
  journal =      TOPLAS,
  year =     {1984},
  OPTkey =   {},
  volume =   {6},
  number =   {4},
  pages =    {632-646},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ChaMis:1986:DC,
  author =   {K. M. Chandy and J. Misra},
  title =    {{How Processes Learn}},
  journal =  DC,
  year =     {1986},
  OPTkey =   {},
  volume =   {1},
  number =   {1},
  pages =    {40-52},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@Book{ChaMis:1988:Book,
  author =   {K. M. Chandy and J. Misra},
  title =    {{Parallel Program Design: A Foundation}},
  publisher =    AW,
  year =     1988
}

@Article{ChaTou:1996:JACM,
  author =   {T. D. Chandra and S. Toueg},
  title =    {{Unreliable Failure Detectors for Reliable Distributed Systems}},
  journal =  JACM,
  year =     {1996},
  volume =   {43},
  number =   {2},
  pages =    {225-267}
}

@Article{ChaVen:1990:JPDC,
  author =   {S. Chandrasekaran and S. Venkatesan},
  title =    {{A Message-Optimal Algorithm for Distributed
                  Termination Detection}},
  journal =  JPDC,
  year =     {1990},
  OPTkey =   {},
  volume =   {8},
  number =   {3},
  pages =    {245-252},
  month =    MAR,
  OPTnote =  {},
  OPTannote =    {}
}

@Article{Charron-Bost:size,
  author =   {B. Charron-Bost},
  title =    {{Concerning the Size of Logical Clocks in Distributed Systems}},
  journal =  IPL,
  year =     1991,
  month =    JUL,
  volume =   {39},
  pages =    {11-16},
}

@InProceedings{Che:1993:WAD,
  author =   {J. Cheng},
  title =    {{Slicing Concurrent Programs---A Graph-Theoretical Approach}},
  booktitle =    PROC # " " # WAD,
  pages =    {223-240},
  year =     1993
}

@Article{ChoMil+:1991:TOPLAS,
  author =   {J. Choi and B. P. Miller and R. Netzer},
  title =    {{Techniques for Debugging Parallel Programs with Flowback Analysis}},
  journal =  TOPLAS,
  year =     1991,
  volume =   13,
  number =   4,
  pages =    {491-530},
  month =    OCT
}

@InProceedings{ClaEme:1981:WLP,
  author =   {E. M. Clarke and E. A. Emerson},
  title =    {{Design and Synthesis of Synchronization Skeletons using
                   Branching Time Temporal Logic}},
  booktitle =    PROC # " " # WLP,
  address =  {Yorktown Heights, New York},
  month =    MAY,
  series =   LNCS,
  volume =   131,
  year =     1981
}

@InProceedings{CohLeh:1982:PODC,
  author =   {S. Cohen and D. Lehmann},
  title =    {{Dynamic Systems and their Distributed Termination}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 1st " # PODC,
  pages =    {29-33},
  year =     {1982},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Ottawa},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ColDol:1994:IPL,
  author =   {Z. Collin and S. Dolev},
  title =    {{Self-Stabilizing Depth-First Search}},
  journal =      IPL,
  year =     1994,
  volume =   49,
  number =   6,
  pages =    {297-301}
}

@InProceedings{CooMar:1991:WPDD,
  author =   {R. Cooper and K. Marzullo},
  title =    {{Consistent Detection of Global Predicates}},
  booktitle =    PROC # " " # WPDD,
  pages =    {163-173},
  year =     1991,
  address =  {Santa Cruz, California}
}

@Book{CorLei+:1991:MIT,
  author =   {T. H. Cormen and C. E. Leiserson and R. L. Rivest},
  title =    {{Introduction to Algorithms}},
  publisher =    MIT,
  address =  {Cambridge, Massachusetts},
  year =     {1991},
}

@InProceedings{CowBea+:2001:USS,
  author =   {C. Cowan and S. Beattie and C. Wright and
                  G. Korah-Hartman},
  title =    {{RaceGuard: Kernel Protection from Temporary File
                   Race Vulnerabilities}},
  booktitle =    PROC # " 10th " # USS,
  pages =    {165-172},
  year =     2001,
  month =    AUG
}

@Book{CoxGoo:1994:PH,
  author =   {J. Cox and B. Goodheart},
  title =    {{The Magic Garden Explained: The Internals of Unix
                   System V Release 4: An Open Systems Design}},
  publisher =    PH,
  year =     1994
}

@InProceedings{CypLeu:1995:SPDP,
  author =   {R. Cypher and E. Leu},
  title =    {{Efficient Race Detection for Message-Passing
                   Programs with Nonblocking Sends and Receives}},
  booktitle =    PROC # " " # SPDP,
  pages =    {534-541},
  year =     1995
}

@Manual{DB2SQL:1999:IBM,
  title =    {DB2 UDB SQL Reference},
  organization = {IBM},
  edition =  {V6.1},
  year =     1999
}

@Article{DarMay:2003:JPDC,
  author =   {D. Darling and J. Mayo},
  title =    {{Stable Predicate Detection in Dynamic Systems}},
  journal =      "Submitted to the " # JPDC,
  OPTpages =     {},
  year =     {2003},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Manual{Dav:1999:IBM,
  title =    {{DataLinks: Managing External Data with DB2
                   Universal Database}},
  organization = {IBM Corporation},
  month =    FEB,
  year =     {1999},
  note =     {White paper prepared by J. R. Davis}
}

@Book{DavPri:1990:CUP,
  author =   {B. A. Davey and H. A. Priestley},
  title =    {{Introduction to Lattices and Order}},
  publisher =    CUP,
  address =  {Cambridge, UK},
  year =     {1990},
}

@TechReport{DemAro:2000:TR:05,
  author =   {M. Demirbas and A. Arora},
  title =    {{An Optimal Termination Detection Algorithm for
                   Rings}},
  institution =  OSU,
  year =     2000,
  number =   {OSU-CISRC-2/00-TR05},
  month =    FEB
}

@Article{Den:1987:TSE,
  author =   {D. Denning},
  title =    {{An Intrusion Detection Model}},
  journal =  TSE,
  volume =   {13},
  number =   {2},
  month =    FEB,
  year =     {1987},
  pages =    {222-232}
}

@Article{DhaIye+:1997:PC,
  author =   {D. M. Dhamdhere and S. R. Iyer and E. K. K. Reddy},
  title =    {{Distributed Termination Detection for Dynamic Systems}},
  journal =      PC,
  year =     {1997},
  OPTkey =   {},
  volume =   {22},
  OPTnumber =    {},
  pages =    {2025-2045},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dij:1965:CACM,
  author =   {E. W. Dijkstra},
  title =    {{Solution of a Problem in Concurrent Programming
                   Control}},
  journal =  CACM,
  pages =    569,
  year =     1965,
  volume =   8,
  number =   9,
  organization = {ACM}
}

@Article{Dij:1971:ACTA,
  author =   {E. W. Dijkstra},
  title =    {{Hierarchical Ordering of Sequential Processes}},
  journal =      ACTA,
  year =     1971,
  volume =   1,
  number =   2,
  pages =    {115-138},
  month =    OCT
}

@Article{Dij:1974:CACM,
  author =   {E. W. Dijkstra},
  title =    {{Self-Stabilizing Systems in spite of Distributed Control}},
  journal =  CACM,
  year =     {1974},
  volume =   {17},
  number =   {11},
  pages =    {643-644}
}

@InCollection{Dij:1985:SV,
  author =   {E. W. Dijsktra},
  title =    {{The Distributed Snapshot of K. M. Chandy and L. Lamport}},
  booktitle =    {Control Flow and Data Flow: Concepts of Distributed
                  Programming},
  OPTcrossref =  {},
  OPTkey =   {},
  OPTpages =     {},
  publisher =    SV,
  year =     {1985},
  editor =   {M. Broy},
  volume =   {F14},
  OPTnumber =    {},
  series =   {NATO ASI},
  OPTtype =  {},
  OPTchapter =   {},
  address =  {New York, NY},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@Article{Dij:1986:DC,
  author =   {E. W. Dijkstra},
  title =    {{A Belated Proof of Self-Stabilization}},
  journal =  DC,
  year =     {1986},
  volume =   {1},
  pages =    {5-6}
}

@Article{DijFei+:1983:IPL,
  author =   {E. W. Dijkstra and W. H. J. Feijen and A. J. M. van
                  Gasteren},
  title =    {{Derivation of a Termination Detection Algorithm for
                   Distributed Computations}},
  journal =  IPL,
  volume =   {16},
  pages =    {217-219},
  OPTkey =   {},
  OPTmonth =     {},
  year =     {1983},
  OPTannote =    {}
}

@Article{DijSch:1980:IPL,
  author =   {E. W. Dijkstra and C. S. Scholten},
  title =    {{Termination Detection for Diffusing Computations}},
  journal =  IPL,
  year =     1980,
  volume =   11,
  number =   1,
  pages =    {1-4}
}

@Article{Dil:1950:AM,
  author =   {R. P. Dilworth},
  title =    {{A Decomposition Theorem for Partially Ordered Sets}},
  journal =  AM,
  year =     1950,
  volume =   51,
  pages =    {161-166}
}

@Article{DolIsr+:1993:DC,
  author =   {S. Dolev and A. Israeli and S. Moran},
  title =    {{Self-Stabilization of Dynamic Systems Assuming Only Read/Write Atomicity}},
  journal =      DC,
  year =     1993,
  volume =   7,
  number =   1,
  pages =    {3-16}
}

@InProceedings{DueGup+:1992:WLCPC,
  author =   {E. Duesterwald and R. Gupta and M. L. Soffa},
  title =    {{Distributed Slicing and Partial Re-execution for Distributed Programs}},
  booktitle =    PROC # " 5th " # WLCPC,
  pages =    {329-337},
  year =     1992
}

@Article{DusMil:1941:AJM,
  author =   {B. Dushnik and E. W. Miller},
  title =    {{Partially Ordered Sets}},
  journal =  AJM,
  year =     1941,
  volume =   63,
  pages =    {600-610}
}

@PhdThesis{Ell:1995:PhD,
  author =   {G. Ellis},
  title =    {{Managing Complex Objects}},
  school =   {University of Queensland},
  year =     1995
}

@Article{ElnAlv+:2002:CS,
  author =   {E. N. Elnozahy and L. Alvisi and Y.-M. Wang and
                  D. B. Johnson},
  title =    {{A Survey of Rollback-Recovery Protocols in
                   Message-Passing Systems}},
  journal =  CS,
  volume =   {34},
  number =   {3},
  year =     {2002},
  pages =    {373-408},
}

@Article{FelHab+:1994:SIAMJDM,
  author =   {S. Felsner and M. Habib and R. H. M{\"o}hring},
  title =    {{On the Interplay of Interval Dimension and Dimension}},
  journal =  SIAMJDM,
  volume =   7,
  pages =    {32-40},
  year =     1994,
  OPTurl =       {http://www.inf.fu-berlin.de/{\symbol{126}}felsner/Paper/Idim-dim.ps.gz},
}

@Article{FelTro:1994:DM,
  author =   {S. Felsner and W. T. Trotter},
  title =    {{On the Fractional Dimension of Partially Ordered Sets}},
  journal =  DM,
  volume =   136,
  pages =    {101-117},
  year =     1994,
  OPTurl =       {http://www.inf.fu-berlin.de/{\symbol{126}}felsner/Paper/fdim.ps.gz},
}

@Article{Fid:1991:Com,
  author =   {C. Fidge},
  title =    {{Logical Time in Distributed Computing Systems}},
  journal =  Com,
  year =     1991,
  volume =   24,
  number =   8,
  pages =    {28-33},
  month =    AUG
}

@InProceedings{FisLyn+:1979:FCS,
  author =   {M. J. Fischer and N. A. Lynch and  J. E. Burns and A. Borodin},
  title =    {{Resource Allocation with Immunity to Limited Process Failure
                   (preliminary report)}},
  booktitle =    PROC # " 20th " # FOCS,
  pages =    {234-254},
  year =     1979,
  month =    OCT
}

@Article{Fra:1980:TOPLAS,
  author =   {N. Francez},
  title =    {{Distributed Termination}},
  journal =  TOPLAS,
  year =     1980,
  volume =   2,
  number =   1,
  pages =    {42-55},
  month =    JAN
}

@InProceedings{FroRay+:1994:ICPP,
  author =   {E. Fromentin and M. Raynal and V. K. Garg and
                  A. I. Tomlinson},
  title =    {{On the Fly Testing of Regular Patterns in Distributed Computations}},
  booktitle =    PROC # " 23rd " # ICPP,
  pages =    {73-76},
  year =     1994,
  number =   2,
  address =  {Chicago, Illinois},
  month =    AUG
}

@InProceedings{FroRay:1994:SPDP,
  author =   {E. Fromentin and M. Raynal},
  title =    {{Inevitable Global States: A Concept to Detect
                   Unstable Properties of Distributed Computations in
                   an Observer Independent Way}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 6th " # SPDP,
  pages =    {242-248},
  year =     {1994},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization ={},
  OPTpublisher = {},
  OPTnote =  {},
  OPTannote =    {}
}

@Misc{GDB,
  OPTkey =   {},
  OPTauthor =    {},
  title =    {{GDB: The GNU Project Debugger}},
  OPThowpublished = {},
  OPTmonth =     {},
  OPTyear =      {},
  note =     {Available at
                  \texttt{http://www.gnu.org/software/gdb/gdb.html}},
  OPTannote =    {}
}

@TechReport{Gae:2003:TR:38,
  author =   {F. C. G{\"a}rtner},
  title =    {{A Survey of Self-Stabilizing Spanning-Tree Construction Algorithms}},
  institution =  SCCS # ", " # EPFL,
  address =      {Lausanne, Switzerland},
  year =     2003,
  number =   {IC 2003/38}
}

@InProceedings{GaeKlo:2000:SRDS,
  author =   {F. C. G{\"a}rtner and S. Kloppenburg},
  title =    {{Consistent Detection of Global Predicates under a Weak Fault Assumption}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # ", " # SRDS,
  pages =    {94-103},
  year =     {2000},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {N{\"u}rnberg, Germany},
  month =    OCT,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{GaePle:2001:DISC,
  author =   {F. C. G{\"a}rtner and S. Pleisch},
  title =    {{(Im)Possibilities of Predicate Detection in
                  Crash-Affected Systems using
                  Interrupt-Style Failure Detectors (Brief Announcement)}},
  booktitle =    PROC # " " # DISC,
  year =     2001,
  address =  {Lisbon, Portugal},
  month =    {October}
}
@TechReport{GaePle:2001:TR,
  author =   {F. C. G{\"a}rtner and S. Pleisch},
  title =    {{(Im)Possibilities of Predicate Detection in Crash-Affected Systems}},
  institution =  IBMZ,
  year =     2001,
  number =   {RZ 3361 (\# 93407)},
  month =    AUG
}
@InProceedings{GaePle:2001:WSS,
  author =   {F. C. G{\"a}rtner and S. Pleisch},
  title =    {{(Im)Possibilities of Predicate Detection in Crash-Affected Systems}},
  booktitle =    PROC # " 5th " # WSS,
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {98-113},
  year =     {2001},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   LNCS # " 2194",
  address =  {Lisbon, Portugal},
  month =    {October},
  OPTorganization ={},
  publisher =    SV,
  OPTnote =  {},
  OPTannote =    {}
}
@InProceedings{GaePle:2002:DISC,
  author =   {F. C. G{\"a}rtner and S. Pleisch},
  title =    {{Failure Detection Sequencers: Necessary and Sufficient
                  Information about Failures to Solve Predicate Detection}},
  booktitle =    PROC # " 16th " #  DISC,
  pages =    {280-294},
  year =     2002,
  number =   2508,
  series =   LNCS,
  publisher =    SV
}
@InProceedings{GamNes+:1987:ICALP,
  author =   {G. Gambosi and J. Ne\v{s}et\v{r}il and M. Talamo},
  title =    {{Posets, Boolean Representations and Quick
                   Path Searching}},
  booktitle =    PROC # " 14th " # ICALP,
  year =     1987,
  pages =    {404-424},
  number =   267,
  series =   LNCS
}
@Article{GamNes+:1990:TCS,
  author =   {G. Gambosi and J. Ne\v{s}et\v{r}il and M. Talamo},
  title =    {{On Locally Presented Posets}},
  journal =  TCS,
  year =     {1990},
  OPTkey =   {},
  volume =   {70},
  number =   {2},
  pages =    {251-260},
  month =    JAN,
  OPTnote =  {},
  OPTannote =    {}
}
@InProceedings{Gar:1996:ICSKE,
  author =   {V. K. Garg},
  title =    {{Observation of Global Properties in Distributed Systems}},
  booktitle =    ICSKE,
  pages =    {418-425},
  year =     1996,
  address =  {Lake Tahoe, Nevada},
  month =    JUN
}
@Book{Gar:1996:KAP,
  author =   {V. K. Garg},
  OPTeditor =    {~},
  title =    {{Principle of Distributed Systems}},
  publisher =    KAP,
  year =     1996
}
@InProceedings{Gar:1997:WAD,
  author =   {V. K. Garg},
  title =    {{Observation and Control for Debugging
                   Distributed Computations}},
  booktitle =    PROC # " " # WAD,
  pages =    {1-12},
  year =     1997,
  address =  {Link{\"o}ping, Sweden},
  note =     {Keynote Presentation}
}
@Book{Gar:2002:Book,
  author =   {V. K. Garg},
  title =    {{Elements of Distributed Computing}},
  publisher =    JWSUS,
  address =  {New York, NY},
  year =     {2002},
}
@InProceedings{Gar:2002:FSTTCS,
  author =   {V. K. Garg},
  title =    {{Algorithmic Combinatorics based on Slicing Posets}},
  booktitle =    PROC # " 22nd " # FSTTCS,
  year =     2002,
  address =  {Kanpur, India},
  month =    {December}
}
@Article{GarBar:1985:ACM,
  author =   {H. Garcia-Molina and D. Barbar},
  title =    {{How to Assign Votes in a Distributed System}},
  journal =  JACM,
  year =     {1985},
  volume =   {32},
  number =   {4},
  pages =    {841-860},
  month =    OCT
}
@InProceedings{GarCha+:1995:CSS,
  author =   {V. K. Garg and C. Chase and R. Kilgore and
                  J. R. Mitchell},
  title =    {{Detecting Conjunctive Channel Predicates in
                   a Distributed Programming Environment}},
  booktitle =    PROC # " " # CSS,
  pages =    {232-241},
  year =     1995,
  volume =   2,
  address =  {Maui, Hawaii},
  month =    JAN
}
@Article{GarCha+:1997:JPDC,
  author =   {V. K. Garg and C. Chase and R. Kilgore and
                  J. R. Mitchell},
  title =    {{Efficient Detection of Channel Predicates in
                   Distributed Systems}},
  journal =  JPDC,
  year =     {1997},
  volume =   {45},
  number =   {2},
  pages =    {134-147},
  month =    SEP
}
@InProceedings{GarCha:1995:ICDCS,
  author =   {V. K. Garg and C. Chase},
  title =    {{Distributed Algorithms for Detecting
                   Conjunctive Predicates}},
  booktitle =    PROC # " " # ICDCS,
  pages =    {423-430},
  year =     1995,
  address =  {Vancouver, Canada},
  month =    JUN
}

@Book{GarJoh:1991:Fre,
  author =   {M. R. Garey and D. S. Johnson},
  OPTeditor =    {Victor Klee},
  title =    {{Computer and Intractability: A Guide to the
                   Theory of \mbox{NP-Completeness}}},
  publisher =    Fre,
  year =     1991
}
@InProceedings{GarLun:1991:NCSC,
  author =   {T. D. Garvey and T. F. Lunt},
  title =    {{Model-Based Intrusion Detection}},
  booktitle =    PROC # " 14th " # NCSC,
  pages =    {372-385},
  year =     1991
}
@Article{GarMit+:2003:SIGACT,
  author =   {V. K. Garg and N. Mittal and A. Sen},
  title =    {{Applications of Lattice Theory to Distributed
                  Computing}},
  journal =  SIGACT # " News Distributed Computing Column",
  year =     2003,
  OPTpublisher = {ACM Press},
  editor =   {Sergio Rajsbaum},
  volume =   34,
  number =   3,
  pages =    {40-61},
  month =    SEP
}
@InProceedings{GarMit:1998:FSTTCS,
  author =   {V. K. Garg and J. R. Mitchell},
  title =    {{Implementable Failure Detectors in
                   Asynchronous Systems}},
  booktitle =    PROC # " " # FSTTCS,
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {158-169},
  year =     {1998},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =  {Chennai, India},
  OPTmonth =     {},
  OPTorganization ={},
  OPTpublisher = {},
  OPTnote =  {},
  OPTannote =    {}
}
@InProceedings{GarMit:1998:ICDCS,
  author =   {V. K. Garg and J. R. Mitchell},
  title =    {{Distributed Predicate Detection in a Faulty
                   Environment}},
  booktitle =    PROC # " " # ICDCS,
  pages =    {416-423},
  year =     {1998},
  address =  {Amsterdam, The Netherlands},
  month =    MAY
}
@InProceedings{GarMit:2001:ICDCS,
  author =   {V. K. Garg and N. Mittal},
  title =    {{On Slicing a Distributed Computation}},
  booktitle =    PROC # " 21st " # ICDCS,
  pages =    {322-329},
  year =     2001,
  address =  {Phoenix, Arizona},
  month =    APR,
  OPTnote =  {Available at \texttt{http://www.cs.utexas.edu/users/neerajm/research.html}}
}
@InProceedings{GarSka:2001:PODC,
  author =   {V. K. Garg and C. Skawratananond},
  title =    {{String Realizers of Posets with Applications
                   to Distributed Computing}},
  booktitle =    PROC # " 20th " # PODC,
  year =     2001,
  address =  {Newport, Rhode Island},
  month =    AUG,
  pages =    {72-80}
}
@InProceedings{GarTom+:1995:SPDP,
  author =   {V. K. Garg and A. I. Tomlinson and E. Fromentin and
                  Michel Raynal},
  title =    {{E}xpressing and {D}etecting {G}eneral {C}ontrol
                  {F}low {P}roperties of {D}istributed {C}omputations},
  booktitle =    PROC # " 7th " # SPDP,
  pages =    {432-438},
  year =     1995,
  address =  {San Antonio, Texas},
  month =    OCT
}
@InProceedings{GarWal:1991:WPDD,
  author =   {V. K. Garg and B. Waldecker},
  title =    {{D}etection of {U}nstable {P}redicates},
  booktitle =    PROC # " " # WPDD,
  address =  {Santa Cruz, California},
  month =    MAY,
  year =     {1991},
  OPTorganization ={ACM/ONR},
}
@InProceedings{GarWal:1992:FSTTCS,
  author =   {V. K. Garg and B. Waldecker},
  title =    {{D}etection of {U}nstable {P}redicates in
                  {D}istributed {P}rograms},
  booktitle =    PROC # " 12th " # FSTTCS,
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {253-264},
  year =     {1992},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   LNCS,
  address =  {New Delhi, India},
  OPTmonth =     {},
  OPTorganization ={},
  OPTpublisher = {},
  OPTnote =  {},
  OPTannote =    {}
}
@Article{GarWal:1994:TPDS,
  author =   {V. K. Garg and B. Waldecker},
  title =    {{Detection of Weak Unstable Predicates in Distributed Programs}},
  journal =  TPDS,
  year =     1994,
  volume =   5,
  number =   3,
  pages =    {299-307},
  month =    MAR
}
@Article{GarWal:1996:TPDS,
  author =   {V. K. Garg and B. Waldecker},
  title =    {{Detection of Strong Unstable Predicates in Distributed Programs}},
  journal =  TPDS,
  year =     1996,
  volume =   7,
  number =   12,
  pages =    {1323-1333},
  month =    DEC
}
@Article{GhoGup+:1996:JCI,
  author =   {S. Ghosh and A. Gupta and S. V. Pemmaraju},
  title =    {{A Fault-containing Self-stabilizing Spanning Tree Algorithm}},
  journal =      JCI,
  year =     1996,
  volume =   2,
  number =   1,
  pages =    {322-328}
}
@Book{God:1996:SV,
  author =   {P. Godefroid},
  ALTeditor =    {},
  title =    {{P}artial-{O}rder {M}ethods for the {V}erification of
                  {C}oncurrent {S}ystems},
  publisher =    SV,
  year =     {1996},
  volume =   {1032},
  series =   {Lecture Notes in Computer Science}
}
@Book{GodCox:1993:PH,
  author =   {B. Goodheart and J. Cox},
  title =    {The Magic Garden Explained: The Internals of Unix
                  System V Release 4},
  publisher =    PH,
  year =     {1993}
}
@Misc{GoySit+:2003:SCISS,
  author =   {B. Goyal and S. Sitaraman and N. Mittal and S. Venkatesan},
  title =    {{A Partial Order Approach to Detect Race Condition Attacks}},
  howpublished = "Abstract published in " # SCISS ,
  month =    APR,
  year =     2003
}
@TechReport{GoySit+:2003:TR:03,
  author =       {B. Goyal and S. Sitaraman and S. Venkatesan},
  title =        {{A Unified Approach to Detect Binding Based Race Condition Attacks}},
  number =       {UTDCS-02-03},
  year =         2003,
  institution =  DCS # ", " # UTD # ", " # "\textsf{http://www.utdallas.edu/{\textasciitilde}venky/publications/race.pdf}"
}
@InProceedings{GoySri+:2003:TWSIS,
  author =   {B. Goyal and S. Sitaraman and N. Mittal and S. Venkatesan},
  title =    {{Methods To Tackle Vulnerabilities Caused by Lack of Mutual Exclusion}},
  booktitle =    PROC # " " # TWSIS,
  year =     2003,
  pages =        {17-21},
  address =      {College Station, Texas},
  month =    APR
}
@Book{GraReu:1993:MK,
  author =   {J. Gray and A. Reuter},
  title =    {Transaction Processing: Concepts and Techniques},
  publisher =    MK,
  year =     {1993}
}
@InProceedings{GraVol:1993:MVPP,
  author =   {S. Grabner and J. Volkert},
  title =    {{Debugging Parallel Programs Using Event Graph Manipulation}},
  booktitle =    PROC # " " # MVPP,
  pages =    {443-450},
  year =     1993,
  month =    OCT
}
@Book{Gratzer,
  author =       {G. Gratzer},
  title =        {{General Lattice Theory}},
  publisher =    {Academic Press},
  address =      {New York, NY},
  year =         1978
}
@InProceedings{HabHuc+:1995:KRUSE,
  author =   {M. Habib and M. Huchard and L. Nourine},
  title =    {{Embedding Partially Ordered Sets into Chain-Products}},
  booktitle =    PROC # " " # KRUSE,
  pages =    {147-161},
  year =     1995,
  address =      {University of California, Santa Cruz},
  month =    AUG
}
@InProceedings{HabNou:1994:ORDAL,
  author =   {M. Habib and L. Nourine},
  title =    {{Bit-Vector Encoding for Partially Ordered Sets}},
  booktitle =    PROC # " " # ORDAL,
  pages =    {1-12},
  year =     1994,
  number =   831,
  series =   LNCS,
  address =      {Lyon, France},
  month =    JUL,
  publisher = SV
}


@inproceedings{KuznetsovRavi:ConcurrencyTM:OPODIS:2011,
  author    = {Petr Kuznetsov and
               Srivatsan Ravi},
  title     = {On the Cost of Concurrency in Transactional Memory},
  booktitle = {Principles of Distributed Systems - 15th International Conference,
               {OPODIS} 2011, Toulouse, France, December 13-16, 2011. Proceedings},
  pages     = {112--127},
  year      = {2011},
  url       = {https://doi.org/10.1007/978-3-642-25873-2\_9},
  doi       = {10.1007/978-3-642-25873-2\_9},
  timestamp = {Wed, 17 May 2017 14:24:33 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/opodis/KuznetsovR11},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@InProceedings{Had:2001:PODC,
  author =   {V. Hadzilacos},
  title =    {{A Note on Group Mutual Exclusion}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 20th " # PODC,
  OPTpages =     {},
  year =     {2001},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    AUG,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@article{Hadzilacos:1988:JACM,
 author = {Hadzilacos, Vassos},
 title = {A theory of reliability in database systems},
 journal = {J. ACM},
 issue_date = {Jan. 1988},
 volume = {35},
 number = {1},
 month = jan,
 year = {1988},
 issn = {0004-5411},
 pages = {121--145},
 numpages = {25}
} 


@InProceedings{HelJar+:1987:PODC,
  author =       {J.-M. H{\'e}lary and C. Jard and N. Plouzeau and M. Raynal},
  title =        {{Detection of Stable Properties in Distributed Applications}},
  booktitle =    PROC # " " # PODC,
  pages =        {125-136},
  year =         {1987}
}
@article{HelRay:1994:DC,

  author =       {J.-M. H{\'e}lary and M. Raynal},
  title =        {{Towards the Construction of Distributed Detection Programs, with
                   an Application to Distributed Termination}},
  journal =      DC,
  volume =       {7},
  number =       {3},
  pages =        {137-147},
  year =         "1994"
}
@Article{Hir:1951:SRKU,
  author =   {T. Hiraguchi},
  title =    {{On the Dimension of Partially Ordered Sets}},
  journal =      SRKU,
  year =     1951,
  volume =   1,
  pages =    {77-94}
}
@Article{Hir:1955:SRKU,
  author =   {T. Hiraguchi},
  title =    {{O}n the {D}imension of {O}rders},
  journal =      SRKU,
  year =     1955,
  volume =   4,
  pages =    {1-20}
}
@Article{HoRam:1982:TSE,
  author =   {G. S. Ho and C. V. Ramamoorthy},
  title =    {{Protocols for Deadlock Detection in Distributed Database Systems}},
  journal =      TSE,
  year =     {1982},
  OPTkey =   {},
  volume =   {8},
  number =   {6},
  pages =    {554-557},
  month =    NOV,
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Hol:1997:TSE,
  author =   {G. Holzmann},
  title =    {{The Model Checker SPIN}},
  journal =      TSE,
  year =     1997,
  OPTkey =   {},
  volume =   23,
  number =   5,
  pages =    {279-295},
  month =    MAY,
  OPTnote =      {},
  OPTannote =    {}
}
@TechReport{HsiMit:2000:TC,
  author =   {H. Hsiao and N. Mittal},
  title =    {{Database Managed External File Update}},
  institution =  IBMARC,
  year =     2000,
  number =   {RJ10183},
  address =  {San Jose, California, 95120}
}
@Manual{HsiNar:1999:IBMARC,
  author =   {H. Hsiao and I. Narang},
  title =    {{Update In-Place Support with DataLinks}},
  organization = IBMARC,
  year =     {1999},
  note =     {Internal Document}
}
@InProceedings{HsiNar:2000:SIGMOD,
  author =   {H. Hsiao and I. Narang},
  title =    {{DLFM: A Transactional Resource Manager}},
  booktitle =    PROC # " 19th " # SIGMOD,
  pages =    {518-528},
  year =     2000,
  address =  {Dallas, Texas},
  month =    MAY
}
@InProceedings{Hua:1989:ICDCS,
  author =   {S.-T. Huang},
  title =    {{Detecting Termination of Distributed Computations by External Agents}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICDCS,
  pages =    {79-84},
  year =     {1989},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Hua:1989:IPL,
  author =   {S.-T. Huang},
  title =    {{Termination Detection by using Distributed Snapshots}},
  journal =      IPL,
  year =     {1989},
  OPTkey =   {},
  volume =   {32},
  OPTnumber =    {},
  pages =    {113-119},
  month =    AUG,
  OPTnote =      {},
  OPTannote =    {}
}
@Article{HuaChe:1992:IPL,
  author =   {S.-T. Huang and N.-S. Chen},
  title =    {{A Self-Stabilizing Algorithm for Constructing Breadth-First Trees}},
  journal =      IPL,
  year =     1992,
  volume =   41,
  number =   2,
  pages =    {109-117},
  month =    FEB
}
@InProceedings{HuaKin:1993:FTCS,
  author =   {Y. Huang and C. Kintala},
  title =    {{S}oftware {I}mplemented {F}ault {T}olerance:
                  {T}echnologies and {E}xperience},
  booktitle =    PROC # " " # FTCS,
  pages =    {138-144},
  year =     1993,
  month =    JUN
}
@InProceedings{HurMiz+:1996:SPDP,
  author =   {M. Hurfin and M. Mizuno and M. Raynal and
                  M. Singhal},
  title =    {{Efficient Distributed Detection of Conjunctions of Local Predicates in
                   Asynchronous Computations}},
  booktitle =    PROC # " 8th " # SPDP,
  pages =    {588-594},
  year =     1996,
  address =  {New Orleans},
  month =    OCT
}
@Article{HurPlo+:1993:JCC,
  author =   {M. Hurfin and N. Plouzeau and M. Raynal},
  title =    {{A Debugging Tool for Distributed Estelle Programs}},
  journal =  JCC,
  year =     1993,
  volume =   16,
  number =   5,
  pages =    {328-333},
  month =    MAY
}
@InProceedings{HurPlo+:1993:WPDD,
  author =   {M. Hurfin and N. Plouzeau and M. Raynal},
  title =    {{D}etecting {A}tomic {S}equences of {P}redicates in
                  {D}istributed {C}omputations},
  booktitle =    PROC # " " # WPDD,
  pages =    {32-42},
  year =     1993
}
@InProceedings{HurRay:1996:WGCS,
  author =   {M. Hurfin and M. Raynal},
  title =    {{D}etecting {D}iamond {N}ecklaces in {L}abeled {D}ags
                  ({A} {P}roblem from {D}istributed  {D}ebugging},
  booktitle =    PROC # " " # WGCS,
  pages =    {211-223},
  year =     1996,
  series =   LNCS,
  publisher =    SV
}
@Manual{ISO:1993,
  author =       {ISO},
  title =        {{S}pecification of the {A}synchronous {T}ransfer {M}ode
                  {R}ing {(ATMR)} {P}rotocol},
  month =        JAN,
  year =         1993,
}
@InProceedings{JarJer+:1994:ICDCS,
  author =       {C. Jard and T. J{\'e}ron and G.-V. Jourdan and J.-X. Rampon},
  title =        {{A} {G}eneral {A}pproach to {T}race-{C}hecking in
                  {D}istributed {C}omputing {S}ystems},
  booktitle =    PROC # " " # ICDCS,
  pages =        {396-403},
  year =         {1994},
  url =          {http://citeseer.nj.nec.com/jard94general.html}
}
@InProceedings{JegMed+:1995:WSCT,
  author =   {R. Jegou and R. Medina and L. Nourine},
  title =    {{L}inear {S}pace {A}lgorithm for {O}n-line
                  {D}etection of {G}lobal {P}redicates},
  booktitle =    PROC # " " # WSCT,
  pages =        {175-189},
  year =     1995,
  editor =   {J. Desel},
  publisher =    SV
}
@InProceedings{JohZwa:1988:PODC,
  author =   {D. B. Johnson and W. Zwaenepoel},
  title =    {{R}ecovery in {D}istributed {S}ystems {U}sing
                  {O}ptimistic {M}essage {L}ogging and
                  {C}heckpointing},
  booktitle =    PROC # " 6th " # PODC,
  pages =    {171-181},
  year =     1988,
  month =    AUG
}
@Article{JohZwa:1990:JA,
  author =       {D. B. Johnson and W. Zwaenepoel},
  title =        {{R}ecovery in {D}istributed {S}ystems using {O}ptimistic {M}essage {L}ogging
                 and {C}heckpointing},
  journal =      JA,
  volume =       {11},
  number =       {3},
  month =        SEP,
  year =         {1990},
  pages =        {462-491},
}
@Article{Jou:2000:DC,
  author =       {Y.-J. Joung},
  title =        {{A}synchronous {G}roup {M}utual {E}xclusion},
  journal =      DC,
  volume =       {13},
  number =       {4},
  pages =        {189-206},
  year =         {2000},
}
@Article{Jou:2002:DC,
  author =       {Y.-J. Joung},
  title =        {{T}he {C}ongenial {T}alking {P}hilosophers {P}roblem in {C}omputer
                  {N}etworks},
  journal =       DC,
  pages =        {155-175},
  year =         {2002},
}
@Article{Jou:2003:TPDS,
  author =       {Y.-J. Joung},
  title =        {{Q}uorum-{B}ased {A}lgorithms for {G}roup {M}utual {E}xclusion},
  journal =      TPDS,
  pages =        {463-475},
  year =         {2003},
  volume =       {14},
  number =       {5},
  month =        MAY
}
@Article{KaeMoh:1978:SIAM,
  author =   {R. Kaerkes and R. H. M{\"o}hring},
  title =    {{V}orlesungen u{\"b}er {O}rdnungen und {N}etzplantheorie},
  journal =      {Schriften zur Informatik und Angewandten Mathematik 45, RWTH Aachen},
  year =     1978
}
@InProceedings{KanNao+:1988:STOC,
  author =   {S. Kannan and M. Naor and S. Rudich},
  title =    {{I}mplicit {R}epresentation of {G}raphs},
  booktitle =    PROC # " 20th " # STOC,
  pages =    {334-343},
  year =     1988,
  address =      {Chicago},
  month =    MAY
}
@Article{KanNao+:1992:SIAMJDM,
  author =   {S. Kannan and M. Naor and S. Rudich},
  title =    {{I}mplicit {R}epresentation of {G}raphs},
  journal =      SIAMJDM,
  year =     1992,
  volume =   5,
  number =   4,
  pages =    {596-603},
  month =    NOV
}
@InProceedings{KanWil+:2003:ICDCS,
  author =   {B. B. H. Kang and R. Wilensky and J, Kubiatowicz},
  title =    {{The Hash History Approach for Reconciling Mutual Inconsistency}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 23rd " # ICDCS,
  pages =    {670-677},
  year =     {2003},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Providence, Rhode Island},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{KeaMoi:1999:PODC,
  author =   {P. Keane and M. Moir},
  title =    {{A} {S}imple {L}ocal-{S}pin {G}roup {M}utual {E}xclusion {A}lgorithm},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PODC,
  pages =    {23-32},
  year =     {1999},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{KhoHam+:2003:JPDC,
  author =   {A. A. Khokhar and S. E. Hambrusch and E. Kocalar},
  title =    {{Termination Detection in Data-Driven Parallel Computations/Applications}},
  journal =      JPDC,
  year =     2003,
  volume =   63,
  number =   3,
  pages =    {312-326},
  month =    MAR
}
@Article{KilCha:1997:CJ,
  author =   {R. Kilgore and C. Chase},
  title =    {{T}esting {D}istributed {P}rograms {C}ontaining
                  {R}acing {M}essages},
  journal =  CJ,
  year =     1997,
  volume =   40,
  number =   8,
  pages =    {489-498},
  month =    NOV
}
@InProceedings{KilCha:1997:CSS,
  author =   {R. Kilgore and C. Chase},
  title =    {{R}e-execution of {D}istributed {P}rograms to
                  {D}etect {B}ugs {H}idden by {R}acing {M}essages},
  booktitle =    PROC # " " # CSS,
  pages =        {423-432},
  year =     1997,
  address =  {Hawaii},
  month =    JAN
}
@PhdThesis{KoChe:1996:Thesis,
  author =       {C. Ko and W. Cheuk},
  title =        {{Execution Monitoring Of Security Critical Programs in a Distributed
                   System: A Specification Based Approach}},
  year =         1996,
  school =       UCD
},
  month =        {August},
  year =         1997
}
@InProceedings{KoRed:2002:SP,
  author =   {C. Ko and T. Redmond},
  title =    {{Noninterference and Intrusion Detection}},
  year =     2002,
  booktitle =    PROC # " " # SP,
  pages =        {177-187},
  address =      {Berkeley, California},
  month =    MAY
}
@InProceedings{KocKho+:1999:PDC,
  author =   {E. Kocalar and A. A. Khokhar and S. E. Hambrusch},
  title =    {{T}ermination {D}etection: {M}odels and {A}lgorithms for {SPMD}
                  {C}omputing {P}aradigms},
  booktitle =    PROC # " " # PDC,
  year =     1999
}
@Book{Koh:1978:MH,
  author =   {Z. Kohavi},
  OPTeditor =    {~},
  title =    {{S}witching and {F}inite {A}utomata {T}heory},
  publisher =    MH,
  year =     1978,
  edition =  {2nd}
}
@Misc{KohGei:1995,
  OPTkey =   {},
  author =   {J. A. Kohl and G. A. Geist},
  title =    {{T}he {PVM 3.4} {T}racing {F}acility and {XPVM 1.1}},
  howpublished = {Computer Science and Mathematics Divison, Oak Ridge National Laboratory, TN, USA},
  OPTmonth =     {},
  year =     {1995},
  note =     {},
  OPTannote =    {}
}
@Article{KorFer:1992:AMCSJ,
  author =   {B. Korel and R. Ferguson},
  title =    {{Dynamic Slicing of Distributed Programs}},
  journal =  AMCSJ,
  year =     1992,
  volume =   2,
  number =   2,
  pages =    {199-215}
}
@Article{KorLas:1988:IPL,
  author =   {B. Korel and J. Laski},
  title =    {{Dynamic Program Slicing}},
  journal =  IPL,
  year =     1988,
  volume =   29,
  number =   3,
  pages =    {155-163}
}
@InProceedings{KorRil:1997:WAD,
  author =   {B. Korel and J. Rilling},
  title =    {{Application of Dynamic Slicing in Program Debugging}},
  booktitle =    PROC # " 3rd " # WAD,
  pages =    {43-57},
  year =     1997,
  editor =   {Mariam Kamkar},
  address =  {Link{\" o}ping, Sweden},
  month =    MAY
}
@Article{Ksh:1998:TCS,
  author =   {A. D. Kshemkalyani},
  title =    {{A Framework for Viewing Atomic Events in Distributed Computations}},
  journal =      TCS,
  year =     {1998},
  OPTkey =   {},
  volume =   {196},
  number =   {1-2},
  pages =    {45-70},
  month =    APR,
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{KshSin:1990:SPDP,
  author =       {A. D. Kshemkalyani and M. Singhal},
  title =        {{Correct Two-phase and One-phase Deadlock Detection
                   Algorithms for Distributed Systems}},
  booktitle =    PROC # " " # SPDP,
  pages =        {126-129},
  month =        DEC,
  year =         {1990}
}
@Article{KunBla+:1997:CJ,
  author =   {T. Kunz and J. P. Black and D. J. Taylor and T. Basten},
  title =    {{POET}: {T}arget-{S}ystem {I}ndependent {V}isualizations of {C}omplex
                  {D}istributed-{A}pplications {E}xecutions},
  journal =      CJ,
  year =     {1997},
  OPTkey =   {},
  volume =   {40},
  number =   {8},
  OPTpages =     {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Lai:1986:JPDC,
  author =   {T. H. Lai},
  title =    {{Termination Detection for Dynamic Distributed Systems with
                  Non-First-In-First-Out Communication}},
  journal =      JPDC,
  year =     {1986},
  OPTkey =   {},
  volume =   {3},
  OPTnumber =    {},
  pages =    {577-599},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{LaiTse+:1992:IPPS,
  author =       {T.-H. Lai and Y.-C. Tseng and X. Dong},
  title =        {{A More Efficient Message-Optimal Algorithm for
                  Distributed Termination Detection}},
  booktitle =    PROC # " 6th " # IPPS,
  year =         {1992},
  pages =        {646--649},
  publisher = {IEEE Computer Society},
}
@Article{LaiWu:1995:TPDS,
  author =   {T.-H. Lai and L.-F. Wu},
  title =    {{An $(N -1)$-Resilient Algorithm for Distributed Termination Detection}},
  journal =      TPDS,
  year =     1995,
  volume =   6,
  number =   1,
  pages =    {63-78}
}
@Article{LaiYan:1987:IPL,
  author =   {T.-H. Lai and T. H. Yang},
  title =    {{On Distributed Snapshots}},
  journal =      IPL,
  year =     {1987},
  OPTkey =   {},
  volume =   {25},
  number =   {3},
  pages =    {153-158},
  month =    MAY,
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Lam:1974:CACM,
  author =   {L. Lamport},
  title =    {{A New Solution of Dijkstra's Concurrent Programming Problem}},
  journal =      CACM,
  year =     {1974},
  OPTkey =   {},
  volume =   {18},
  number =   {8},
  pages =    {453-455},
  month =    AUG,
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Lam:1978:CACM,
  author =   {L. Lamport},
  title =    {{T}ime, {C}locks, and the {O}rdering of {E}vents in
                  a {D}istributed {S}ystem},
  journal =  CACM,
  year =     1978,
  volume =   21,
  number =   7,
  pages =    {558-565},
  month =    JUL
}
@Article{LanBul+:1994:CS,
  author =   {C. E. Landwehr and A. R. Bull and J. P. McDermott and W. S. Choi},
  title =    {{A} {T}axonomy of {C}omputer {P}rogram {S}ecurity {F}laws},
  journal =      CS,
  year =     1994,
  volume =   26,
  number =   3,
  pages =    {211-254},
  issn =         {0360-0300}
}
@Article{Law:1976:MCT,
  author =   {E. L. Lawler},
  title =    {{G}raphical {A}lgorithms and their {C}omplexity},
  journal =      MCT,
  year =     1976,
  volume =   81,
  pages =    {3-32}
}
@Article{LebMel:1987:TC,
  author =   {T. J. LeBlanc and J. M. Mellor-Crummey},
  title =    {{D}ebugging {P}rograms with {I}nstant {R}eplay},
  journal =  TC,
  year =     1987,
  volume =   {C-36},
  number =   4,
  pages =    {471-482},
  month =    APR
}
@Article{MadWes:1991:DM,
  author =   {T. Madej and D. B. West},
  title =    {{T}he {I}nterval {I}nclusion {N}umber of a {P}artially {O}rdered {S}et},
  journal =      DM,
  year =     1991,
  volume =   88,
  pages =    {259-277},
  note =     ES
}
@Article{Mae:1985:TrCS,
  author =       {M. Maekawa},
  title =        {{A}lgorithm for {M}utual {E}xclusion in {D}ecentralized {S}ystem},
  journal =      TrCS,
  pages =        {145-159},
  year =         {1985},
  volume =       {3},
  number =       {2},
  month =        MAY,
  OPTorganization = {ACM}
}
@Book{Mae:1987:Book,
  author =   {M. Maekawa and A. E. Oldehoft and R. R. Oldehoft},
  OPTeditor =    {},
  title =    {{Operating Systems Advanced Concepts}},
  publisher =    BCPC,
  year =     {1987},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Menlo Park, California},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Book{MaeOld+:1987:Book,
  author =   {M. Maekawa and A. E. Oldehoft and R. R. Oldehoft},
  title =    {{O}perating {S}ystems {A}dvanced {C}oncepts},
  publisher =    BCPC,
  year =     1987,
  address =      {Menlo Park, California}
}
@Article{MagWel+:1981:TCS,
  author =   {A. Maggiolo-Schettini and H. Welde and J. Winkowski},
  title =    {{M}odeling a {S}olution for a {C}ontrol {P}roblem in
                  {D}istributed {S}ystems by {R}estrictions},
  journal =  TCS,
  year =     1981,
  volume =   13,
  number =   1,
  pages =    {61-83},
  month =    JAN
}
@Unpublished{MahDut:2004:JPDC,
  author =   {N. R. Mahapatra and S. Dutt},
  title =    {{An Efficient Delay-Optimal Distributed Termination Detection Algorithm}},
  note =     "To Appear in " # JPDC,
  OPTkey =   {},
  OPTmonth =     {},
  year =     {2004},
  OPTannote =    {}
}
@Misc{Man:Rdist,
   title =      {{Man pages: Rdist - Remote File Distribution Program}},
   organization = {Sun Microsystems}
}
@article{ManIma:1992:JPDC,
  author =       {Y. Manabe and M. Imase},
  title =        {{G}lobal {C}onditions in {D}ebugging {D}istributed {P}rograms},
  journal =      JPDC,
  volume =       {15},
  number =       {1},
  pages =        {62-69},
  year =         {1992}
}
@InProceedings{MarNei:1991:WDAG,
  author =       {K. Marzullo and G. Neiger},
  title =        {{D}etection of {G}lobal {S}tate {P}redicates},
  booktitle =    PROC # " " # WDAG,
  pages =        {254-272},
  year =         {1991}
}
@Article{MarSab:1994:DC,
  author = {K. Marzullo and L. Sabel},
  title = {{E}fficient {D}etection of a {C}lass of {S}table {P}roperties},
  journal = DC,
  volume = {8},
  number = {2},
  pages = {81-91},
  year = {1994},
  url = "citeseer.nj.nec.com/marzullo94efficient.html"
}
@Article{Mat:1987:DC,
  author =   {F. Mattern},
  title =    {{Algorithms for Distributed Termination Detection}},
  journal =      DC,
  year =     {1987},
  OPTkey =   {},
  volume =   {2},
  number =   {3},
  pages =    {161-175},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Mat:1989:IPL,
  author =   {F. Mattern},
  title =    {{Global Quiescence Detection based on Credit Distribution
                   and Recovery}},
  journal =      IPL,
  year =     {1989},
  OPTkey =   {},
  volume =   {30},
  number =   {4},
  pages =    {195-200},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{Mat:1989:WDAG,
  author =   {F. Mattern},
  title =    {{Virtual Time and Global States of Distributed Systems}},
  booktitle =    "Parallel and Distributed Algorithms: " # PROC # " "
                  # WDAG,
  pages =    {215-226},
  year =     1989,
  publisher =    ES
}
@Article{Mat:1993:JPDC,
  author =       {F. Mattern},
  title =        {{E}fficient {A}lgorithms for {D}istributed {S}napshots and {G}lobal
                  {V}irtual {T}ime {A}pproximation},
  journal =      JPDC,
  volume =       {18},
  number =       {4},
  pages =        {423-434},
  year =         {1993},
  url =          {http://citeseer.nj.nec.com/mattern93efficient.html}
}
@Article{MatCap:1999:JSS,
  author =   {J. Matocha and T. Camp},
  title =    {{A Taxonomy of Distributed Termination Detection Algorithms}},
  journal =      JSS,
  year =     1999,
  volume =   43,
  number =   3,
  pages =    {207-221},
  month =    NOV
}
@Techreport{MatMeh+:1991:TR:32,
  author =       {F. Mattern and H. Mehl and A. Schoone and G. Tel},
  title =        {{Global Virtual Time Approximation with Distributed
                  Termination Detection Algorithms}},
  institution =  {University of Utrecht, The Netherlands},
  number =       {RUU-CS-91-32},
  year =         {1991},
  url =          {http://citeseer.nj.nec.com/mattern91global.html}
}
@Manual{MatMel+:1997:ISO,
  author =   {N. Mattos and J. Melton and J. Richey},
  title =    {Database Language SQL - Part 9: Management of
                  External Data (SQL/MED)},
  organization = {ISO working draft},
  month =    JUN,
  year =     1997
}
@InProceedings{McMLi:1993:COMPSAC,
  author =   {P. Li and B. McMillin},
  title =    {{Fault-Tolerant Distributed Deadlock Detection/Resolution}},
  booktitle =    PROC # " 17th " # COMPSAC,
  pages =    {224-230},
  year =     1993,
  month =    NOV
}
@InProceedings{MilCho:1988:ICDCS,
  author =   {B. P. Miller and J. Choi},
  title =    {{B}reakpoints and {H}alting in {D}istributed
                  {P}rograms},
  booktitle =    PROC # " 8th " # ICDCS,
  pages =    {316-323},
  year =     1988
}
@InProceedings{Mis:1983:PODC,
  author =   {J. Misra},
  title =    {{Detecting Termination of Distributed Computations using Markers}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # PODC,
  pages =    {290-294},
  year =     {1983},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@PhdThesis{Mit:2002:Thesis,
  author =       {N. Mittal},
  title =        {{T}echniques for {A}nalyzing {D}istributed {C}omputations},
  school =       UTA,
  year =         2002,
  month =        MAY,
  note =         {Available at \texttt{http://www.utdallas.edu/{\symbol{126}}neerajm}}
}
@InProceedings{MitGar:1998:ICDCS,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Consistency Conditions for Multi-Object Distributed Operations}},
  booktitle =    PROC # " 18th " # ICDCS,
  pages =    {582-589},
  year =     {1998},
  address =      {Amsterdam, The Netherlands},
  month =    MAY
}
@TechReport{MitGar:1998:TR:005,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Consistency Conditions for Multi-Object Distributed Operations}},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     1998,
  number =   {TR-PDS-1998-005},
  address =      {Austin, TX 78712}
}
@InProceedings{MitGar:2000:PODC,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Debugging Distributed Programs using Controlled Re-execution}},
  booktitle =    PROC # " 19th " # PODC,
  pages =    {239-248},
  year =     2000,
  address =  {Portland, Oregon},
  month =    JUL
}
@TechReport{MitGar:2000:TR:002,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Debugging Distributed Programs using Controlled Re-execution}},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     2000,
  number =   {TR-PDS-2000-002},
  address =  {Austin, TX 78712},
  month =    MAY
}
@InProceedings{MitGar:2001:DISC,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Computation Slicing: Techniques and Theory}},
  booktitle =    PROC # " " # DISC,
  pages =    {78-92},
  year =     2001,
  address =      {Lisbon, Portugal},
  month =    OCT
}
@InProceedings{MitGar:2001:ICDCS,
  author =   {N. Mittal and V. K. Garg},
  title =    {{On Detecting Global Predicates in Distributed Computations}},
  booktitle =    PROC # " 21st " # ICDCS,
  pages =    {3-10},
  year =     2001,
  address =      {Phoenix, Arizona},
  month =    APR,
  OPTnote =  {Available at
                  \texttt{http://www.cs.utexas.edu/users/neerajm/research.html}}
}
@TechReport{MitGar:2001:TR:002,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Computation Slicing: Techniques and Theory}},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     2001,
  number =   {TR-PDS-2001-002},
  OPTaddress =   {Austin, TX 78712},
  month =    APR,
  note =         {Available at \texttt{http://www.cs.utexas.edu/users/neerajm}}
}
@TechReport{MitGar:2001:TR:005,
  author =   {N. Mittal and V. K. Garg},
  title =    {{A Rigorous Proof of $O(n^2)$ Bound on the Number of Moves
                  for Stabilization of Dijkstra's 3-State Algorithm}},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {TR-PDS-2001-005},
  address =      {Austin, TX 78712},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{MitGar:2003:ICDCS,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Software Fault Tolerance of Distributed Programs using Computation Slicing}},
  booktitle =    PROC # " 23rd " # ICDCS,
  pages =    {105-113},
  year =     2003,
  address =  {Providence, Rhode Island},
  month =    MAY
}
@TechReport{MitGar:2003:TR:15,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Techniques and Applications of Computation Slicing}},
  institution =  DCS # ", " # UTD,
  year =     2003,
  number =   {UTDCS-15-03},
  OPTaddress =   {Richardson, TX 75083},
  month =    APR
}
@Article{MitGar:2004:DC,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Finding Missing Synchronization in a Distributed Computation using
                  Controlled Re-execution}},
  journal =      DC,
  year =     {2004},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  month =    MAR,
  note =     {Online First},
  OPTannote =    {}
}
@InProceedings{MitHsi:2000:ICDE,
  author =   {N. Mittal and H. Hsiao},
  title =    {{D}atabase {M}anaged {E}xternal {F}ile {U}pdate},
  booktitle =    PROC # " 17th " # ICDE,
  pages =    {557-564},
  year =     2001,
  address =  {Heidelberg, Germany},
  month =    APR
}
@InProceedings{MitSen+:2004:IPDPS,
  author =   {N. Mittal and A. Sen and V. K. Garg and R. Atreya},
  title =    {{Finding Satisfying Global States: All for One and One for All}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # IPDPS,
  OPTpages =     {},
  year =     {2004},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    APR,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{MitVen+:2004:DISC,
  author =   {N. Mittal and S. Venkatesan and S. Peri},
  title =    {{Message-Optimal and Latency-Optimal Termination Detection
                  Algorithms for Arbitrary Topologies}},
  booktitle =    PROC # " " # DISC,
  pages =        {290-304},
  year =     2004,
  address =      {Amsterdam, The Netherlands},
  month =    OCT
}
@TechReport{MitVen+:2004:TR,
  author =   {N. Mittal and S. Venkatesan and S. Peri},
  title =    {{Message-Optimal and Latency-Optimal Termination Detection
                  Algorithms for Arbitrary Topologies}},
  institution =  UTD,
  number =       {UTDCS-08-04},
  month =        FEB,
  year =     2004,
  note =     {Available at
                  \texttt{http://www.utdallas.edu/{\textasciitilde}neerajm/}}
}
@InProceedings{MurGar:1997:ICDCS,
  author =   {V. V. Murty and V. K. Garg},
  title =    {{C}haracterization of {M}essage {O}rdering
                  {S}pecifications and {P}rotocols},
  booktitle =    PROC # " 17th " # ICDCS,
  year =     1997,
  month =    MAY
}
@Article{Nas:1961:JLMS,
  author =   {C. Nash-Williams},
  title =    {{E}dge-{D}isjoint {S}panning {T}rees of {F}inite {G}raphs},
  journal =      JLMS,
  year =     1961,
  volume =   36,
  pages =    {445-450}
}
@InProceedings{NetBre+:1996:SPDT,
  author =   {R. Netzer and T. Brennan and S. Damodaran-Kamal},
  title =    {{D}ebugging {R}ace {C}onditions in
                  {M}essage-{P}assing {P}rograms},
  booktitle =    PROC # " " # SPDT,
  pages =    {31-40},
  year =     1996,
  month =    MAY
}
@Article{NetMil:1995:JS,
  author =   {R. H. B. Netzer and B. P. Miller},
  title =    {{O}ptimal {T}racing and {R}eplay for {D}ebugging
                  {M}essage-{P}assing {P}rograms},
  journal =  JS,
  year =     1995,
  volume =   8,
  number =   4,
  pages =    {371-388}
}
@Article{NetXu:1995:TPDS,
  author =   {R. H. B. Netzer and J. Xu},
  title =    {{N}ecessary and {S}ufficient {C}onditions for {C}onsistent
                  {G}lobal {S}napshots},
  journal =      TPDS,
  year =     1995,
  volume =   6,
  number =   2,
  pages =    {165-169},
  month =    FEB
}
@Unpublished{POTAwebsite,
  author =   {A. Sen and V. K. Garg},
  title =    {{P}artial {O}rder {T}race {A}nalyzer {(POTA)}},
  note =     {http://maple.ece.utexas.edu/{\textasciitilde}sen/POTA.html},
  OPTkey =   {},
  OPTmonth =     {},
  OPTyear =      {},
  OPTannote =    {}
}
@Article{PapWas+:1999:SIGMOD,
  author =   {M. Papiani and J. Wason and A. Dunlop and D. Nicole},
  title =    {{A} {D}istributed {S}cientific {A}rchive {U}sing the
                  {W}eb, {XML} and {SQL}/{MED}},
  journal =  {SIGMOD Record},
  volume =   {28},
  number =   {3},
  pages =    {56-62},
  month =    SEP,
  year =     {1999}
}
@Article{ParPop+:1983:TSE,
  author =   {D. S. Parker and G. J. Popek and G. Rudisin and A. Stoughton
                  and B. J. Walker and E. Walton and J. M. Chow and D. A. Edwards
                  and S. Kiser and C. S. Kline},
  title =    {{Detection of Mutual Inconsistency in Distributed Systems}},
  journal =      TSE,
  year =     {1983},
  OPTkey =   {},
  volume =   {9},
  number =   {3},
  pages =    {240-247},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{PerMit:2004:PDCS,
  author =   {S. Peri and N. Mittal},
  title =    {{On Termination Detection in an Asynchronous Distributed System}},
  booktitle =    PROC # " " # PDCS,
  pages =        {209-215},
  year =     2004,
  address =      {San Francisco, California},
  month =    SEP
}
@TechReport{PerMit:2004:TR,
  author =   {S. Peri and N. Mittal},
  title =    {{An Efficient Snapshot Protocol for a Dynamic System}},
  institution =  DCS # ", " # UTD,
  year =     {2004},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@TechReport{PerMit:2004:TR:15,
  author =   {S. Peri and N. Mittal},
  title =    {{On Termination Detection in an Asynchronous Distributed System}},
  institution =  DCS # ", " # UTD,
  year =     {2004},
  OPTkey =   {},
  OPTtype =      {},
  number =   {UTDCS-15-04},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{PlaBec+:1995:UWTC,
  author =   {J. S. Plank and M. Beck and G. Kingsley},
  title =    {{Libckpt: Transparent Checkpointing under UNIX}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # UWTC,
  pages =    {213-223},
  year =     {1995},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {New Orleans, Louisiana},
  month =    JAN,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@Misc{Pom:2000:TUT,
  OPTkey =   {},
  author =   {W. Torres-Pomales},
  title =    {{S}oftware {F}ault {T}olerance: {A} {T}utorial},
  OPThowpublished = {},
  OPTmonth =     {},
  year =     {2000},
  note =     {NASA Langley Research Center},
  OPTannote =    {}
}
@InProceedings{PraSin:1994:SPDP,
  author =   {R. Prakash and M. Singhal},
  title =    {{Maximal Global Snapshot with Concurrent Initiators}},
  booktitle =    PROC # " 6th " # SPDP,
  pages =    {344-351},
  year =     1994,
  address =      {Dallas, Texas},
  month =    OCT
}
@InProceedings{QueSif:1982:ISP,
  author =       {J. P. Queille and J. Sifakis},
  title =        {{S}pecification and {V}erification of {C}oncurrent {S}ystems in {CESAR}},
  address =      {New York},
  booktitle =    PROC # " 5th " # ISP,
  pages =        {337-351},
  publisher =    SV,
  series =       LNCS,
  volume =       137,
  year =         1982
}
@Article{Ran:1983:IPL,
  author =   {S. P. Rana},
  title =    {{A Distributed Solution of the Distributed Termination
                   Problem}},
  journal =      IPL,
  year =     {1983},
  OPTkey =   {},
  volume =   {17},
  number =   {1},
  pages =    {43-46},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{RaoAlv+:2000:KDE,
  author =       {S. Rao and L. Alvisi and H. Vin},
  title =        {{T}he {C}ost of {R}ecovery in {M}essage {L}ogging {P}rotocols},
  journal =      KDE,
  volume =       {12},
  number =       {2},
  year =         {2000},
  pages =        {160-173},
}
@Book{Ray:1988:JWS,
  author =       {M. Raynal},
  title =        {{D}istributed {A}lgorithms and {P}rotocols},
  publisher =    JWS,
  year =         {1988}
}
@Article{Ray:1989:TrCS,
  author =   {K. Raymond},
  title =    {{A} {T}ree based {A}lgorithm for {D}istributed {M}utual {E}xclusion},
  journal =      TrCS,
  year =     1989,
  volume =   7,
  number =   1,
  pages =    {61-77}
}
@Article{RicAgr:1981:CACM,
  author =       {G. Ricart and A. K. Agrawala},
  title =        {{An Optimal Algorithm for Mutual Exclusion in Computer Networks}},
  journal =      CACM,
  volume =       {24},
  number =       {1},
  year =         {1981},
  pages =        {9-17},
  publisher =    {ACM Press},
  month =        JAN,
}
@Article{Riv:1974:AMS,
  author =   {I. Rival},
  title =    {{M}aximal {S}ublattices of {F}inite {D}istributive {L}attices {II}},
  journal =      PROC # " " # AMS,
  year =     1974,
  volume =   44,
  number =   2,
  pages =    {263-268}
}
@Book{STA,
  author =       {R. Stanley},
  title =        {{E}numerative {C}ombinatorics {V}olume 1},
  publisher =    {Wadsworth and Brookes/Cole},
  address =      {Monterey, California},
  year =         1986
}
@Unpublished{SafDij:1987:998,
  author =   {E. W. Dijkstra},
  title =    {{Shmuel Safra's Version of Termination Detection}},
  note =     {EWD Manuscript 998. Available at \texttt{http://www.cs.utexas.edu/users/EWD}},
  OPTkey =   {},
  OPTmonth =     {},
  year =     {1987},
  OPTannote =    {}
}
@TechReport{Sai:2002:TR:51,
  author =   {Y. Saito},
  title =    {{Unilateral Version Vector Pruning using Loosely Synchronized Clocks}},
  institution =  HPL,
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {HPL-2002-51},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{SchGet:1987:TOG,
  author =       {R.W. Scheifler and J. Gettys},
  title =        {{The X Window System}},
  journal =      TOG,
  month =        APR,
  year =         1987,
  volume =       5,
  number =       2,
  pages =        {79-109}
}
@Article{SchMat:1994:DC,
  author =   {R. Schwartz and F. Mattern},
  title =    {{D}etecting {C}ausal {R}elationships in {D}istributed  {C}omputations:
                  {I}n {S}earch of the {H}oly {G}rail},
  journal =      DC,
  year =     1994,
  volume =   7,
  number =   3,
  pages =    {149-174}
}
@InProceedings{SchWyl:1991:SOSP,
  author =   {F. Schmuck and J. Wyllie},
  title =    {{Experience with Transactions in QuickSilver}},
  booktitle =    PROC # " 13th " # SOSP,
  pages =    {239-253},
  year =     1991,
  month =    OCT
}
@InProceedings{SenGar:2002:IPDPS,
  author =   {A. Sen and V. K. Garg},
  title =    {{D}etecting {T}emporal {L}ogic {P}redicates in the {H}appened-{B}efore {M}odel},
  booktitle =    PROC # " " # IPDPS,
  year =     2002,
  address =      {Florida},
  month =    APR
}
@TechReport{SenGar:2002:TR:001,
  author =   {A. Sen and V. K. Garg},
  title =    {{A}utomatic {G}eneration of {C}omputation {S}lices for
                  {D}etecting {T}emporal {L}ogic {P}redicates},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     {2003},
  OPTkey =   {},
  OPTtype =      {},
  number =   {TR-PDS-2003-001},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{SenGar:2003:OPODIS,
  author =       {A. Sen and V. K. Garg},
  title =        {{Detecting Temporal Logic Predicates in Distributed
                   Programs using Computation Slicing}},
  booktitle =    PROC # " " # OPODIS,
  OPTpages =     {},
  month =        DEC,
  year =         {2003}
}
@InProceedings{SenGar:2003:RV,
  author =       {A. Sen and V. K. Garg},
  title =        {{P}artial {O}rder {T}race {A}nalyzer ({POTA}) for
                  {D}istributed {P}rograms},
  booktitle =    PROC # " Third " # RV,
  OPTseries =    {Electronic Notes in Theoretical Computer Science},
  volume =       {89},
  issue =        {2},
  publisher =    {Elsevier},
  year =         {2003}
}


@InProceedings{ShaFra:1986:ICALP,
  author =   {N. Shavit and N. Francez},
  title =    {{A New Approach to Detection of Locally Indicative Stability}},
  booktitle =    PROC # " " # ICALP,
  pages =    {344-358},
  year =     1986,
  address =      {Rennes, France}
}


@TechReport{ShaTou:1984:TR:624,
  author =   {A. Shah and S. Toueg},
  title =    {{Distributed Snapshots in spite of Failures}},
  institution =  DCS # ", " # CORNELL,
  year =     1984,
  number =   {TR84-624},
  address =      {Ithaca, NY},
  month =    JUL,
  note =     {(Revised February 1985)}
}


@InProceedings{SheDea:2002:WETICE,
  author =       {J. S. Sherif and T. G. Dearmond},
  title =        {{Intrusion Detection: Systems and Models}},
  booktitle =    PROC # " " # WETICE,
  pages =        {115-136},
  month =        JUN,
  year =         {2002},
  address =      {Pittsburgh, Pennsylvania}
}


@Book{SinShi:1994:Book,
  author =       {M. Singhal and N. G. Shivaratri},
  title =        {{Advanced Concepts in Operating Systems}},
  publisher =    MH # " and " # MIT,
  year =         {1994},
  ISBN =         {0-07-057572-X}
}

@InProceedings{SkaMit+:1999:PDCS,
  author =   {C. Skawratananond and N. Mittal and V. K. Garg},
  title =    {{A} {L}ightweight {A}lgorithm for {C}ausal {M}essage
                  {O}rdering in {M}obile {C}omputing {S}ystems},
  booktitle =    PROC # " 12th " # PDCS,
  pages =    {245-250},
  year =     {1999},
  address =      {Florida}
}


@Unpublished{SolDes,
  author =   {Solar Designer},
  title =    {{Root Programs and Links}},
  note =     {Available at \texttt{http://www.openwall.com/linux/}},
  OPTkey =   {},
  OPTmonth =     {},
  OPTyear =      {},
  OPTannote =    {}
}


@Unpublished{SolDes:OP,
  author =   {Openwall Project},
  title =    {{Linux Kernel Patch}},
  note =     {\textsf{http://www.openwall.com/linux}},
  OPTkey =   {},
  OPTmonth =     {},
  OPTyear =      {},
  OPTannote =    {}
}


@InProceedings{SpeKea:1986:ICDCS,
  author =   {M. Spezialetti and P. Kearns},
  title =    {{Efficient Distributed Snapshots}},
  booktitle =    PROC # " 6th " # ICDCS,
  pages =    {382-388},
  year =     1986
}


@Article{SpiBra:1987:DAM,
  author =   {J. Spinrad and A. Brandstadt and L. Stewart},
  title =    {{Bipartite Permutation Graphs}},
  journal =      DAM,
  year =     1987,
  volume =   18,
  pages =    {279-292}
}



@InProceedings{SriSiv:2002:ICPDCS,
  author =   {N. Sridhar and P. A. G. Sivilotti},
  title =    {{L}azy {S}napshots},
  booktitle =    PROC # " 14th " # ICPDCS,
  pages =    {96-101},
  year =     {2002},
  OPTeditor =    {S.G. Akl and T.Gonzalez},
  address =      {Cambridge, MA},
  month =    NOV,
  OPTorganization = {IASTED},
  OPTpublisher =    {ACTA Press},
  OPTurl =          {http://citeseer.nj.nec.com/sridhar02lazy.html}
}



@InProceedings{SroSch+:1998:WNTS,
  author =   {J. Srouji and P. Schuster and M. Bach and Y. Kuzmin},
  title =    {{A Transparent Checkpoint Facility on NT}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 2nd " # WNTS,
  OPTpages =     {},
  year =     {1998},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Seattle, Washington},
  month =    {August},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{Sta:2001:PH,
  author =   {W. Stallings},
  title =    {{O}perating {S}ystems: {I}nternals and {D}esign {P}rinciples},
  publisher =    PH,
  year =     2001
}




@InCollection{StoLiu:1998:CAV,
  author =   {S. D. Stoller and Y. A. Liu},
  title =    {{E}fficient {S}ymbolic {D}etection of {G}lobal
                  {P}roperties in {D}istributed {S}ystems},
  booktitle =    PROC # " 10th " # CAV,
  pages =    {357-368},
  publisher =    {Springer-Verlag},
  year =     1998,
  editor =   {Alan J. Hu and Moshe Y. Vardi},
  volume =   1427,
  series =   LNCS
}



@InProceedings{StoSch:1995:WDAG,
  author =   {S. D. Stoller and F. Schneider},
  title =    {{F}aster {P}ossibility {D}etection by {C}ombining
                  {T}wo {A}pproaches},
  booktitle =    PROC # " " # WDAG,
  pages =        {318-332},
  year =     1995,
  volume =       {972},
  series =       LNCS,
  address =  {France},
  month =    SEP
}


@InProceedings{StoUnn+:2000:CAV,
  author =   {S. D. Stoller and L. Unnikrishnan and Y. A. Liu},
  title =    {{Efficient Detection of Global Properties in
                  Distributed Systems Using Partial-Order Methods}},
  booktitle =    PROC # " 12th " # CAV,
  pages =    {264-279},
  year =     2000,
  volume =   1855,
  series =   LNCS,
  month =    JUL,
  publisher =    {Springer-Verlag}
}



@InProceedings{Stu:2002:DISC,
  author =   {G. Stupp},
  title =    {{Stateless Termination Detection}},
  booktitle =    PROC # " 16th " # DISC,
  pages =    {163-172},
  year =     2002,
  address =      {Toulouse, France}
}


@InProceedings{Tai:1997:ICDCS,
  author =   {K. Tai},
  title =    {{R}ace {A}nalysis of {T}races of {A}synchronous
                  {M}essage-{P}assing {P}rograms},
  booktitle =    PROC # " 17th " # ICDCS,
  pages =    {261-268},
  year =     1997
}



@PhdThesis{Tar:2000:Thesis,
  author =   {A. Tarafdar},
  title =    {{S}oftware {F}ault {T}olerance in {D}istributed {S}ystems
                  {U}sing {C}ontrolled {R}e-execution},
  school =   {The University of Texas at Austin},
  year =     2000,
  month =    AUG
}


@InProceedings{TarGar:1998:ICDCS,
  author =   {A. Tarafdar and V. K. Garg},
  title =    {{A}ddressing {F}alse {C}ausality while {D}etecting
                  {P}redicates in {D}istributed {P}rograms},
  booktitle =    PROC # " 9th " # ICDCS,
  pages =    {94-101},
  year =     1998,
  address =  {Amsterdam, The Netherlands},
  month =    MAY
}

@InProceedings{TarGar:1998:SPDP,
  author =   {A. Tarafdar and V. K. Garg},
  title =    {{P}redicate {C}ontrol for {A}ctive {D}ebugging of
                  {D}istributed {P}rograms},
  booktitle =    PROC # " 9th " # SPDP,
  pages =        {763-769},
  year =     1998,
  address =  {Orlando}
}

@InProceedings{TarGar:1999:DISC,
  author =   {A. Tarafdar and V. K. Garg},
  title =    {{S}oftware {F}ault {T}olerance of {C}oncurrent
                  {P}rograms {U}sing {C}ontrolled {R}e-execution},
  booktitle =    PROC # " 13th " # DISC,
  pages =    {210-224},
  year =     1999,
  address =  {Bratislava, Slovak Republic},
  month =    SEP
}


@Book{Tel:2000:CUP,
  author =   {G. Tel},
  title =    {{Introduction to Distributed Algorithms}},
  publisher =    CUP # "~(US Server)",
  year =     2000,
  edition =      {Second},
  month =    SEP
}

@Article{TelMat:1993:TOPLAS,
  author =   {G. Tel and F. Mattern},
  title =    {{The Derivation of Distributed Termination Detection Algorithms from Garbage Collection Schemes}},
  journal =      TOPLAS,
  year =     1993,
  volume =   15,
  number =   1,
  pages =    {1-35},
  month =    JAN
}



@Article{Tip:1995:JPL,
  author =   {F. Tip},
  title =    {{A Survey of Program Slicing Techniques}},
  journal =      JPL,
  year =     1995,
  volume =   3,
  number =   3,
  pages =    {121-189}
}

@InProceedings{TomGar:1993:WPDS,
  author =   {A. I. Tomlinson and V. K. Garg},
  title =    {{An Algorithm for Minimally Latent Global Virtual Time}},
  booktitle =    PROC # " 7th " # WPDS,
  pages =        {35-42},
  year =     1993,
  address =  {San Diego, California},
  month =    MAY
}


@InProceedings{TomGar:1994:CSE,
  author =   {A. I. Tomlinson and V. K. Garg},
  title =    {{Maintaining Global Assertions in Distributed Systems}},
  booktitle =    CSE,
  pages =    {257-272},
  year =     1994,
  publisher =    TMH
}


@Article{TomGar:1994:JPDC,
  author =   {A. I. Tomlinson and V. K. Garg},
  title =    {{M}onitoring {F}unctions on {G}lobal {S}tates of
                  {D}istributed {P}rograms},
  journal =  JPDC,
  year =     1997,
  volume =       {41},
  number =       {},
  pages  =       {173-189},
  month =        MAR,
  OPTnote =  "A revised version of ``Detecting Relational Global
                  Predicates in Distributed Systems'', In " # PROC #
                  " " # WPDD # ", San Diego, California, " # MAY # "
                  1993, pages 21-31"
}


@InProceedings{TomGar:1995:FSTTCS,
  author =       {A. I. Tomlinson and V. K. Garg},
  title =        {{Observation of Software for Distributed Systems with RCL}},
  booktitle =    PROC # " 15th " # FSTTCS,
  pages =        {195-209},
  year =         {1995},
  url =          {http://citeseer.nj.nec.com/tomlinson95observation.html}
}

@Article{TomGar:1997:JPDC,
  author =   {A. I. Tomlinson and V. K. Garg},
  title =    {{M}onitoring {F}unctions on {G}lobal {S}tates of
                  {D}istributed {P}rograms},
  journal =  JPDC,
  year =     1997,
  volume =       {41},
  number =       {2},
  pages  =       {173-189},
  month =        MAR,
  OPTnote =  "A revised version of ``Detecting Relational Global
                  Predicates in Distributed Systems'', In " # PROC #
                  " " # WPDD # ", San Diego, California, " # MAY # "
                  1993, pages 21-31"
}


@Book{Tro:1992:JHUP,
  author =   {W. T. Trotter},
  title =    {{C}ombinatorics and {P}artially {O}rdered {S}ets: {D}imension {T}heory},
  publisher =    JHUP,
  year =     1992,
  address =      {Baltimore, MD}
}

@article{Tse:1995:JPDC,
  author =       {Y.-C. Tseng},
  title =        {{Detecting Termination by Weight-Throwing in a Faulty Distributed System}},
  journal =      JPDC,
  volume =       {25},
  number =       {1},
  pages =        {7-15},
  year =         "1995",
  OPTnote =      "previous label was Tse:1992:JPDC"
}

@Article{TseTan:2001:TPDS,
  author =       {Y.-C. Tseng and C.-C. Tan},
  title =        {{On Termination Detection Protocols in a Mobile Distributed
                   Computing Environment}},
  journal =      TPDS,
  year =         2001,
  volume =       12,
  number =       6,
  pages =        {558-566}
}


@InProceedings{TsyYee:2003:USS,
  author =   {E. Tsyrklevich and B. Yee},
  title =    {{Dynamic Detection and Prevention of Race Conditions in File Accesses}},
  booktitle =    PROC # " 12th " # USS,
  pages =    {243-255},
  year =     2003,
  month =    AUG
}

@Article{Tur:1984:DAM,
  author =   {G. Turan},
  title =    {{Succinct Representations of Graphs}},
  journal =      DAM,
  year =     1984,
  volume =   8,
  pages =    {289-294}
}

@Book{Vah:1996:PH,
  author =   {U. Vahalia},
  title =    {Unix Internals: The New Frontiers},
  publisher =    PH,
  year =     1996,
  month =    JAN
}

@Article{ValTar+:1982:SIAMJC,
  author =   {J. Valdes and R. E. Tarjan and E. L. Lawler},
  title =    {{T}he {R}ecognition of {S}eries-{P}arallel {D}igraphs},
  journal =      SIAMJC,
  year =     1982,
  volume =   11,
  pages =    {298-314}
}

@Article{Ven:1989:TR,
  author =   {S. Venkatesan},
  title =    {{Reliable Protocols for Distributed Termination Detection}},
  journal =      TR,
  year =     1989,
  volume =   38,
  number =   1,
  pages =    {103-110},
  month =    APR
}




@Article{Ven:1995:TOPLAS,
  author =   {G. Venkatesh},
  title =    {{Experimental Results from Dynamic Slicing of C Programs}},
  journal =      TOPLAS,
  year =     1995,
  volume =   17,
  number =   2,
  pages =    {197-216}
}







@Article{SuzKas:1985:TrCS,
  author =   {I. Suzuki and T. Kasami},
  title =    {{A Distributed Mutual Exclusion Algorithm}},
  journal =      TrCS,
  year =     1985,
  volume =   3,
  number =   4,
  pages =    {344-349}
}



@Article{VenDat:1995:TSE,
  author =   {S. Venkatesan and B. Dathan},
  title =    {{T}esting and {D}ebugging {D}istributed {P}rograms {U}sing
                  {G}lobal {P}redicates},
  journal =      TSE,
  year =     1995,
  volume =   21,
  number =   2,
  pages =    {163-177},
  month =    FEB
}


@InProceedings{VieBlo+:2000:CSAC,
  author =   {J. Viega, J. Bloch, T. Kohno and G. McGraw},
  title =    {{ITS4: A Static Vulnerability Scanner for C and C++ Code}},
  booktitle =    PROC # " " # CSAC,
  year =     2000,
  month =    DEC
}


@InProceedings{WalGar:1991:WPDD,
  author =       {B. Waldecker and V. K. Garg },
  title =        {{U}nstable {P}redicate {D}etection in {D}istributed
                  {P}rogram {D}ebugging},
  booktitle =    PROC # " " # WPDD,
  address =  {Santa Cruz, California},
  pages =        {276-278},
  month =    MAY,
  year =     1991
}

@Article{Wan:1997:TC,
  author =   {Y.-M. Wang},
  title =    {{C}onsistent {G}lobal {C}heckpoints that {C}ontain a
                  {G}iven {S}et of {L}ocal {C}heckpoints},
  journal =      TC,
  year =     1997,
  volume =   46,
  number =   4,
  pages =    {456-468},
  month =    APR
}


@InProceedings{WanDam+:1997:ICDCS,
  author =       {Y. M. Wang and O. P. Damani and V. K. Garg},
  title =        {{D}istributed {R}ecovery with {K}-{O}ptimistic Logging},
  pages =        {60-67},
  booktitle =    PROC # " 17th " # ICDCS,
  address =      {Baltimore, Maryland},
  month =        JUN,
  publisher =    {IEEE},
  address =  {Washington - Brussels - Tokyo},
  year =         1997,
}



@Article{WanHua+:1997:TC,
  author =   {Y.-M. Wang and Y. Huang and W. K. Fuchs and
                  C. Kintala and G. Suri},
  title =    {{P}rogressive {R}etry for {S}oftware {F}ailure
                  {R}ecovery in {M}essage-{P}assing {A}pplications},
  journal =  TC,
  year =     1997,
  volume =   46,
  number =   10,
  pages =    {1137-1141},
  month =    OCT
}



@InProceedings{WanMay:2004:IPDPS,
  author =   {X. Wang and J. Mayo},
  title =    {{A General Model for Detecting Termination in Dynamic Systems}},
  booktitle =    PROC # " 18th " # IPDPS,
  year =     2004,
  address =      {Santa Fe, New Mexico},
  month =    APR
}


@Article{Wei:1982:CACM,
  author =   {M. Weiser},
  title =    {{P}rogrammers {U}se {S}lices when {D}ebugging},
  journal =  CACM,
  year =     1982,
  volume =   25,
  number =   7,
  pages =    {446-452}
}

@Article{WuJou:2000:CDS,
  author =   {K.-P. Wu and Y.-J. Joung},
  title =    {{Asynchronous Group Mutual Exclusion in Ring Networks}},
  OPTcrossref =  {},
  OPTkey =   {},
  journal =      CDS,
  pages =    {1-8},
  year =     {2000},
  OPTeditor =    {},
  volume =   {147},
  number =   {1}
}



@Article{Yan:1982:SIAMHADM,
  author =   {M. Yannakakis},
  title =    {{T}he {C}omplexity of the {P}artial {O}rder {D}imension {P}roblem},
  journal =      SIAMJADM,
  year =     1982,
  volume =   3,
  pages =    {351-358}
}




@InProceedings{ZibGil:1997:OOPSLA,
  author =   {Y. Zibin and Y. Gil},
  title =    {{E}fficient {S}ubtyping {T}ests with {PQ}-{E}ncoding},
  booktitle =    PROC # " 16th Annual " # OOPSLA,
  pages =    {96-107},
  year =     1997,
  address =      {Tampa Bay, Florida},
  month =    OCT
}

@Manual{iFS:1999,
  author =   {Oracle},
  title =    {iFS: Oracle Internet File System},
  note =     {\\ {\sf
                  http://www.oracle.com/database/options/ifs.html}},
  year =     1999
}

@InProceedings{WuLai+:1992:ICPADS,
  author =   {L.-F. Wu and T.-H. Lai and Y.-C. Tseng},
  title =    {{Consensus and Termination Detection in the Presence of Faulty Processes}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICPADS,
  pages =    {267-274},
  year =     {1992},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Hsinchu, Taiwan},
  month =    DEC,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{DwoLyn+:1988:JACM,
  author =       {C. Dwork and N. Lynch and L. Stockmeyer},
  title =        {{Consensus in the presence of partial synchrony}},
  OPTcrossref =  "",
  OPTkey =       "",
  journal =      JACM,
  year =         "1988",
  volume =       "35",
  number =       "2",
  pages =        {288-323},
  month =        APR,
  OPTnote =      "",
  annote =       "The authors study practically motivated models of
                  synchrony that lie between fully asynchronous and
                  fully synchronous systems in which consensus shall
                  be achieved. The models of partial synchrony studied
                  include: (1) upper bounds on processor speeds and
                  message latency exist but are unknown, and (2) upper
                  bounds exists and are known, but only hold after
                  some unknown time (eventually). In both cases
                  consensus with different resiliency can be achieved."
}


@InProceedings{DelFau+:2004:PODC,
  author =   {C. Delporte-Gallet and H. Fauconnier and R. Guerraoui and
                  V. Hadzilacos and P. Kouznetsov and S. Toueg},
  title =    {{The Weakest Failure Detector to Solve Certain Fundamental Problems
                   in Distributed Computing}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # PODC,
  OPTpages =     {},
  year =     {2004},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {St. Johns, Newfoundland, Canada},
  month =    JUL,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{MitGae+:2004:TR:37,
  author =   {N. Mittal and F. G{\"a}rtner and S. Venkatesan and L. D. Penso},
  title =    {{ Detecting Termination in a Crash-Prone Distributed System}},
  institution =  DCS # ", " # UTD,
  year =     {2004},
  OPTkey =   {},
  OPTtype =      {},
  number =   {UTDCS-37-04},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{HurMiz+:1998:TSE,
  author =       {M. Hurfin and M. Mizuno and M. Singhal and M. Raynal},
  title =        {Efficient Distributed Detection of Conjunctions of Local Predicates},
  journal =      TSE,
  volume =       {24},
  number =       {8},
  year =         {1998},
  issn =         {0098-5589},
  pages =        {664--677},
  doi =          {http://dx.doi.org/10.1109/32.707701},
  publisher =    {IEEE Press},
}

@Book{Lyn:1996:MK,
  author =   {N. Lynch},
  OPTeditor =    {},
  title =    {{Distributed Algorithms}},
  publisher =    MK,
  year =     {1996},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{Awe:1987:STOC,
  author =       {B. Awerbuch},
  title =        {{Optimal Distributed Algorithms for Minimum Weight Spanning Tree, Counting,
                   Leader Election, and Related Problems}},
  booktitle =    PROC # " 19th " # STOC,
  year =         {1987},
  pages =        {230-240},
  address =      {New York, New York, United States},
  publisher =    {ACM Press},
}

@Article{SchSan:1994:DC,
  author =   {A. Schiper and A. Sandoz},
  title =    {{Strong Stable Properties in Distributed Systems}},
  journal =      DC,
  year =     {1994},
  OPTkey =   {},
  volume =   {8},
  number =   {2},
  pages =    {93-103},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{SinKal+:1993:TR:93-11,
  author =   {A. Sinha and L. Kal{\'e} and B. Ramkumar},
  title =    {{A Dynamic and Adaptive Quiescence Detection Algorithm}},
  institution =  PPL # ", " #  DCS # ", "  # UIUC,
  year =     {1993},
  OPTkey =   {},
  OPTtype =      {},
  number =   {93-11},
  OPTaddress =   {Urbana-Champaign, IL 61801},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ChaMis:1986:TOPLAS,
  author =   {K. M. Chandy and J. Misra},
  title =    {{An Example of Stepwise Refinement of Distributed Programs: Quiescence Detection}},
  journal =      TOPLAS,
  year =     {1986},
  OPTkey =   {},
  volume =   {8},
  number =   {3},
  pages =    {326-343},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{KshSin:1994:TSE,
  author =   {A. D. Kshemkalyani and M. Singhal},
  title =    {{Efficient Detection and Resolution of Generalized Distributed Deadlocks}},
  journal =      TSE,
  year =     {1994},
  OPTkey =   {},
  volume =   {20},
  number =   {1},
  pages =    {43-54},
  month =    JAN,
  OPTnote =      {},
  OPTannote =    {}
}



@Article{BraTou:1987:DC,
  author =   {G. Bracha and S. Toueg},
  title =    {{Distributed Deadlock Detection}},
  journal =      DC,
  year =     {1987},
  OPTkey =   {},
  volume =   {2},
  number =   {3},
  pages =    {127-138},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Kna:1987:CS,
  author =   {E. Knapp},
  title =    {{Deadlock Detection in Distributed Databases}},
  journal =      CS,
  year =     {1987},
  OPTkey =   {},
  volume =   {19},
  number =   {4},
  pages =    {303-328},
  month =    DEC,
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{LynMal+:2002:WPPS,
  author =   {N. Lynch and D. Malkhi and D. Ratajczak},
  title =    {{Atomic Data Access in Content Addressable Networks}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 1st " # WPPS,
  pages =    {295-305},
  year =     {2002},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    MAR,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{LiMis+:2004:DISC,
  author =   {X. Li and J. Misra and C. G. Plaxton},
  title =    {{Active and Concurrent Topology Maintenance}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # DISC,
  OPTpages =     {},
  year =     {2004},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{ZhaHua+:2003:SAC,
  author =   {B. Y. Zhao and L. Huang and J. Stribling and S. C. Rhea and A. D. Joseph and J. Kubiatowicz},
  title =    {{Tapestry: A Resilient Global-Scale Overlay for Service Deployment}},
  journal =      SAC,
  year =     {2003},
  OPTkey =   {},
  volume =   {22},
  number =   {1},
  pages =    {41-53},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{StoMor+:2003:TN,
  author =   {I. Stoica and R. Morris and D. Liben-Nowell and D. R. Karger and M. F. Kaashoek
                  and F. Dabek and H. Balakrishnan},
  title =    {{Chord: A Scalable Peer-to-Peer Lookup Service for Internet Applications}},
  journal =      TN,
  year =     {2003},
  OPTkey =   {},
  volume =   {11},
  number =   {1},
  pages =    {17-32},
  month =    FEB,
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{AspSha:2003:SDA,
  author =   {J. Aspnes and G. Shah},
  title =    {{Skip Graphs}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 14th Annual " # SDA,
  pages =    {384-393},
  year =     {2003},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    JAN,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{BanMay:2004:SIU,
  author =   {S. Bansod and J. Mayo},
  title =    {{A Distributed Algorithm for Unstable Global Predicate Evaluation with Approximately Synchronized Clocks}},
  journal =      SIU,
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {2},
  pages =    {151-168},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Unpublished{AgaGar:2004:TR,
  author =   {A. Agarwal and V. K. Garg},
  title =    {{Chain Clock: Efficient Causality Tracking for Shared Memory Systems}},
  note =     "Submitted to the " # ICDCS,
  OPTkey =   {},
  month =    JUN,
  year =     {2005},
  OPTannote =    {}
}



@Article{Lee:2004:TSE,
  author =   {S. Lee},
  title =    {{Fast, Centralized Detection and Resolution of Distributed Deadlocks in the
                   Generalized Model}},
  journal =      TSE,
  year =     {2004},
  OPTkey =   {},
  volume =   {30},
  number =   {9},
  pages =    {561-573},
  month =    SEP,
  OPTnote =      {},
  OPTannote =    {}
}


@Article{BouTro:1998:TPDS,
  author =   {A. Boukerche and C. Tropper},
  title =    {{A Distributed Graph Algorithm for the Detection of Local Cycles and Knots}},
  journal =      TPDS,
  year =     {1998},
  OPTkey =   {},
  volume =   {9},
  number =   {8},
  pages =    {748-757},
  month =    AUG,
  OPTnote =      {},
  OPTannote =    {}
}



@InProceedings{CheDen+:1996:ICDCS,
  author =   {S. Chen and Y. Deng and P. C. Attie and W. Sun},
  title =    {{Optimal Deadlock Detection in Distributed Systems based on
                   Locally Constructed Wait-For Graphs}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICDCS,
  pages =    {613-619},
  year =     {1996},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    MAY,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hol:1972:CS,
  author =   {R. C. Holt},
  title =    {{Some Deadlock Properties of Computer Systems}},
  journal =      CS,
  year =     {1972},
  OPTkey =   {},
  volume =   {4},
  OPTnumber =    {},
  pages =    {179-195},
  month =    SEP,
  OPTnote =      {},
  OPTannote =    {}
}


@Article{KshSin:1999:KDE,
  author =   {A. D. Kshemkalyani and M. Singhal},
  title =    {{A One-Phase Algorithm to Detect Distributed Deadlocks in
                   Replicated Databases}},
  journal =      KDE,
  year =     {1999},
  OPTkey =   {},
  volume =   {11},
  number =   {6},
  pages =    {880-895},
  month =    NOV,
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{ManSin:2002:ICPP,
  author =   {D. Manivannan and M. Singhal},
  title =    {{A Distributed Algorithm for Knot Detection in a Distributed Graph}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICPP,
  OPTpages =     {},
  year =     {2002},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ManSin:2003:TPDS,
  author =   {D. Manivannan and M. Singhal},
  title =    {{An Efficient Distributed Algorithm for Detecting Knots and
                   Cycles in a Distributed Graph}},
  journal =      TPDS,
  year =     {2003},
  OPTkey =   {},
  volume =   {14},
  OPTnumber =    {10},
  pages =    {961-972},
  month =    OCT,
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Sin:1989:Com,
  author =   {M. Singhal},
  title =    {{Deadlock Detection in Distributed Systems}},
  journal =      Com,
  year =     {1989},
  OPTkey =   {},
  volume =   {22},
  OPTnumber =    {},
  pages =    {37-48},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{KshSin:1994:JPDC,
  author =   {A. D. Kshemkalyani and M. Singhal},
  title =    {{On Characterization and Correctness of Distributed Deadlock Detection}},
  journal =      JPDC,
  year =     {1994},
  OPTkey =   {},
  volume =   {22},
  number =   {1},
  pages =    {44-59},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{JagVas:1983:TSE,
  author =   {J. R. Jagannathan and R. Vasudevan},
  title =    {{Comments on ``Protocols for Deadlock Detection in
                  Distributed Database Systems''}},
  journal =      TSE,
  year =     {1983},
  OPTkey =   {},
  volume =   {9},
  number =   {3},
  pages =    {371},
  month =    MAY,
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Awe:1985:JACM,
  author =   {B. Awerbuch},
  title =    {{Complexity of Network Synchronization}},
  journal =      JACM,
  year =     {1985},
  OPTkey =   {},
  volume =   {32},
  number =   {4},
  pages =    {804-823},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@inproceedings{XiaPlax:2002:POMC,
 author = {Xiaozhou Li and C. Greg Plaxton},
 title = {On name resolution in peer-to-peer networks},
 booktitle = {POMC '02: Proceedings of the second ACM international workshop on Principles of mobile computing},
 year = {2002},
 isbn = {1-58113-511-4},
 pages = {82--89},
 location = {Toulouse, France},
 doi = {http://doi.acm.org/10.1145/584490.584507},
 publisher = {ACM Press},
 address = {New York, NY, USA},
 }

@URL{dist,
  author =       {},
  title =        "www.distributed.net/rc5",
  howpublished = {},
  year =         "2002",
  month =        "Dec",
  note =         {},
  abstract =     {},
  keywords =     {},
  source =       {},
  file = F
}

@CONFERENCE{SatNeer:2005:FSTTCS,
  author =       {Sathya Peri and Neeraj Mittal},
  title =        {Monitoring Stable Properties in Dynamic Peer-to-Peer Distributed Systems},
  booktitle =    PROC # " 25th " # FSTTCS,
  year =         {2005},
  pages  =       {420-431},
  address =      {Hyderabad, India},
  month =        {December},
  note =         {},
  key =          {},
  crossref =     {},
  annote =       {},
}

@TECHREPORT{BalHelPier:2004:TR,
  AUTHOR =       {R. Baldoni and J. Helary and S. Tucci Piergiovanni},
  TITLE =        {Maintaining group connectivity in dynamic asynchronous distributed systems},
  INSTITUTION =  {``Dipartimento di Informatica e Sistemistica, A.Ruberti, Universit?? di Roma la Sapienza"},
  YEAR =         {2004},
  doi=           {"http://www.dis.uniroma1.it/~midlab"},
}

@article{PageJacChen:1993:TPDS,
 author = {I. Page and T. Jacob and E. Chern},
 title = {Fast Algorithms for Distributed Resource Allocation},
 journal = {IEEE Trans. Parallel Distrib. Syst.},
 volume = {4},
 number = {2},
 year = {1993},
 issn = {1045-9219},
 pages = {188--197},
 doi = {http://dx.doi.org/10.1109/71.207594},
 publisher = {IEEE Press},
 address = {Piscataway, NJ, USA},
}

@article{ChoiSing:1995:TOPLAS,
 author = {Manhoi Choy and Ambuj K. Singh},
 title = {Efficient fault-tolerant algorithms for distributed resource allocation},
 journal = {ACM Trans. Program. Lang. Syst.},
 volume = {17},
 number = {3},
 year = {1995},
 issn = {0164-0925},
 pages = {535--559},
 doi = {http://doi.acm.org/10.1145/203095.203101},
 publisher = {ACM Press},
 address = {New York, NY, USA},
 }

@TECHREPORT{SatNeer:2006:TR,
  AUTHOR =       {Sathya Peri and Neeraj Mittal},
  TITLE =        {Lower bounds on Departures for Dynamic Asynchronous Peer-to-Peer systems},
  INSTITUTION =  {University of Texas at Dallas},
  YEAR =         {2006},
}

@INPROCEEDINGS{WeidPagPerv:1991:SPDP,
  AUTHOR =       {Weidman.E.B and Page.I.P and Pervin.W.J},
  TITLE =        {{Explicit dynamic exclusion algorithm}},
  BOOKTITLE =    {Proceedings of the Third IEEE Symposium on Parallel and Distributed Processing},
  YEAR =         {1991},
  pages =        {142-149},
  month =        {DEC},
  organization = {IEEE},
}

@INPROCEEDINGS{LynMalRata:2002:IPTPS,
  AUTHOR =       {N. Lynch and D. Malkhi and D. Ratajczak},
  TITLE =        {{Atomic Data Access in Content Addressable Networks}},
  BOOKTITLE =    {Proceedings for the 1st International Workshop on Peer-to-Peer Systems (IPTPS '02)},
  YEAR =         {2002},
  month =        {Mar},
  publisher =    {Springer-Verlag},
}
%% Citations included by Sat in the area of STMs

@article{HerlMoss:1993:SigArch,
 author = {Maurice Herlihy and J. Eliot B.Moss },
 title = {{Transactional memory: {A}rchitectural {S}upport for {L}ock-{F}ree {D}ata {S}tructures}},
 journal = {SIGARCH Comput. Archit. News},
 volume = {21},
 number = {2},
 year = {1993},
 issn = {0163-5964},
 pages = {289--300},
 doi = {},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{ShavTou:1995:PODC,
 author = {Shavit, Nir and Touitou, Dan},
 title = {{{S}oftware {T}ransactional {M}emory}},
 booktitle = {PODC},
 year = {1995},
 isbn = {0-89791-710-3},
 pages = {204--213},
 location = {Ottowa, Ontario, Canada},
 doi = {},
 publisher = {},
 address = {},
 }

@inproceedings{Harretal:2005:PPoPP,
 author = {Tim Harris and Simon Marlow and Simon Peyton-Jones and Maurice Herlihy},
 title = {{Composable memory transactions}},
 booktitle = {PPoPP},
 year = {2005},
 isbn = {1-59593-080-9},
 pages = {48--60},
 location = {Chicago, IL, USA},
 doi = {},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{Yangetal:2007:PPoPP,
 author = {Ni, Yang and Menon, Vijay S. and Adl-Tabatabai, Ali-Reza and Hosking, Antony L. and Hudson, Richard L. and Moss, J. Eliot B. and Saha, Bratin and Shpeisman, Tatiana},
 title = {{Open nesting in software transactional memory}},
 booktitle = {PPoPP},
 year = {2007},
 isbn = {978-1-59593-602-8},
 pages = {68--78},
 location = {San Jose, California, USA},
 doi = {http://doi.acm.org/10.1145/1229428.1229442},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{AgarLeiSukh:2006:MSPC,
 author = {Agrawal, Kunal and Leiserson, Charles E. and Sukha, Jim},
 title = {{Memory models for open-nested transactions}},
 booktitle = {MSPC '06: Proceedings of the 2006 workshop on Memory system performance and correctness},
 year = {2006},
 isbn = {1-59593-578-9},
 pages = {70--81},
 location = {San Jose, California},
 doi = {http://doi.acm.org/10.1145/1178597.1178610},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@article{MossAnt:2006:SCP,
 author = {Moss, J. Eliot B. and Hosking, Antony L.},
 title = {{Nested transactional memory: model and architecture sketches}},
 journal = {Sci. Comput. Program.},
 volume = {63},
 number = {2},
 year = {2006},
 issn = {0167-6423},
 pages = {186--201},
 doi = {http://dx.doi.org/10.1016/j.scico.2006.05.010},
 publisher = {Elsevier North-Holland, Inc.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 }

@inproceedings{AgarFinSukh:2008:PPoPP,
 author = {Agrawal, Kunal and Fineman, Jeremy T. and Sukha, Jim},
 title = {{Nested parallelism in transactional memory}},
 booktitle = {PPoPP '08: Proceedings of the 13th ACM SIGPLAN Symposium on Principles and practice of parallel programming},
 year = {2008},
 isbn = {978-1-59593-795-7},
 pages = {163--174},
 location = {Salt Lake City, UT, USA},
 doi = {http://doi.acm.org/10.1145/1345206.1345232},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{Moretal:2006:ASPLOS,
 author = {Moravan, Michelle J. and Bobba, Jayaram and Moore, Kevin E. and Yen, Luke and Hill, Mark D. and Liblit, Ben and Swift, Michael M. and Wood, David A.},
 title = {{Supporting nested transactional memory in logTM}},
 booktitle = {ASPLOS-XII: Proceedings of the 12th international conference on Architectural support for programming languages and operating systems},
 year = {2006},
 isbn = {1-59593-451-0},
 pages = {359--370},
 location = {San Jose, California, USA},
 doi = {http://doi.acm.org/10.1145/1168857.1168902},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@Article{Moss:2006:MPI,
	author = {J.E.B.Moss},
	journal = {In Workshop on Memory Performance Issues},
	year = {2006},
	title = {{Open Nested Transactions: Semantics and Support}}
}


@inproceedings{GuerKap:Opacity:PPoPP:2008,
 author = {Guerraoui, Rachid and Kapalka, Michal},
 title = {On the Correctness of Transactional Memory},
 booktitle = {Proceedings of the 13th ACM SIGPLAN Symposium on Principles and Practice of Parallel Programming},
 series = {PPoPP '08},
 year = {2008},
 isbn = {978-1-59593-795-7},
 location = {Salt Lake City, UT, USA},
 pages = {175--184},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1345206.1345233},
 doi = {10.1145/1345206.1345233},
 acmid = {1345233},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {correctness, lower bound, model, transactional memory},
}

@inproceedings{ImbsRay:LockSTM:OPODIS:2008,
 author = {Imbs, Damien and Raynal, Michel},
 title = {{A Lock-Based STM Protocol That Satisfies Opacity and Progressiveness}},
 booktitle = {OPODIS '08: Proceedings of the 12th International Conference on Principles of Distributed Systems},
 year = {2008},
 isbn = {978-3-540-92220-9},
 pages = {226--245},
 location = {Luxor, Egypt},
 doi = {http://dx.doi.org/10.1007/978-3-540-92221-6_16},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
 }

@article{Herlihy+:Linearizability:TPLS:1990,
 author = {Herlihy, Maurice P. and Wing, Jeannette M.},
 title = {{Linearizability: a correctness condition for concurrent objects}},
 journal = {ACM Trans. Program. Lang. Syst.},
 volume = {12},
 number = {3},
 year = {1990},
 issn = {0164-0925},
 pages = {463--492},
 doi = {},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

 @article{Papad:1979:JACM,
 author = {Papadimitriou, Christos H.},
 title = {The Serializability of Concurrent Database Updates},
 journal = {J. ACM},
 issue_date = {Oct. 1979},
 volume = {26},
 number = {4},
 month = oct,
 year = {1979},
 issn = {0004-5411},
 pages = {631--653},
 numpages = {23},
 url = {http://doi.acm.org/10.1145/322154.322158},
 doi = {10.1145/322154.322158},
 acmid = {322158},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@BOOK{tm-book,
  author    = {Rachid Guerraoui and
               Michal Kapalka},
  title     = {Principles of Transactional Memory},
  series    = {Synthesis Lectures on Distributed Computing Theory},
  publisher = {Morgan {\&} Claypool Publishers},
  year      = {2010},
  url       = {https://doi.org/10.2200/S00253ED1V01Y201009DCT004},
  doi       = {10.2200/S00253ED1V01Y201009DCT004},
  timestamp = {Tue, 16 May 2017 01:00:00 +0200},
  biburl    = {https://dblp.org/rec/bib/series/synthesis/2010Guerraoui},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Vidya:1987:AINF,
 author = {Vidyasankar, K.},
 title = {{Generalized theory of serializability}},
 journal = {Acta Inf.},
 volume = {24},
 number = {1},
 year = {1987},
 issn = {0001-5903},
 pages = {105--109},
 doi = {http://dx.doi.org/10.1007/BF00290709},
 publisher = {Springer-Verlag New York, Inc.},
 address = {Secaucus, NJ, USA},
 }

@article{RenAbba:1994:IPL,
 author = {Resende, R. F. and El Abbadi, A.},
 title = {{On the serializability theorem for nested transactions}},
 journal = {Inf. Process. Lett.},
 volume = {50},
 number = {4},
 year = {1994},
 issn = {0020-0190},
 pages = {177--183},
 doi = {http://dx.doi.org/10.1016/0020-0190(94)00033-6},
 publisher = {Elsevier North-Holland, Inc.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 }

@book{WeiVoss:TIS:2002:Morg,
  author    = {Gerhard Weikum and
               Gottfried Vossen},
  title     = {{Transactional Information Systems: Theory, Algorithms, and
               the Practice of Concurrency Control and Recovery}},
  publisher = {Morgan Kaufmann},
  year      = {2002},
  isbn      = {1-55860-508-8},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{Imbs+:2009:PODC,
 author = {Imbs, Damien and de Mendivil, Jos\'{e} Ramon and Raynal, Michel},
 title = {{Brief announcement: virtual world consistency: a new condition for STM systems}},
 booktitle = {PODC '09: Proceedings of the 28th ACM symposium on Principles of distributed computing},
 year = {2009},
 isbn = {978-1-60558-396-9},
 pages = {280--281},
 location = {Calgary, AB, Canada},
 doi = {http://doi.acm.org/10.1145/1582716.1582764},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{ImbsRay:2009:SIROCCO,
 author = {Imbs, Damien and Raynal, Michel},
 title = {{A versatile {STM} protocol with invisible read operations that satisfies the virtual world consistency condition}},
 booktitle = {Proceedings of the 16th international conference on Structural Information and Communication Complexity},
 series = {SIROCCO'09},
 year = {2010},
 isbn = {3-642-11475-X, 978-3-642-11475-5},
 location = {Piran, Slovenia},
 pages = {266--280},
 numpages = {15},
 url = {http://dx.doi.org/10.1007/978-3-642-11476-2_21},
 doi = {10.1007/978-3-642-11476-2_21},
 acmid = {2174448},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
 keywords = {atomic object, causal past, commit/abort, concurrency control, consistency condition, consistent global state, lock, read-from relation, regular read/write object, serializability, shared memory, software transactional memory, transaction, vector clock},
} 

@inproceedings{CIR11,
  author    = {Tyler Crain and
               Damien Imbs and
               Michel Raynal},
  title     = {{Read Invisibility, Virtual World Consistency and Probabilistic
               Permissiveness are Compatible}},
  booktitle = {ICA3PP (1)},
  year      = {2011},
  pages     = {244-257}
}

@inproceedings{israeli-disjoint,
 author = {Israeli, Amos and Rappoport, Lihu},
 title = {{Disjoint-access-parallel implementations of strong shared memory primitives}},
 booktitle = {Proceedings of the thirteenth annual ACM symposium on Principles of distributed computing},
 series = {PODC '94},
 year = {1994},
 isbn = {0-89791-654-9},
 location = {Los Angeles, California, United States},
 pages = {151--160},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/197917.198079},
 doi = {http://doi.acm.org/10.1145/197917.198079},
 acmid = {198079},
 publisher = {ACM},
 address = {New York, NY, USA},
} 


@inproceedings{AHM09,
 author = {Attiya, Hagit and Hillel, Eshcar and Milani, Alessia},
 title = {{Inherent limitations on disjoint-access parallel implementations of transactional memory}},
 booktitle = {Proceedings of the twenty-first annual symposium on Parallelism in algorithms and architectures},
 series = {SPAA '09},
 year = {2009},
 isbn = {978-1-60558-606-9},
 location = {Calgary, AB, Canada},
 pages = {69--78},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1583991.1584015},
 doi = {http://doi.acm.org/10.1145/1583991.1584015},
 acmid = {1584015},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {disjoint-access parallelism, impossibility result, lower bound, partial snapshots, transactional memory},
} 

@InProceedings{Doherty+:2009:REFINE,
	booktitle = {REFINE},
	year = {2009},
	author = {Simon Doherty and Lindsay Groves and Victor Luchangco and Mark Moir},
	title = {{Towards Formally Specifying and Verifying Transactional Memory}}
}

@TechReport{SatVid:2010:TR,
	author = {Sathya Peri and K.Vidyasankar},
	institution = {Memorial University of Newfoundland},
	title = {{Correctness of Concurrent Executions of Closed Nested Transactions in Transactional Memory Systems}},
	year = {July, 2011}
}

@inproceedings{SatVid:2011:ICDCN,
 author = {Sathya Peri and K.Vidyasankar},
 title = {{Correctness of Concurrent Executions of Closed Nested Transactions in Transactional Memory Systems}},
 booktitle = {12th International Conference on Distributed Computing and Networking},
 pages = {95--106},
 year = {2011},
 location = {Bangalore, Canada},
 }

@inproceedings{SatVid:2012:ICDCN,
 author = {Sathya Peri and K.Vidyasankar},
 title = {{An efficient scheduler for closed nested transactions that satisfies all-read-consistency and non-interference}},
 booktitle = {13th International Conference on Distributed Computing and Networking},
 year = {2012},
 location = {Bangalore, Canada},
 }

@inproceedings{Guer+:disc:2008,
  author	= {Guerraoui, Rachid and Henzinger, Thomas and Singh, Vasu},
  title		= {{Permissiveness in {T}ransactional {M}emories}},
  booktitle	= {DISC~'08: Proc. 22nd International Symposium on Distributed Computing},
  note		= {Springer-Verlag Lecture Notes in Computer Science volume 5218},
  urlpage	= {http://dx.doi.org/10.1007/978-3-540-87779-0_21},
  pdf		= {http://infoscience.epfl.ch/record/125702/files/main.pdf},
  pages		= {305--319},
  year		= {2008},
  month		= {sep},
}

@InProceedings{Baretto+:PPoPP:2010,
   address     = { },
   affiliation = {EPFL},
   author      = {Baretto, Joao and Dragojevic, Aleksandar and Ferreira,
                 Paulo and Guerraoui, Rachid and Kapalka, Michal},
   booktitle   = {Proceedings of the 15th {ACM} {SIGPLAN} symposium on
                 {P}rinciples and {P}ractice of {P}arallel {C}omputing},
   details     = {http://infoscience.epfl.ch/record/144050},
   documenturl = {http://infoscience.epfl.ch/getfile.py?recid=144050&mode=best},
   doi         = {10.1145/1693453.1693466},
   keywords    = {Nested parallel programs; Fork-join; Work-stealing; Transactional memory},
   location    = {Bangalore, India},
   pages       = {91--100},
   publisher   = {ACM},
   review      = {REVIEWED},
   series      = { },
   status      = {PUBLISHED},
   title       = {{Leveraging {P}arallel {N}esting in {T}ransactional {M}emory}},
   unit        = {LPD},
   url         = { },
   year        = 2010
}

@InProceedings{RanVid:Tran:2011,
	author = {Ranjeet Kumar and Krishnamurthy Vidyasankar},
	booktitle = {TRANSACT 2011},
	title = {{HParSTM: A Hierarchy-based STM Protocol for Supporting Nested Parallelism}},
	month = {June},
	year = {2011}
}

@Article{RaviSat:IJCCT:2012,
	title = {{A Correctness Criterion for Eager Approach Validation for Transactional Memory System}},
	year = {2012},
	pages = {43-49},
	author = {Ravi Kumar and Sathya Peri},
	volume = {3},
	journal = {International Journal of Computer and Communication Technology (IJCCT)},
	number = {2}
}

@article{KuzSat:Corr:2012,
  author    = {Petr Kuznetsov and
               Sathya Peri},
  title     = {{On Non-Interference of Transactions}},
  journal   = {CoRR},
  volume    = {abs/1211.6315},
  year      = {2012},
  ee        = {http://arxiv.org/abs/1211.6315},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{Bernstein+:MCC:TDS:1983,
 author = {Bernstein, Philip A. and Goodman, Nathan},
 title = {{{M}ultiversion {C}oncurrency {C}ontrol: {T}heory and {A}lgorithms}},
 journal = {ACM Trans. Database Syst.},
 issue_date = {Dec. 1983},
 volume = {8},
 number = {4},
 month = dec,
 year = {1983},
 issn = {0362-5915},
 pages = {465--483},
 numpages = {19},
 url = {http://doi.acm.org/10.1145/319996.319998},
 doi = {10.1145/319996.319998},
 acmid = {319998},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {transaction processing},
}
 
@Article{CachRito:2006:CP,
	title = {{{V}ersioned {B}oxes as the basis for {M}emory {T}ransactions}},
	year = {2006},
	number = {2},
	author = {J. Cachopo and A. Rito-Silva},
	pages = {172--185},
	journal = {Science of Computer Programming},
	volume = {63}
}

@inproceedings{AydAbd:2008:Serial:transact,
  author	= {Aydonat, Utku and Abdelrahman, Tarek},
  title		= {{Serializability of {T}ransactions in {S}oftware {T}ransactional {M}emory}},
  booktitle	= {TRANSACT~'08: 3rd Workshop on Transactional Computing},
  pdf		= {http://www.unine.ch/transact08/papers/Aydonat-Serializability.pdf},
  year		= {2008},
  month		= {feb},
}

@article{PapadKanel:1984:MultVer:TDS,
 author = {Papadimitriou, Christos H. and Kanellakis, Paris C.},
 title = {{On Concurrency Control by Multiple Versions}},
 journal = {ACM Trans. Database Syst.},
 issue_date = {March 1984},
 volume = {9},
 number = {1},
 month = mar,
 year = {1984},
 issn = {0362-5915},
 pages = {89--99},
 numpages = {11},
 url = {http://doi.acm.org/10.1145/348.318588},
 doi = {10.1145/348.318588},
 acmid = {318588},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{Perel+:2011:SMV:DISC,
  author    = {Dmitri Perelman and
               Anton Byshevsky and
               Oleg Litmanovich and
               Idit Keidar},
  title     = {{SMV}: {S}elective {M}ulti-{V}ersioning {STM}},
  booktitle = {DISC},
  year      = {2011},
  pages     = {125-140},
  ee        = {http://dx.doi.org/10.1007/978-3-642-24100-0_9},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{herlihy+:2003:stm-dynamic:podc,
  author	= {Herlihy, Maurice and Luchangco, Victor and Moir, Mark and {William N. Scherer}, III},
  title		= {{Software Transactional Memory for Dynamic-Sized Data Structures}},
  booktitle	= {PODC~'03: Proc. 22nd ACM Symposium on Principles of Distributed Computing},
  pages		= {92--101},
  month		= {Jul},
  urlpage	= {http://doi.acm.org/10.1145/872035.872048},
  year		= {2003},
}

@inproceedings{dice:2006:tl2:disc,
  author	= {Dice, Dave and Shalev, Ori and Shavit, Nir},
  title		= {{Transactional Locking II}},
  booktitle	= {DISC~'06: Proc. 20th International Symposium on Distributed Computing},
  note		= {Springer-Verlag Lecture Notes in Computer Science volume 4167},
  pages		= {194--208},
  year		= {2006},
  month		= {sep},
}

@inproceedings{perel+:2010:MultVer:PODC,
 author = {Perelman, Dmitri and Fan, Rui and Keidar, Idit},
 title = {On Maintaining Multiple Versions in STM},
 booktitle = {Proceedings of the 29th ACM SIGACT-SIGOPS Symposium on Principles of Distributed Computing},
 series = {PODC '10},
 year = {2010},
 isbn = {978-1-60558-888-9},
 location = {Zurich, Switzerland},
 pages = {16--25},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1835698.1835704},
 doi = {10.1145/1835698.1835704},
 acmid = {1835704},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {transactional memory},
} 

@incollection{riegel+:2006:LSA:DISC,
  author	= {Riegel, Torvald and Felber, Pascal and Fetzer, Christof},
  editor	= {},
  title		= {{A {L}azy {S}napshot {A}lgorithm with {E}ager {V}alidation}},
  booktitle	= {Proceedings of the 20th International Symposium on Distributed Computing, {DISC} 2006},
  publisher	= {Springer},
  month		= {Sep},
  year		= {2006},
  volume	= {4167},
  isbn		= {3-540-44624-9},
  pages		= {284--298},
  series	= {Lecture Notes in Computer Science},
  urlpage	= {http://dx.doi.org/10.1007/11864219_20}
}

@inproceedings{riegel+:sistm:transact:2006,
  author	= {Riegel, Torvald and Fetzer, Christof and Felber, Pascal},
  booktitle	= {Proceedings of the First ACM SIGPLAN Workshop on Languages, Compilers, and Hardware Support for Transactional Computing},
  month		= {Jun},
  title		= {{Snapshot Isolation for Software Transactional Memory }},
  year		= {2006}
}

@article{attiyaHill:sinmvperm:tcs:2012,
  author    = {Hagit Attiya and
               Eshcar Hillel},
  title     = {{A {S}ingle-{V}ersion {STM} that is {M}ulti-{V}ersioned {P}ermissive}},
  journal   = {Theory Comput. Syst.},
  volume    = {51},
  number    = {4},
  year      = {2012},
  pages     = {425-446},
  ee        = {http://dx.doi.org/10.1007/s00224-012-9406-3},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{prisat:mvto:corr:2013,
  author    = {Priyanka Kumar and
               Sathya Peri},
  title     = {{A TimeStamp based Multi-version STM Protocol that satisfies
               Opacity}},
  journal   = {CoRR},
  volume    = {abs/1305.6624},
  year      = {2013},
  ee        = {http://arxiv.org/abs/1305.6624},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{Fern+:LSMVSTM:PPoPP:2011,
 author = {Fernandes, S{\'e}rgio Miguel and Cachopo, Joao},
 title = {{Lock-free and {S}calable {M}ulti-version {S}oftware {T}ransactional {M}emory}},
 booktitle = {Proceedings of the 16th ACM symposium on Principles and practice of parallel programming},
 series = {PPoPP '11},
 year = {2011},
 isbn = {978-1-4503-0119-0},
 location = {San Antonio, TX, USA},
 pages = {179--188},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1941553.1941579},
 doi = {10.1145/1941553.1941579},
 acmid = {1941579},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {garbage collection, lock-free synchronization, multi-version concurrency control, transactional memory},
} 

@Article{LuScott:UMV:Transact:2012,
	journal = {Transact},
	title = {{Unmanaged Multiversion STM}},
	year = {2012},
	author = {Li Lu and Michael L. Scott}
}

@inproceedings{SinhaMalik:RuntimeSee:IPDPS:2010,
  author    = {Arnab Sinha and
               Sharad Malik},
  title     = {{Runtime checking of serializability in software transactional
               memory}},
  booktitle = {IPDPS},
  year      = {2010},
  pages     = {1-12},
  ee        = {http://dx.doi.org/10.1109/IPDPS.2010.5470389},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{HadzPapad:AAMVCC:PODS:1985,
 author = {Hadzilacos, Thanasis and Papadimitriou, Christos H.},
 title = {{Algorithmic aspects of multiversion concurrency control}},
 booktitle = {Proceedings of the fourth ACM SIGACT-SIGMOD symposium on Principles of database systems},
 series = {PODS '85},
 year = {1985},
 isbn = {0-89791-153-9},
 location = {Portland, Oregon, USA},
 pages = {96--104},
 numpages = {9},
 url = {http://doi.acm.org/10.1145/325405.325417},
 doi = {10.1145/325405.325417},
 acmid = {325417},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@article{KuznetsovPeri:Non-interference:TCS:2017,
  author    = {Petr Kuznetsov and
               Sathya Peri},
  title     = {Non-interference and local correctness in transactional memory},
  journal   = {Theor. Comput. Sci.},
  volume    = {688},
  pages     = {103--116},
  year      = {2017},
  url       = {https://doi.org/10.1016/j.tcs.2016.06.021},
  doi       = {10.1016/j.tcs.2016.06.021},
  timestamp = {Thu, 28 Dec 2017 00:00:00 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/tcs/KuznetsovP17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Kumar+:MVTO:ICDCN:2014,
 author = {Kumar, Priyanka and Peri, Sathya and Vidyasankar, K.},
 title = {A TimeStamp Based Multi-version STM Algorithm},
 booktitle = {Proceedings of the 15th International Conference on Distributed Computing and Networking - Volume 8314},
 series = {ICDCN 2014},
 year = {2014},
 isbn = {978-3-642-45248-2},
 location = {Coimbatore, India},
 pages = {212--226},
 numpages = {15},
 url = {http://dx.doi.org/10.1007/978-3-642-45249-9_14},
 doi = {10.1007/978-3-642-45249-9_14},
 acmid = {2741924},
 publisher = {Springer-Verlag New York, Inc.},
 address = {New York, NY, USA},
} 



@book{Har+:TMBook:2010,
  author    = {Tim Harris and
               James R. Larus and
               Ravi Rajwar},
  title     = {{Transactional Memory, 2nd edition}},
  booktitle = {Transactional Memory (2.ed.)},
  publisher = {Morgan {\&} Claypool Publishers},
  series    = {Synthesis Lectures on Computer Architecture},
  year      = {2010},
  ee        = {http://dx.doi.org/10.2200/S00272ED1V01Y201006CAC011},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{OluHamm:MicroBook:Queue:2005,
 author = {Olukotun, Kunle and Hammond, Lance},
 title = {{The Future of Microprocessors}},
 journal = {Queue},
 issue_date = {September 2005},
 volume = {3},
 number = {7},
 month = sep,
 year = {2005},
 issn = {1542-7730},
 pages = {26--29},
 numpages = {4},
 url = {http://doi.acm.org/10.1145/1095408.1095418},
 doi = {10.1145/1095408.1095418},
 acmid = {1095418},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@book{Herlihy:ArtBook:2012,
  title={{The Art of Multiprocessor Programming}},
  author={Herlihy, M. and Shavit, N.},
  isbn={9780080569581},
  url={},
  year={2012},
  publisher={Elsevier Science}
}

@inproceedings{Harris:NBList:DISC:2001,
 author = {Harris, Timothy L.},
 title = {A Pragmatic Implementation of Non-blocking Linked-Lists},
 booktitle = {Proceedings of the 15th International Conference on Distributed Computing},
 series = {DISC '01},
 year = {2001},
 isbn = {3-540-42605-1},
 pages = {300--314},
 numpages = {15},
 url = {http://dl.acm.org/citation.cfm?id=645958.676105},
 acmid = {676105},
 publisher = {Springer-Verlag},
 address = {London, UK, UK},
}

@article{Herlihy:WaitFree:1991,
  title={{Wait-free synchronization}},
  author={Herlihy, Maurice},
  journal={ACM Transactions on Programming Languages and Systems (TOPLAS)},
  volume={13},
  number={1},
  pages={124--149},
  year={1991},
  publisher={ACM}
}

@INPROCEEDINGS{Attiya+:DUOp:ICDCS:2013,
author={Attiya, H. and Hans, S. and Kuznetsov, P. and Ravi, S.},
booktitle={Distributed Computing Systems (ICDCS), 2013 IEEE 33rd International Conference on},
title={{Safety of Deferred Update in Transactional Memory}},
year={2013},
month={July},
pages={601-610},
keywords={concurrency control;transaction processing;committed transactions;deferred update safety;deferred-update semantics;opacityc riterion;prefix serializations;sequential execution;sequential order;speculative transactions;transactional memory;unique-write assumption;History;Law;Real-time systems;Safety;Semantics;Silicon;Limit-closure;Safety;Transactional Memory},
doi={10.1109/ICDCS.2013.57},
ISSN={1063-6927},}

@article{PriSat:MVC:Corr:2015,
  author    = {Priyanka Kumar and
               Sathya Peri},
  title     = {{Multi-Version Conflict Notion}},
  journal   = {CoRR},
  volume    = {abs/1307.8256},
  year      = {2013},
  url       = {http://arxiv.org/abs/1307.8256},
  timestamp = {Thu, 15 Aug 2013 15:30:58 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/KumarP13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Attiya+:TMS:DISC:2014,
  author    = {Hagit Attiya and
               Alexey Gotsman and
               Sandeep Hans and
               Noam Rinetzky},
  title     = {{Safety of Live Transactions in Transactional Memory: {TMS} is Necessary
               and Sufficient}},
  booktitle = {Distributed Computing - 28th International Symposium, {DISC} 2014,
               Austin, TX, USA, October 12-15, 2014. Proceedings},
  pages     = {376--390},
  year      = {2014},
  crossref  = {DBLP:conf/wdag/2014},
  url       = {http://dx.doi.org/10.1007/978-3-662-45174-8_26},
  doi       = {10.1007/978-3-662-45174-8_26},
  timestamp = {Tue, 30 Sep 2014 10:44:00 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/wdag/AttiyaGHR14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{Herlihy:WFS:TPLS:1991,
 author = {Herlihy, Maurice},
 title = {{Wait-free Synchronization}},
 journal = {ACM Trans. Program. Lang. Syst.},
 issue_date = {Jan. 1991},
 volume = {13},
 number = {1},
 month = jan,
 year = {1991},
 issn = {0164-0925},
 pages = {124--149},
 numpages = {26},
 url = {http://doi.acm.org/10.1145/114005.102808},
 doi = {10.1145/114005.102808},
 acmid = {102808},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {linearization, wait-free synchronization},
} 

@book{HerlihyShavit:AMP:Book:2012,
 author = {Herlihy, Maurice and Shavit, Nir},
 title = {{The Art of Multiprocessor Programming, Revised Reprint}},
 year = {2012},
 isbn = {9780123973375, 9780123977953},
 edition = {1st},
 publisher = {Morgan Kaufmann Publishers Inc.},
 address = {San Francisco, CA, USA},
} 

@inproceedings{LuScott:GMV:DISC:2013,
  author    = {Li Lu and
               Michael L. Scott},
  title     = {{Generic Multiversion {STM}}},
  booktitle = {Distributed Computing - 27th International Symposium, {DISC} 2013,
               Jerusalem, Israel, October 14-18, 2013. Proceedings},
  pages     = {134--148},
  year      = {2013},
  crossref  = {DBLP:conf/wdag/2013},
  url       = {http://dx.doi.org/10.1007/978-3-642-41527-2_10},
  doi       = {10.1007/978-3-642-41527-2_10},
  timestamp = {Mon, 28 Oct 2013 18:03:50 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/wdag/LuS13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{CachAnt:VBoxes:SCOOL:2005,
  author	= {Cachopo, Joao and Rito-Silva, Antonio},
  title		= {{Versioned Boxes as the Basis for Memory Transactions}},
  booktitle	= {OOPSLA 2005 Workshop on Synchronization and Concurrency in Object-Oriented Languages (SCOOL)},
  urlpage	= {http://hdl.handle.net/1802/2101},
  year		= {2005},
  month		= {oct},
}

@article{Thomas:TWR:TDS:1979,
 author = {Thomas, Robert H.},
 title = {{A Majority Consensus Approach to Concurrency Control for Multiple Copy Databases}},
 journal = {ACM Trans. Database Syst.},
 issue_date = {June 1979},
 volume = {4},
 number = {2},
 month = jun,
 year = {1979},
 issn = {0362-5915},
 pages = {180--209},
 numpages = {30},
 url = {http://doi.acm.org/10.1145/320071.320076},
 doi = {10.1145/320071.320076},
 acmid = {320076},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {clock synchronization, computer networks, concurrency control, distributed computation, distributed control, distributed databases, multiprocess systems, update synchronization},
} 

@inproceedings{Gramoli+:OptListSet:DISC-BA:2015,
  TITLE = {{Brief Announcement: A Concurrency-Optimal List-Based Set}},
  AUTHOR = {Gramoli, Vincent and Kuznetsov, Petr and Ravi, Srivatsan and Shang, Di},
  URL = {https://hal.archives-ouvertes.fr/hal-01207872},
  BOOKTITLE = {{DISC 2015}},
  ADDRESS = {Tokyo, Japan},
  ORGANIZATION = {{Toshimitsu Masuzawa and Koichi Wada}},
  EDITOR = {Yoram Moses and Matthieu Roy},
  PUBLISHER = {{Springer-Verlag Berlin Heidelberg}},
  SERIES = {29th International Symposium on Distributed Computing},
  VOLUME = {LNCS 9363},
  YEAR = {2015},
  MONTH = Oct,
  PDF = {https://hal.archives-ouvertes.fr/hal-01207872/file/37-BA.pdf},
  HAL_ID = {hal-01207872},
  HAL_VERSION = {v1},
}

@article{Gramoli+:OptListSet:CoRR:2015,
  author    = {Vincent Gramoli and
               Petr Kuznetsov and
               Srivatsan Ravi and
               Di Shang},
  title     = {{A Concurrency-Optimal List-Based Set}},
  journal   = {CoRR},
  volume    = {abs/1502.01633},
  year      = {2015},
  url       = {http://arxiv.org/abs/1502.01633},
  timestamp = {Mon, 02 Mar 2015 14:17:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/GramoliKRS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Heller+:LazyList:PPL:2007,
  author    = {Steve Heller and
               Maurice Herlihy and
               Victor Luchangco and
               Mark Moir and
               William N. Scherer III and
               Nir Shavit},
  title     = {{A Lazy Concurrent List-Based Set Algorithm}},
  journal   = {Parallel Processing Letters},
  volume    = {17},
  number    = {4},
  pages     = {411-424},
  year      = {2007},
  url       = {},
  doi       = {},
  timestamp = {Mon, 23 Jun 2008 13:43:26 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/ppl/HellerHLMSS07},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Ziv+:Composing:POPL:2015,
  title={{Composing Concurrency Control}},
  author={Ziv, Ofri and Aiken, Alex and Golan-Gueta, Guy and Ramalingam, G and Sagiv, Mooly},
  booktitle={Proceedings of the 36th ACM SIGPLAN Conference on Programming Language Design and Implementation},
  pages={240--249},
  year={2015},
  organization={ACM}
}

@article{marathe2004qualitative,
  title={{A qualitative survey of modern software transactional memory systems}},
  author={Marathe, Virendra J and Scott, Michael L},
  journal={University of Rochester Computer Science Dept., Tech. Rep},
  year={2004}
}

@inproceedings{Vafeiadis:2006:PCH:1122971.1122992,
 author = {Vafeiadis, Viktor and Herlihy, Maurice and Hoare, Tony and Shapiro, Marc},
 title = {{Proving Correctness of Highly-concurrent Linearisable Objects}},
 booktitle = {PPoPP},
 series = {},
 year = {2006},
 isbn = {1-59593-189-9},
 location = {},
 pages = {129--136},
 numpages = {8},
 url = {},
 doi = {},
 acmid = {1122992},
 publisher = {},
 address = {},
 keywords = {concurrent programming, formal verification, linearisability, rely-guarantee reasoning, shared-memory concurrency},
}


@techreport{marathe:stm-survey:urcs-tr:2004,
  author	= {Marathe, Virendra J. and Scott, Michael L.},
  title		= {{A Qualitative Survey of Modern Software Transactional Memory Systems}},
  number	= {TR 839},
  institution	= {University of Rochester Computer Science Dept.},
  month		= {Jun},
  year		= {2004},
  pdf		= {http://www.cs.rochester.edu/u/scott/papers/2004_TR839.pdf}
}

@phdthesis{Fraser:PracticalLF:2004,
  title={{Practical lock-freedom}},
  author={Fraser, Keir},
  year={2004},
  school={University of Cambridge}
}

@inproceedings{Herlihy+:STM-DynamicSize:PODC:2003,
  title={{Software transactional memory for dynamic-sized data structures}},
  author={Herlihy, Maurice and Luchangco, Victor and Moir, Mark and Scherer III, William N},
  booktitle={Proceedings of the twenty-second annual symposium on Principles of distributed computing},
  pages={92--101},
  year={2003},
  organization={ACM}
}
@inproceedings{Marathe+:STM-Tradeoff:LCRS:2004,
  title={{Design tradeoffs in modern software transactional memory systems}},
  author={Marathe, Virendra J and Scherer, William N and Scott, Michael L},
  booktitle={Proceedings of the 7th workshop on Workshop on languages, compilers, and run-time support for scalable systems},
  pages={1--7},
  year={2004},
  organization={ACM}
}

@article{Barghouti:1991:CCA:116873.116875,
 author = {Barghouti, Naser S. and Kaiser, Gail E.},
 title = {{Concurrency Control in Advanced Database Applications}},
 journal = {ACM Comput. Surv.},
 issue_date = {Sept. 1991},
 volume = {23},
 number = {3},
 month = sep,
 year = {1991},
 issn = {0360-0300},
 pages = {269--317},
 numpages = {49},
 url = {http://doi.acm.org/10.1145/116873.116875},
 doi = {10.1145/116873.116875},
 acmid = {116875},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {advanced database applications, concurrency control, cooperative transactions, design environments, extended transaction models, long transactions, object-oriented databases, relaxing serializability},
}

@article{Beeri+:Nested:JACM:1989,
 author = {Beeri, Catriel and Bernstein, Philip A. and Goodman, Nathan},
 title = {{A Model for Concurrency in Nested Transactions Systems}},
 journal = {J. ACM},
 issue_date = {April 1989},
 volume = {36},
 number = {2},
 month = apr,
 year = {1989},
 issn = {0004-5411},
 pages = {230--269},
 numpages = {40},
 url = {http://doi.acm.org/10.1145/62044.62046},
 doi = {10.1145/62044.62046},
 acmid = {62046},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{HerlihyKosk:Boosting:PPoPP:2008,
	author    = {Maurice Herlihy and
	Eric Koskinen},
	title     = {Transactional boosting: a methodology for highly-concurrent transactional
	objects},
	booktitle = {Proceedings of the 13th {ACM} {SIGPLAN} Symposium on Principles and
	Practice of Parallel Programming, {PPOPP} 2008, Salt Lake City, UT,
	USA, February 20-23, 2008},
	pages     = {207--216},
	year      = {2008},
	url       = {http://doi.acm.org/10.1145/1345206.1345237},
	doi       = {10.1145/1345206.1345237},
	timestamp = {Tue, 22 May 2012 15:24:56 +0200},
	biburl    = {https://dblp.org/rec/bib/conf/ppopp/HerlihyK08},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{Hassan+:OptBoost:PPoPP:2014,
 author = {Hassan, Ahmed and Palmieri, Roberto and Ravindran, Binoy},
 title = {Optimistic Transactional Boosting},
 booktitle = {Proceedings of the 19th ACM SIGPLAN Symposium on Principles and Practice of Parallel Programming},
 series = {PPoPP '14},
 year = {2014},
 isbn = {978-1-4503-2656-8},
 location = {Orlando, Florida, USA},
 pages = {387--388},
 numpages = {2},
 url = {http://doi.acm.org/10.1145/2555243.2555283},
 doi = {10.1145/2555243.2555283},
 acmid = {2555283},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {STM, transactional boosting, transactional data structures},
} 


@inproceedings{Hassan:OptTransLazy:Opodis:2014,
	title={{On developing optimistic transactional lazy set}},
	author={Hassan, Ahmed and Palmieri, Roberto and Ravindran, Binoy},
	booktitle={OPODIS},
	pages={437--452},
	year={2014},
	organization={Springer}
}

@inproceedings{Spiegelman+:TransDS:PLDI:2016,
	title={{Transactional data structure libraries}},
	author={Spiegelman, Alexander and Golan-Gueta, Guy and Keidar, Idit},
	booktitle={PLDI},
	pages={682--696},
	year={2016},
	organization={ACM}
}

@article{Anand+:CaPRa:Corr:2015,
  author    = {Anshu S. Anand and
               R. K. Shyamasundar and
               Sathya Peri},
  title     = {{Opacity Proof for CaPR+ Algorithm}},
  journal   = {CoRR},
  volume    = {abs/1510.06967},
  year      = {2015},
  url       = {http://arxiv.org/abs/1510.06967},
  timestamp = {Sun, 01 Nov 2015 17:30:45 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/AnandSP15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Lev-Ari+:OnCorrectness:DISC:2014,
	author    = {Kfir Lev{-}Ari and
	Gregory V. Chockler and
	Idit Keidar},
	title     = {{On Correctness of Data Structures under Reads-Write Concurrency}},
	booktitle = {DISC},
	pages     = {273--287},
	year      = {2014},
	crossref  = {DBLP:conf/wdag/2014},
	url       = {},
	doi       = {},
	timestamp = {Fri, 19 May 2017 01:25:17 +0200},
	biburl    = {http://dblp.uni-trier.de/rec/bib/conf/wdag/Lev-AriCK14},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Lev-Ari+:ConsApproachLinz:DISC:2015,
	author = {Lev-Ari, Kfir and Chockler, Gregory V and Keidar, Idit},
	booktitle = {DISC},
	doi = {},
	editor = {Moses, Yoram},
	isbn = {978-3-662-48652-8},
	pages = {356--370},
	publisher = {Springer},
	series = {},
	title = {{A Constructive Approach for Proving Data Structures' Linearizability}},
	url = {},
	volume = {},
	year = {2015}
}

@article{zhang2016high,
  title={{High-Performance Composable Transactional Data Structures}},
  author={Zhang, Deli},
  year={2016}
}

@techreport{zhang2010composability,
  author={Zhang, Rui and Budimli{\'c}, Zoran and Scherer III, William N},
  title={{Composability for application-specific transactional optimizations}},
  institution={Department of Computer Science, Rice University},
  year={2010}
}

@article{DBLP:journals/corr/abs-0910-0366,
  author    = {Daniel Cederman and
               Philippas Tsigas},
  title     = {{Supporting Lock-Free Composition of Concurrent Data Objects}},
  journal   = {CoRR},
  volume    = {abs/0910.0366},
  year      = {2009},
  url       = {},
  timestamp = {Wed, 07 Jun 2017 14:40:49 +0200},
  biburl    = {http://dblp.dagstuhl.de/rec/bib/journals/corr/abs-0910-0366},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Hassan2015,
author = {Hassan, Ahmed and Wang, Chao and Broadwater, Robert P},
mendeley-groups = {PhD Thesis},
title = {{Designing , Modeling , and Optimizing Transactional Data Structures}},
year = {2015}
}

@article{harris2007abstract,
	title={{Abstract nested transactions}},
	author={Harris, Tim and others},
	year={2007},
	publisher={Citeseer}
}

@article{Peri+:OSTM:Corr:2017,
	author    = {Sathya Peri and
	Ajay Singh and
	Archit Somani},
	title     = {{Efficient means of Achieving Composability using Transactional Memory}},
	journal   = {CoRR},
	volume    = {abs/1709.00681},
	year      = {2017},
	url       = {http://arxiv.org/abs/1709.00681},
	archivePrefix = {arXiv},
	eprint    = {1709.00681},
	timestamp = {Thu, 05 Oct 2017 09:42:55 +0200},
	biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1709-00681},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Peri+:OSTM:Netys:2018,
  author    = {Sathya Peri and
               Ajay Singh and
               Archit Somani},
  title     = {Efficient Means of Achieving Composability Using Object Based Semantics
               in Transactional Memory Systems},
  booktitle = {Networked Systems - 6th International Conference, {NETYS} 2018, Essaouira,
               Morocco, May 9-11, 2018, Revised Selected Papers},
  pages     = {157--174},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-05529-5\_11},
  doi       = {10.1007/978-3-030-05529-5\_11},
  timestamp = {Tue, 08 Jan 2019 16:57:19 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/netys/PeriSS18},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Felber+:ElasticTrans:2017:jpdc,
 author = {Felber, Pascal and Gramoli, Vincent and Guerraoui, Rachid},
 title = {{Elastic Transactions}},
 journal = {J. Parallel Distrib. Comput.},
 issue_date = {February 2017},
 volume = {100},
 number = {C},
 month = feb,
 year = {2017},
 issn = {0743-7315},
 pages = {103--127},
 numpages = {25},
 url = {https://doi.org/10.1016/j.jpdc.2016.10.010},
 doi = {10.1016/j.jpdc.2016.10.010},
 acmid = {3066828},
 publisher = {Academic Press, Inc.},
 address = {Orlando, FL, USA},
 keywords = {Concurrent data structures, Transactional memory},
} 


@inproceedings{ZhangDech:LockFreeTW:SPAA:2016,
 author = {Zhang, Deli and Dechev, Damian},
 title = {Lock-free Transactions Without Rollbacks for Linked Data Structures},
 booktitle = {Proceedings of the 28th ACM Symposium on Parallelism in Algorithms and Architectures},
 series = {SPAA '16},
 year = {2016},
 isbn = {978-1-4503-4210-0},
 location = {Pacific Grove, California, USA},
 pages = {325--336},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/2935764.2935780},
 doi = {10.1145/2935764.2935780},
 acmid = {2935780},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {lock-free, transactional boosting, transactional data structure, transactional memory},
} 

@inproceedings{Dalessandro+:NoRec:PPoPP:2010,
  added-at = {2010-01-19T00:00:00.000+0100},
  author = {Dalessandro, Luke and Spear, Michael F. and Scott, Michael L.},
  biburl = {https://www.bibsonomy.org/bibtex/2bb4ff560750c574e33fceb87457d3cce/dblp},
  booktitle = {PPOPP},
  editor = {Govindarajan, R. and Padua, David A. and Hall, Mary W.},
  ee = {http://doi.acm.org/10.1145/1693453.1693464},
  interhash = {65ad98c6f111ce3b454219b4fd45ebb8},
  intrahash = {bb4ff560750c574e33fceb87457d3cce},
  isbn = {978-1-60558-877-3},
  keywords = {dblp},
  pages = {67-78},
  publisher = {ACM},
  timestamp = {2012-05-23T11:41:17.000+0200},
  title = {{NOrec: Streamlining STM by Abolishing Ownership Records}},
  url = {http://dblp.uni-trier.de/db/conf/ppopp/ppopp2010.html#DalessandroSS10},
  year = 2010
}


@inproceedings{Juyal+:MVOSTM:SSS:2018,
  author    = {Chirag Juyal and
               Sandeep S. Kulkarni and
               Sweta Kumari and
               Sathya Peri and
               Archit Somani},
  title     = {An Innovative Approach to Achieve Compositionality Efficiently Using
               Multi-version Object Based Transactional Systems},
  booktitle = {Stabilization, Safety, and Security of Distributed Systems - 20th
               International Symposium, {SSS} 2018, Tokyo, Japan, November 4-7, 2018,
               Proceedings},
  pages     = {284--300},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-03232-6\_19},
  doi       = {10.1007/978-3-030-03232-6\_19},
  timestamp = {Thu, 06 Dec 2018 00:00:00 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/sss/JuyalKKPS18},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


==> Submitted MVOSTM Journal-2019/con_future.tex <==
\section{Conclusion}
\label{sec:confu}
With the rise of multi-core systems, concurrent programming becomes popular. Concurrent programming using multiple threads has become necessary to utilize all the cores present in the system effectively. But concurrent programming is usually challenging due to synchronization issues between the threads. 

In the past few years, several STMs have been proposed which address these synchronization issues and provide greater concurrency. STMs hide the synchronization and communication difficulties among the multiple threads from the programmer while ensuring correctness and hence making programming easy. Another advantage of STMs is that they facilitate compositionality of concurrent programs with great ease. Different concurrent operations that need to be composed to form a single atomic unit is achieved by encapsulating them in a single transaction.
 
In literature, most of the STMs are \rwtm{s} which export read and write operations. To improve the performance, a few researchers have proposed \otm{s} \cite{HerlihyKosk:Boosting:PPoPP:2008,Hassan+:OptBoost:PPoPP:2014, Peri+:OSTM:Netys:2018} which export higher level objects operation such as \tab{} insert, delete, and lookup etc. By leveraging the semantics of these higher level \op{s}, these STMs provide greater concurrency. On the other hand, it has been observed in STMs and databases that by storing multiple versions for each \tobj in case of \rwtm{s} provides greater concurrency \cite{perel+:2010:MultVer:PODC,Kumar+:MVTO:ICDCN:2014}.

\ignore{
	
\todo{SK: Remove this para}
So, we get inspired from literature and proposed a new STM as \mvotm which is the combination of both of these ideas (multi-versions in OSTMs). It provides greater concurrency and reduces number of abort while maintaining multiple versions corresponding to each key. \mvotm ensures compositionality by making the transactions atomic. In addition to that, we develop garbage collection for MVOSTM (MVOSTM-GC) to delete unwanted versions corresponding to the each keys to reduce traversal overhead. \mvotm satisfies \ccs{} as \emph{opacity}.
%\color{blue}

%\color{black}
}

This paper proposed the notion of the optimized multi-version object based STMs (\opmvotm{s}) and compares their effectiveness with multi-version object based STMs (MVOSTMs), single-version object based STMs and multi-version read-write STMs. We find that \opmvotm provides a significant benefit over above-mentioned state-of-the-art STMs for different types of workloads. Specifically, we  have  evaluated the effectiveness of OPT-MVOSTM for the \tab{} and list data structure as \ophmvotm and \oplmvotm respectively. 

\ophmvotm and \oplmvotm use the unbounded number of versions for each key. To utilize the memory efficiently, we limit the number of versions and develop two variants for both \tab and list data structures: (1) A garbage collection method in \opmvotm to delete the unwanted versions of a key, denoted as \opmvotmgc. (2) Placing a limit of $K$ on the number of versions in \opmvotm, resulting in \opkotm. Both these variants (\opmvotmgc and \opkotm) gave a performance gain of over 16\% and 24\% over \opmvotm in the best case. \opkotm consumes minimum memory among all the variants of it. We represent \opmvotmgc in hash-table and list as \ophmvotmgc and \oplmvotmgc  respectively. Similarly, We represent \opkotm in hash-table and list as \ophkotm  and \oplkotm  respectively.


\ophkotm performs best among its variants and
outperforms state-of-the-art hash-table based STMs  (HT-OSTM, ESTM, RWSTM, HT-MVTO, HT-KSTM) by a factor of 3.62, 3.95, 3.44, 2.75, 1.85 for workload W1,  1.44, 2.36, 4.45, 9.84, 7.42 for workload W2, and 2.11, 4.05, 7.84, 12.94, 10.70 for workload W3 respectively. Similarly, \oplkotm performs best among its variants and outperforms state-of-the-art list based STMs (list-OSTM, Trans-list, Boosting-list, NOrec-list, list-MVTO, list-KSTM)  by a factor of  2.56, 25.38, 23.57, 27.44, 13.34, 5.99 for W1, 1.51, 20.54, 24.27, 29.45, 24.89, 19.78 for W2, and 2.91, 32.88, 28.45, 40.89, 173.92, 124.89 for W3 respectively.  We rigorously proved that \opmvotm{s} satisfy the correctness criteria as \opty.


%Garbage collection gave a performance gain of 15\%  over \mvotm without garbage collection in the best case. Thus, the overhead of garbage collection is less than the performance improvement due to improved memory usage. This gave performance gain of 22\% over \mvotm without garbage collection in the best case. 

%Furthermore, we optimize \mvotm with limited (say $K$) number of versions corresponding to each key. We find that this optimization improves the performance even further.
%compare our proposed \mvotm with limited number of version.


 

==> Submitted MVOSTM Journal-2019/correctness.tex <==
\section{Correctness of \opmvotm}
\label{sec:cmvostm}
In this section, we will prove that our implementation satisfies opacity. Consider the history $H$ generated by \emph{OPT-MVOSTM} algorithm. Recall that only the \emph{t\_begin}, \rvmt{}, t\_insert(), \upmt{} (or $tryC$) access shared memory. 

Note that $H$ is not necessarily sequential: the transactional \mth{s} can execute in an overlapping manner. To reason about correctness, we have to prove $H$ is opaque. Since we defined opacity for histories which are sequential, we order all the overlapping \mth{s} in $H$ to get an equivalent sequential history. We then show that this resulting sequential history satisfies \mth{}.

We order overlapping \mth{s} of $H$ as follows: (1) two overlapping \emph{t\_begin} \mth{s} based on the order in which they obtain lock over the $counter$; (2) two \rvmt{s} accessing the same key $k$ by their order of unlocking over $\langle \bp, \rp, \rc, \\\bc \rangle$ of $k$; (3) an \rvmt{} $rvm_i(k)$ and a $t\_insert_j()$, of a transaction $T_j$ accessing the same key $k$, are ordered by their order of unlocking over $\langle \bp, \rp, \\\rc, \bc \rangle$ of $k$; (4) an \rvmt{} $rvm_i(k)$ and a $\tryc_j$, of a transaction $T_j$ which has written to $k$, are similarly ordered by their order of unlocking over $\langle \bp, \rp, \rc, \bc \rangle$ of $k$; (5) two t\_insert{()} methods accessing the same key $k$ by their order of unlocking over $\langle \bp, \rp, \rc, \bc \rangle$ of $k$; (6) a $t\_insert_i()$ and a $\tryc_j$, of a transaction $T_j$ which has written to $k$, are similarly ordered by their order of unlocking over $\langle \bp, \rp, \rc, \bc \rangle$ of $k$; (7) similarly, two \tryc{} \mth{s} based on the order in which they unlock over $\langle \bp, \rp, \rc, \bc \rangle$ of same key $k$.

Combining the real-time order of events with above-mentioned order, we obtain a partial order which we denote as \emph{$\locko_H$}. (It is a partial order since it does not order overlapping \rvmt{s} on different $keys$ or an overlapping \rvmt{} and a \tryc{} which do not access any common $key$). 



In order for $H$ to be sequential, all its \mth{s} must be ordered. Let $\alpha$ be a total order or \emph{linearization} of \mth{s} of $H$ such that when this order is applied to $H$, it is sequential. We denote the resulting history as $H^{\alpha} = \seq{\alpha}{H}$. 
% ~
We now argue about the \validity{} of histories generated by the algorithm. 
\begin{lemma}
	\label{lem:histvalid}
	Consider a history $H$ generated by the \opmvotm algorithm. Let $\alpha$ be a linearization of $H$ which respects $\locko_H$, i.e. $\locko_H \subseteq \alpha$. Then $H^{\alpha} = \seq{\alpha}{H}$ is \valid. 
\end{lemma}

\begin{proof}
	Consider a successful \rvmt{} $rvm_i(k)$ that returns value $v$. The \rvmt{} first obtains the lock on $\langle \bp, \rp, \rc, \bc \rangle$ of key $k$. Thus the value $v$ returned by the \rvmt{} must have already been stored in $k$'s version list by a transaction, say $T_j$ when it successfully returned OK from its \tryc{} \mth{}. For this to have occurred, $T_j$ must have successfully locked and released $\langle \bp, \rp, \rc, \\\bc \rangle$ of $k$ prior to $T_i$'s locking \mth. Thus from the definition of $\locko_H$, we get that $\tryc_j(ok)$ occurs before $rvm_i(k,v)$ which also holds in $\alpha$. 
	
	%If $T_j$ is $T_0$, then by our assumption we have that $T_j$ committed before the start of any \mth{} in $H$. Hence, this automatically implies that in both cases $H^{\alpha}$ is \valid.  
\end{proof}

It can be seen that for proving correctness, any linearization of a history $H$ is sufficient as long as the linearization respects $\locko_H$. The following lemma formalizes this intuition, 

\begin{lemma}
	\label{lem:histseq}
	Consider a history $H$. Let $\alpha$ and $\beta$ be two linearizations of $H$ such that both of them respect $\locko_H$, i.e. $\locko_H \subseteq \alpha$ and $\locko_H \subseteq \beta$. Then, $H^{\alpha} = \seq{\alpha}{H}$ is opaque if $H^{\beta} = \seq{\beta}{H}$ is opaque. 
\end{lemma}

\begin{proof} From \lemref{histvalid}, we get that both $H^{\alpha}$ and $H^{\beta}$ are \valid{} histories. Now let us consider each case \\
	\textbf{If:}  Assume that $H^{\alpha}$ is opaque. Then, we get that there exists a legal \tseq{} history $S$ that is equivalent to $\overline{H^{\alpha}}$. From the definition of $H^{\beta}$, we get that $\overline{H^{\alpha}}$ is equivalent to $\overline{H^{\beta}}$. Hence, $S$ is equivalent to $\overline{H^{\beta}}$ as well. We also have that, $\prec_{H^{\alpha}}^{RT} \subseteq \prec_{S}^{RT}$. From the definition of $\locko_H$, we get that $\prec_{H^{\alpha}}^{RT} = \prec_{\locko_H}^{RT} = \prec_{H^{\beta}}^{RT}$. This automatically implies that $\prec_{H^{\beta}}^{RT} \subseteq \prec_{S}^{RT}$. Thus $H^{\beta}$ is opaque as well. 
	
	~ \\
	\textbf{Only if:} This proof comes from symmetry since $H^{\alpha}$ and $H^{\beta}$ are not distinguishable. 
\end{proof}

This lemma shows that, given a history $H$, it is enough to consider one sequential history $H^{\alpha}$ that respects $\locko_H$ for proving correctness. If this history is opaque, then any other sequential history that respects $\locko_H$ is also opaque.

Consider a history $H$ generated by \opmvotm{} algorithm. We then generate a sequential history that respects $\locko_H$. For simplicity, we denote the resulting sequential history of \opmvotm{} as $H_{to}$. Let $T_i$ be a committed transaction in $H_{to}$ that writes to $k$ (i.e. it creates a new version of $k$). 

To prove the correctness, we now introduce some more notations. We define $\stl{T_i}{k}{H_{to}}$ as a committed transaction $T_j$ such that $T_j$ has the \emph{smallest timestamp larger (or stl)} than $T_i$ in $H_{to}$ that writes to $k$ in $H_{to}$. Similarly, we define $\lts{T_i}{k}{H_{to}}$ as a committed transaction $T_k$ such that $T_k$ has the \emph{largest timestamp smaller (or lts)} than $T_i$ that writes to $k$ in $H_{to}$. \cmnt{ We denote $\vli{ts}{x}{H_{to}}$, as the $v\_tuple$ in $x.vl$ after executing all the events in $H_{to}$ created by transaction $T_{ts}$. If no such $v\_tuple$ exists then it is nil. }Using these notations, we describe the following properties and lemmas on $H_{to}$,

\begin{property}
	\label{prop:uniq-ts}
	Every transaction $T_i$ is assigned a unique numeric timestamp $i$.
\end{property}

\begin{property}
	\label{prop:ts-inc}
	If a transaction $T_i$ begins after another transaction $T_j$ then $j < i$.
\end{property}

\begin{lemma}
	\label{lem:readsfrom}
	If a transaction $T_k$ looks up key $k_x$ from (a committed transaction) $T_j$ then $T_j$ is a committed transaction updating to $k_x$ with $j$ being the largest timestamp smaller than $k$. Formally, $T_j = \lts{T_k}{k_x}{H_{to}}$. 
\end{lemma}

\begin{proof}
    We prove it by contradiction. So, assume that transaction $T_k$ looks up key $k_x$ from $T_i$ that has committed before $T_j$ so, from \propref{ts-inc}, $i<k$ and $k<j$ i.e. $i$ is not largest timestamp smaller than $k$. But given statement in this lemma is $i<j<k$ which contradicts our assumption. Hence, $T_k$ looks up key $k_x$ from $T_j$ which is the largest timestamp smaller than $k$.
\end{proof}

\cmnt{
	\begin{definition}
		\label{def:fLP}
		%For each successful method, $LP$ is the first unlocking point of that method. 
		Linearization Point (LP) is the first unlocking point of each successful method.
	\end{definition}
}

\begin{lemma}
	\label{lem:readswrite}
	Suppose a transaction $T_k$ looks up $k_x$ from (a committed transaction) $T_j$ in $H_{to}$, i.e. $\{\up_j(k_{x,j}, v), \rvm_k(k_{x,i}, v)\} \in \evts{H_{to}}$. Let $T_i$ be a committed transaction that updates to $k_x$, i.e. $\up_i(k_{x,i}, u) \in \evts{T_i}$. Then, the timestamp of $T_i$ is either less than $T_j$'s timestamp or greater than $T_k$'s timestamp, i.e. $i<j \oplus k<i$ (where $\oplus$ is XOR operator). 
\end{lemma}

\begin{proof}
	We will prove this by contradiction. Assume that $i<j \oplus k<i$ is not true. This implies that, $j<i<k$. But from the implementation of \rvmt{} and \tryc{} \mth{s}, we get that either transaction $T_i$ is aborted or $T_k$ looks up $k$ from $T_i$ in $H$. Since neither of them are true, we get that $j<i<k$ is not possible. Hence, $i<j \oplus k<i$. 
\end{proof}

To show that $H_{to}$ satisfies opacity, we use the graph characterization developed above in \secref{gcofo}. For the graph characterization, we use the version order defined using timestamps. Consider two committed transactions $T_i, T_j$ such that $i < j$. Suppose both the transactions write to key $k$. Then the versions created are ordered as $k_i \ll k_j$. We denote this version order on all the $keys$ created as $\ll_{to}$. Now consider the opacity graph of $H_{to}$ with version order as defined by $\ll_{to}$, $G_{to} = \opg{H_{to}}{\ll_{to}}$. In the following lemmas, we will prove that $G_{to}$ is acyclic.

\begin{lemma}
	\label{lem:edgeorder}
	All the edges in $G_{to} = \opg{H_{to}}{\ll_{to}}$ are in timestamp order, i.e. if there is an edge from $T_j$ to $T_i$ then the $j < i$. 
\end{lemma}

\begin{proof}
	To prove this, let us analyze the edges one by one, 
	\begin{itemize}
		\item \rt{} edges: If there is an \rt{} edge from $T_j$ to $T_i$, then $T_j$ terminated before $T_i$ started. Hence, from \propref{ts-inc} we get that $j < i$.
		
		\item \rvf{} edges: This follows directly from \lemref{readsfrom}.
		
		\item \mv{} edges: The \mv{} edges relate a committed transaction $T_k$ updates to a key $k$, $up_k(k,v)$; a successful \rvmt{} $rvm_j(k,u)$ belonging to a transaction $T_j$ looks up $k$ updated by a committed transaction $T_i$, $up_i(k, u)$. Transactions $T_i, T_k$ create new versions $k_i, k_k$ respectively. According to $\ll_{to}$, if $k_k \ll_{to} k_i$, then there is an edge from $T_k$ to $T_i$. From the definition of $\ll_{to}$ this automatically implies that $k < i$.
		
		On the other hand, if $k_i \ll_{to} k_k$ then there is an edge from $T_j$ to $T_k$. Thus, in this case, we get that $i < k$. Combining this with \lemref{readswrite}, we get that $j < k$. 
		
		
		%	\item \mv{} edges: The \mv{} edges relate a committed transaction $T_i$ updates to a key $k$, $up_i(k,u)$; a successful \rvmt{} $rvm_k(k,v)$ belonging to a transaction $T_k$ lookup $k$ updated by a committed transaction $T_j$, $up_j(k, v)$ and transaction $T_j$. Transactions $T_j, T_i$ create new versions $k_i, k_j$ respectively. According to $\ll_{to}$, if $k_i \ll_{to} k_j$, then there is an edge from $T_i$ to $T_j$. From the definition of $\ll_{to}$ this automatically implies that $i < j$.
		
		%	On the other hand, if $k_j \ll_{to} k_i$ then there is an edge from $T_k$ to $T_i$. Thus in this case, we get that $j < i$. Combining this with \lemref{readswrite}, we get that $k < i$. 
	\end{itemize}
	Thus in all the cases, we have shown that if there is an edge from $T_j$ to $T_i$ then the $j < i$.
\end{proof}


\begin{theorem}
	\label{thm:to-opaque}
	Any history $H_{to}$ generated by \opmvotm is \opq. 
\end{theorem}

\begin{proof}
	From the definition of $H_{to}$ and \lemref{histvalid}, we get that $H_{to}$ is \valid. We show that $G_{to} = \opg{H_{to}}{\ll_{to}}$ is acyclic. We prove this by contradiction. Assume that $G_{to}$ contains a cycle of the form, $T_{c1} \rightarrow T_{c2} \rightarrow .. T_{cm} \rightarrow T_{c1}$. From \lemref{edgeorder} we get that, $c1 < c2 < ... < cm < c1$ which implies that $c1 < c1$. Hence, a contradiction. This implies that $G_{to}$ is acyclic. Thus from \thmref{opg}, we get that $H_{to}$ is opaque.
\end{proof}

Now, it is left to show that our algorithm is \emph{live}, i.e., under certain conditions, every operation eventually completes. We have to show that the transactions do not deadlock. This is because all the transactions lock all $\langle \bp, \rp, \rc, \bc \rangle$ of $keys$ in a predefined order. As discussed earlier, the STM system orders all $\langle \bp, \rp, \rc, \bc \rangle$ of $keys$. We denote this order as \aco and denote it as $\prec_{ao}$. Thus $k_1 \prec_{ao} k_2 \prec_{ao} ... \prec_{ao} k_n$. 

From \aco, we get the following property


\begin{property}
	\label{prop:aco}
	Suppose transaction $T_i$ accesses shared objects $p$ and $q$ in $H$. If $p$ is ordered before $q$ in \aco, then $lock(p)$ by transaction $T_i$ occurs before $lock(q)$. Formally, $(p \prec_{ao} q) \Leftrightarrow (lock(p) <_H lock(q))$. 
\end{property}

\begin{theorem}
	\label{thm:prog}
	\opmvotm with unbounded versions ensures that \rvmt{s} do not abort.
\end{theorem}
\begin{proof}
	This is self-explanatory with the help of \opmvotm{} algorithm because each $key$ is maintaining multiple versions in the case of unbounded versions. So \rvmt{} always finds a correct version to read it from. Thus, \rvmt{s} do not $abort$. 
\end{proof}

%\noindent \thmref{prog} gives us a nice property a transaction with \tlook only \mth{s} will not abort. 

==> Submitted MVOSTM Journal-2019/design.tex <==
\section{\emph{\opmvotm{s}} Design and Data Structure}
\label{sec:mvdesign}
This section describes the design and data structure of optimized \emph{\mvotm{s}} (or \emph{\opmvotm{s}}). Here, we propose hash-table and list based \emph{\opmvotm{s}} as \emph{\ophmvotm} and \emph{\oplmvotm} respectively. \emph{\opmvotm{s}} are generic for other data structure as well. \emph{\ophmvotm} is a \tab based \opmvotm that explores the idea of multiple versions in \otm{s} for \tab object to achieve greater concurrency. The design of \ophmvotm is similar to \hmvotm{} \cite{Juyal+:MVOSTM:SSS:2018} consisting of $B$ buckets. All the keys of the \tab in the range $\mathcal{K}$ are statically allocated to one of these buckets. 

Each bucket consists of linked-list of nodes along with two sentinel nodes \emph{head} and \emph{tail} with values -$\infty$ and +$\infty$ respectively. The structure of each node is as $\langle key, ~ lock, ~ \\ marked, ~ vl, ~ nnext \rangle$. The $key$ is a unique value from the set of all keys $\mathcal{K}$. All the nodes are stored in increasing order in each bucket as shown in \figref{1mvostmdesign} (a), similar to any linked-list based concurrent set implementation \cite{Heller+:LazyList:PPL:2007, Harris:NBList:DISC:2001}. In the rest of the document, we use the terms key and node interchangeably. To perform any operation on a key, the corresponding $lock$ is acquired. $marked$ is a boolean field which represents whether the key is deleted or not. The deletion is performed in a lazy manner similar to the concurrent linked-lists structure \cite{Heller+:LazyList:PPL:2007}. If the $marked$ field is true then key corresponding to the node has been logically deleted; otherwise, it is present. The $vl$ field of the node points to the version list (shown in \figref{1mvostmdesign} (b)) which stores multiple versions corresponding to the key. The last field of the node is $nnext$ which stores the address of the next node. It can be seen that the list of keys in a bucket is as an extension of \emph{\lazy} \cite{Heller+:LazyList:PPL:2007}. Given a node $n$ in the linked-list of bucket $B$ with key $k$, we denote its fields as $n.key$ (or $k.key$), $~ n.lock$ (or $k.lock$), $~ n.marked$ (or $k.marked$), $~ n.vl$ (or $k.vl$), $~ n.nnext$ (or $k.nnext$).

%\hmvotm is a \tab based \mvotm that explores the idea of using multiple versions in \otm{s} for \tab object to achieve greater concurrency. The design of \hmvotm is similar as \hotm{}\cite{Peri+:OSTM:Netys:2018} consisting of $m$ buckets. Each bucket consists of linked-list of nodes along with two sentinel nodes head and tail with values -$\infty$ and +$\infty$ respectively. The structure of each node is as $\langle key, ~ lock, ~ marked, ~ vl, ~ nnext \rangle$. The $key$ $\langle k_1, k_2, ...k_n \rangle$ are unique and store in increasing order in each bucket refer \figref{1mvostmdesign} (a). To perform any operation on the corresponding key $lock$ should be acquired. $marked$ is a Boolean field which represents the key is deleted or not. Here, we perform lazy deletion which is popular in literature lazy-lists \cite{Heller+:LazyList:PPL:2007, Herlihy:ArtBook:2012}. If the $marked$ field is true then key corresponding to the node has been logically deleted otherwise it's present. The $vl$ field of node points to a list as version list to store multiple version corresponding to each key that reduces the number of aborts and provides greater concurrency. The last field of the node is $nnext$ which stores the address of the next node. 

%that addresses a concurrent \textit{hash-table} as a shared data structure 

%\vspace{-.3cm}
\cmnt{
\begin{figure}
	\centering
	\captionsetup{justification=centering}
	\centerline{\scalebox{0.47}{\input{figs/mvostm10.pdf_t}}}
	\caption{\htmvotm design}
	\label{fig:1mvostmdesign1}
\end{figure}
%\vspace{-.3cm}
}
%\vspace{-.7cm}
\begin{figure}
	\centering
	\captionsetup{justification=centering}
	\centerline{\scalebox{0.4}{\input{figs/design.pdf_t}}}
	\caption{Optimized \emph{HT-MVOSTM} design}
	\label{fig:1mvostmdesign}
\end{figure}

%\vspace{-.7cm}
The structure of each version in the $vl$ of a key $k$ is $\langle ts, ~ val, ~ rvl, ~ max_{rvl}, ~ vnext \rangle$ as shown in \figref{1mvostmdesign} (b). The field $ts$ denotes the unique timestamp of the version. In our algorithm, every transaction is assigned a unique timestamp when it begins which is also its $id$. Thus $ts$ of this version is the timestamp of the transaction that created it. All the versions in the $vl$ of $k$ are sorted by $ts$. Since the timestamps are unique, we denote a version, $ver$ of a node $n$ with key $k$ having $ts$ $j$ as $n.vl[j].ver$ or $k.vl[j].ver$. The corresponding fields in the version as $k.vl[j].ts, ~ k.vl[j].val, ~ k.vl[j].rvl, ~ k.vl[j].max_{rvl}, \\~ k.vl[j].vnext$. 

The field $val$ contains the value updated by an update transaction. If this version is created by an insert \mth $\tins_i(ht, k, v)$ by transaction $T_i$, then $val$ will be $v$. On the other hand, if the \mth is $\tdel_i(ht, k, v)$ then $val$ will be $null$. In this case, as per the algorithm, the node of key $k$ will also be marked. \ophmvotm algorithm does not immediately physically remove deleted keys from the \tab. The need for this is explained below. Thus an \rvmt (\tdel or \tlook) on key $k$ can return $null$ when it does not find the key or encounters a $null$ value for $k$. 

The $rvl$ field stands for \emph{return value list} which is a list of all the transactions that executed \rvmt{} on this version, i.e., those transactions which returned $val$. The first optimization in \emph{\ophmvotm} to reduce the traversal time of $rvl$, we have used $max_{rvl}$  which contains the maximum $ts$ of the transaction that executed \rvmt{} on this version. The field $vnext$ points to the next available version of that key. 

In order to increase the efficiency and utilize the memory properly, We propose two variants of \emph{\ophmvotm} as follows: First, we apply garbage collection (or GC) on the versions and propose \emph{\ophmvotmgc}. It maintains unbounded versions in $vl$ (the length of the list) while deleting the unwanted versions using garbage collection scheme. Second, we propose \emph{\ophkotm} which maintains the bounded number of versions such as $K$ and improves the efficiency further. Whenever a new version $ver$ is created and is about to be added to $vl$, the length of $vl$ is checked. If the length becomes greater than $K$, the version with lowest $ts$ (i.e., the oldest) is replaced with the new version $ver$ and thus maintaining the length back to $K$. 

We propose \emph{\oplmvotm{s}} while considering the bucket size as 1 in \emph{\ophmvotm}. Along with this, we propose two variants of \emph{\oplmvotm}
as \emph{\oplmvotmgc} and \emph{\oplkotm} which applies the garbage collection scheme in unbounded versions and bounded $K$ versions for list based object respectively  similar to \emph{\ophmvotm}.
\ignore{
%The need of adding the $ts$ field in the version list to identify the cyclic conflict which violates \opty{} \cite{GuerKap:Opacity:PPoPP:2008}. %This is shown by the graph characterization in \secref{conflicts} of \figref{1mvostm1} if any cyclic conflict will occur then the generated history leads to non \opq{} history.    
%	\vspace{-.3cm}

	\begin{figure}
	\captionsetup{justification=centering}
		%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
		%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
		\centerline{\scalebox{0.40}{\input{figs/pnetys5.pdf_t}}}
		\caption{Need of maintaining deleted node in underlying DS to satisfy opacity}
		\label{fig:mvostm81}
	\end{figure}	
%	\vspace{-.3cm}

\textbf{Why do we need to store the deleted node?} This will be clear by the \figref{mvostm81}, where we have two concurrent transactions $T_2$ and $T_3$. History in the \figref{mvostm81} (a) is not opaque because we can't come up with any serial order. To make it serial (or opaque) the second method $ins_2(ht, k_{3,2})$ of transaction $T_2$ has to return abort. For that \hmvotm scheduler have to keep the information about the already executed conflicting method $del_3(ht, k_{3,0}, NULL)$ of transaction $T_3$ using $ts$. Therefore, $del_3(ht, k_{3,0}, NULL)$ of transaction $T_3$ add itself into $T_1.rvl$ (assume that transaction $T_1$ has already inserted a version on key $k_3$ refer \figref{mvostm81} (c). So in future if any lower time-stamp transaction less than $T_3$ will come then that lower transaction will ABORT (in this case transaction $T_2$ is aborting in (\figref{mvostm81} (b)) because higher time-stamp already present in the $rvl$ (\figref{mvostm81} (c)) of the same version. After aborting $T_2$ we will get the equivalent serial history $T_2$ followed by $T_3$ %\todo{Change according to updated fig,}.
}

\vspace{1mm}
\noindent
\textbf{Marked Version Nodes:} \ophmvotm stores keys even after they have been deleted (the version of the nodes which have $marked$ field as true). This is because some other concurrent transactions could read from a different version of this key and not the $null$ value inserted by the deleting transaction. Consider for instance the transaction $T_1$ performing $lu_1(ht, k_2, v_0)$ as shown in \figref{pop} (b). Due to the presence of previous version $v_0$, \ophmvotm returns this earlier version $v_0$ for $lu_1(ht, k_2, v_0)$ \mth. Whereas, it is not possible for \hotm to return the version $v_0$  because $k_1$ has been removed from the system by delete method of higher timestamp transaction $T_2$ than $T_1$. In that case, $T_1$ would have to be aborted. Thus as explained in \secref{intro}, storing multiple versions increases the concurrency. 

To store deleted keys along with the live keys (or unmarked node) in a \lazy will increase the traversal time to access unmarked nodes. Consider \figref{nostm2}, in which there are four keys $\langle k_2, k_4, k_8, k_{11}\rangle$ present in the list. Here $\langle k_2, k_4, k_8 \rangle$ are marked (or deleted) nodes while $k_{11}$ is unmarked. Now, consider accessing the key $k_{11}$ by \ophmvotm as a part of one of its methods. Then \ophmvotm would have to unnecessarily traverse the marked nodes to reach key $k_{11}$. %So, this motivates us to maintain a data structure \lsl{} corresponding to each bucket of \tab{} \cite{DBLP:journals/corr/abs-1709-00681}. Along with it also stores version list corresponding to each key that reduces number of aborts. 

%corresponding to each bucket of \tab{} where each key also maintains the version list to reduces number of aborts.  
%\vspace{-.7cm}
\begin{figure}
	\centering
	\begin{minipage}[b]{0.49\textwidth}
		\centering
		\captionsetup{justification=centering}
		\scalebox{.38}{\input{figs/pnetys6.pdf_t}}
		% \vspace{-16cm}
		\caption{Searching $k_{11}$ over \emph{lazy-list}}
		\label{fig:nostm2}
	\end{minipage}   
	\hfill
	\begin{minipage}[b]{0.49\textwidth}
		\scalebox{.38}{\input{figs/pnetys9.pdf_t}}
		\centering
		\captionsetup{justification=centering}
		% \vspace{-16cm}
		\caption{Searching $k_{11}$ over $\lsl{}$}
		\label{fig:nostm}
	\end{minipage}
\end{figure}
%\vspace{-.7cm}
This motivated us to modify the \lazy structure of nodes in each bucket to form a skip list based on red and blue links. We denote it as \emph{red-blue lazy-list} or \emph{\lsl}. This idea was earlier explored by Peri et al. in developing \otm{s} \cite{Peri+:OSTM:Netys:2018}. $\lsl{}$ consists of nodes with two links, red link (or \rn) and blue link (or \bn). The node which is not marked (or not deleted) are accessible from the head via \bn{}. While all the nodes including the marked ones can be accessed from the head via \rn. With this modification, let us consider the above example of accessing unmarked key $k_{11}$. It can be seen that $k_{11}$ can be accessed much more quickly through \bn as shown in \figref{nostm}. Using the idea of $\lsl{}$, we have modified the structure of each node as \emph{$\langle$ key, lock, marked, vl, \rn, \bn $\rangle$}. Further, for a bucket $B$, we denote its linked-list as $B.\lsl$. 

\ignore{

Now, if node corresponding to the key doesn't exist in the underlying DS then \textbf{How we will maintain the node time-stamp by \rvmt{}?} This case will occur when node corresponding to the key is not present in \bn{} as well as \rn{}. Then \rvmt{} will create the node corresponding to the key in \rn{} with marked field as true and append the $0^{th}$ version in its $vl$ and add itself into $0^{th}.rvl$. Inserting the $0^{th}$ version ensures that the transactions which contain only \rvmt{s} will never abort. 
%\vspace{-.7cm}
\begin{figure}
	\centering
	\captionsetup{justification=centering}
	\scalebox{.4}{\input{figs/pnetys10.pdf_t}}
	% \vspace{-16cm}
	\caption{Execution under \lsl{}. $k_{20}$ is added in \lsl{} if not present.}
	\label{fig:nostm1}
\end{figure}
%\vspace{-.7cm}

Consider the \figref{nostm}, in which \npluk{} want to search a key $k_{20}$. Here, the key $k_{20}$ is not present in the \bn{} as well as \rn{}. So it will create the node corresponding to the key in \rn{} with marked field as true and append the $0^{th}$ version in its $vl$ and add itself into $0^{th}.rvl$ refer \figref{nostm1}. 

Each transaction maintains local log in the form of $L\_txlog$ where they store unique transaction id, status and $L\_list$. If transaction is currently executing or committed or aborted due to some inconsistency then status will be live, commit or abort, respectively. $L\_list$ is a vector which contains $\langle bucket\_id, key, val, preds, currs, op\_status, opn \rangle$. The $op\_status$ is an operation status which could be $OK$ or $FAIL$.
Each \mth{} identifies the location corresponding to the key in \bn{} and \rn{} from \lsl{} where they have to work and store the $preds$ and $currs$ in the form of an array. $opn$ stands for operation name which could be \npluk, \npins{}, \npdel{} which will work on $key$. 

}


==> Submitted MVOSTM Journal-2019/dpcode.tex <==
\section{Detailed Pcode of MVOSTM}
\label{apn:rpcode}
%\vspace{-.3cm}


\subsection{Global DS}
\begin{lstlisting}{language = C++}
struct G_node{
int G_key;
struct G_vl;
G_lock;			
node G_knext;    
};
\end{lstlisting}

\begin{lstlisting}{language = C++}
struct G_vl{
int G_ts;
int G_val;
bool G_mark; 	
/*rvl stands for return value list*/
int G_rvl[];			
vl G_vnext;    
};
\end{lstlisting}

\subsection{Local DS}

\begin{lstlisting}{language = C++}
class L_txlog{
int L_t_id;			
STATUS L_tx_status;
vector <L_rec> L_list;
find();
getList();
};
\end{lstlisting}

\begin{lstlisting}{language = C++}
class L_rec{
int L_obj_id;
int L_key; 
int L_val;		
node* L_knext, G_pred, G_curr, node;
STATUS L_op_status;		
OP_NAME L_opn;
getOpn();	getPreds&Currs();  getOpStatus();
getKey&Objid();	getVal();	   getAptCurr();
setVal();	setPreds&Currs();  setOpStatus();   setOpn();
};
enum OP_NAME = {INSERT, DELETE, LOOKUP}
enum STATUS = {ABORT = 0, OK, FAIL, COMMIT}
\end{lstlisting}

\begin{table}[H]
	\centering
	\begin{tabular}{ || m{8em} | m{9cm}|| } 
		\hline
		\textbf{Functions} & \textbf{Description} \\ 
		\hline 		\hline
		setOpn() & set method name into transaction local log\\ 
		\hline
		setVal() & set value of the key into transaction local log\\ 
		\hline
		setOpStatus() & set status of method into transaction local log\\ 
		\hline
		setPred\&Curr() & set location of $G\_pred$ and $G\_curr$ according to the node corresponding to the key into transaction local log\\ 
		\hline
		getOpn() & get method name from transaction local log\\ 
		\hline
		getVal() & get value of the key from transaction local log\\ 
		\hline
		getOpStatus() & get status of the method from transaction local log\\ 
		\hline
		getKey\&Objid() & get key and obj\_id corresponding to the method from transaction local log\\ 
		\hline
		getPred\&Curr() & get location of $G\_preds$ and $G\_currs$ according to the node corresponding to the key from transaction local log \\ 
		\hline		
	\end{tabular}
	\caption{Description of accessing transaction local log methods}
	\label{tabel:1}
\end{table}


\begin{table}[H]
	\centering
	\begin{tabular}{ || m{2.3cm} | m{2.3cm} | m{2.3cm} | m{2.3cm} | m{2.3cm}|| } 
		\hline
		\textbf{p/q} & \textbf{\npins{}} & \textbf{\npdel{}} & \textbf{\npluk{}} & \textbf{\nptc} \\ 
		\hline 		
		\textbf{\npins{}} & + & + & + & +\\
		\hline
		\textbf{\npdel{}} & + & + & + & -\\
		\hline
		\textbf{\npluk{}} & + & + & + & -\\
		\hline
		\textbf{\nptc{}} & + & - & - & -\\
		\hline
	\end{tabular}
	\caption{Commutative table}
	\label{tabel:2}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STM_init()
 %Return the transaction id ($L\_t\_id$) at \Lineref{begin8}.

%Transaction id ($L\_t\_id$), object id (L\_obj\_id), node corresponding to the key (L\_key) and value(L\_val) are the inputs of this function.  

\cmnt{
\setlength{\textfloatsep}{0pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%rv_method()%%%%%%%%%%%%%
\begin{algorithm} [H]
%\label{alg:llsearch} 
\scriptsize
\caption{\emph{\rvmt()} }
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{0}\makeatother
\Procedure{\rvmt{()}}{}
\If{(($m_{ij}(k)$ == \npluk{}) $||$ ($m_{ij}(k)$ == \npdel{}))}
\If{(k $\in$ local\_log(key))}
\State Update the local log \& return;
\Else
\State Search into the $CDS$ to identify the $preds$ \& $currs$ for key in \bn{} \& \rn.
\State Acquire the locks in increasing order.
\If{($!rv\_Validation()$)}
\State Release the locks and retry;
\ElsIf{(k $\notin$ $CDS$)} 
\State Create the new node in \rn{} and add the $T_0$ version in it. 
\EndIf
\State $find\_lts():$ Identify the version with largest TS as $T_j$ but less then TS($T_i$);
\State Add TS($T_i$) into $rvl$ of $T_j$;
\State Release the locks and update the local log;
\EndIf
\EndIf
\EndProcedure
\end{algorithmic}
%\end{multicols}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%rv_validation()%%%%%%%%%%%%%
\begin{algorithm} [H]
%\label{alg:llsearch} 
\scriptsize
\caption{\emph{rv\_Validation()} }
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{0}\makeatother
\Procedure{rv\_validation{()}}{}
\If{$((\bp.marked) || (\bc.marked) ||(\bp.\bn) \neq \bc || (\rp.\rn) \neq {\rc})$}
\State return $false$;
\Else 
\State return $true$;
\EndIf 
\EndProcedure
\end{algorithmic}
%\end{multicols}
\end{algorithm}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%try_C()%%%%%%%%%%%%%
\begin{algorithm} [H]
%\label{alg:llsearch} 
\scriptsize
\caption{\emph{tryC()} }
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{0}\makeatother
\Procedure{tryC{()}}{}
\State Get the local log list for corresponding transaction;
\ForAll{(opn $\in$ local\_log\_list)}
\If{(($m_{ij}(k)$ == \npins{}) $||$ ($m_{ij}(k)$ == \npdel{}))}
\State Search into the $CDS$ to identify the $preds$ \& $currs$ for key in \bn{} \& \rn;
\State Acquire the locks in increasing order;
\If{($!rv\_Validation()$)}
\State Release the locks and retry;
\EndIf
\State $find\_lts():$ If (k $\in$ $CDS$) then identify the version with largest TS as $T_j$ but less then TS($T_i$);
\If{($!tryC\_Validation()$)}
\State return $Abort$;
\EndIf
\EndIf
\EndFor
\ForAll{(opn $\in$ local\_log\_list)}
\If{(($m_{ij}(k)$ == \npins{}) $||$ ($m_{ij}(k)$ == \npdel{}))}
\State $intraTransValidation():$ Update the preds and currs of consecutive operation working on same region.
\If{(k $\notin$ CDS)}
\State Create the new node in \rn{}, \bn{} and add the $T_0$ version in it;
\EndIf
\State $find\_lts():$ Identify the version with largest TS as $T_j$ but less then TS($T_i$);
\State Add TS($T_i$) into $rvl$ of $T_j$;
\State Update the local log;
\EndIf
\EndFor
%\EndFor
\State Release the locks;
\EndProcedure
\end{algorithmic}
%\end{multicols}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%tryC_validation()%%%%%%%%%%%%%
\begin{algorithm} [H]
%\label{alg:llsearch} 
\scriptsize
\caption{\emph{tryC\_Validation()} }
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{0}\makeatother
\Procedure{tryC\_validation{()}}{}
\ForAll {$T_k$ in $rvl$ of $T_j$}
\If{(TS($(T_k)$ $>$ TS($T_i$)))}
\State return $false$;
\EndIf 
\EndFor
\EndProcedure
\end{algorithmic}
%\end{multicols}
\end{algorithm}

 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Local Log Search()%%%%%%%%%%%%%
\begin{algorithm} [H]
\label{alg:llsearch} 
\scriptsize
\caption{\emph{MV-OSTM} Algorithm}
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{0}\makeatother
%\Procedure{STM local log search}{key} \label{lin:ll1}
\If{($G\_key$ $\in$ local\_log($L\_key$))} \label{lin:ll2}\Comment{Search into local log}
\If{$(($\textup{INSERT} $=$ \textup{$L\_opn$} $)||($ \textup{LOOKUP} $=$ \textup{$L\_opn$}$))$} \label{lin:ll3};
\State $L\_val$ $\gets$ $L\_getVal(L\_opn,L\_key)$ \label{lin:ll4};
\State $L\_op\_status$ $\gets$  $L\_getOpStatus$(L\_opn, L\_key) \label{lin:ll5};
%\State Update the local log.\label{lin:ll6}
			\ElsIf{$($\textup{DELETE} $=$ \textup{$L\_opn$}$)$} \label{lin:ll7}
			\State $L\_val$ $\gets$ NULL \label{lin:ll8}; 
			\State $L\_op\_status$ $\gets$ FAIL \label{lin:ll9}; 
\EndIf
\State Update the local log.
\State return $\langle L\_val$, $L\_op\_status \rangle$.\label{lin:ll10}
\EndIf

\State \Comment{Traversal phase}
\State $\bp$ $\gets$ $G\_head$ \label{lin:ltraversal2}; 
\State $\bc$ $\gets$ $\bp.\bn$ \label{lin:ltraversal3};
\While{$((\bc.key) < L\_key)$} \label{lin:ltraversal4};
\State $\bp$ $\gets$ $\bc$ \label{lin:ltraversal5};
\State $\bc$ $\gets$ $\bc.\bn$ \label{lin:ltraversal6};
\EndWhile \label{lin:ltraversal12}
\State $\rp$ $\gets$ $\bp$ \label{lin:ltraversal7}; 
\State $\rc$ $\gets$ $\rp.\rn$ \label{lin:ltraversal8};
\While{$((\rc.key) < L\_key)$} \label{lin:ltraversal9}
\State $\rp$ $\gets$ $\rc$ \label{lin:ltraversal10};
\State $\rc$ $\gets$ $\rc.\rn$ \label{lin:ltraversal11};
\EndWhile \label{lin:ltraversal14}
\State Update the \preds{} and \currs{} into local log.
\State \Comment{Validation phase}
\If{(($\bp$.marked) || ($\bc$.marked) ||($\bp.\bn$) $\neq$ $\bc$ || ($\rp.\rn$) $\neq$ {$\rc$})}\Comment{Validation}
\State return $\langle RETRY \rangle$;
\Else
\State return $\langle OK \rangle$;
\EndIf
\State /*Find the largest time-stamp but less then itself($T_i$).*/
\State $find\_lts$(max(closest\_tuple(TS($T_j$))) $<$ TS($T_i$))
\ForAll {($T_k$ $\in$ rvl($T_i$))}
\If{(TS($T_i$) < TS($T_k$))}
\State return $\langle ABORT \rangle$;
\Else
\State return $\langle OK \rangle$;
\end{algorithmic}
%\end{multicols}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------------------------------TryCommit----------------------------------%---------
%----
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[H]
\scriptsize
	\caption{\tabspace[0.2cm] STM $tryC()$ }
	\label{algo:trycommit}
	\setlength{\multicolsep}{0pt}
		%\begin{multicols}{2}
	\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{33}\makeatother
		\Procedure{STM tryC}{($L\_t\_id$)} \label{lin:tryc1}
    \State $L\_list$ $\gets$ $getList$($L\_t\_id$) \label{lin:tryc3};
		\While{$(\textbf{$L\_rec_{i} \gets \textup{next}(L\_list$}))$} \label{lin:tryc5}
		\State ($L\_key, L\_obj\_id$) $\gets$ \llgkeyobj{} \label{lin:tryc6};
		\State \lsls{$COMMIT \downarrow$} \label{lin:tryc8};
			
		\If {$((\bc.key = L\_key) \& (\checkv(L\_t\_id \downarrow,\bc \downarrow) = FALSE))$}\label{lin:tryc9}
\State Unlock all the variables;\label{lin:tryc10}
\State return $ABORT$;\label{lin:tryc11}
\ElsIf {$((\rc.key = L\_key) \& (\checkv(L\_t\_id \downarrow,\rc \downarrow) = FALSE))$}\label{lin:stryc9}
\State Unlock all the variables;\label{lin:stryc10}
\State return $ABORT$;\label{lin:stryc11}

\EndIf;\label{lin:tryc12}
		\State \llspc{} \label{lin:tryc14};
		\EndWhile \label{lin:tryc15}
	\While{$(\textbf{$L\_rec_{i} \gets \textup{next}(L\_list$}))$} \label{lin:tryc17}
		\State ($L\_key, L\_obj\_id$) $\gets$ \llgkeyobj{} \label{lin:tryc18};
		\State $L\_opn$ $\gets$ $(L\_rec)_{i}$.$L\_opn$ \label{lin:tryc20};
		\State intraTransValdation($L\_rec_{i} \downarrow$, $\preds \uparrow$, $\currs \uparrow$) \label{lin:tryc42};
		\If{$($\textup{INSERT} $=$ \textup{$L\_opn$}$)$} \label{lin:tryc22}
		\If{$(\bc.key) = L\_key)$} \label{lin:tryc23}
	\State insert $v\_tuple \langle L\_t\_id,val,F,NULL,NULL \rangle$ into $G\_curr.vl$ in the increasing order;	\label{lin:tryc24}
	
	\ElsIf{$(\rc.key) = L\_key)$} \label{lin:stryc23}
	\State \lslins{$RL\_BL \downarrow$} \label{lin:stryc24}
	\State insert $v\_tuple \langle L\_t\_id,val,F,NULL,NULL \rangle$ into $G\_curr.vl$ in the increasing order;	\label{lin:stryc25}
	
		\Else \label{lin:tryc25}
		\State \lslins{$BL \downarrow$} \label{lin:tryc27};
		\State insert $v\_tuple \langle L\_t\_id,val,F,NULL,NULL \rangle$ into $node.vl$ in the increasing order;	\label{lin:tryc28}
	\EndIf \label{lin:tryc29}
\ElsIf{$($\textup{DELETE} $=$ $L\_opn)$} \label{lin:tryc31}
	\If{$(\bc.key) = L\_key)$} \label{lin:tryc33}
		\State insert $v\_tuple \langle L\_t\_id,NULL,T,NULL,NULL \rangle$ into $G\_curr.vl$ in the increasing order;	\label{lin:tryc34}
			\State \lsldel{} \label{lin:stryc35};
		\EndIf \label{lin:tryc39}
	
		\EndIf \label{lin:tryc40}
		\EndWhile \label{lin:tryc43}
        \State \rlsol{} \label{lin:tryc45};  
        \State $L\_tx\_status$ $\gets$ OK \label{lin:tryc47};
		\State return $\langle L\_tx\_status\rangle$\label{lin:tryc48};
		\EndProcedure \label{lin:tryc49}
	\end{algorithmic}
	%	\end{multicols}
\end{algorithm}

}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STM_init()

\begin{algorithm} 
\label{alg:init} 
\scriptsize

\caption{STM $\init()$: This method invokes at the start of the STM system. Initialize the global counter ($\cnt$) as 1 at \Lineref{init1} and return it.}
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{52}\makeatother	
\Procedure{STM init}{$\cnt \uparrow$}
\cmnts{Initializing the global counter}
\State $\cnt$ $\gets$ 1; \label{lin:init1}
\cmnt{
\ForAll {key $G\_k$ used by the STM System}
%\State /* $T_0$ is initializing key $k$ */
\State /*$T_0$ is initializing key $k$*/
\State add $\langle 0, 0, T, NULL, NULL \rangle$ to $G\_k.vl$;  \label{lin:init} %\Comment{Implies that $T_0$ has initialized $x$}
\EndFor;
}
\State return $\langle \cnt \rangle$; 
\EndProcedure
\end{algorithmic}
	
%	\end{multicols}
\end{algorithm}




\cmnt{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Traversal Phase%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[H]
\scriptsize
	\caption{list\_traversal() : It finds the location of the node corresponding to the key in underlying DS. First it identifies the node in \bn{} then in \rn{}. After finding the appropriate $\preds$ and $\currs$ corresponding to the key, it acquires the locks and validate it.}
	\label{algo:traversal}
	\setlength{\multicolsep}{0pt}
		%\begin{multicols}{2}
	\begin{algorithmic}[1]
	\makeatletter\setcounter{ALG@line}{166}\makeatother	
	\Procedure{list\_traversal}{$L\_Bucket\_id, L\_key$} \label{lin:ltraversal1}

%\cmnts{By default setting the $L\_op\_status$ as RETRY}\label{lin:lslsearch2}
	    %\State STATUS $L\_op\_status$ $\gets$ RETRY; \label{lin:lslsearch3}
	 %\cmnts{Identify the \preds and \currs for node corresponding to the key if $L\_op\_status$ is RETRY}\label{lin:lslsearch4}   
		%\While{($L\_op\_status$ = \textup{RETRY})} \label{lin:lslsearch5}
	%	\cmnts{Get the head of the bucket in chaining hash-table with the help of $L\_obj\_id$ and $L\_key$}\label{lin:lslsearch6}
		%\State $G\_head$ $\gets$ \glslhead \label{lin:lslsearch7};
	%	\cmnts{Initialize $\bp$ to head}\label{lin:lslsearch8}
		\State $\bp$ $\gets$ $G\_head$ \label{lin:ltraversal2}; 
	%	\cmnts{Initialize $\bc$ to $\bp.\bn$}\label{lin:lslsearch10}
		\State $\bc$ $\gets$ $\bp.\bn$ \label{lin:ltraversal3};
	%	\cmnts{Searching node corresponding to the key into \bn}
		\While{$((\bc.key) < L\_key)$} \label{lin:ltraversal4};
		\State $\bp$ $\gets$ $\bc$ \label{lin:ltraversal5};
				
		\State $\bc$ $\gets$ $\bc.\bn$ \label{lin:ltraversal6};
			
	%\EndWhile \label{lin:lslsearch15}
		
%		\cmnts{Initialize $\rp$ to head}\label{lin:slslsearch8}
		\State $\rp$ $\gets$ $\bp$ \label{lin:ltraversal7}; 
%		\cmnts{Initialize $\rc$ to $\rp.\rn$}\label{lin:slslsearch10}
		\State $\rc$ $\gets$ $\rp.\rn$ \label{lin:ltraversal8};
	%	\cmnts{Searching node corresponding to the key into \rn}
		\While{$((\rc.key) < L\_key)$} \label{lin:ltraversal9}
		\State $\rp$ $\gets$ $\rc$ \label{lin:ltraversal10};
				
		\State $\rc$ $\gets$ $\rc.\rn$ \label{lin:ltraversal11};
			
		\EndWhile \label{lin:ltraversal12}
		
		
		%\State    /*get the value*/
		%\State $L\_val$ $\gets$ $G\_curr.value$
		%\cmnts{Acquire the locks on increasing order of keys}\label{lin:lslsearch16}
	    \State acquirePred\&CurrLocks($ \preds$, $ \currs$); \label{lin:ltraversal13}
%\cmnts{Method validation to identify the changes done by concurrent conflicting method}\label{lin:lslsearch19}
		%\State methodValidation($\preds$ $\downarrow$, $\currs$ $\downarrow$, $L\_op\_status \uparrow$)\label{lin:lslsearch20};	
		%\State $op\_status$ $\gets$ \validation \label{lin:lslsearch21};
%\cmnts{If $L\_op\_status$ is RETRY then release all the locks}		\label{lin:lslsearch21}
	%	\If{(($L\_op\_status$ = \textup{RETRY}))} \label{lin:lslsearch22}
	   % \State releasePred\&CurrLocks($ \preds \downarrow$, $ \currs \downarrow$);
	    %\EndIf \label{lin:lslsearch25}
			
		\EndWhile \label{lin:ltraversal14}
		
		\State return $\langle G\_preds[], G\_currs[]\rangle$ \label{lin:ltraversal15};
	
	\EndProcedure \label{lin:ltraversal16}
	
	\end{algorithmic}
	%	\end{multicols}
\end{algorithm}
%\end{spacing}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STM_begin()
\begin{algorithm} 
\label{alg:begin} 
\scriptsize
\caption{STM $begin()$: It invoked by a thread to being a new transaction $T_i$. It creates transaction local log and allocate unique id at \Lineref{begin3} and \Lineref{begin5} respectively.}
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{88}\makeatother
\Procedure{STM begin}{$\cnt \downarrow$, $L\_t\_id \uparrow$} \label{lin:begin1}
\cmnts{Creating a local log for each transaction}\label{lin:begin2}
\State \txll $\gets$ create new \txllf;  \label{lin:begin3}
%\State /*Acquiring lock on live set of transaction*/
%\State $\livetx.lock()$;  
\cmnts{Getting transaction id ($L\_t\_id$) from $\cnt$}\label{lin:begin4}
\State \txll.$L\_t\_id$ $\gets$ $\cnt$;  \label{lin:begin5}
\cmnts{Incremented global counter atomically $\cnt$}\label{lin:begin6}
\State $\cnt$ $\gets$ \gi; //$\Phi_{lp}(Linearization Point)$ \label{lin:begin7}
%\State add $t\_id$ to $\livetx$; 
%\State /*Release lock on live set of transaction*/
%\State $\livetx.unlock()$; 
\State return $\langle L\_t\_id \rangle$; \label{lin:begin8}
\EndProcedure\label{lin:begin9}
\end{algorithmic}
%\end{multicols}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STM_ Insert()

\begin{algorithm}[H]

	\caption{STM $insert():$ Optimistically, the actual insertion will happen in the \nptc{} method. First, it will identify the node corresponding to the key in local log. If the node exists then it just update the local log with useful information like value, operation name and status for the node corresponding to the key at \Lineref{insert8}, \Lineref{insert9} and \Lineref{insert10} respectively for later use in \nptc{}. Otherwise, it will create a local log and update it.}
    \scriptsize
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
	\label{algo:insert}
	\begin{algorithmic}[1]
	\makeatletter\setcounter{ALG@line}{97}\makeatother
	\Procedure{STM insert}{$L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_val \downarrow$}\label{lin:insert1}
	\cmnts{First identify the node corresponding to the key into local log using $find()$ funciton}\label{lin:insert2}
		\If{$(!$\txlfind$)$}\label{lin:insert3}
		\cmnts{Create local log record and append it into increasing order of keys} \label{lin:insert4}
		\State $L\_rec$ $\gets$ create new $L\_rec \langle L\_obj\_id, L\_key \rangle$; \label{lin:insert5}
		\EndIf \label{lin:insert6}
		\cmnts{Updating the local log} \label{lin:insert7}		\State \llsval{$L\_val \downarrow$};//$\Phi_{lp} (Linearization Point)$ \label{lin:insert8}
		\State \llsopn{$INSERT \downarrow$}; \label{lin:insert9}
		\State \llsopst{$OK \downarrow$}; \label{lin:insert10}
		\State return $\langle void \rangle$; \label{lin:insert11} 
    	%\State loclog.setOpStatus$(obj\_id \downarrow, key \downarrow, OK \downarrow)$;
    \EndProcedure	\label{lin:insert12}
	\end{algorithmic}
%\end{multicols}	
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------------------------------STM\_LOOKUP-------------------------------------%------
%----
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{spacing}{2}
\begin{algorithm}[H]
	%\algsetup{linenosize=\tiny}
	
	\caption{\tabspace[0.2cm] STM $lookup_{i}()$: If \npluk{} is not the first method on a particular key means if its a subsequent method of the same transaction on that key then first it will search into the local log from \Lineref{lookup3} to \Lineref{lookup14}. If the previous method on the same key of same transaction was insert or lookup (from \Lineref{lookup7} to \Lineref{lookup9}) then \npluk{} will return the value and operation status based on previous operation value and status. If the previous method on the same key of same transaction was delete (from \Lineref{lookup11} to \Lineref{lookup13}) then \npluk{} will return the value and operation status as NULL and FAIL respectively. If \npluk{} is the first method on that key (from \Lineref{lookup16} to \Lineref{lookup22}) then it will identify the location of node corresponding to the key in underlying DS with the help of \nplsls{} inside the \npcld{} method at \Lineref{lookup17}.} %: If the transaction to which this operation belongs has locally done an operation on the same key then returns apt value and status(wrt the previous local operation). Else do the \nplsls{} to find the correct location of the key and validate it.
		%\emph{DESCP}\tabspace: If the Tx has locally done an operation returns apt value and status else does TO \tabspace[2.2cm] and method validation traversal phase in only.\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $obj\_id$, $key$\\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $value$, $op\_status$     }
	\scriptsize
	\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
		
		\label{algo:lookup}
		%	\setlength{\multicolsep}{0pt}
		%	\begin{multicols}{2}
		
		\begin{algorithmic}[1]
			\makeatletter\setcounter{ALG@line}{109}\makeatother
			\Procedure{STM lookup}{$L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_val \uparrow, L\_op\_status \uparrow$} \label{lin:lookup1}
			%\State $op\_status$ $\gets$ RETRY \label{lin:lookup2};
			\cmnts{First identify the node corresponding to the key into local log}\label{lin:lookup2}
			\If{$($\txlfind$)$} \label{lin:lookup3}
			\cmnts{Getting the previous operation's name}\label{lin:lookup4}
			\State $L\_opn$ $\gets$ \llgopn{} \label{lin:lookup5}; %\Comment{$\Phi_{lp}$}
			\cmnts{If previous operation is insert/lookup then get the value/op\_status based on the previous operations value/op\_status}\label{lin:lookup6}
			\If{$(($\textup{INSERT} $=$ \textup{$L\_opn$} $)||($ \textup{LOOKUP} $=$ \textup{$L\_opn$}$))$} \label{lin:lookup7}
			
			\State $L\_val$ $\gets$ \llgval{} \label{lin:lookup8};
			\State $L\_op\_status$ $\gets$  $L\_rec.L\_getOpStatus$($L\_obj\_id \downarrow, L\_key \downarrow$) \label{lin:lookup9};
			\cmnts{If previous operation is delete then set the value as NULL and op\_status as FAIL}\label{lin:lookup10}
			\ElsIf{$($\textup{DELETE} $=$ \textup{$L\_opn$}$)$} \label{lin:lookup11}
			\State $L\_val$ $\gets$ NULL \label{lin:lookup12}; 
			\State $L\_op\_status$ $\gets$ FAIL \label{lin:lookup13}; 
			\EndIf \label{lin:lookup14}
			%	\EndIf \label{lin:lookup11}
			\Else \label{lin:lookup15}
			\cmnts{ Common function for \rvmt{}, if node corresponding to the key is not part of local log}\label{lin:lookup16}
			\State \cld{};\label{lin:lookup17}
			\cmnt{		
				%\State $op\_status $ $\gets$ lslSearch($obj\_id$ $\downarrow$, $key$ $\downarrow$, $preds[]$ $\uparrow$, $currs[]$ $\uparrow$, $value_{BL}$ $\uparrow$, $RV$ $\downarrow$);	
				\State    /*if key is not present in local log then search in underlying DS with the help of list\_lookup*/
				\State \lsls{} \label{lin:lookup13}; 
				%State    /*if list\_lookup return op\_status as ABORT then method will return ABORT*/
				%If{$(op\_status_{ll}$ $=$ \textup{ABORT}$)$} \label{lin:lookup14}
				%			\State release all the locks
				%State \handlea{} \label{lin:lookup15}; 
				%Else \label{lin:lookup16}
				%			\State    /*check node corresponding to the key is part of underlying DS or not*/	
				%			\If{$((G\_curr.key) == L\_key)$} \label{lin:lookup17}
				\State /*From $G\_k.vls$, identify the right $version\_tuple$*/ 
				\State \find($L\_t\_id \downarrow,L\_key \downarrow, closest\_tuple \uparrow)$;	
				\State /*Adding $L\_t\_id$ into $j$'s $rvl$*/
				\State Append $L\_t\_id$ into $rvl$; 
				%                   \State \emph{unlock $x$};
				%                    \State return $(v)$; \Comment{v is the value returned}
				\If{$(closest\_tuple.m = TRUE)$}
				
				\State $L\_op\_status$ $\gets$ FAIL \label{lin:lookup18};
				\State $L\_val$ $\gets$ NULL \label{lin:lookup20};
				\Else
				\State $L\_op\_status$ $\gets$ OK;
				\State $L\_val$ $\gets$ $closest\_tuple.v$;
				\EndIf    
				%            \Else
				%                    \State /*Adding $i$ into $0$'s $rvl$*/
				%                    \State Append $i$ into $rvl$; 
				%                    \State $L\_op\_status$ $\gets$ FAIL;
				%                    \State $L\_val$ $\gets$ $NULL$;
				%\EndIf \label{lin:lookup30}
				
				
				\State $G\_pred.unlock()$;//$\Phi_{lp}$
				\State $G\_curr.unlock()$;
				\State    /*new log entry created to help upcoming method on the same key of the same tx*/
				\State $L\_rec$ $\gets$ Create new $L\_rec\langle L\_obj\_id, L\_key \rangle$\label{lin:lookup31}; 
				%\State ll.setPreds&Currs($obj\_id$ $\downarrow$, $key$ $\downarrow$, $preds[]$ $\downarrow$, $currs[]$ $\downarrow$);
				\State \llsval{$L\_val \downarrow$}
				\State \llspc{} \label{lin:lookup32};
			}						  
			
			%\EndIf \label{lin:lookup38}
			
			\EndIf \label{lin:lookup18}
			\cmnts{Update the local log} \label{lin:lookup19}
			\State \llsopn{$LOOKUP \downarrow$} \label{lin:lookup20};
			\State \llsopst{$L\_op\_status \downarrow$} \label{lin:lookup21};
			
			\State return $\langle L\_val, L\_op\_status\rangle$\label{lin:lookup22}; 
			
			\EndProcedure \label{lin:lookup23}
		\end{algorithmic}
		
%	\end{multicols}
	
\end{algorithm}



%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------------------------------STM\_DELETE-------------------------------------%------
%----
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{spacing}{2}
\begin{algorithm}[H]
%\algsetup{linenosize=\tiny}
\scriptsize
	\caption{\tabspace[0.2cm] STM $delete_{i}()$ : It will work same as a \npluk{}. If it is not the first method on a particular key means if its a subsequent method of the same transaction on that key then first it will search into the local log from \Lineref{delete3} to \Lineref{delete23}. If the previous method on the same key of same transaction was insert (from \Lineref{delete77} to \Lineref{delete10}) then \npdel{} will return the value based on previous operation value and status as OK and set the value and operation as NULL and DELETE respectively. 
    If previous method on the same key of same transaction was delete (from \Lineref{delete12} to \Lineref{delete15}) then \npdel{} will return the value and operation status as NULL and FAIL respectively.
    If previous method on the same key of same transaction was lookup (from \Lineref{delete16} to \Lineref{delete21}) then \npdel{} will return the value and operation status based on the previous operation value and status. If \npdel{} is the first method on that key (from \Lineref{delete24} to \Lineref{delete30}) then it will identify the location of node corresponding to the key in underlying DS with the help of \nplsls{} inside the \npcld{} method at \Lineref{delete25}.}
		%\emph{DESCP}\tabspace: If the Tx has locally done an operation returns apt value and status else does TO \tabspace[2.2cm] and method validation traversal phase in only.\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $obj\_id$, $key$\\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $value$, $op\_status$     }
	\label{algo:delete}
	\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
	
	\begin{algorithmic}[1]
	\makeatletter\setcounter{ALG@line}{132}\makeatother
		\Procedure{STM delete}{$L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_val \uparrow, L\_op\_status \uparrow$} \label{lin:delete1}
		%\State $op\_status$ $\gets$ RETRY \label{lin:lookup2};
			\cmnts{First identify the node corresponding to the key into local log}\label{lin:delete2}
		\If{$($\txlfind$)$} \label{lin:delete3}
	    \cmnts{Getting the previous operation's name}\label{lin:delete4}
			\State $L\_opn$ $\gets$ \llgopn{} ;\label{lin:delete5} %\Comment{$\Phi_{lp}$}
		\cmnts{If previous operation is insert then get the value based on the previous operations value and set the value and operation name as NULL and DELETE respectively}\label{lin:delete6}
		\If{$($\textup{INSERT} $=$ \textup{$L\_opn$}$)$} \label{lin:delete77}
		\State $L\_val$ $\gets$ \llgval{} \label{lin:delete7};
		
		\State \llsval{NULL $\downarrow$} \label{lin:delete8};

		\State \llsopn{DELETE $\downarrow$} \label{lin:delete9};
		
		\State $L\_op\_status$ $\gets$ OK \label{lin:delete10};
		\cmnts{If previous operation is delete then set the value as NULL}\label{lin:delete11}
		\ElsIf{$($\textup{DELETE} $=$ \textup{$L\_opn$}$)$} \label{lin:delete12}
		\State \llsval{NULL $\downarrow$} \label{lin:delete13};
		\State $L\_val$ $\gets$ NULL \label{lin:delete14}; 
		\State $L\_op\_status$ $\gets$ FAIL \label{lin:delete15}; 
		\Else \label{lin:delete16}
		
		\cmnts{If previous operation is lookup then get the value based on the previous operations value and set the value and operation name as NULL and DELETE respectively}\label{lin:delete17}
		\State $L\_val$ $\gets$ \llgval{} \label{lin:delete18}; 
		
		\State \llsval{NULL$ \downarrow$} \label{lin:delete19};
		
		
		\State \llsopn{DELETE $\downarrow$} \label{lin:delete20};
		\State $L\_op\_status$ $\gets$  $L\_rec.getOpStatus$($L\_obj\_id \downarrow$, $L\_key \downarrow$) \label{lin:delete21};
		
		\EndIf \label{lin:delete22}
		
		\Else \label{lin:delete23}
						  
					
	%	\EndIf 
		    \cmnts{Common function for \rvmt{}, if node corresponding to the key is not part of local log}\label{lin:delete24}
			\State \cld{};		\label{lin:delete25}
		\EndIf \label{lin:delete26}
		\cmnts{Update the local log}\label{lin:delete27}
		\State \llsopn{$DELETE \downarrow$} ;\label{lin:delete28}
			\State \llsopst{$L\_op\_status \downarrow$} ;\label{lin:delete29}
			
			\State return $\langle L\_val, L\_op\_status\rangle$; \label{lin:delete30}
				
	\EndProcedure\label{lin:delete31}
	\end{algorithmic}
	
%	\end{multicols}
	
\end{algorithm}
\cmnt{
\begin{figure}[H]
	\captionsetup{justification=centering}
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centerline{\scalebox{0.38}{\input{figs/pnetys5.pdf_t}}}
	\caption{Need of inserting $0^{th}$ version by \rvmt{} to satisfy opacity}
	\label{fig:mvostm8}
\end{figure}	
}
\begin{figure}[H]
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centerline{\scalebox{0.35}{\input{figs/mvostm8.pdf_t}}}
	\caption{Need of inserting $0^{th}$ version by \rvmt{} to satisfy opacity}
	\label{fig:mvostm8}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------------------------------commonLu\&Del-------------------------------------%------
%----
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{spacing}{2}
\begin{algorithm}[H]
%\algsetup{linenosize=\tiny}
%\scriptsize
	\caption{\tabspace[0.2cm] $commonLu\&Del()$ : This method is invoked by a \rvmt{} (\npluk{} and \npdel{}$)$, if node corresponding to the key is not part of local log. At \Lineref{com3} it identify the $\preds$ and $\currs$ for the node corresponding to the key in underlying DS with the help of \nplsls{}. If node corresponding to the key is in \bn{} of underlying DS then (from \Lineref{com5} to \Lineref{com17}) it finds the version tuple corresponding to the key which is having the largest timestamp less than itself as $closest\_tuple$ at \Lineref{com7}. After that, it will add itself into $closest\_tuple.rvl$ at \Lineref{com9}. If identified version mark field is TRUE then it will set the $L\_op\_status$ and $L\_val$ as FAIL and NULL otherwise, OK and value of identified tuple from \Lineref{com11} to \Lineref{com17} respectively. If node corresponding to the key is in \rn{} of underlying DS then (from \Lineref{scom5} to \Lineref{scom17}) it finds the version tuple corresponding to the key which is having the largest timestamp less than itself as $closest\_tuple$ at \Lineref{scom7}. After that, it will add itself into $closest\_tuple.rvl$ at \Lineref{scom9}. If identified version mark field is TRUE then it will set the $L\_op\_status$ and $L\_val$ as FAIL and NULL otherwise, OK and value of identified tuple from \Lineref{scom11} to \Lineref{scom17} respectively. 
	If node corresponding to the key is not part of underlying DS then (from \Lineref{com19} to \Lineref{com27}) it will create the new node corresponding to the key and add it into \rn{} of underlying DS with the help of \nplslins{} at \Lineref{com20}. After that it creates the $0^{th}$ version (at \Lineref{com22}) and add itself into $0^{th}.rvl$ at \Lineref{com23}. Then, it will set the $L\_op\_status$ and $L\_val$ as FAIL and NULL respectively at \Lineref{com25} and \Lineref{com26}. Finally, it will release the lock which is acquired in \nplsls{} at \Lineref{com3} and update the local log to help the upcoming method of the same transaction on the same key. \textbf{Why do we need to create a $0^{th}$ version by \rvmt{} in \rn{}?} This will be clear by the \figref{mvostm8}, where we have two concurrent transactions $T_1$ and $T_2$. History in the \figref{mvostm8}.a) is not opaque because we can't come up with any serial order. To make it serial (or opaque) first method $lu_2(ht, k_3, NULL)$ of transaction $T_2$ have to create the $0^{th}$ version in \rn{} if its not present in the underlying DS and add itself into $0^{th}.rvl$. So in future if any lower timestamp transaction less than $T_2$ will come then that lower transaction will ABORT (in this case transaction $T_1$ is aborting in (\figref{mvostm8}.b))) because higher timestamp already present in the $rvl$ (\figref{mvostm8}.c)) of the same version. After aborting $T_1$ we will get the serial history.}
	\scriptsize
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
	
	\label{algo:commonlu&del}
%	\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
	
	\begin{algorithmic}[1]
	\makeatletter\setcounter{ALG@line}{164}\makeatother
		\Procedure{commonLu\&Del}{$L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_val \uparrow, L\_op\_status \uparrow$} \label{lin:com1} %\label{lin:commonlu&del}
		%\State $op\_status$ $\gets$ RETRY \label{lin:lookup2};
    \cmnts{If node corresponding to the key is not present in local log then search into underlying DS with the help of list\_lookup} \label{lin:com2}
			\State \lsls{}\label{lin:com3};
			\cmnts{ If node corresponding to the key is part of \bn{}}\label{lin:com4}
			\If{$(\bc.key = L\_key)$}\label{lin:com5}
						\cmnts{From $\bc.vls$, identify the right $version\_tuple$} \label{lin:com6}
                    \State \find($L\_t\_id \downarrow,\bc \downarrow, closest\_tuple \uparrow)$;\label{lin:com7}
                    
                    \cmnts{ Closest\_tuple is $\langle j,val,mark,rvl,vnext \rangle$} \label{lin:com8}

                    \State Adding $L\_t\_id$ into $j$'s $rvl$; \label{lin:com9}
                    %\State Append $L\_t\_id$ into $rvl$; 
 %                   \State \emph{unlock $x$};
%                    \State return $(v)$; \Comment{v is the value returned}
\cmnts{If the $closest\_tuple$ mark field is TRUE then $L\_op\_status$ and $L\_val$ set as FAIL and NULL otherwise set OK and value of $closest\_tuple$ respectively}\label{lin:com10}
                \If{$(closest\_tuple.mark = TRUE)$}\label{lin:com11}
                    
                    \State $L\_op\_status$ $\gets$ FAIL \label{lin:com12};
                    \State $L\_val$ $\gets$ NULL \label{lin:com13};
                \Else\label{lin:com14}
                    \State $L\_op\_status$ $\gets$ OK;\label{lin:com15}
                    \State $L\_val$ $\gets$ $closest\_tuple.val$; \label{lin:com16}
                \EndIf    \label{lin:com17}
        \cmnts{If node corresponding to the the key is part of \rn }
			\ElsIf{$(\rc.key = L\_key)$}\label{lin:scom5}
						\cmnts{From $\rc.vls$, identify the right $version\_tuple$} \label{lin:scom6}
                    \State \find($L\_t\_id \downarrow,\rc \downarrow, closest\_tuple \uparrow)$;\label{lin:scom7}
                    
                    \cmnts{Closest\_tuple is $\langle j,val,mark,rvl,vnext \rangle$} \label{lin:scom8}
\algstore{myalg}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}                     
	\begin{algorithmic} [1]                   % enter the algorithmic environment
			\scriptsize
		\algrestore{myalg}
                    \State Adding $L\_t\_id$ into $j$'s $rvl$; \label{lin:scom9}
                    %\State Append $L\_t\_id$ into $rvl$; 
 %                   \State \emph{unlock $x$};
%                    \State return $(v)$; \Comment{v is the value returned}
\cmnts{If the $closest\_tuple$ mark field is TRUE then $L\_op\_status$ and $L\_val$ set as FAIL and NULL otherwise set OK and value of $closest\_tuple$ respectively}\label{lin:scom10}
                \If{$(closest\_tuple.mark = TRUE)$}\label{lin:scom11}
                    
                    \State $L\_op\_status$ $\gets$ FAIL \label{lin:scom12};
                    \State $L\_val$ $\gets$ NULL \label{lin:scom13};
                \Else\label{lin:scom14}
                    \State $L\_op\_status$ $\gets$ OK;\label{lin:scom15}
                    \State $L\_val$ $\gets$ $closest\_tuple.val$; \label{lin:scom16}
                \EndIf    \label{lin:scom17}
 
        
        
                
        \Else\label{lin:com18}
        		\cmnts{If node corresponding to the key is not part of \rn as well as \bn then create the node into \rn with the help of list\_Ins()}\label{lin:com19}
		        \State \lslins{$RL \downarrow$};\label{lin:com20}
		        \cmnts{Insert the $0^{th}$ version tuple} \label{lin:com21}
		        \State insert $v\_tuple \langle 0,NULL,T,NULL,NULL \rangle$ into $node.vl$ in the increasing order;	 \label{lin:com22}
                  \State Adding $L\_t\_id$ into $0^{th}.rvl$;\label{lin:com23}
                    %\State Append $L\_t\_id$ into $rvl$;
                \cmnts{Setting $L\_op\_status$ and $L\_val$ as FAIL and NULL because its reading from the marked version, which is TRUE}\label{lin:com24}    
                \State    $L\_op\_status$ $\gets$ FAIL ;\label{lin:com25}
                    \State $L\_val$ $\gets$ NULL ;\label{lin:com26}
			\EndIf\label{lin:com27}
			\cmnts{Releasing the locks in increasing order}\label{lin:com28}
			  	    \State releasePred\&CurrLocks($ \preds \downarrow$, $ \currs \downarrow$);
\cmnts{Create local log record and append it into increasing order of keys}\label{lin:com31}						\State $L\_rec$ $\gets$ Create new $L\_rec\langle L\_obj\_id, L\_key \rangle$\label{lin:com32}; 
						%\State ll.setPreds&Currs($obj\_id$ $\downarrow$, $key$ $\downarrow$, $preds[]$ $\downarrow$, $currs[]$ $\downarrow$);
						\State \llsval{$L\_val \downarrow$} \label{lin:com33}
						\State \llspc{} ;
						  
			
			\State return $\langle L\_val, L\_op\_status\rangle$;\label{lin:com34}
				
	\EndProcedure 
	\end{algorithmic}
	
%	\end{multicols}
	
\end{algorithm}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------------------------------TryCommit----------------------------------%---------
%----
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[H]
\scriptsize
	\caption{\tabspace[0.2cm] STM $tryC()$ : The actual effect of \upmt{s} (\npins{} and \npdel{}) will take place in \nptc{} method. From \Lineref{tryc5} to \Lineref{tryc15} will identify and validate the $\preds$ and $\currs$ of each \upmt{} of same transaction. At \Lineref{tryc9} it will validate if there exist any higher timestamp transaction in the $rvl$ of the $closest\_tuple$ of $\bc$ then returns ABORT at \Lineref{tryc11}. Same as at \Lineref{stryc9} it will validate if there exist any higher timestamp transaction in the $rvl$ of the $closest\_tuple$ of $\rc$ then returns ABORT at \Lineref{stryc11}. Otherwise it will perform the above steps for remaining \upmt{s}. On successful validation of all the \upmt{s}, the actually effect will be taken place from \Lineref{tryc17} to \Lineref{tryc43}. If the \upmt{} is insert and node corresponding to the key is part of \bn{} then it creates the new version tuple and add it in increasing order of version list from \Lineref{tryc22} to \Lineref{tryc24}. If node corresponding to the key is part of \rn{} then it adds the same node in the \bn{} as well with the help of \nplslins{} at \Lineref{stryc24} and creates the new version tuple and add it in increasing order of version list from \Lineref{stryc23} to \Lineref{stryc25}. Otherwise it will create the node and insert it into \bn{} with the help of \nplslins{} and insert the version tuple from \Lineref{tryc25} to \Lineref{tryc29}. If the \upmt{} is delete and node corresponding to the key is part of \bn{} then it creates the new version tuple and set its mark field as TRUE and add it in increasing order of version list from \Lineref{tryc31} to \Lineref{stryc35}. After successful completion of each \upmt{}, it will validate the $\preds$ and $\currs$ of upcoming \upmt{} of the same transaction with the help of \npintv{} at \Lineref{tryc42}. Eventually, it will release all the locks at \Lineref{tryc45} in the same order of lock acquisition.} %: All update methods will takes effect in underlying data-structure atomically if the validation will succeed. 
		%\emph{DESCP}\tabspace: All update methods of the transaction take ordered locks, validate and update underlying \tabspace[2.2cm]  data-structure atomically. \\
		%\emph{IN}\tabspace \tabspace[0.72cm]: \\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $txstatus$     }
	\label{algo:trycommit}
	\setlength{\multicolsep}{0pt}
%		\begin{multicols}{2}
	\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{213}\makeatother
		\Procedure{STM tryC}{$L\_t\_id \downarrow, L\_tx\_status \uparrow$} \label{lin:tryc1}

%\State    /*get the tx id*/
%		\State $L\_t\_id$ $\gets$ getTS($t_i \downarrow$) \label{lin:tryc2};
		\cmnts{Get the local log list corresponding to each transaction which is in increasing order of keys}\label{lin:tryc2}
		\State $L\_list$ $\gets$ $L\_txlog.getList$($L\_t\_id \downarrow$) \label{lin:tryc3};
%		\State    /*sort the local log in increasing order of keys and copy into ordered list*/
%		\State $L\_ordered$ $\gets$ \llsort{} \label{lin:tryc4};
\cmnts{Identify the new $\preds$ and $\currs$ for all update methods of a transaction and validate it}\label{lin:tryc4}
		\While{$(\textbf{$L\_rec_{i} \gets \textup{next}(L\_list$}))$} \label{lin:tryc5}
		\State ($L\_key, L\_obj\_id$) $\gets$ \llgkeyobj{} \label{lin:tryc6};
		\cmnts{Identify the new $G\_pred$ and $G\_curr$ location with the help of list\_lookup()}\label{lin:tryc7}
		\State \lsls{$COMMIT \downarrow$} \label{lin:tryc8};
			
		\If {$((\bc.key = L\_key) \& (\checkv(L\_t\_id \downarrow,\bc \downarrow) = FALSE))$}\label{lin:tryc9}
%\State $\remid(i)$;
\State Unlock all the variables;\label{lin:tryc10}
\State return $ABORT$;\label{lin:tryc11}
\ElsIf {$((\rc.key = L\_key) \& (\checkv(L\_t\_id \downarrow,\rc \downarrow) = FALSE))$}\label{lin:stryc9}
%\State $\remid(i)$;
\State Unlock all the variables;\label{lin:stryc10}
\State return $ABORT$;\label{lin:stryc11}

\EndIf;\label{lin:tryc12}

					%State    /*if list\_lookup return op\_status as ABORT then method will return ABORT*/
		%If{$(op\_status_{ll}$ $=$ \textup{ABORT}$)$} \label{lin:tryc8}
%		\State release all the locks
		%State \handlea{} \label{lin:tryc9};
		
		%\State return \label{lin:tryc10};
		
		%EndIf \label{lin:tryc11}
			\cmnts{Update the log entry} \label{lin:tryc13}

		\State \llspc{} \label{lin:tryc14};
		\EndWhile \label{lin:tryc15}
	\cmnts{Get each update method one by one and take effect in underlying DS}\label{lin:tryc16}
		\While{$(\textbf{$L\_rec_{i} \gets \textup{next}(L\_list$}))$} \label{lin:tryc17}
		\State ($L\_key, L\_obj\_id$) $\gets$ \llgkeyobj{} \label{lin:tryc18};
		\cmnts{Get the operation name from local log record}\label{lin:tryc19}
		\State $L\_opn$ $\gets$ $(L\_rec)_{i}$.$L\_opn$ \label{lin:tryc20};
		
					\cmnts{Modify the $\preds$ and $\currs$ for the consecutive update methods which are working on overlapping zone in lazy-list}\label{lin:tryc41}
		\State intraTransValdation($L\_rec_{i} \downarrow$, $\preds \uparrow$, $\currs \uparrow$) \label{lin:tryc42};
\cmnts{If operation is insert then after successful completion of it node corresponding to the key should be part of \bn}\label{lin:tryc21}
\algstore{myalg}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}                     
	\begin{algorithmic} [1]                   % enter the algorithmic environment
			\scriptsize
		\algrestore{myalg}
		\If{$($\textup{INSERT} $=$ \textup{$L\_opn$}$)$} \label{lin:tryc22}
	%\State    /*if node corresponding to the key is part of \bn*/
		\If{$(\bc.key) = L\_key)$} \label{lin:tryc23}
	\State insert $v\_tuple \langle L\_t\_id,val,F,NULL,NULL \rangle$ into $G\_curr.vl$ in the increasing order;	\label{lin:tryc24}
	
	\ElsIf{$(\rc.key) = L\_key)$} \label{lin:stryc23}
	\State \lslins{$RL\_BL \downarrow$} \label{lin:stryc24}
	\State insert $v\_tuple \langle L\_t\_id,val,F,NULL,NULL \rangle$ into $G\_curr.vl$ in the increasing order;	\label{lin:stryc25}
	
		\Else \label{lin:tryc25}
		\cmnts{If node corresponding to the key is not part underlying DS then create the node with the help of list\_Ins() and insert it into \bn}\label{lin:tryc26}
		\State \lslins{$BL \downarrow$} \label{lin:tryc27};
		\State insert $v\_tuple \langle L\_t\_id,val,F,NULL,NULL \rangle$ into $node.vl$ in the increasing order;	\label{lin:tryc28}
%	\State    /*set the op\_status as OK in local log*/
%		\State \llsopst{$OK \downarrow$} \label{lin:tryc30};
	%\State    /*update the max\_ts of insert for node corresponding to the key into underlying DS*/		
	%	\State $\texttt{write}$(node.max\_ts.insert, TS($t_i$)) \label{lin:tryc31};
		\EndIf \label{lin:tryc29}
		\cmnts{If operation is delete then after successful completion of it node corresponding to the key should part of \rn only}\label{lin:tryc30}
		\ElsIf{$($\textup{DELETE} $=$ $L\_opn)$} \label{lin:tryc31}
	\cmnts{If node corresponding to the key is part of \bn}\label{lin:tryc32}
	

	
		\If{$(\bc.key) = L\_key)$} \label{lin:tryc33}
	%\State    /*delete the node corresponding to the key from the \bn with the help of lslDel()*/	
			\State insert $v\_tuple \langle L\_t\_id,NULL,T,NULL,NULL \rangle$ into $G\_curr.vl$ in the increasing order;	\label{lin:tryc34}
			\State \lsldel{} \label{lin:stryc35};
%		\State    /*set the op\_status as OK in local log*/
%		\State \llsopst{$OK \downarrow$} \label{lin:tryc36};
		%\State    /*update the max\_ts of delete for node corresponding to the key into underlying DS*/	
		%\State $\texttt{write}$(\textcolor{blue}{$currs[1]$}.max\_ts.delete, TS($t_i$)) \label{lin:tryc37};
\cmnt{
		\Else \label{lin:tryc35}
		\State    /*If node corresponding to the key is not part underlying DS then create the node with the help of list\_Ins() */\label{lin:tryc36}
		\State \lslins{$RL \downarrow$};\label{lin:tryc37}
		
		\State insert $v\_tuple \langle L\_t\_id,NULL,T,NULL,NULL \rangle$ into $node.vl$ in the increasing order;	\label{lin:tryc38}
		%\State \llsopst{$FAIL \downarrow$} \label{lin:tryc39};
		
		%\State $write$(\textcolor{red}{$currs[0]$}.max\_ts.delete, TS($t_i$)) \label{lin:tryc40};
}	
		\EndIf \label{lin:tryc39}
	
		\EndIf \label{lin:tryc40}
		

			
		\EndWhile \label{lin:tryc43}
		\cmnts{Release all the locks in increasing order}\label{lin:tryc44}
		\State \rlsol{} \label{lin:tryc45};  
		\cmnts{Set the transaction status as OK}\label{lin:tryc46}
		\State $L\_tx\_status$ $\gets$ OK \label{lin:tryc47};
%		
%		\State \txsetst{} \label{lin:tryc46};
		\State return $\langle L\_tx\_status\rangle$\label{lin:tryc48};
		\EndProcedure \label{lin:tryc49}
	\end{algorithmic}
%		\end{multicols}
\end{algorithm}


	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%------------------- lazyrblist-delete -----------------------
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\begin{algorithm}[H]
		\scriptsize
		\caption{\tabspace[0.2cm] \dell() : Delete a node from blue link in underlying hash table at location corresponding to $\preds$ \& $\currs$.}
			%\emph{DESCP}\tabspace: Deletes a node from blue list in underlying hash table at location corresponding to \tabspace[2.2cm] preds[] \& currs[].\\
			%\emph{IN}\tabspace \tabspace[0.72cm]: $preds[], currs[]$  \\
			%\emph{OUT}\tabspace \tabspace[0.37cm]:  }
		\label{algo:lsldelete}
		\setlength{\multicolsep}{0pt}
%		\begin{multicols}{2}
			\begin{algorithmic}[1]
				\makeatletter\setcounter{ALG@line}{265}\makeatother
				\Function{list\_del}{$\preds \downarrow, \currs \downarrow$} \label{lin:lsldel1}
				
				%\cmnts{mark the node$ \langle obj\_id, key \rangle$ for deletion}
				%\State $\texttt{write}$($\bc$.marked, True) \label{lin:lsldel2};
				\cmnts{Update the blue links}
				\State $\bp$.\bn $\gets$ $\bc$.\bn \label{lin:lsldel3};
				\State return $\langle void \rangle$;
				\EndFunction \label{lin:lsldel4}
			\end{algorithmic}
			
%		\end{multicols}
	\end{algorithm}
	



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%----------------- List lookup() ---------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{spacing}{0.8}
\begin{algorithm}[H]
\scriptsize
%lslSearch($obj\_id \downarrow, key \downarrow, preds[] \uparrow, currs[] \uparrow, value \uparrow, val\_type \downarrow$)
	\caption{list\_lookup() : This method is called by \rvmt{} and \upmt{}. It finds the location of the node corresponding to the key in underlying DS from \Lineref{lslsearch5} to \Lineref{slslsearch15}. First it identifies the node in \bn{} (from \Lineref{lslsearch5} to \Lineref{lslsearch15}) then in \rn{} (from \Lineref{slslsearch9} to \Lineref{slslsearch15}). After finding the appropriate location of the node corresponding to the key in the form of $\preds$ and $\currs$, it will acquire the locks on it at \Lineref{lslsearch17} and validate it at \Lineref{lslsearch20}.}
		%\emph{DESCP}\tabspace: Finds location of the corresponding $\left\langle obj\_id, key  \right\rangle$ in underlying hash table. color of preds[] \tabspace[2.2cm] \& currs[] depicts the red or blue node.\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $\left\langle obj\_id, key  \right\rangle$, $val\_type$  \\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $preds[], currs[], value$     }
	\label{algo:lslsearch}
	\setlength{\multicolsep}{0pt}
%		\begin{multicols}{2}
	\begin{algorithmic}[1]
	\makeatletter\setcounter{ALG@line}{270}\makeatother	
		\Procedure{list\_lookup}{$L\_obj\_id \downarrow, L\_key \downarrow, G\_preds[] \uparrow, G\_currs[] \uparrow$} \label{lin:lslsearch1}

	\cmnts{By default setting the $L\_op\_status$ as RETRY}\label{lin:lslsearch2}
	    \State STATUS $L\_op\_status$ $\gets$ RETRY; \label{lin:lslsearch3}
	 \cmnts{Identify the \preds and \currs for node corresponding to the key if $L\_op\_status$ is RETRY}\label{lin:lslsearch4}   
		\While{($L\_op\_status$ = \textup{RETRY})} \label{lin:lslsearch5}
		\cmnts{Get the head of the bucket in chaining hash-table with the help of $L\_obj\_id$ and $L\_key$}\label{lin:lslsearch6}
		\State $G\_head$ $\gets$ \glslhead \label{lin:lslsearch7};
		\cmnts{Initialize $\bp$ to head}\label{lin:lslsearch8}
		\State $\bp$ $\gets$ $G\_head$ \label{lin:lslsearch9}; 
		\cmnts{Initialize $\bc$ to $\bp.\bn$}\label{lin:lslsearch10}
		\State $\bc$ $\gets$ $\bp.\bn$ \label{lin:lslsearch11};
		\cmnts{Searching node corresponding to the key into \bn}
		\While{$((\bc.key) < L\_key)$} \label{lin:lslsearch12}
		\State $\bp$ $\gets$ $\bc$ \label{lin:lslsearch13};
				
		\State $\bc$ $\gets$ $\bc.\bn$ \label{lin:lslsearch14};
			
		\EndWhile \label{lin:lslsearch15}
		
		\cmnts{Initialize $\rp$ to head}\label{lin:slslsearch8}
		\State $\rp$ $\gets$ $\bp$ \label{lin:slslsearch9}; 
		\cmnts{Initialize $\rc$ to $\rp.\rn$}\label{lin:slslsearch10}
		\State $\rc$ $\gets$ $\rp.\rn$ \label{lin:slslsearch11};
		\cmnts{Searching node corresponding to the key into \rn}
		\While{$((\rc.key) < L\_key)$} \label{lin:slslsearch12}
		\State $\rp$ $\gets$ $\rc$ \label{lin:slslsearch13};
				
		\State $\rc$ $\gets$ $\rc.\rn$ \label{lin:slslsearch14};
			
		\EndWhile \label{lin:slslsearch15}
		
		
		%\State    /*get the value*/
		%\State $L\_val$ $\gets$ $G\_curr.value$
		\cmnts{Acquire the locks on increasing order of keys}\label{lin:lslsearch16}
	    \State acquirePred\&CurrLocks($ \preds \downarrow$, $ \currs \downarrow$); \label{lin:lslsearch17}
\cmnts{Method validation to identify the changes done by concurrent conflicting method}\label{lin:lslsearch19}
		\State methodValidation($\preds$ $\downarrow$, $\currs$ $\downarrow$, $L\_op\_status \uparrow$)\label{lin:lslsearch20};	
		%\State $op\_status$ $\gets$ \validation \label{lin:lslsearch21};
\cmnts{If $L\_op\_status$ is RETRY then release all the locks}		\label{lin:lslsearch21}
		\If{(($L\_op\_status$ = \textup{RETRY}))} \label{lin:lslsearch22}
	    \State releasePred\&CurrLocks($ \preds \downarrow$, $ \currs \downarrow$);
	    \EndIf \label{lin:lslsearch25}
			
		\EndWhile \label{lin:lslsearch26}
		
		\State return $\langle G\_preds[], G\_currs[]\rangle$ \label{lin:lslsearch27};
	
	\EndProcedure \label{lin:lslsearch28}
	\end{algorithmic}
%		\end{multicols}
\end{algorithm}
%\end{spacing}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%------------------- acquirepreds&currs -----------------------
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\begin{algorithm}[H]
		\scriptsize
		\caption{\tabspace[0.2cm] acquirePred\&CurrLocks() : acquire all locks taken during \nplsls{}.}
			%\emph{DESCP}\tabspace: releases all locks taken during tryCommit\\
			%\emph{IN}\tabspace \tabspace[0.72cm]: $ordered\_ll\_list$\\
			%\emph{OUT}\tabspace \tabspace[0.37cm]:   }
		\label{algo:acquirepreds&currs}
		\setlength{\multicolsep}{0pt}
%		\begin{multicols}{2}
			\begin{algorithmic}[1]
				\makeatletter\setcounter{ALG@line}{306}\makeatother
				\Function{acquirePred\&CurrLocks}{$ \preds \downarrow$, $ \currs \downarrow$}
				\State $\bp$.$\texttt{lock()}$;
				\State $\rp$.$\texttt{lock()}$;
				\State $\rc$.$\texttt{lock()}$;
				\State $\bc$.$\texttt{lock()}$;
				\State return $\langle void \rangle$;        
				\EndFunction
			\end{algorithmic}
			
%		\end{multicols}
	\end{algorithm}
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%------------------- releasepreds&currs -----------------------
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\begin{algorithm}[H]
		\scriptsize
		\caption{\tabspace[0.2cm] releasePred\&CurrLocks() : Release all locks taken during \nplsls{}.}
			%\emph{DESCP}\tabspace: releases all locks taken during tryCommit\\
			%\emph{IN}\tabspace \tabspace[0.72cm]: $ordered\_ll\_list$\\
			%\emph{OUT}\tabspace \tabspace[0.37cm]:    }
		\label{algo:releasepreds&currs}
		\setlength{\multicolsep}{0pt}
%		\begin{multicols}{2}
			\begin{algorithmic}[1]
				\makeatletter\setcounter{ALG@line}{313}\makeatother
				\Function{releasePred\&CurrLocks}{$ \preds \downarrow$, $ \currs \downarrow$}
				\State $\bp$.$\texttt{unlock()}$\label{lin:rpandc};//$\Phi_{lp}$ 
				\State $\rp$.$\texttt{unlock()}$;
				\State $\rc$.$\texttt{unlock()}$;
				\State $\bc$.$\texttt{unlock()}$;
				\State return $\langle void \rangle$;        
				\EndFunction
			\end{algorithmic}
			
%		\end{multicols}
	\end{algorithm}
	%\end{multicols}
	

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%----------------------------list-insert --------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\vspace{-.5cm}
\begin{algorithm}[H]
\scriptsize
	\caption{\tabspace[0.2cm] list\_Ins(): This method is called by the \rvmt{} and \upmt{}. Color of preds \& currs depicts the red or blue node.}
		%\emph{DESCP}\tabspace: Inserts or overwrites a node in underlying hash table at location corresponding to \tabspace[2.2cm] preds[] \& currs[]. Color of preds[] \& currs[] depicts the red or blue node.\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $preds[], currs[], list\_type$  \\
		%\emph{OUT}\tabspace \tabspace[0.37cm]:     }
	\label{algo:lslins}
		\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
	\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{320}\makeatother
		\Procedure{list\_Ins}{$\preds \downarrow, \currs \downarrow, list\_type \downarrow, node \uparrow$} \label{lin:lslins1}


\cmnts{Inserting the node from redlist to bluelist}
				\If{$((list\_type)$ $=$ $($\textcolor{black}{$RL$}$\_$\textcolor{black}{$BL$}$))$} \label{lin:lslins2}
				
				%\State $\texttt{write}$($\rc$.marked, false) \label{lin:lslins3}; 
				\State $\rc$.\bn $\gets$ $\bc$ \label{lin:lslins4};
				\State $\bp$.\bn $\gets$ $\rc$ \label{lin:lslins5};
				\cmnts{Inserting the node into redlist only}
				\ElsIf{$((list\_type$) $=$ \textcolor{black}{$RL$}$)$} \label{lin:lslins6}
				\State node = Create new node()
				\label{lin:lslins7};
						\cmnts{After created the node acquiring the lock on it}\label{lin:lslins4}
		\State node.lock();\label{lin:lslins5}
		
				\State node.\rn $\gets$ $\rc$ \label{lin:lslins9};
				\State $\rp$.\rn $\gets$ node \label{lin:lslins10};
				
				\Else \label{lin:lslins11}
				\cmnts{Inserting the node into red as well as blue list}
				\State node = new node() \label{lin:lslins12}; %\Comment{default locked state for thread validation}
				\cmnts{After creating the node acquiring the lock on it}
				\State node.lock();
				\State node.\rn $\gets$ $\rc$ \label{lin:lslins13};
				\State node.\bn $\gets$ $\bc$ \label{lin:lslins14};
				
				\State $\rp$.\rn $\gets$ node \label{lin:lslins15};
				
				\State $\bp$.\bn $\gets$ node \label{lin:lslins16};
				\EndIf \label{lin:lslins17}
				\State return $\langle node \rangle$;
			
\cmnt{

        \State    /*Inserting the new node corresponding to the key into Underlying DS/\label{lin:lslins2}
		\State node = Create new node() \label{lin:lslins3}; %\Comment{default locked state for thread validation}
		\State    /*After created the node acquiring the lock on it*/\label{lin:lslins4}
		\State node.lock();\label{lin:lslins5}
		\State /*Adding the new node at appropriate location (in increasing order of the keys) with the help of $G\_pred$ and $G\_curr$*/\label{lin:lslins6}
		\State node.knext $\gets$ $G\_curr$ \label{lin:lslins7};
		\State $G\_pred$.knext $\gets$ node \label{lin:lslins8};
		\State return $\langle node \rangle$;\label{lin:lslins9}}
		\EndProcedure \label{lin:lslins10}
	\end{algorithmic}
%	\end{multicols}
\end{algorithm}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% find_lts(largest timestamp but less then itself)   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}  
\scriptsize
\label{alg:select}
\caption{$\find()$: This method is called by \rvmt{} and \upmt{} to identify a  $closest\_tuple$ $\langle j,val,mark,rvl,vnext \rangle$ created by the transaction $T_j$ with the largest timestamp smaller than $L\_t\_id$ from \Lineref{findlts5} to \Lineref{findlts10}.}
		\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{344}\makeatother
\Procedure{find\_lts}{$L\_t\_id \downarrow, \currs \downarrow, closest\_tuple \uparrow$} \label{lin:findlts1}
\cmnts{Initialize $closest\_tuple$} \label{lin:findlts2}
\State $closest\_tuple = \langle 0,NULL,F,NULL,NULL \rangle$;\label{lin:findlts3}
\cmnts{For all the version of $\currs$ identify the largest timestamp less than $L\_t\_id$} \label{lin:findlts4}
\ForAll {$\langle p,val,mark,rvl,vnext \rangle \in \currs.vl$} \label{lin:findlts5}
\If {$(p < L\_t\_id)$ and $(closest\_tuple.ts < p)$} \label{lin:findlts6}
\cmnts{Assign closest tuple as $\langle p,val,mark,rvl,vnext \rangle$, if any version tuple is having largest timestamp less then L\_t\_id exist} \label{lin:findlts7}
\State $closest\_tuple = \langle p,val,mark,rvl,vnext \rangle$; \label{lin:findlts8}
\EndIf\label{lin:findlts9}
\EndFor\label{lin:findlts10}
\State return $\langle closest\_tuple\rangle$; \label{lin:findlts11}
\EndProcedure\label{lin:findlts12}
\end{algorithmic}
%\end{multicols}
\end{algorithm}

\begin{figure} [tbph]
	\captionsetup{justification=centering}
	%\centering
	%\includegraphics[scale=.5]{figs/fig3.png}
	%\includegraphics[scale=.5]{figs/fig3.pdf_t}
	\centerline{\scalebox{0.5}{\input{figs/disc2.pdf_t}}}
	\caption{Validation by $check\_version$}
	\label{fig:mvostmm12}
\end{figure}


\cmnt{
\begin{figure} [tbph]
	%\centering
	%\includegraphics[scale=.5]{figs/fig3.png}
	%\includegraphics[scale=.5]{figs/fig3.pdf_t}
	\centerline{\scalebox{0.5}{\input{figs/mvostm12.pdf_t}}}
	\caption{Validation by $check\_version$}
	\label{fig:mvostm12}
\end{figure}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%---------------------------------Check Version -------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{algorithm}  
\scriptsize
\label{alg:checkVersion} 
\caption{$\checkv()$: This method is called by the \nptc{}. First it will find the $closest\_tuple$ $\langle j,val,mark,rvl,vnext \rangle$ created by the transaction $T_j$ with the largest timestamp smaller than $L\_t\_id$ at \Lineref{checkVersion3}. Then, it checks the version list to identify is there any higher timestamp already present in the $rvl$ of $closest\_tuple$ from \Lineref{checkVersion5} to \Lineref{checkVersion11}. If it presents then it will returns FALSE at \Lineref{checkVersion9} otherwise, TRUE at \Lineref{checkVersion13}. It will be more clear by the \figref{mvostmm12}.a) where second method $ins_1(ht, k_3, ABORT)$ of transaction $T_1$ will ABORT because higher transaction $T_2$ timestamp is already present in the $rvl$ of $closest\_tuple$ as $0^{th}$ version in \figref{mvostmm12}.b).}
		\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{356}\makeatother
\Procedure{check\_versions}{$L\_t\_id \downarrow,\currs \downarrow$} \label{lin:checkVersion1}
\cmnts{From $\currs.vls$, identify the correct $version\_tuple$ means identfy the tuple which is having higher time-stamp but less then it} \label{lin:checkVersion2}
\State $\find(L\_t\_id \downarrow, \currs \downarrow, closest\_tuple \uparrow)$;\label{lin:checkVersion3}	
\cmnts{Got the closest\_tuple as $\langle j,val,mark,rvl,vnext \rangle$}\label{lin:checkVersion4}
%\ForAll {$v\_tuples \langle j,v,rl \rangle $ in $x \cdot vl$}
\ForAll {$T_k$ in $rvl$ of $closest\_tuple.j$}\label{lin:checkVersion5}
\cmnts{$T_k$ has already read the version created by $T_j$}\label{lin:checkVersion6}
\If {$(L\_t\_id < k)$}   \label{lin:checkVersion7}
\cmnts{If in $rvl$ of $closest\_tuple.j$, any higher time-stamp exists then $L\_t\_id$ then return $FALSE$}\label{lin:checkVersion8}
\State return $\langle FALSE\rangle$;  \label{lin:checkVersion9}
\EndIf\label{lin:checkVersion10}
\EndFor\label{lin:checkVersion11}
%\EndFor;
\cmnts{If in $rvl$ of $closest\_tuple.j$, there is no higher time-stamp exists then $L\_t\_id$ then return $TRUE$}\label{lin:checkVersion12}
\State return $\langle TRUE\rangle$;\label{lin:checkVersion13}
\EndProcedure\label{lin:checkVersion14}
\end{algorithmic}
%\end{multicols}
\end{algorithm}

\begin{figure}[tbph]
	\captionsetup{justification=centering}
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centerline{\scalebox{0.47}{\input{figs/disc1.pdf_t}}}
	\caption{Method validation}
	\label{fig:mvostm9}
\end{figure}
\cmnt{
\begin{figure}[tbph]
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centerline{\scalebox{0.5}{\input{figs/mvostm9.pdf_t}}}
	\caption{Method validation}
	\label{fig:mvostm9}
\end{figure}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%---------------------------------methodValidation -------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[H]
\scriptsize
	\caption{\tabspace[0.2cm] methodValidation() : This method is called by the \rvmt{} and \upmt{}. It will identify the conflicts among the concurrent methods of different transactions at \Lineref{iv2}. It will be more clear by the \figref{mvostm9}, where two concurrent conflicting methods of different transactions are working on the same key $k_3$. Initially, at stage $s_1$ in \figref{mvostm9}.c) both the conflicting method optimistically (without acquiring locks) identify the same $\preds$ and $\currs$ for key $k_3$ from underlying DS in \figref{mvostm9}.a). At stage $s_2$ in \figref{mvostm9}.c), method $ins_1(k_3)$ of transaction $T_1$ acquired the lock on $\preds$ and $\currs$ and inserted the node into it (\figref{mvostm9}.b)). After successful insertion by $T_1$, $\preds$ and $\currs$ will change for $lu_2(k_3)$ at stage $s_3$ in \figref{mvostm9}.c). It will caught via method validation function at \Lineref{iv2} when $(\preds.\bn \neq G\_curr)$ for $lu_2(k_3)$. After that again it will find the new $\preds$ and $\currs$ for $lu_2(k_3)$ with the help of \nplsls{} method and eventually it will commit.}
		%\emph{DESCP}\tabspace: method validation for conflicting concurrent operations.\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $preds[]$, $currs[]$\\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $RETRY$, $OK$     }
	\label{algo:interferenceValidation}
			\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
	\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{370}\makeatother	
		\Procedure{methodValidation}{$\preds \downarrow, \currs \downarrow, L\_op\_status \uparrow$} \label{lin:iv1}
	    \cmnts{Validating $\preds$ and $\currs$}
		\If{$((\bp.marked) || (\bc.marked) ||(\bp.\bn) \neq \bc || (\rp.\rn) \neq {\rc})$}  \label{lin:iv2}
		\cmnts{If validation fail then $L\_op\_status$ set as $RETRY$}
        \State $L\_op\_status$ $\gets$ RETRY

		\Else \label{lin:iv4}
		
	    \State $L\_op\_status$ $\gets$ OK

		\EndIf \label{lin:iv6}
				\State return $\langle L\_op\_status\rangle$ \label{lin:iv5};
	
		\EndProcedure \label{lin:iv7}
	\end{algorithmic}
%\end{multicols}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%------------------- find -----------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{algorithm}[H]
\scriptsize
	\caption{\tabspace[0.2cm] $L\_find()$ : This method is called by \npins{}, \rvmt{} and \upmt{}. It will check whether any method corresponding to $\left\langle L\_obj\_id, L\_key  \right\rangle$ is present in local log from \Lineref{findll4} to \Lineref{findll8}.}
		%\emph{DESCP}\tabspace: Checks weather any operation corresponding to $\left\langle obj\_id, key  \right\rangle$ is present in ll\_list.\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $\left\langle obj\_id, key  \right\rangle$  \\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $true, false$     }
	\label{algo:findInLL}
				\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
	\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{380}\makeatother		
		\Procedure{L\_find}{$L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_rec \uparrow$} \label{lin:findll1}
		
		%\State    /*get the tx id*/
		%\State $L\_t\_id$ $\gets$ getTS($t_i$) \label{lin:findll2};
		
		\State $L\_list$ $\gets$ \txgllist{} \label{lin:findll3}; 
	\cmnts{Every method first identify the node corresponding to the key into local log}
		\While{$(L\_rec_{i} \gets next(L\_list))$} \label{lin:findll4}
		\cmnts{Taking one by one $L\_obj\_id$ and $L\_key$ form $L\_rec$}
		\If{$((L\_rec_{i}.first = L\_obj\_id) \& (L\_rec_{i}.sec = L\_key))$} \label{lin:findll5}

		\State return $\langle TRUE, L\_rec \rangle$ \label{lin:findll6};
		\EndIf \label{lin:findll7}
		\EndWhile \label{lin:findll8}
		\State return $\langle FALSE, NULL \rangle$ \label{lin:findll9};
		\EndProcedure \label{lin:findll10}
	\end{algorithmic}
%	\end{multicols}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%------------------- releaseorderedlocks -----------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[H]
\scriptsize
	\caption{\tabspace[0.2cm] releaseOrderedLocks(): Release all locks in increasing order of their keys from \Lineref{rlock2} to \Lineref{rlock7}.}
		%\emph{DESCP}\tabspace: releases all locks taken during tryCommit\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $ordered\_ll\_list$\\
		%\emph{OUT}\tabspace \tabspace[0.37cm]:    }
	\label{algo:releaseorderedlocks}
			\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
	\begin{algorithmic}[1]
	\makeatletter\setcounter{ALG@line}{391}\makeatother
		\Procedure{releaseOrderedLocks}{$L\_list \downarrow$} \label{lin:rlock1}
	\State    /*Releasing all the locks in increasing order of the keys */
		\While{($\textbf{$L\_rec_{i} \gets next(L\_list$})$)} \label{lin:rlock2}
		
		\State $L\_rec_{i}$.$\preds$.$\texttt{unlock()}$ \label{lin:rlock3};//$\Phi_{lp}$ 
		\State $L\_rec_{i}$.$\currs$.$\texttt{unlock()}$ \label{lin:rlock4};
		
		%\State $ll\_entry_i$.\textcolor{red}{$currs[0]$}.$\texttt{unlock()}$ \label{lin:rlock5};
		%\State $ll\_entry_i$.\textcolor{blue}{$currs[1]$}.$\texttt{unlock()}$ \label{lin:rlock6}; 
		\EndWhile \label{lin:rlock7}
		\State return $\langle void \rangle$;
		\EndProcedure \label{lin:rlock8}
	\end{algorithmic}
			
%	\end{multicols}
\end{algorithm}
%\end{multicols}

\begin{figure} [H]
	\captionsetup{justification=centering}
	%\centering
	%\includegraphics[scale=.5]{figs/fig3.png}
	%\includegraphics[scale=.5]{figs/fig3.pdf_t}
	\centerline{\scalebox{0.45}{\input{figs/disc3.pdf_t}}}
	\caption{Intra transaction validation}
	\label{fig:mvostmm11}
\end{figure}

\cmnt{
\begin{figure} [H]
	%\centering
	%\includegraphics[scale=.5]{figs/fig3.png}
	%\includegraphics[scale=.5]{figs/fig3.pdf_t}
	\centerline{\scalebox{0.5}{\input{figs/mvostm11.pdf_t}}}
	\caption{Intra transaction validation}
	\label{fig:mvostm11}
\end{figure}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%intraTransValidation%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[H]
\scriptsize
	\caption{\tabspace[0.2cm] intraTransValidation() : This method is called by \nptc{} only. If two $\upmt{s}$ within same transaction have at least one shared node among its recorded $\preds$ and $\currs$, in this case the previous $\upmt{}$ effect might be overwritten if the next $\upmt{}$ $\preds$ and $\currs$ are not updated according to the updates done by the previous $\upmt{}$. Thus to solve this we have intraTransValidation() after each $\upmt{}$ in $\nptc$. This will be more clear by the \figref{mvostmm11}, where two \upmt{s} of same transaction $T_1$ are $ins_{11}(k_3)$ and $ins_{12}(k_5)$ (\figref{mvostmm11}.c)). At stage $s_1$ in \figref{mvostmm11}.c) both the \upmt{s} identify the same $\preds$ and $\currs$ from underlying DS (\figref{mvostmm11}.a)). After the successful insertion done by first \upmt{} at stage $s_2$ in \figref{mvostmm11}.c), key $k_3$ is part of underlying DS (\figref{mvostmm11}.b)). At stage $s_3$ in \figref{mvostmm11}.c) if we will not update the $\preds$ and $\currs$ for $ins_{12}(k_5)$ then it will overwrite the previous method updates. To resolve this issue we are doing the intraTransValidation() after each \upmt{} to assign the appropriate $\preds$ and $\currs$ for the upcoming \upmt{} of same transaction.}
		%\emph{DESCP}\tabspace: program order validation\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $ll\_entry_i$  \\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $preds[], currs[]$}
	\label{algo:povalidation}
	\setlength{\multicolsep}{0pt}
%		\begin{multicols}{2}
	\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{399}\makeatother		
		\Procedure{intraTransValidation}{$L\_rec_{i} \downarrow, \preds \uparrow, \currs \uparrow$} \label{lin:threadv1}

	\State $L\_rec.getAllPreds\&Currs(L\_rec$ $\downarrow$, $\preds$ $\uparrow$, $\currs$ $\uparrow$) \label{lin:threadv2};	
				%\State \llgallpc{} \label{lin:threadv2};
				\cmnts{if $\bp$ is marked or $\bc$ is not reachable from $\bp.\bn$ then modify the next consecutive \upmt{} $\bp$ based on previous \upmt{}}
				\If{$(($$\bp$.\textup{marked}$) ||$ $($ $\bp$.\textup{\bn}$)$ != $\bc$$))$} \label{lin:threadv3}
				\cmnts{find $k$ < $i$; such that $le_k$ contains previous update method on same bucket }
				\If{$(($$L\_rec_{k}$.\textup{opn}$)$ $=$ INSERT$)$} \label{lin:threadv4}
				
				\State $L\_rec_{i}$.$\bp$.$\texttt{unlock()}$ \label{lin:thredv4-5};
				\State $\bp$ $\gets$ ($L\_rec_{k}.\bp.\bn)$ \label{lin:threadv5};
				\State $L\_rec_{i}$.$\bp$.$\texttt{lock()}$ \label{lin:thredv5-5};		
				\Else \label{lin:threadv6}
				\cmnts{\upmt{} method $\bp$ will be previous method $\bp$}
				\State $L\_rec_{i}$.$\bp$.$\texttt{unlock()}$ \label{lin:thredv6-5};
				\State $\bp$ $\gets$ ($L\_rec_{k}$.$\bp$) \label{lin:threadv7};
				
				\State $L\_rec_{i}$.$\bp$.$\texttt{lock()}$ \label{lin:thredv7-5};
				\EndIf \label{lin:threadv8}
				
				\EndIf \label{lin:threadv9}
				\cmnts{if $\rc$ \& $\rp$ is modified by prev operation then update them also}
				\If{$($$\rp$.\textup{\rn} != $\rc$$)$} \label{lin:threadv10}
				\State $L\_rec_{i}$.$\rp$.$\texttt{unlock()}$
				\State $\rp$ $\gets$ ($L\_rec_{k}$.$\rp.\rn$)  \label{lin:threadv11}; 
				\State $L\_rec_{i}$.$\rp$.$\texttt{lock()}$
				\EndIf \label{lin:threadv12}
				\State return $\langle \preds, \currs\rangle$;
	\cmnt{		


	
	
	
	        \State $L\_rec.getAllPreds\&Currs(L\_rec_{i}$ $\downarrow$, $G\_pred$ $\uparrow$, $G\_curr$ $\uparrow$) \label{lin:threadv2};	
		%\State \llgallpc{} \label{lin:threadv2};
	%\State    /*if $\bp$ is marked or $\bc$ is not reachable from $\bp.\bn$ then modify the next consecutive \upmt{} $\bp$ based on previous \upmt{}*/
		\If{$(G\_pred.knext \neq G\_curr)$} \label{lin:threadv3}
		\State    /*Find $k$ $>$ $i$; such that $L\_rec_{k}$ contains next update method on same bucket */
		\If{$((($$L\_rec_{k}$.\textup{L\_opn}$)$ $=$ INSERT$)$ $||$ $(($$L\_rec_{k}$.\textup{L\_opn}$)$ $=$ DELETE$))$} \label{lin:threadv4}
		
	\State $L\_rec_{k}$.$G\_pred$.$\texttt{unlock()}$ \label{lin:thredv4-5};
		\State $G\_pred$ $\gets$ ($L\_rec_{i}.G\_pred.knext)$ \label{lin:threadv5};
	\State $L\_rec_{k}$.$G\_pred$.$\texttt{lock()}$ \label{lin:thredv5-5};		
		%\Else \label{lin:threadv6}
	%\State    /*\upmt{} method $\bp$ will be previous method $\bp$*/
	%\State $L\_rec_{i}$.$G\_pred$.$\texttt{unlock()}$ \label{lin:thredv6-5};
	%	\State $G\_pred$ $\gets$ ($L\_rec_{i}$.$G\_pred$) \label{lin:threadv7};
		
	%		\State $L\_rec_{i}$.$G\_pred$.$\texttt{lock()}$ \label{lin:thredv7-5};
		\EndIf \label{lin:threadv8}
		
		\EndIf \label{lin:threadv9}
	\State return $\langle G\_pred, G\_curr\rangle$;
	}
	\EndProcedure	
	\end{algorithmic}
%		\end{multicols}
\end{algorithm}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%% Garbage Collection 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Garbage Collection}
\label{sec:gc}
We have performed garbage collection method to delete the unwanted version of keys i.e. if the particular version corresponding to any key is not going to use in future then we can delete that version. For the better understanding of it please consider \figref{mvostm4}. Here, we are having 3 versions of key $k_1$ with timestamp 0, 15 and 25 respectively. Each version is having 5 fields described in \secref{mvdesign}. Now, consider the version 15, there exist the next version 25 and all the transactions between 15 to 25 has been terminated (either commit or abort) then we are deleting version 15. Similarly, we can delete other versions corresponding to each key as well and optimize the memory. 

\begin{figure} [H]
	%\centering
	%\includegraphics[scale=.5]{figs/fig3.png}
	%\includegraphics[scale=.5]{figs/fig3.pdf_t}
	\centerline{\scalebox{0.35}{\input{figs/mvostm4.pdf_t}}}
	\caption{Data Structures for Garbage Collection}
	\label{fig:mvostm4}
\end{figure}

\begin{algorithm}[H] 
\scriptsize
\label{alg:begin1} 
\caption{STM $begin()$: Invoked by a thread to being a new transaction $T_i$}
	\setlength{\multicolsep}{0pt}
	%	\begin{multicols}{2}
\begin{algorithmic}[1]
%\State lock $\tcntr$;
\makeatletter\setcounter{ALG@line}{423}\makeatother
\Procedure{STM begin}{$L\_t\_id \uparrow$}
\State /*Creating a local log for each transaction*/
\State \txll $\gets$ create new \txllf;  
%\State /*Acquiring lock on live set of transaction*/
%\State $\livetx.lock()$;  
\State /*Get $t\_id$ from $\cnt$*/
\State \txll.$L\_t\_id$ $\gets$ $\cnt$;  
\State /*Incremented $\cnt$*/
\State $\cnt$ $\gets$ \gi;  
%\State add $t\_id$ to $\livetx$; 
%\State /*Release lock on live set of transaction*/
%\State $\livetx.unlock()$;
\State $\livel.lock()$; \label{lin:beginit}
\State add $L\_t\_id$ to $\livel$; 
\State $\livel.unlock()$;
\State return $\langle L\_t\_id \rangle$; 
\EndProcedure
%\State unlock $\tcntr$;
%\State return $i$; \label{lin:begfin}
%\EndFunction{$\begtrans${}}
\end{algorithmic}
%\end{multicols}
\end{algorithm}


\begin{algorithm}[H]  
\scriptsize
\label{alg:instuple}
\caption{$\instup()$: Inserts the version tuple for $(L\_t\_id,v)$ created by the transaction $T_i$ into the version list of $L\_key$}
	\setlength{\multicolsep}{0pt}
%		\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{435}\makeatother
\Procedure{ins\_tuple}{$L\_key \downarrow, L\_t\_id\downarrow, v\downarrow, NULL\downarrow, NULL\downarrow$}
\State /*Initialize $cur\_tuple$*/
\State $cur\_tuple = \langle L\_t\_id, val, F, NULL, NULL \rangle$; 
\State /* Finds the tuple with the largest timestamp smaller than i */
\State $\find(L\_t\_id \downarrow, L\_key \downarrow, prev\_tuple \uparrow)$; \label{lin:prevtup}
\State /*$prev\_tuple$ is $\langle ts, val, mark, rvl, nts\rangle$*/
\State $cur\_tuple.nts = prev\_tuple.nts$;
\State $prev\_tuple.nts = L\_t\_id$;
\State insert $cur\_tuple$ into $L\_key.vl$ in the increasing order of timestamps;  
\State /* $\lvert L\_key.vl \lvert$ denotes number of versions of $L\_key$ created and threshold is a predefined value. */
\If {($\lvert L\_key.vl \lvert > threshold$)} 
\State /*If number of created versions for $L\_key$ crossed the threshold value then calling the Garbage Collection*/ 
\State $gc(L\_key)$;
\EndIf 
\State return $\langle void \rangle$
\EndProcedure
\end{algorithmic}
%\end{multicols}
\end{algorithm}




\begin{algorithm}[H]
\scriptsize
\caption{STM $\gc()$: Unused version of a \tobj{} $L\_key$ will deleted from $L\_key.vl$}
	\setlength{\multicolsep}{0pt}
%		\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{451}\makeatother
\Procedure{gc}{$L\_key \downarrow$}
\State $\livel.lock()$;
\State /*\tobj{} $L\_key$ is already locked*/
\ForAll {$(cur\_tuple \in L\_key.vl)$} 
\If {$(cur\_tuple.nts == NULL)$}
\State /* If $nts$ is NULL, check the next tuple in the version list */
\State continue; 
\EndIf
\State $j = cur\_tuple.ts + 1$;
\State /*Check for all ids $j$ in the range $j < nts$*/
\While {$(j < cur\_tuple.nts)$} 
\If {$(j \in \livel)$}
\State /* If any tuples with timestamp $j$, such that  $i< j < nts$ have not terminated (means exist in $liveList$) then $cur\_tuple$ can't be deleted*/

\State break;
\EndIf
\EndWhile
\State /* If all the tuples with timestamp $j$, such that  $i< j < nts$ have terminated then $cur\_tuple$ can be deleted*/
\State delete $cur\_tuple$;
\EndFor 
\State /* $\livel$ is not unlocked when this function returns */
%\State unlock $\livel$;
\State return $\langle void \rangle$
\EndProcedure
\end{algorithmic}
%\end{multicols}
\end{algorithm}


==> Submitted MVOSTM Journal-2019/graphC.tex <==

\section{Graph Characterization of Opacity}
\label{sec:gcofo}

To prove that an STM system satisfies opacity, it is useful to consider graph characterization of histories. In this section, we describe the graph characterization of Guerraoui and Kapalka \cite{tm-book} modified for sequential histories.

Consider a history $H$ which consists of multiple version for each \tobj. The graph characterization uses the notion of \textit{version order}. Given $H$ and a \tobj{} $k$, we define a version order for $k$ as any (non-reflexive) total order on all the versions of $k$ ever created by committed transactions in $H$. It must be noted that the version order may or may not be the same as the actual order in which the versions of $k$ are generated in $H$. A version order of $H$, denoted as $\ll_H$ is the union of the version orders of all the \tobj{s} in $H$. 

Consider the history $H3$ as shown in \figref{mvostm3} $: lu_1(k_{x, 0}, null), lu_2(k_{x, 0}, null), lu_1\\(k_{y, 0}, null), lu_3(k_{z, 0}, null), ins_1(k_{x, 1}, v_{11}), ins_3(k_{y, 3}, v_{31}), ins_2(k_{y, 2}, v_{21}), ins_1(k_{z, 1},\\ v_{12}), c_1, c_2, lu_4(k_{x, 1}, v_{11}), lu_4(k_{y, 2}, v_{21}), ins_3(k_{z, 3}, v_{32}), c_3, lu_4(k_{z, 1}, v_{12}), lu_5(k_{x, 1}, \\v_{11}), lu_6(k_{y, 2}, v_{21}), c_4, c_5, c_6$. Using the notation that a committed transaction $T_i$ writing to $k_x$ creates a version $k_{x, i}$, a possible version order for $H3$ $\ll_{H3}$ is: $\langle k_{x, 0} \ll k_{x, 1} \rangle, \langle k_{y, 0} \ll k_{y, 2} \ll k_{y, 3} \rangle, \langle k_{z, 0} \ll k_{z, 1} \ll k_{z, 3} \rangle $.
\cmnt{
Consider the history $H4: l_1(ht, k_{x, 0}, NULL) l_2(ht, k_{x, 0}, NULL) l_1(ht, k_{y, 0}, NULL) l_3(ht, k_{z, 0},\\ NULL) i_1(ht, k_{x, 1}, v_{11}) i_3(ht, k_{y, 3}, v_{31}) i_2(ht, k_{y, 2}, v_{21}) i_1(ht, k_{z, 1}, v_{12}) c_1 c_2 l_4(ht, k_{x, 1}, v_{11}) l_4(ht,\\ k_{y, 2}, v_{21}) i_3(ht, k_{z, 3}, v_{32}) c_3 l_4(ht, k_{z, 1}, v_{12}) l_5(ht, k_{x, 1}, v_{11}), l_6(ht, k_{y, 2}, v_{21}) c_4, c_5, c_6$. In our representation, we abbreviate \tins{} as $i$, \tdel{} as $d$ and \tlook{} as $l$. Using the notation that a committed transaction $T_i$ writing to $k_x$ creates a version $k_{x, i}$, a possible version order for $H4$ $\ll_{H4}$ is: $\langle k_{x, 0} \ll k_{x, 1} \rangle, \langle k_{y, 0} \ll k_{y, 2} \ll k_{y, 3} \rangle, \langle k_{z, 0} \ll k_{z, 1} \ll k_{z, 3} \rangle $. 
}
%\vspace{-.3cm}
\begin{figure}[H]
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centering
	\captionsetup{justification=centering}
	\centerline{\scalebox{0.45}{\input{figs/ppopp2.pdf_t}}}
	\caption{History $H3$ in time line view}
	\label{fig:mvostm3}
\end{figure}
%\vspace{-.3cm}
\cmnt{
\begin{figure}[tbph]
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centerline{\scalebox{0.45}{\input{figs/mvostm3.pdf_t}}}
	\caption{History $H4$ in time line view}
	\label{fig:mvostm3}
\end{figure}
}
We define the graph characterization based on a given version order. Consider a history $H$ and a version order $\ll$. We then define a graph (called opacity graph) on $H$ using $\ll$, denoted as $\opg{H}{\ll} = (V, E)$. The vertex set $V$ consists of a vertex for each transaction $T_i$ in $\overline{H}$. The edges of the graph are of three kinds and are defined as follows:
\begin{enumerate}
\setlength\itemsep{0em}
\item \textit{\rt}(real-time) edges: If the commit of $T_i$ happens before beginning of  $T_j$ in $H$, then there exist a real-time edge from $v_i$ to $v_j$. We denote set of such edges as $\rt(H)$.
%\vspace{-.2cm}
\item \textit{\rvf}(return value-from) edges: If $T_j$ invokes \rvmt on key $k_1$ from $T_i$ which has already been committed in $H$, then there exists a return value-from edge from $v_i$ to $v_j$. If $T_i$ is having \upmt{} as insert on the same key $k_1$ then $ins_i(k_{1, i}, v_{i1}) <_H c_i <_H \rvm_j(k_{1, i}, v_{i1})$. If $T_i$ is having \upmt{} as delete on the same key $k_1$ then $del_i(k_{1, i}, null) <_H c_i <_H \rvm_j(k_{1, i}, null)$. We denote set of such edges as $\rvf(H)$.
%\vspace{-.2cm}
\item \textit{\mv}(multi-version) edges: This is based on version order. Consider a triplet with successful methods as  $\up_i(k_{1, i},u)$, $\rvm_j(k_{1, i},u)$, $\up_k(k_{1, k},v)$ , where $u \neq v$. As we can observe it from $\rvm_j(k_{1,i},u)$, $c_i <_H\rvm_j(k_{1,i},u)$. if $k_{1,i} \ll k_{1,k}$ then there exist a multi-version edge from $v_j$ to $v_k$. Otherwise ($k_{1,k} \ll k_{1,i}$), there exist a multi-version edge from $v_k$ to $v_i$. We denote set of such edges as $\mv(H, \ll)$.
\end{enumerate}
\cmnt{
\begin{enumerate}

\item \textit{\rt}(real-time) edges: If commit of $T_i$ happens before beginning of  $T_j$ in $H$, then there exist a real-time edge from $v_i$ to $v_j$. We denote set of such edges as $\rt(H)$.

\item \textit{\rvf}(return value-from) edges: If $T_j$ invokes \rvmt on key $k_1$ from $T_i$ which has already been committed in $H$, then there exist a return value-from edge from $v_i$ to $v_j$. If $T_i$ is having \upmt{} as insert on the same key $k_1$ then $i_i(k_{1, i}, v_{i1}) <_H c_i <_H \rvm_j(k_{1, i}, v_{i1})$. If $T_i$ is having \upmt{} as delete on the same key $k_1$ then $d_i(k_{1, i}, nil_{i1}) <_H c_i <_H \rvm_j(k_{1, i}, nil_{i1})$. We denote set of such edges as $\rvf(H)$.

\item \textit{\mv}(multi-version) edges: This is based on version order. Consider a triplet with successful methods as  $\up_i(k_{1,i},u)$ $\rvm_j(k_1,u)$ $\up_k(k_{1,k},v)$ , where $u \neq v$. As we can observe it from $\rvm_j(k_1,u)$, $c_i <_H\rvm_j(k_1,u)$. if $k_{1,i} \ll k_{1,k}$ then there exist a multi-version edge from $v_j$ to $v_k$. Otherwise ($k_{1,k} \ll k_{1,i}$), there exist a multi-version edge from $v_k$ to $v_i$. We denote set of such edges as $\mv(H, \ll)$.
\vspace{-.3cm}
\end{enumerate}
}
\noindent We now show that if a version order $\ll$ exists for a history $H$ such that it is acyclic, then $H$ is \opq. 

\begin{figure}[H]
%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
\centerline{\scalebox{0.7}{\input{figs/mvostm2.pdf_t}}}
\caption{$\opg{H3}{\ll_{H3}}$}
\label{fig:mvostm1}
\end{figure}

Using this construction, the $\opg{H3}{\ll_{H3}}$ for history $H3$ and $\ll_{H3}$ is given above is shown in \figref{mvostm1}. The edges are annotated. The only \mv{} edge from $T_4$ to $T_3$ is because of \tobj{s} $k_y, k_z$. $T_4$ lookups value $v_{12}$ for $k_z$ from $T_1$ whereas $T_3$ also inserts $v_{32}$ to $k_z$ and commits before $lu_4(k_{z,1}, v_{12})$. 



Given a history $H$ and a version order $\ll$, consider the graph $\opg{\overline{H}}{\ll}$. While considering the $\rt{}$ edges in this graph, we only consider the real-time relation of $H$ and not $\overline{H}$. It can be seen that $\prec_H^{RT} \subseteq \prec_{\overline{H}}^{RT}$ but with this assumption, $\rt(H) = \rt(\overline{H})$. Hence,  we get the following property, 

\begin{property}
\label{prop:hoverh}
The graphs $\opg{H}{\ll}$ and $\opg{\overline{H}}{\ll}$ are the same for any history $H$ and $\ll$. 
\end{property}
%~
\begin{definition}
\label{def:seqver}
For a \tseq{} history $S$, we define a version order $\ll_S$ as follows: For two version $k_{x,i}, k_{x,j}$ created by committed transactions $T_i, T_j$ in $S$, $\langle k_{x,i} \ll_S k_{x,j} \Leftrightarrow T_i <_S T_j \rangle $. 
\end{definition}
%~
%Now, consider the following lemmas,
Now we show the correctness of our graph characterization using the following lemmas and theorem. 

\begin{lemma}
\label{lem:seracycle}
Consider a \legal{} \tseq{} history $S$. Then the graph $\opg{S, \ll_S}$ is acyclic.
\end{lemma}

\begin{proof}
We numerically order all the transactions in $S$ by their real-time order by using a function \textit{\ordfn}. For two transactions $T_i, T_j$, we define $\ord{T_i} < \ord{T_j} \Leftrightarrow T_i <_S T_j$. Let us analyze the edges of $\opg{S, \ll_S}$ one by one: 
\begin{itemize}
\item \rt{} edges: It can be seen that all the \rt{} edges go from a lower \ordfn{} transaction to a higher \ordfn{} transaction. 

\item \rvf{} edges: If $T_j$ lookups $k_x$ from $T_i$ in $S$ then $T_i$ is a committed transaction with $\ord{T_i} < \ord{T_j}$. Thus, all the \rvf{} edges from a lower \ordfn{} transaction to a higher \ordfn{} transaction.

\item \mv{} edges: Consider a successful \rvmt{} $\rvm_j(k_x, u)$ and a committed transaction $T_k$ writing $v$ to $k_x$ where $u \neq v$. Let $c_i$ be $\rvm_j(k_x, u)$'s \lastw. Thus, $\up_i(k_{x,i}, u) \in \evts{T_i}$. Thus, we have that $\ord{T_i} < \ord{T_j}$. Now there are two cases w.r.t $T_i$: (1) Suppose $\ord{T_k} < \ord{T_i}$. We now have that $T_k \ll T_i$. In this case, the mv edge is from $T_k$ to $T_i$. (2) Suppose $\ord{T_i} < \ord{T_k}$ which implies that $T_i \ll T_k$. Since $S$ is legal, we get that $\ord{T_j} < \ord{T_k}$. This case also implies that there is an edge from $\ord{T_j}$ to $\ord{T_k}$. Hence, in this case as well the \mv{} edges go from a transaction with lower \ordfn{} to a transaction with higher \ordfn{}. 

%\item \mv{} edges: Consider a successful \rvmt{} $\rvm_k(k_x, v)$ and a committed transaction $T_i$ writing $u$ to $k_x$ where $u \neq v$. Let $c_j$ be $\rvm_k(k_x, v)$'s \lastw. Thus, $\up_j(k_{x,j}, v) \in \evts{T_j}$. Thus, we have that $\ord{T_j} < \ord{T_k}$. Now there are two cases w.r.t $T_i$: (1) Suppose $\ord{T_i} < \ord{T_j}$. We now have that $T_i \ll T_j$. In this case, the mv edge is from $T_i$ to $T_j$. (2) Suppose $\ord{T_j} < \ord{T_i}$ which implies that $T_j \ll T_i$. Since $S$ is legal, we get that $\ord{T_k} < \ord{T_i}$. This case also implies that there is an edge from $\ord{T_k}$ to $\ord{T_i}$. Hence, in this case as well the \mv{} edges go from a transaction with lower \ordfn{} to a transaction with higher \ordfn{}. 
\end{itemize}

Thus, in all the three cases the edges go from a lower \ordfn{} transaction to higher \ordfn{} transaction. This implies that the graph is acyclic. 
\end{proof}

\begin{lemma}
\label{lem:eqv_hist_mvorder}
Consider two histories $H, H'$ that are equivalent to each other. Consider a version order $\ll_H$ on the \tobj{s} created by $H$. The mv edges $\mv(H, \ll_H)$ induced by $\ll_H$ are the same in $H$ and $H'$.
\end{lemma}

\begin{proof}
Since the histories are equivalent to each other, the version order $\ll_H$ is applicable to both of them. It can be seen that the \mv{} edges depend only on events of the history and version order $\ll$. It does not depend on the ordering of the events in $H$. Hence, the \mv{} edges of $H$ and $H'$ are equivalent to each other. 
\end{proof}

\noindent Using these lemmas, we prove the following theorem. 


\begin{theorem}
\label{thm:opg}
A \valid{} history H is opaque iff there exists a version order $\ll_H$ such that $\opg{H}{\ll_H}$ is acyclic.
\end{theorem}

\begin{proof}
\textbf{(if part):} Here we have a version order $\ll_H$ such that $G_H=\opg{H}{\ll}$ is acyclic. Now we have to show that $H$ is opaque. Since the $G_H$ is acyclic, a topological sort can be obtained on all the vertices of $G_H$. Using the topological sort, we can generate a \tseq{} history $S$. It can be seen that $S$ is equivalent to $\overline{H}$. Since $S$ is obtained by a topological sort on $G_H$ which maintains the real-time edges of $H$, it can be seen that $S$ respects the \rt{} order of $H$, i.e $\prec_H^{RT} \subseteq \prec_S^{RT}$. 

Similarly, since $G_H$ maintains return value-from (\rvf{}) order of $H$, it can be seen that if $T_j$ lookups $k_x$ from $T_i$ in $H$ then $T_i$ terminates before $lu_j(k_x)$ and $T_j$ in $S$. Thus, $S$ is \valid. Now it remains to be shown that $S$ is \legal. We prove this using contradiction. Assume that $S$ is not legal. Thus, there is a successful \rvmt{} $\rvm_j(k_x, u)$ such that its \lastw{} in $S$ is $c_k$ and $T_k$ updates value $v (\neq u)$ to $k_x$, i.e $\up_k(k_{x,k}, v) \in \evts{T_k}$. Further, we also have that there is a transaction $T_i$ that inserts $u$ to $k_x$, i.e $\up_i(k_{x,i}, u) \in \evts{T_i}$. Since $S$ is \valid, as shown above, we have that $T_i \prec_{S}^{RT} T_k \prec_{S}^{RT} T_j$.

Now in $\ll_H$, if $k_{x,k} \ll_H k_{x,i}$ then there is an edge from $T_k$ to $T_i$ in $G_H$. Otherwise ($k_{x,i} \ll_H k_{x,k}$), there is an edge from $T_j$ to $T_k$. Thus, in either case, $T_k$ can not be in between $T_i$ and $T_j$ in $S$ contradicting our assumption. This shows that $S$ is legal. 


%Similarly, since $G_H$ maintains return value-from (\rvf{}) order of $H$, it can be seen that if $T_j$ lookups $k_x$ from $T_i$ in $H$ then $T_i$ terminates before $lu_j(k_x)$ and $T_j$ in $S$. Thus, $S$ is \valid. Now it remains to be shown that $S$ is \legal. We prove this using contradiction. Assume that $S$ is not legal. Thus, there is a successful \rvmt{} $\rvm_k(k_x, v)$ such that its \lastw{} in $S$ is $c_i$ and $T_i$ updates value $u (\neq v)$ to $k_x$, i.e $\up_i(k_{x,i}, u) \in \evts{T_i}$. Further, we also have that there is a transaction $T_j$ that insert $v$ to $k_x$, i.e $\up_j(k_{x,j}, v) \in \evts{T_j}$. Since $S$ is \valid, as shown above, we have that $T_j \prec_{S}^{RT} T_i \prec_{S}^{RT} T_k$.

%Now in $\ll_H$, if $k_{x,i} \ll_H k_{x,j}$ then there is an edge from $T_i$ to $T_j$ in $G_H$. Otherwise ($k_{x,j} \ll_H k_{x,i}$), there is an edge from $T_k$ to $T_i$. Thus in either case $T_i$ can not be in between $T_j$ and $T_k$ in $S$ contradicting our assumption. This shows that $S$ is legal. 

\textbf{(Only if part):} Here we are given that $H$ is opaque and we have to show that there exists a version order $\ll$ such that $G_H=\opg{H}{\ll} (=\opg{\overline{H}}{\ll}$, \propref{hoverh}) is acyclic. Since $H$ is opaque there exists a \legal{} \tseq{} history $S$ equivalent to $\overline{H}$ such that it respects real-time order of $H$. Now, we define a version order for $S$, $\ll_S$ as in \defref{seqver}. Since the $S$ is equivalent to $\overline{H}$, $\ll_S$ is applicable to $\overline{H}$ as well. From \lemref{seracycle}, we get that $G_S=\opg{S}{\ll_S}$ is acyclic. Now consider $G_H = \opg{\overline{H}}{\ll_S}$. The vertices of $G_H$ are the same as $G_S$. Coming to the edges, 

\begin{itemize}
\item \rt{} edges: We have that $S$ respects real-time order of $H$, i.e $\prec_{H}^{RT} \subseteq \prec_{S}^{RT}$. Hence, all the \rt{} edges of $H$ are a subset of $S$. 

\item \rvf{} edges: Since $\overline{H}$ and $S$ are equivalent, the return value-from relation of $\overline{H}$ and $S$ are the same. Hence, the \rvf{} edges are the same in $G_H$ and $G_S$. 

\item \mv{} edges: Since the version-order and the \op{s} of the $H$ and $S$ are the same, from \lemref{eqv_hist_mvorder} it can be seen that $\overline{H}$ and $S$ have the same \mv{} edges as well.
\end{itemize}

Thus, the graph $G_H$ is a subgraph of $G_S$. Since we already know that $G_S$ is acyclic from \lemref{seracycle}, we get that $G_H$ is also acyclic. 
\end{proof}



==> Submitted MVOSTM Journal-2019/intro.tex <==
%\vspace{-12pt}
\section{Introduction}
\label{sec:intro}

%\vspace{1mm}
%\noindent
%\textbf{History of STMs.}

Nowadays, multi-core systems are in trend which necessitated the need for concurrent programming to exploit the cores appropriately. Howbeit, developing the correct and efficient concurrent programs is difficult.  Software Transactional Memory Systems (STMs) are a convenient programming interface which assist the programmer to access the shared memory concurrently using multiple threads without worrying about consistency issues such as deadlock, livelock, priority-inversion, etc. STMs facilitate one more feature compositionality of concurrent programs with great ease which makes it more approachable. Different concurrent operations that need to be composed to form a single atomic unit is achieved by encapsulating them in a transaction. In this paper, we discuss various STMs such as read-write STMs (or RWSTMs), object based STMs (or OSTMs) available in the literature along with the benefits of OSTMs over RWSTMs. After that, we motivated from multi-version RWSTMs and propose multi-version object based STMs (or MVOSTMs) \cite{Juyal+:MVOSTM:SSS:2018} which maintain multiple versions and improves the concurrency further. Later, we made a couple of modifications (discussed in \secref{mvdesign}, \secref{pcode}, and \secref{exp}) to optimize the MVOSTMs and propose optimized MVOSTMs (or \emph{\opmvotm{s}}).
%\color{blue}
%Next, we discuss different types of STMs considered in the literature and identify the need to develop \todo{name} developed in this paper. 
%\color{black}

%With the rise of multi-core systems, concurrent programming is popular. Software Transaction Memory Systems (STMs) are a convenient programming interface for a programmer to access shared memory without worrying about concurrency issues such as locking, races, deadlocks, etc. To access the shared memory, concurrently running transactions uses the methods of \textit{STMs}. Another advantage of STMs is that they facilitate compositionality of concurrent programs with great ease. Different concurrent operations that need to be composed to form a single atomic unit is achieved by encapsulating all these operations as a single transaction.

\vspace{1mm}
\noindent
\textbf{Read-Write STMs:} There exists a lot of popular STMs in the literature such as ESTM \cite{Felber+:ElasticTrans:2017:jpdc}, NOrec \cite{Dalessandro+:NoRec:PPoPP:2010} which executes read/write operations on \emph{transaction objects} or \emph{\tobj{s}}. We represent these STMs as \emph{Read-Write STMs} or \emph{RWSTMs}. RWSTMs typically export following methods: (1) \tbeg{}: which begins a transaction with a unique identity, (2) \tread{} (or $r$): which reads the value of \tobj from shared memory, (3) \twrite{} (or $w$): which writes the new value to \tobj in its local memory, (4) \tryc{}: which validates the values written to \tobj{s} by the transaction and tries to commit. If all the updates made by the transaction is consistent then updates reflect to the shared memory and transaction returns commit, and (5) \trya{}: which returns abort on any inconsistency. %through \trya{} method.

%Any \textit{STMs} which uses read/write operations(or methods) to access shared memory is known as \textit{\textbf{Read-Write STMs} (or \rwtm{}}). In literature, most of the \textit{STMs} are \rwtm{}. NOrec \cite{conf/ppopp/DalessandroSS10}, ESTM \cite{Felber:2017:jpdc} etc. and several other renowned STMs that work at read-write level. It is a library which exports following methods: a) \tbeg{}: begins a transaction, b) \tread{} (or $r$): reads from shared memory, c) \twrite{} (or $w$): writes into its local memory, d) \tryc{}: validates and tries to commit the transaction by writing values on to the shared memory. If validation is successful,  then it returns commit. Otherwise, it returns abort. %through \trya{} method.

\ignore {
Most of the \textit{STMs} proposed in the literature are specifically based on read/write primitive operations (or methods) on memory buffers (or memory registers). These \textit{STMs} typically export the following methods: \tbeg{} which begins a transaction, \tread{} (or $r$) which reads from a buffer, \twrite{} (or $w$) which writes onto a buffer, \tryc{} which validates the \op{s} of the transaction and tries to commit. If validation is successful then it returns commit otherwise STMs export \trya{} which returns abort. We refer to these as \textit{\textbf{Read-Write STMs} or \rwtm{}}. 
As a part of the validation, the STMs typically check for \emph{conflicts} among the \op{s}. Two \op{s} are said to be conflicting if at least one of them is a write (or update) \op. Normally, the order of two conflicting \op{s} can not be commutated.  %Two \op{s} are said to be conflicting if the relative execution order of these \op{s} can not be reversed or commutated without affecting the behaviour of the \op{s} following them. 
}

%\vspace{-.5cm}
\begin{figure}
	\centering
	\captionsetup{justification=centering}
	\centerline{\scalebox{0.4}{\input{figs/pnetys1.pdf_t}}}
	\caption{Advantages of OSTMs over RWSTMs}
	\label{fig:tree-exec}
\end{figure}
%\vspace{-.7cm}

%Literature of databases shows that object-based systems ensure greater concurrency than read-write systems. Hence, Herlihy et al.\cite{HerlihyKosk:Boosting:PPoPP:2018}, Hassan et al. \cite{Hassan+:OptBoost:PPoPP:2014}, and Weikum \& Vossen \cite[Chap 6]{WeiVoss:2002:Morg} extended this concept to STMs as  \textit{\textbf{Object-based STMs} (or \otm{s}}) which works on higher level objects than \rwtm{}.  We have considered an \otm{}\footnote{\otm{} has been accepted as a full paper in NETYS-2018.} using \emph{\tab} \cite{DBLP:journals/corr/abs-1709-00681}. It exports these methods: a) \tbeg{}: begins a transaction, b) \tins{} (or $ins$): inserts a value for a given key, c) \tdel{} (or $del$): deletes the value corresponding to the key and return its value, d) \tlook{} (or $lu$): lookup the value corresponding to the key and e) \tryc{}: validates the \op{s} and tries to commit the transaction.
 
%\vspace{1mm}
%\noindent
%\textbf{An example to illustrate benefits of \otm over \rwtm{}.} 

\vspace{1mm}
\noindent
\textbf{Object based STMs:} There are few STMs available in the literature which executes higher level operations such as insert, delete, lookup on \tab. We represent these STMs as \emph{Object based STMs} or \emph{OSTMs}. The concept of Boosting by Herlihy et al. \cite{HerlihyKosk:Boosting:PPoPP:2008}, the optimistic variant by Hassan et al. \cite{Hassan+:OptBoost:PPoPP:2014} and recently \hotm system by Peri et al. \cite{Peri+:OSTM:Netys:2018} are some examples that demonstrate the performance benefits achieved by \otm{s}. Peri et al. \cite{Peri+:OSTM:Netys:2018} showed that \otm{s} provide greater concurrency than RWSTMs while reducing the number of aborts.

\vspace{1mm}
\noindent 
\textbf{Benefits of \otm{s} over \rwtm{s}: } To show the benefits of \otm{s}, We consider a \tab based STM system which invokes insert (or $ins$), lookup (or $lu$) and delete (or $del$) method. Each \tab consists of $B$ buckets with the elements in each bucket arranged in the form of a linked-list. \figref{tree-exec} (a) represents a \tab{} with the first bucket containing keys $\langle k_3,~ k_6,~ k_8 \rangle$. \figref{tree-exec} (b) shows the execution by two transaction $T_1$ and $T_2$ represented in the form of a tree. $T_1$ performs lookup \op{s} on keys $k_3$ and $k_8$ while $T_2$ performs a delete on $k_6$. The delete on key $k_6$ generates read on the keys $k_3,k_6$ and writes the keys $k_6,k_3$ assuming that delete is performed similar to delete \op in \lazy \cite{Heller+:LazyList:PPL:2007}. The lookup on $k_3$ generates read on $k_3$ while the lookup on $k_8$ generates read on $k_3, k_8$. Note that in this execution $k_6$ has already been deleted by the time lookup on $k_8$ is performed. 

%\rwtm{} and \otm{s} \op{s} as layer-0 (or leaves) and layer-1 respectively in the form of transactional forest. Suppose transactions  $T_1$ and $T_2$ are concurrently executing. History $H0$ at layer-0 (while ignoring higher-level \op{s})  is not \opq \cite{GuerKap:2008:PPoPP} because between the two reads of $k_2$ by $T_1$, $T_2$ writes to $k_2$. So, history $H0$ is forming a cycle shown in \figref{tree-exec} (c). To ensure opacity for $H0$, one of the transactions among $T_1$ or $T_2$ would be aborted. \cmnt{Now, consider the history $H1$ at layer-1,

%In this setting, suppose a transaction $T_1$ of \otm{} invokes methods \tlook{} on the keys $k_5, k_8$. This would internally cause the \otm{} to invoke \lookk{} method on keys $\langle k_2, k_5 \rangle$ and $\langle k_2, k_5, k_7, k_8 \rangle$ respectively. Concurrently, suppose transaction $T_2$ invokes the method \tdel{} on key $k_7$ between the two \tlook{s} of $T_1$. This would cause, \otm{} to invoke \dell{} method of \llist{} on $k_7$. Since, we are using lazy-list approach on the underlying \llist, \dell{} involves pointing the next field of element $k_5$ to $k_8$ and marking element $k_7$ as deleted. Thus \dell{} of $k_7$ would execute the following sequence of read/write level operations- $r(k_2) r(k_5) r(k_7) w(k_5) w(k_7)$ where $r(k_5), w(k_5)$ denote read \& write on the element $k_5$ with some value respectively. The execution of \otm{} denoted as a \emph{history} can be represented as a transactional forest as shown in \figref{tree-exec} b). Here the execution of each transaction is a tree. 
  
In this execution, we denote the read-write \op{s} (leaves) as layer-0 and $lu, del$ methods as layer-1. Consider the history (execution) at layer-0 (while ignoring higher-level \op{s}), denoted as $H0$. It can be verified this history is not \opq \cite{GuerKap:Opacity:PPoPP:2008}. This is because, between the two reads of $k_3$ by $T_1$, $T_2$ writes to $k_3$. It can be seen that if history $H0$ is input to an \rwtm{s} one of the transactions between $T_1$ or $T_2$ would be aborted to ensure opacity \cite{GuerKap:Opacity:PPoPP:2008}. \figref{tree-exec} (c) shows the presence of a cycle in the conflict graph of $H0$. 
% correctness (in this case opacity \cite{GuerKap:2008:PPoPP})
  
Now, consider the history $H1$ at layer-1 consists of $lu$, and $del$ \mth{s}, while ignoring the read/write \op{s} since they do not overlap (referred to as pruning in \cite[Chap 6]{WeiVoss:TIS:2002:Morg}). These methods work on distinct keys ($k_3$, $k_6$, and $k_8$). They do not overlap and are not conflicting. So, they can be re-ordered in either way. Thus, $H1$ is \opq{} \cite{GuerKap:Opacity:PPoPP:2008} with equivalent serial history $T_1 T_2$ (or $T_2 T_1$) and the corresponding conflict graph shown in \figref{tree-exec} (d). Hence, a \tab based \otm{} system does not abort any of $T_1$ or $T_2$. This shows that \otm{s} can reduce the number of aborts and provide greater concurrency. 

%\vspace{1mm}
%\noindent
%\noindent{\textbf{Goals of the paper. } }
%The goal of this paper is to present hash table multi-version object STM as a way to increase concurrency and reduce unnecessary aborts in transactions operating on these STMs. Before we present the main summary of our results, next, we define the history of STMs and their limitations to identify the need for developing multi-version object STM. 

\ignore{
\color{red}
\vspace{1mm}
\noindent
\textbf{Multi-Version Object STMs:} Having shown the advantage achieved by \otm{s},\todo{issue 1} We now explore the notion of \emph{Multi-Version Object STMs} or \emph{\mvotm{s}}. It was observed in databases and \rwtm{s} that by storing multiple versions for each \tobj, greater concurrency can be obtained \cite{Kumar+:MVTO:ICDCN:2014}. Maintaining multiple versions can ensure that more read operations succeed because the reading \op{} will have an appropriate version to read. This motivated us to develop \mvotm{s}. 

issue1 = We did not show this. The writeup suggests that we did this. 

\color{blue}
}

\vspace{1mm}
\noindent
\textbf{Multi-Version Object Based STMs:} Some of the \otm{s} such as \cite{HerlihyKosk:Boosting:PPoPP:2008}, \cite{Hassan+:OptBoost:PPoPP:2014}, \cite{Peri+:OSTM:Netys:2018} exploits the advantages of it. In this paper, we propose and analyze \emph{Optimized Multi-version Object Based STMs} or \emph{\opmvotm{s}} along with the rigorous correctness proof. This work is motivated by the observation that databases and \rwtm{s} achieves greater concurrency by storing multiple versions corresponding to each \tobj \cite{Kumar+:MVTO:ICDCN:2014}. Specifically, maintaining multiple versions can ensure that more read operations succeed because the reading \op{} will obtain an appropriate version to read. Our goal is to analyze the benefit of \emph{OPT-\mvotm{s}} over both single version \otm{s} and multi-version \rwtm{s}. %\todo{check for truth}

%\color{black}
%It exports these methods: a) \tbeg{}: begins a transaction, b) \tins{} (or $ins$): inserts a version corresponding to the key, c) \tdel{} (or $del$): deletes a version corresponding to the key and returns its value, d) \tlook{} (or $lu$): looks up an appropriate version corresponding to the key and e) \tryc{}: validates the \op{s} of the transaction.
%\vspace{-.9cm}
%\color{blue}
%\vspace{-.7cm}
\begin{figure}
	\centering
	\captionsetup{justification=centering}
	\scalebox{.4}{\input{figs/pnetys3.pdf_t}}
	% \vspace{-16cm}
	\caption{Advantages of optimized multi-version over single version \otm{}}
	\label{fig:pop}
\end{figure}
%\vspace{-.7cm}
%\vspace{1mm}
\noindent 
\textbf{The potential benefit of \emph{OPT-\mvotm{s}} over \otm{s} and multi-version \rwtm{s}:} We now illustrate the advantage of \emph{OPT-\mvotm{s}} as compared to single-version \otm{s} (\sotm{s}) using the \tab object with $B$ buckets having the same \op{s} as discussed above: $ins, lu, del$. \figref{pop} (a) represents a history H with two concurrent transactions $T_1$ and $T_2$ operating on a \tab{} $ht$. $T_1$ first tries to perform a $lu$ on key $k_3$. But due to the absence of key $k_3$ in $ht$, it obtains a value of $null$. Then $T_2$ invokes $ins$ method on the same key $k_3$ and inserts the value $v_3$ in $ht$. Then $T_2$ deletes the key $k_2$ from $ht$ and returns $v_0$ implying that some other transaction had previously inserted $v_0$ into $k_2$. The second method of $T_1$ is $lu$ on the key $k_2$. With this execution, any \sotm system has to return abort for $T_1$'s $lu$ \op  to ensure correctness, i.e., \opty. Otherwise, if $T_1$ would have obtained a return value $v_0$ for $k_2$, then the history would not be \opq anymore. This is reflected by a cycle in the corresponding conflict graph between $T_1$ and $T_2$, as shown in \figref{pop} (c). Thus to ensure \opty, \sotm system has to return abort for $T_1$'s lookup on $k_2$.

 In an \emph{OPT-\mvotm{s}} based on \tab, denoted as \emph{OPT-\hmvotm}, whenever a transaction inserts or deletes a key $k$, a new version is created. Consider the above example with an \emph{OPT-\hmvotm}, as shown in \figref{pop} (b). Even after $T_2$ deletes $k_2$, the previous value of $v_0$ is still retained. Thus, when $T_1$ invokes $lu$ on $k_2$ after the delete on $k_2$ by $T_2$, \emph{OPT-\hmvotm} return $v_0$ (as previous value). With this, the resulting history is \opq{} with equivalent serial history being $T_1 T_2$. The corresponding conflict graph is shown in \figref{pop} (d) does not have a cycle. 

Thus, \emph{OPT-\mvotm} reduces the number of aborts and achieve greater concurrency than \sotm{s} while ensuring the compositionality. We believe that the benefit of \emph{OPT-\mvotm} over multi-version \rwtm is similar to \sotm over single-version \rwtm as explained above.
%This paper is an extension of work originally presented by Juyal et al. \cite{Juyal+:MVOSTM:SSS:2018} in SSS 2018. We made couple of modifications in MVOSTMs to make it more efficient and called Optimized MVOSTM (or Opt-MVOSTM). 
\emph{OPT-\mvotm} is a generic concept which can be applied to any data structure. In this paper, we have considered the \tab{} and list  based \emph{OPT-\mvotm{s}} as \emph{OPT-\hmvotm} and \emph{OPT-\lmvotm} respectively. If the bucket size $B$ of \tab{} becomes 1 then \tab based \emph{OPT-\mvotm{s}} boils down to the list based \emph{OPT-\mvotm{s}}. 

\emph{OPT-\hmvotm} and \emph{OPT-\lmvotm} use an unbounded number of versions for each key. To address this issue, we develop two variants for both \tab and list data structures (or DS): (1) A garbage collection method in \emph{OPT-\mvotm{s}} to delete the unwanted versions of a key, denoted as \emph{OPT-\mvotmgc}. Garbage collection gave an average performance gain of 16\%  over \emph{OPT-\mvotm} without garbage collection in the best case. Thus, the overhead of garbage collection scheme is less than the performance improvement due to improved memory usage. (2) Placing a limit of $K$ on the number versions in \emph{OPT-\mvotm}, resulting in \emph{OPT-\kotm}. This gave an average performance gain of 24\% over \emph{OPT-\mvotm} without garbage collection in the best case. 

 Experimental results show that \ophkotm performs best among its variants and
outperforms state-of-the-art hash-table based STMs  (HT-OSTM, ESTM, RWSTM, HT-MVTO, HT-KSTM) by a factor of 3.62, 3.95, 3.44, 2.75, 1.85 for workload W1 (90\% lookup, 8\% insert and 2\% delete),  1.44, 2.36, 4.45, 9.84, 7.42 for workload W2 (50\% lookup,  25\% insert and 25\% delete), and 2.11, 4.05, 7.84, 12.94, 10.70 for workload W3 (10\% lookup,  45\% insert and 45\% delete) respectively. Similarly, \oplkotm performs best among its variants and outperforms state-of-the-art list based STMs (list-OSTM, Trans-list, Boosting-list, NOrec-list, list-MVTO, list-KSTM)  by a factor of  2.56, 25.38, 23.57, 27.44, 13.34, 5.99 for W1, 1.51, 20.54, 24.27, 29.45, 24.89, 19.78 for W2, and 2.91, 32.88, 28.45, 40.89, 173.92, 124.89 for W3 respectively. To the best of our knowledge, this is the first work to explore the idea of using multiple versions in \otm{s} to achieve greater concurrency. 

%\color{blue} Thus, the overhead of garbage collection is less than the performance improvement due to improved memory usage.\color{black}
%\todo{This paragraph has to be revisted.}

\noindent 
\textbf{Contributions of the paper:}
\begin{itemize}
\item We propose a new notion of optimized multi-version objects based STM system as \emph{OPT-\mvotm} in \secref{mvdesign}. In this paper, we develop it for list and \tab{} objects as \emph{OPT-\lmvotm} and \emph{OPT-\hmvotm} respectively. \emph{OPT-\mvotm} is generic for other data structures as well.

\item For efficient space utilization in \emph{\opmvotm{s}} with unbounded versions, we develop \emph{Garbage Collection} for \emph{OPT-\mvotm} (i.e. \emph{OPT-\mvotmgc}) and bounded version \emph{OPT-\mvotm} (i.e. \emph{OPT-\kotm}).

\item \secref{cmvostm} shows that \emph{OPT-\lmvotm} and \emph{OPT-\hmvotm} satisfy standard \cc of STMs, \emph{opacity} \cite{GuerKap:Opacity:PPoPP:2008}.

%\item Both the \mvotm{s} can have both bounded and unbounded number of versions. If the implementation chooses unbounded versions, then the resulting STM system satisfies the progress condition: \mvpness \cite{perel+:2010:MultVer:PODC} which requires that lookup-only transaction never gets aborted.

\item  Experimental analysis of both \emph{OPT-\lmvotm} and \emph{OPT-\hmvotm} with state-of-the-art STMs are present in \secref{exp}. Proposed \emph{OPT-\lmvotm} and \emph{OPT-\hmvotm} provide greater concurrency and reduces the number of aborts as compared to  \emph{MVOSTMs}, \sotm{s}, single-version \rwtm{s} and, multi-version \rwtm{s} while maintaining multiple versions corresponding to each key. 

%\item We develop the \emph{garbage collection} method to delete unwanted versions from \mvotm with unbounded versions.%


%\item \mvotm shows significant performance gain over renowned state-of-the-art STMs. %\emph{list-OSTM}\cite{DBLP:journals/corr/abs-1709-00681}.
\end{itemize}

\noindent
\textit{Roadmap:} The paper is organized as follows. We describe our building system model in \secref{model}. In \secref{gcofo}, we formally define the graph characterization of opacity. \secref{mvdesign} represents the \emph{\opmvotm{s}} design and data structure. \secref{pcode} shows the working of \emph{\ophmvotm{s}} and its algorithms. We formally prove the correctness of \emph{\opmvotm{s}} in \secref{cmvostm}.  In \secref{exp} we show the experimental evaluation of \emph{\opmvotm{s}} with state-of-art-STMs. Finally, we conclude in \secref{confu}. %Due to space constraints, we have only outlined the main idea. The full details can be found in \cite{prisat:mvto:corr:2013} and in appendix.
%\todo{In the previous paragraph, you have some text that this is better than existing STMs. We should have some text about that in the contributions. We show that \mvotm is better than single version otm. We show that \mvotm is better than multi version \rwtm}

%\textbf{Road-map:} We described our system model and preliminaries in \secref{model}. \secref{conflicts} represents the graph characterization of \mvotm. \secref{mvdesign} and \secref{pcode} describes the \hmvotm design, data structure and pseudo code respectively. \secref{cmvostm} and \secref{exp} represents correctness of \mvotm and comparisons with the state-of-the-art. Finally, we conclude our paper followed by future work in \secref{confu}. Due to space constraints, we kept only the main idea in the paper, but for more details, please refer technical report \cite{DBLP:journals/corr/abs-1712-09803}. 

==> Submitted MVOSTM Journal-2019/macros.tex <==
% comment a region

\newcommand{\punt}[1]{}
\newcommand{\cmnt}[1]{}


% a word should not be broken across lines
\newcommand{\nosplit}{\linebreak}

% no hyphenation
\def\nohyphens{\hyphenpenalty=10000\exhyphenpenalty=10000}

% ~ character
\newcommand{\tilda}{\symbol{126}}

% useful mathematical symbols

\newcommand{\ang}[1]{\langle #1 \rangle}
\newcommand{\Ang}[1]{\Big\langle #1 \Big\rangle}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% keywords for pseudocode

%% various theorem environments
%% Commented out because they are already defined in llncs file %%
%% Decommented out because they are not defined in sigplan class %%

\newtheorem{theorem}{Theorem}
\renewcommand{\thetheorem}{\arabic{theorem}}

\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{property}[theorem]{Property}

\newtheorem{definition}{Definition}

\newcounter{history}
\newcommand{\hist}[1]{\refstepcounter{history} {#1}}

\newcommand{\proof}[1][]{\noindent{\bf\boldmath
                     P\hspace{-0.25ex}roof{#1}\/:\unboldmath}\hspace*{0.5em}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------Theorem Notations Defined by Petr --------------------------------------------------------------------------------------------------------
%% Defined by Petr

%\newtheorem{acknowledgement}[theorem]{Acknowledgement}
%\newtheorem{observation}[theorem]{Observation}


%------------------------------------------------------------------------------------------------------------------------------

% various references
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\stref}[1]{step~\ref{step:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\insref}[1]{line~\ref{ins:#1}}
%\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\axmref}[1]{Proposition~\ref{axm:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\eqnref}[1]{Eqn(\ref{eq:#1})}
\newcommand{\eqvref}[1]{Equivalence~(\ref{eqv:#1})}
\newcommand{\ineqref}[1]{Inequality~(\ref{ineq:#1})}
%\newcommand{\invref}[1]{(\ref{inv:#1})}
\newcommand{\exref}[1]{Example~\ref{ex:#1}}
\newcommand{\propref}[1]{Property~\ref{prop:#1}}
\newcommand{\obsref}[1]{Observation~\ref{obs:#1}}
\newcommand{\asmref}[1]{Assumption~\ref{asm:#1}}
\newcommand{\thref}[1]{Thread~\ref{th:#1}}
\newcommand{\trnref}[1]{Transaction~\ref{trn:#1}}

\newcommand{\linref}[1]{Line~\ref{lin:#1}}
%\newcommand{\algoref}[1]{{\sf Algo$_{\ref{algo:#1}}$}}
\newcommand{\algoref}[1]{{Algorithm~\ref{algo:#1}}}
\newcommand{\subsecref}[1]{SubSection{\ref{subsec:#1}}}

\newcommand{\histref}[1]{\ref{hist:#1}}

\newcommand{\apnref}[1]{Appendix~\ref{apn:#1}}
\newcommand{\invref}[1]{Invariant~\ref{inv:#1}}

\newcommand{\Chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\Figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\Tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\Stref}[1]{Step~\ref{step:#1}}
\newcommand{\Thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\Lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\Corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\Axmref}[1]{Proposition~\ref{axm:#1}}
\newcommand{\Defref}[1]{Definition~\ref{def:#1}}
\newcommand{\Eqref}[1]{eq(\ref{eq:#1})}
\newcommand{\Eqvref}[1]{Equivalence~(\ref{eqv:#1})}
\newcommand{\Ineqref}[1]{Inequality~(\ref{ineq:#1})}
\newcommand{\Exref}[1]{Example~\ref{ex:#1}}
\newcommand{\Propref}[1]{Property~\ref{prop:#1}}
\newcommand{\Obsref}[1]{Observation~\ref{obs:#1}}
\newcommand{\Asmref}[1]{Assumption~\ref{asm:#1}}

\newcommand{\Lineref}[1]{Line~\ref{lin:#1}}
\newcommand{\Algoref}[1]{{\sf Algo$_{\ref{algo:#1}}$}}

\newcommand{\Apnref}[1]{Section~\ref{apn:#1}}
\newcommand{\Invref}[1]{Invariant~\ref{inv:#1}}
\newcommand{\Confref}[1]{Conflict~\ref{conf:#1}}




\newcommand{\theqed}{$\Box$}


\newcommand{\nsqed}{\hspace*{\fill} \theqed}


% Renews the footnote command
\renewcommand{\thefootnote}{\alph{footnote}}

\newcommand{\ignore}[1]{}

\newcommand{\myparagraph}[1]{\vspace{1mm}\noindent\textbf{#1}}


%------------------------------------------------------------------------------------------------------------------
% Definitions for Object STM paper
%------------------------------------------------------------------------------------------------------------------
%

\newcommand{\tobj} {t-object\xspace}
\newcommand{\txns}[1] {txns(#1)}
\newcommand {\comm}[1] {committed(#1)}
\newcommand {\aborted}[1] {aborted(#1)}
\newcommand {\incomp}[1] {incomp(#1)}
\newcommand {\live}[1] {live(#1)}
\newcommand {\term}[1] {term(#1)}
\newcommand {\key}[1] {key(#1)}
\newcommand {\confevt}[1] {conf-event(#1)}
\newcommand {\confmth}[1] {conf-method(#1)}
\newcommand {\conf}[1] {conflict(#1)}
\newcommand {\termn}[1] {terminate(#1)}

\newcommand {\tcomp} {t-complete\xspace}
\newcommand {\tinc} {t-incomplete\xspace}

\newcommand{\ssch} {sub-history}
\newcommand{\sschs} {sub-histories}

\newcommand{\nseq} {non-sequential}
\newcommand{\tseq} {t-sequential\xspace}
%\newcommand{\seq} {sequential}
\newcommand{\serial} {serial\xspace}
\newcommand{\serialc} {serial criterion\xspace}

\newcommand{\lastw} {lastWrite}
\newcommand{\lwrite}[2] {#2.lastWrite(#1)}
\newcommand{\vwrite} {valWrite}
\newcommand{\valw}[2] {#2.valWrite(#1)}
\newcommand{\lastup} {lastUpdt}
\newcommand{\lupdt}[2] {#2.lastUpdt(#1)}
\newcommand{\lseen}[2] {#2.lastSeen(#1)}

\newcommand{\mr} {MR}
\newcommand{\tr} {TR}

%\newcommand{\valid} {valid}
\newcommand{\validity} {validity\xspace}
\newcommand{\legal} {legal\xspace}
\newcommand{\legality} {legality\xspace}

\newcommand{\op} {operation\xspace}
\newcommand{\mth} {method\xspace}
%\newcommand{\rvmt} {rv\_method\xspace}
%\newcommand{\upmt} {upd\_method\xspace}
\newcommand{\rvp} {\emph{\rvmt execution} phase}
\newcommand{\cp} {\emph{\upmt execution} phase}

\newcommand{\termop} {terminal operation\xspace}
\newcommand{\cc} {correctness-criterion\xspace}
\newcommand{\ccs} {correctness-criteria\xspace}
\newcommand{\gen}[1] {gen(#1)}

\newcommand{\inv} {$inv$}
\newcommand{\rsp} {$rsp$}
\newcommand{\rmw} {rmw}
\newcommand{\first}[1] {first(#1)}
\newcommand{\last}[1] {last(#1)}

\newcommand{\evts}[1] {evts(#1)}
\newcommand{\met}[1] {methods(#1)}

\newcommand{\sgt} {SGT\xspace}
\newcommand{\memop} {memory operation\xspace}
\newcommand{\pref}[2] {#2.prefix(#1)}

\newcommand{\init} {\emph{init}\xspace}
\newcommand{\tbeg} {\emph{t\_begin}\xspace}
\newcommand{\tread} {\emph{t\_read}\xspace}
\newcommand{\twrite} {\emph{t\_write}\xspace}
\newcommand{\tins} {\emph{t\_insert}\xspace}
\newcommand{\tdel} {\emph{t\_delete}\xspace}
\newcommand{\tlook} {\emph{t\_lookup}\xspace}
\newcommand{\tryc} {\emph{tryC}\xspace}%{\emph{tryC}}
\newcommand{\trya} {\emph{tryA}\xspace}%{\emph{tryA}}


\newcommand{\failed} {failed\xspace}
\newcommand{\unaborted} {unaborted\xspace}

%\newcommand{\ins} {\emph{list\_insert}}
%\newcommand{\del} {\emph{list\_del}}
%\newcommand{\look} {\emph{list\_lookup}}

\newcommand{\inss} {\emph{list\_insert}}
\newcommand{\dell} {\emph{list\_del}}
\newcommand{\lookk} {\emph{list\_lookup}}

\newcommand{\ins} {\emph{lsl\_ins}\xspace}
\newcommand{\del} {\emph{lsl\_del}\xspace}
\newcommand{\look} {\emph{lsl\_Search}\xspace}

\newcommand{\rv} {\emph{rv}}
\newcommand{\up} {\emph{up}}

\newcommand{\rset}[1] {rset(#1)}
\newcommand{\wset}[1] {wset(#1)}
\newcommand{\rvar} {readVar}

\newcommand{\co} {CO\xspace}
\newcommand{\opq} {opaque\xspace}
\newcommand{\opty} {opacity\xspace}
\newcommand{\coop} {co-opaque\xspace}
\newcommand{\coopty} {co\text{-}opacity\xspace}

\newcommand{\vwc} {VWC\xspace}
\newcommand{\lo} {LO\xspace}
\newcommand{\lopty} {LO\xspace}
\newcommand{\lopq} {locally-opaque\xspace}

\newcommand{\tab} {hash-table\xspace}
\newcommand{\set}{table\xspace}
\newcommand{\llist} {list\xspace}
\newcommand{\otm} {\textit{OSTM}\xspace}%{ObjSTM}
\newcommand{\sotm} {\textit{SV-OSTM}\xspace}%{ObjSTM}

\newcommand{\rwtm} {\textit{RWSTM}\xspace}
%\newcommand{\lotm} {Table-OSTM}
\newcommand{\lotm} {OSTMs\xspace}
\newcommand{\bto} {BTO\xspace}
\newcommand{\bst} {BST\xspace}
\newcommand{\lsl} {lazyrb\text{-}list\xspace}
\newcommand{\lazy} {lazy-list\xspace}

\newcommand{\csr} {CSR\xspace}

\newcommand{\perm} {permissive\xspace}
\newcommand{\pness} {permissiveness\xspace}
\newcommand{\permfn}[1] {perm(#1)}

\newcommand{\sspec} {sequential-specification\xspace}
\newcommand{\samp} {sample-stm\xspace}

\newcommand{\cg}[1] {CG(#1)}

\newcommand{\uset} {updtSet\xspace}
\newcommand{\lset} {lookupSet\xspace}
\newcommand{\rvm} {\emph{rvm}\xspace}
%\newcommand{\ht} {\emph{hash table}}

\newcommand{\firste} {firstEvt\xspace}
\newcommand{\laste} {lastEvt\xspace}
\newcommand{\fevt}[1] {#1.firstEvt}
\newcommand{\levt}[1] {#1.lastEvt}

\newcommand{\fkmth}[3] {#3.firstKeyMth(#1, #2)}
\newcommand{\pkmth}[3] {#3.prevKeyMth(#1, #2)}

\newcommand{\bstu} {\emph{bst-update}}
\newcommand{\lllist} {locallog\_list}

\newcommand{\udset}[1] {updtSet(#1)}
\newcommand{\rvset}[1] {rvSet(#1)}
%\newcommand{\bst}{BST}

\newcommand{\refr}[1]{refNode(#1)}
\newcommand{\lin}[1]{#1.LP\xspace}

%\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%

\newcommand\tabspace[1][1cm]{\hspace*{#1}}

%%%%%%% DS macros
%\newcommand{\glslhead}{getLslHead($obj\_id \downarrow, key \downarrow$)}


%\newcommand{\txlfind} {\textup{translog.find\_in\_loclog}$(obj\_id \downarrow, key \downarrow)$}
\newcommand{\txgid} {txlog.getTid()}
%\newcommand{\txgllist} {txlog.getLlList($t_{i} \downarrow$)}
\newcommand{\txsetst}[1] {L\_txlog.setStatus($L\_txstatus \downarrow$, $ OK \downarrow$)}
\newcommand{\txbegin}[1] {begin(#1)}

%\newcommand{\lsls}[1] {list\_lookup($obj\_id \downarrow,  key \downarrow, knext \uparrow, value \uparrow$, #1)}

\newcommand{\rvvalidate} {rvValidate($ key \downarrow$, $preds[] \downarrow$, $currs[] \downarrow$)}

%\newcommand{\lslins}[1] {lslIns($preds[] \downarrow$, $currs[] \downarrow$, #1)}
\newcommand{\lsldel} {lslDel($preds[] \downarrow$, $currs[] \downarrow$)}


%\newcommand{\rlsol} {releaseOrderedLocks($ordered\_ll\_list \downarrow$)}

\newcommand{\ctov} {commitTOValidation($ll\_entry_i \downarrow$)}
\newcommand{\rvtov} {rvTOValidation($ key \downarrow$, $curr \downarrow$)}
\newcommand{\toval} {toValidation($ key \downarrow$, $curr \downarrow$, $val\_type \downarrow$)}
\newcommand{\validation} {validation($ key \downarrow$, $curr \downarrow$, $val\_type \downarrow$)}


\newcommand{\ifvalidation} {$$\textup{interferenceValidation}$(preds[] \downarrow, currs[] \downarrow)$$}
%\newcommand{\handlea}{tryAbort($obj\_id \downarrow$)}

%\newcommand{\llsort}{ll.sort ($ll\_list \downarrow$)}

%%---------------------macro w/o parameter

\newcommand{\npctov} {\emph{commitTOValidation()}}
\newcommand{\nptov} {\emph{toValidation()}}
\newcommand{\npintv} {\emph{intraTransValidation()}}
\newcommand{\nptc} {\emph{STM tryC()}}
\newcommand{\npins} {\emph{STM insert()}}
\newcommand{\npdel} {\emph{STM delete()}}
\newcommand{\npluk} {\emph{STM lookup()}}
\newcommand{\nplsls} {\emph{list\_lookup()}}
\newcommand{\nplsldel} {\emph{lslDel()}}
\newcommand{\nplslins} {\emph{list\_Ins()}}
\newcommand{\npbegin} {\emph{STM begin}}
\newcommand{\nppoval} {\emph{lostUpdateValidation()}}
\newcommand{\tcins} {\emph{tryC_{ins}}}
\newcommand{\npcld}{\emph{commonLu\&Del()}}


\newcommand{\rn} {\textcolor{red}{RL}\xspace}
\newcommand{\bn} {\textcolor{blue}{BL}\xspace}

\newcommand{\rc} {\textcolor{red}{currs[0]}}
\newcommand{\bc} {\textcolor{blue}{currs[1]}}
\newcommand{\bp} {\textcolor{blue}{preds[0]}}
\newcommand{\rp} {\textcolor{red}{preds[1]}}


\newcommand{\eevts}[1] {#1.evts}
\newcommand{\hst}[1] {#1.hist\xspace}
\newcommand{\exec}[1] {#1.exec\xspace}
%\newcommand{\state}[1] {#1.state\xspace}
\newcommand{\alls}[1] {#1.allStates\xspace}
\newcommand{\pres}[1] {#1.pre\text{-}state\xspace}
\newcommand{\posts}[1] {#1.post\text{-}state\xspace}

\newcommand{\shist}[2] {#2.subhist(#1)}
\newcommand{\subhist} {subhist\xspace}
\newcommand{\subh}  {sub\text{-}history\xspace}

\newcommand{\preds} {G\_preds[]}
\newcommand{\currs} {G\_currs[]}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MV-OSTM %%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\mvotm} {\textit{MVOSTM}\xspace}
\newcommand{\mvotms} {\textit{MV-OSTM}\xspace}
\newcommand{\hmvotm} {\textit{HT-MVOSTM}\xspace}
\newcommand{\lmvotm} {\textit{list-MVOSTM}\xspace}
\newcommand{\hotm} {\textit{HT-OSTM}\xspace}
\newcommand{\kotm} {\textit{KOSTM}\xspace}
\newcommand{\hkotm} {\textit{HT-KOSTM}\xspace}
\newcommand{\lkotm} {\textit{list-KOSTM}\xspace}
\newcommand{\mvotmgc} {\textit{MVOSTM-GC}\xspace}
\newcommand{\hmvotmgc} {\textit{HT-MVOSTM-GC}\xspace}
\newcommand{\lmvotmgc} {\textit{list-MVOSTM-GC}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MV-OSTM %%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MV-OSTM %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MV-OSTM %%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%% Local %%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\llog} {txLog\xspace}

\newcommand{\txlfind} {$L\_txlog.find(L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_rec \uparrow)$}
\newcommand{\txll} {$L\_txlog$}
\newcommand{\txllf} {$L\_txlog()$}
\newcommand{\llsopn}[1] {$L\_rec.setOpn(L\_obj\_id \downarrow$, $L\_key \downarrow$, #1)}
\newcommand{\llsval}[1] {$L\_rec.setVal(L\_obj\_id \downarrow$, $ L\_key \downarrow$, #1)}
\newcommand{\llsopst}[1] {$L\_rec.setOpStatus(L\_obj\_id \downarrow$, $ L\_key \downarrow$, #1)}

\newcommand{\llgopn}[1] {$L\_rec.getOpn(L\_obj\_id \downarrow$, $ L\_key \downarrow$)}
%\newcommand{\llsopn}[1] {$L\_getOpn((obj\_id \downarrow$, $key \downarrow$, #1)}

\newcommand{\llgval}[1] {$L\_rec.getVal(L\_obj\_id \downarrow$, $ L\_key \downarrow$)}
%\newcommand{\llsval}[1] {loclog.getVal($obj\_id \downarrow$, $ key \downarrow$, #1)}

\newcommand{\llspc} {$L\_rec.setPred\&Curr(L\_obj\_id \downarrow$, $ L\_key \downarrow$, $G\_pred \downarrow$, $G\_curr \downarrow$)}

\newcommand{\llgaptc}[1] {$L\_rec.getAptCurr$(#1)}
\newcommand{\llgkeyobj} {$L\_rec.getKey\&Objid(L\_rec_{i} \downarrow$)}

\newcommand{\llgopst} {$L\_rec.getOpStatus(L\_obj\_id \downarrow$, $L\_key \downarrow$)}
%\newcommand{\llsopst}[1] {loclog.getOpStatus($obj\_id \downarrow$, $ key \downarrow$, #1)}

\newcommand{\llgallpc}{$L\_rec.getAllPreds\&Currs(L\_rec_{i} \downarrow$, $preds[] \uparrow$, $currs[] \uparrow$ )}

\newcommand{\poval}{lostUpdateValidation($L\_rec_{i}\downarrow$, $preds[]\uparrow$, $currs[]\uparrow$ )}

\newcommand{\llsort}{$L\_txlog.sort$($L\_list \downarrow$)}

\newcommand{\txgllist} {$L\_txlog.getList(L\_t\_id \downarrow$)}

\newcommand{\cld}{$commonLu\&Del$($L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_val \uparrow, L\_op\_status \uparrow$)}
%%%%%%%%%%%%%%%%%%%% Global %%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\cnt} {G\_cnt}
\newcommand{\livetx} {live\_trans}
\newcommand{\gi} {$get\&inc(G\_cnt \downarrow)$}
\newcommand{\glslhead}{getListHead($L\_obj\_id \downarrow, L\_key \downarrow$)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%From MVTO%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\opg}[2] {OPG(#1, #2)}
\newcommand{\ord}[1] {ord(#1)}
\newcommand{\ordfn} {ord}

\newcommand{\mv} {mv}
\newcommand{\rvf} {rvf}
\newcommand{\rt} {rt}
\newcommand{\rvmt} {rv\_method\xspace}
\newcommand{\upmt} {upd\_method\xspace}

%\newcommand{\op} {operation}
\newcommand{\checkv} {check\_versions}
\newcommand{\remid} {removeId}
\newcommand{\instup} {ins\_tuple}
\newcommand{\gc} {gc}
\newcommand{\liveset} {liveSet}
\newcommand{\livel} {liveList}
\newcommand{\locko} {lockOrder}
\newcommand{\mvto} {MV-OSTM}
\newcommand{\valid} {valid}
\newcommand{\seq}[2] {linearize(#2, #1)}
\newcommand{\stl}[3] {#3.stl(#1, #2)}
%\newcommand{\lts}[3] {#3.lts(#1, #2)}
\newcommand{\lts}[3] {#3.lts(#1, #2)}
\newcommand{\aco} {accessOrder}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% methods%%%%%%%%%%%%%%%%%%

\newcommand{\lsls}[1] {list\_lookup($L\_obj\_id \downarrow,  L\_key \downarrow, G\_pred \uparrow, G\_curr \uparrow$)}
\newcommand{\find} {find\_lts}
\newcommand{\handlea}{return ABORT}
\newcommand{\lslins}[1] {list\_Ins($G\_pred \downarrow$, $G\_curr \downarrow$, $node \uparrow$)}
\newcommand{\rlsol} {releaseOrderedLocks($L\_list \downarrow$)}

\newcommand{\mvperm} {mv-permissive\xspace}
\newcommand{\mvpness} {mv-permissiveness\xspace}

\newcommand {\cmnts}[1] {\State{\textcolor{gray}{/* #1 */} }}
\renewcommand{\thefootnote}{\arabic{footnote}}	

%\algrenewcommand{\algorithmiccomment}[1]{$//$ #1}
%\algrenewcommand{\algorithmiccomment}[1]{/* #1 */}







\newcommand{\opmvotm} {\textit{OPT-MVOSTM}\xspace}
\newcommand{\ophmvotm} {\textit{OPT-HT-MVOSTM}\xspace}
\newcommand{\oplmvotm} {\textit{OPT-list-MVOSTM}\xspace}

\newcommand{\opkotm} {\textit{OPT-KOSTM}\xspace}
\newcommand{\ophkotm} {\textit{OPT-HT-KOSTM}\xspace}
\newcommand{\oplkotm} {\textit{OPT-list-KOSTM}\xspace}
\newcommand{\opmvotmgc} {\textit{OPT-MVOSTM-GC}\xspace}
\newcommand{\ophmvotmgc} {\textit{OPT-HT-MVOSTM-GC}\xspace}
\newcommand{\oplmvotmgc} {\textit{OPT-list-MVOSTM-GC}\xspace}

==> Submitted MVOSTM Journal-2019/pcode.tex <==
\section{Working of \ophmvotm{}} 
\label{sec:pcode}

% Within a transaction, a process can invoke layer-1 \mth{s} (or \op{s}) on a \emph{\tab} \tobj. A \tab{}($ht$) consists of multiple key-value pairs of the form $\langle k, v \rangle$. The keys and values are respectively from sets $\mathcal{K}$ and $\mathcal{V}$. The \mth{s} that a thread can invoke are: (1) $\tbeg_i{}$: Begins a transaction and returns an unique id to the invoking thread (2) $\tins_i(ht, k, v)$: Transaction $T_i$ inserts a value $v$ onto key $k$ in $ht$ (3) $\tdel_i(ht, k, v)$: Transaction $T_i$ deletes the key $k$ from the \tab{} $ht$ \& returns the current value $v$ for $T_i$. If Key $k$ does not exist, it return $null$. (4) $\tlook_i(ht, k, v)$: returns the current value $v$ for key $k$ in $ht$  for $T_i$. Similar to \tdel, if the key $k$ does not exist then \tlook returns $null$ (5) $\tryc_i$ which tries to commit all the \op{s} of $T_i$  and (6) $\trya_i$ aborts $T_i$. We assume that each \mth{} consists of an \inv{} and \rsp{} event.

\ophmvotm exports \tbeg, \tins, \tdel, \tlook, and \tryc \mth{s} as explained in \secref{model}. Among them \tdel, \tlook are return-value methods (or \rvmt{s}) while \tins, \tdel are update methods (or \upmt{s}). We treat \tdel as both \rvmt as well as \upmt. The \rvmt{s} return the current value of the key. %The \upmt{s} update the value of the keys in the shared memory after validation as a part of the \tryc \mth. 
The \upmt{s}, update to the keys are first noted down in the local log, \emph{\llog}. Then in the \tryc \mth after successful validations of these updates are transferred to the shared memory.%\todo{Removed the figure as we lack space.} 
%
\ignore{
%\figref{nostm24} shows the life cycle of a transaction in \mvotm.  

\begin{figure}
	\centering	
	\captionsetup{justification=centering}
	\centerline{\scalebox{0.5}{\input{figs/pnetys8.pdf_t}}}
	\caption{Transaction life cycle of \mvotm}	
	\label{fig:nostm24}
\end{figure}
}
We now explain the working of each method as follows: %Additional details including pseudocode are in \apnref{rpcode} and in the accompanying technical report\cite{Juyal+:MVOSTM:Corr:2017}. %\todo{cite only at one place in the pcode} \cite{Juyal+:MVOSTM:Corr:2017}.
%\todo{SK: compressed. Review }
%Due to lack of space, the pseudocode of some of the \mth{s} are shown here. The remaining details are explained in the \apnref{rpcode} and in the accompanying technical report \todo{cite only at one place in the pcode} \cite{Juyal+:MVOSTM:Corr:2017}. 

%\textit{STM\_begin(), STM\_lookup(), STM\_insert(), STM\_delete()} and \textit{STM\_tryC()} methods. Each transaction is divided into two phases. First, \textbf{{\rvp{}}} in which initially each transaction invokes \textit{STM begin()} method by a thread to begin a new transaction $T_i$. It creates transaction local log and allocates unique id. In the case of \npins{} method actual insertion will happen in \cp{}(or \nptc{}). First, it will identify the node corresponding to the key in local log. If the node exists then it just update the local log with useful information like value, operation name and operation status for later use in \nptc{}. Otherwise, it will create a local log and update it. 
%\textit{STM \init()} This method invokes at the start of the STM system. Initialize the global counter as 1. 
%\vspace{-.5cm}

\vspace{1mm}
\noindent 
\textbf{\emph{t\_begin()}:} A thread invokes a new transaction $T_i$ using this method. The transaction $T_i$ local log $\llog_i$ is initialized at \Lineref{bg2}. This \mth returns a unique id to the invoking thread by incrementing an atomic counter at \Lineref{bg3}. This unique id is also the timestamp of the transaction $T_i$. For convenience, we use the notation that $i$ is the timestamp (or id) of the transaction $T_i$. 

\begin{algorithm}
	%\label{alg:llsearch} 
	\scriptsize
	\caption{\emph{t\_begin()}: It provides the local log and unique id to each transaction.}
	\setlength{\multicolsep}{0pt}
	%\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{0}\makeatother
		\Procedure{\emph{t\_begin{()}}}{}\label{lin:bg1}
		\State txLog $\gets$ new txLog(). \Comment{Initialize the local log of transaction} \label{lin:bg2}
		\State $t\_id$ $\gets$ get\&inc(\emph{counter}). \Comment{Get the unique transaction id ($t\_id$) while incrementing the \emph{counter} atomically} \label{lin:bg3}
		\State return $t\_id$.
		\EndProcedure
	\end{algorithmic}
	%\end{multicols}
\end{algorithm}

\vspace{1mm}
\noindent 
\textbf{\rvmt{s}}: It can be either $\tdel(ht, k, v)$ or $\tlook(ht, k, v)$. Both these \mth{s} return the current value of key $k$. \algoref{rvmt} gives the high level overview of these \mth{s}. First, the algorithm checks to see if the given key is already in the local log, $\llog_i$ of $T_i$ (\linref{rvm-chk_log}). If the key is already there then the current \rvmt is not the first method on $k$ and is a subsequent method of $T_i$ on $k$. So, we can return the value of $k$ from the $\llog_i$. 

If the key is not present in the $\llog_i$, then \ophmvotm searches into shared memory. Specifically, it searches the bucket to which $k$ belongs to. Every key in the range $\mathcal{K}$ is statically allocated to one of the $B$ buckets. So the algorithms search for $k$ in the corresponding bucket, say $B_k$ to identify the appropriate location, i.e., identify the correct \emph{predecessor} or $pred$ and \emph{current} or  $curr$ keys in the \lsl of $B_k$ without acquiring any locks similar to the search in \lazy \cite{Heller+:LazyList:PPL:2007}. Since each key has two links, \rn and \bn, the algorithm identifies four node references: two $pred$ and two $curr$ according to red and blue links. They are stored in the form of an array with $\bp$ and $\bc$ corresponding to blue links; $\rp$ and $\rc$ corresponding to red links. If both $\rp$ and $\rc$ nodes are unmarked then the $pred, curr$ nodes of both red and blue links will be the same, i.e., $\bp = \rp$ and $\rc = \bc$. Thus depending on the marking of $pred, curr$ nodes, a total of two, three or four different nodes will be identified. Here, the search ensures that $\bp.key \leq \rp.key < k \leq \rc.key \leq \bc.key$. 

Next, the re-entrant locks on all the $pred, curr$ keys are acquired in increasing order to avoid the deadlock. Then all the $pred$ and $curr$ keys are validated by \emph{rv\_Validation()} in \linref{rvm-chk_valid} as follows: (1) If $pred$ and $curr$ nodes of blue links are not marked, i.e, $(\neg \bp.marked) ~ \&\& ~ (\neg \bc.marked)$. (2) If the next links of both blue and red $pred$ nodes point to the correct $curr$ nodes: $(\bp.\bn = \bc) ~ \&\& ~ (\rp.\rn = \rc)$ at \Lineref{rvv1}. 

If any of these checks fail, then the algorithm retries to find the correct $pred$ and $curr$ keys. It can be seen that the validation check is similar to the validation in concurrent \lazy \cite{Heller+:LazyList:PPL:2007}.%\todo{SK: Removed ref to app} 
%Detailed reasons behind these checks along with pseudocode is given in \apnref{rpcode} and \cite{Juyal+:MVOSTM:Corr:2017}.\todo{cite only at one place in the pcode}

Next, we check if $k$ is in $B_k.\lsl$. If $k$ is not in $B_k$, then we create a new node $n$ for $k$ as: $\langle key=k, lock=false, marked = true, vl=ver, nnext=\phi \rangle$ and insert it into $B_k.\lsl$ such that it is accessible only via \rn. %since this node is marked (\linref{rvm-ver_abs}). 
This node will have a single version $ver$ as $\langle ts=0, val=null, rvl=i, max_{rvl} = i, vnext=\phi \rangle$. Here invoking transaction $T_i$ is creating a version with timestamp $0$ to ensure that \rvmt{s} of other transactions will never abort. As we have explained in \figref{pop} (b) of \secref{intro}, even after $T_2$ deletes $k_2$, the previous value of $v_0$ is still retained. Thus, when $T_1$ invokes $lu$ on $k_2$ after the delete on $k_2$ by $T_2$, \ophmvotm will return $v_0$ (as previous value). Hence, each \rvmt will find a version to read while maintaining the infinite version corresponding to each key $k$. $marked$ field sets to true because it access by $\rn$ only. In $rvl$ and $max_{rvl}$, $T_i$ adds the timestamp as $i$ in it and $vnext$ is initialized to empty value. Since $val$ is null and the $n$, this version and the node are not technically inserted into $B_k.\lsl$. %\todo{Done:Add the reason for this version.}

If $k$ is in $B_k.\lsl$ then, $k$ is the same as $\rc$ or $\bc$ or both. Let $n$ be the node of $k$ in $B_k.\lsl$. We then find the version of $n$, $ver_j$ which has the timestamp $j$ such that $j$ has the largest timestamp smaller than $i$ (timestamp of $T_i$). Add $i$ to $ver_j$'s $rvl$ (\linref{rvm-add_i}). $max_{rvl}$ maintains the maximum timestamp among all rv\_methods read from this version at \Lineref{rvm-max}. Then release the locks, update the local log $\llog_i$ in \linref{rvm-unlock} and return the value stored in $ver_j.val$ in \linref{rvm-ret}. %\todo{Removed rv\_validation from here due to lack of space.} 
%We considered \npluk{} and \npdel{} methods as a \rvmt{}. At \Lineref{rvm2} of algorithm 1, if \npluk{} is not the first method on a particular key means if its a subsequent method of the same transaction for that key then it will search into the local log and return the value and operation status based on the previous operation. If \npluk{} is the first method on that key then it will search into \emph{concurrent data structure (CDS)} to identify the location of the node corresponding to the key in \bn{} as well as \rn{} at \Lineref{rvm5}. Then at \Lineref{rvm7}, it will do the \emph{rv\_Validation()} after acquiring the locks on $preds$ and $currs$ in increasing order of keys to avoid deadlocks. If \emph{rv\_Validation()} succeed and node corresponding to the key is not present in the underlying DS then it will create the node and insert the $0^{th}$ version and add itself into $0^{th}$.$rvl$ refer \figref{mvostm81} and release the locks in same lock acquisition order. From \Lineref{rvm13} to \Lineref{rvm16}, it identifies the version from $CDS$ with largest TS as $T_j$ which is less than TS($T_i$) with the help of \emph{find\_lts()} method. Then add TS($T_i$) into $rvl$ of $T_j$ and finally release the locks and update the local log. \npdel{} will work same as a \npluk{}. The actual deletion will happen in the \nptc{}.
%\setlength{\textfloatsep}{0pt} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%rv_method()%%%%%%%%%%%%%
%\vspace{-.5cm}
\begin{algorithm}
	\scriptsize
	\caption{\emph{\rvmt:} It can be either $\tdel_i(ht, k, v)$ or $\tlook_i(ht, k, v)$ on key $k$ that maps to bucket $B_k$ of hash-table $ht$.} \label{algo:rvmt} 	
	%\setlength{\multicolsep}{0pt}
	%\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{5}\makeatother
		\Procedure{$\rvmt_i$}{$ht, k, v$}		
		\If{($k \in \llog_i$)} \label{lin:rvm-chk_log}
			\State Update the local log and return $val$. \label{lin:rvm-pres_log}
		\Else \label{lin:rvm-els_log}
			\State Search in \lsl to identify the $preds[]$ and $currs[]$ for $k$ using \bn and \rn in bucket $B_k$. \label{lin:rvm-search}
			\State Acquire the locks on $preds[]$ and $currs[]$ in increasing order. \label{lin:rvm-locks}
			\If{($!rv\_Validation()$)} \label{lin:rvm-chk_valid}
				\State Release the locks and goto \linref{rvm-search}. \label{lin:rvm-retry}
			\EndIf %\label{lin:rvm-end_valid}
			\If{($k  ~ \notin ~ B_k.\lsl$)} \label{lin:rvm-chk_k} 
				\State Create a new node $n$ with key $k$ as: $\langle$ \emph{key = k, lock = false, marked = true, vl = ver, nnext = }$\phi \rangle$. \label{lin:rvm-chk_k1} 
				\State /*The $vl$ consists of a single element $ver$ with $ts$ as 0*/
				\State Create the version $ver$ as: $\langle \emph{$ts=0, val=null, rvl=i, max_{rvl}=i, vnext=\phi$}\rangle$.  
				\State Insert $n$ into $B_k.\lsl$ such that it is accessible only via \rn{s}. \Comment{$n$ is marked} \label{lin:rvm-ver_abs}  	\State Release the locks; update the $\llog_i$ with $k$.
				\State return $null$.
			\EndIf %\label{lin:rvm-end-chk_k} 
			\State Identify the version $ver_j$ with $ts=j$ such that $j$ is the largest timestamp smaller than $i$.
%			\If{($ver_j$ == $null$)}
%			\State goto \Lineref{rvm-chk_k1}.
%			\EndIf
			%\State $ver_j = find\_lts(k)$.\label{lin:corr-ver} 
			\State Add $i$ into the $rvl$ of $ver_j$. \label{lin:rvm-add_i} 
			\If{($ver_j.max_{rvl}$ $<$ $i$)}
			\State Set $ver_j.max_{rvl}$ to $i$. \label{lin:rvm-max} 
			\EndIf
			\State $retVal = ver_j.val$.
			\State Release the locks; update the $\llog_i$ with $k$ and $retVal$. \label{lin:rvm-unlock} 
		\EndIf %\label{lin:rvm-end_log}
		\State return $retVal$. \label{lin:rvm-ret}
		\EndProcedure
	\end{algorithmic}
%\end{multicols}
\end{algorithm}
%\vspace{-.7cm}

\ignore {
The \emph{rv\_Validation()} is called by the \rvmt{} and \upmt{}. It will identify the conflicts among the concurrent methods of different transactions. It will be more clear by the \figref{mvostm9}, where two concurrent conflicting methods of different transactions are working on the same key $k_3$. Initially, at stage $s_1$ in \figref{mvostm9} (c) both the conflicting methods $ins_1(k_3)$ and $lu_2(k_3)$ optimistically (without acquiring locks) identify the same $preds$ and $currs$ for key $k_3$ from underlying $CDS$ in \figref{mvostm9} (a). At stage $s_2$ in \figref{mvostm9} (c), method $ins_1(k_3)$ of transaction $T_1$ acquired the lock on $preds$ and $currs$ and inserted the node into it (\figref{mvostm9} (b)). After successful insertion by $T_1$, $preds$ and $currs$ will change for $lu_2(k_3)$ at stage $s_3$ in \figref{mvostm9} (c). It will caught via \emph{rv\_Validation} method at \Lineref{rvv1} when $(\bp.\bn \neq \bc)$ for $lu_2(k_3)$. After that again it will find the new $preds$ and $currs$ for $lu_2(k_3)$ and eventually it will commit.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%rv_validation()%%%%%%%%%%%%%
\begin{algorithm}
	%\label{alg:llsearch} 
	\scriptsize
	\caption{\emph{rv\_Validation()} }
	\setlength{\multicolsep}{0pt}
	%\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{14}\makeatother
		\Procedure{rv\_validation{()}}{}
		\If{$((\bp.marked) || (\bc.marked) ||(\bp.\bn) \neq \bc || (\rp.\rn) \neq {\rc})$}\label{lin:rvv1}
		\State return $false$. \label{lin:rvv2}
		\Else \label{lin:rvv3}
		\State return $true$. \label{lin:rvv4}
		\EndIf 
		\EndProcedure
	\end{algorithmic}
	%\end{multicols}
\end{algorithm}

\cmnt{
\begin{figure}[tbph]
\captionsetup{justification=centering}
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centerline{\scalebox{0.47}{\input{figs/mvostm9.pdf_t}}}
	\caption{Method validation}
	\label{fig:mvostm91}
\end{figure}
}

\begin{figure}[tbph]
\captionsetup{justification=centering}
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centerline{\scalebox{0.42}{\input{figs/disc1.pdf_t}}}
	\caption{Interference validation (or rv\_Validation)}
	\label{fig:mvostm9}
\end{figure}
%\vspace{-.7cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%try_C()%%%%%%%%%%%%%
}	

\ignore {

We are considering the chaining \tab{} as a underlying data structure where chaining is done via lazy-list refer \figref{1mvostmdesign} a). Each bucket of the \tab{} is having two sentinel nodes: $head$ and $tail$. $Head$ and $tail$ are initialized as -$\infty$ and +$\infty$ respectively. Keys $\langle k_1, k_2, ...k_n \rangle$ are added in increasing order in the list between the sentinel nodes. %as represented in \figref{mvostmdesign} a). %We assume that all the keys are ordered as $k_1, k_2, ...k_n$ and belong to the set $\mathcal{T}$. 

Each key is maintaining the multiple versions in increasing order of timestamp (\figref{1mvostmdesign} b)). %as shown in \figref{mvostmdesign} b). 
For each key $k_1$ of transaction $T_i$, we maintain $k_1.vl$ (version list) which is a list consisting of version tuples in the form $\langle ts, val, mark, rvl, vnext \rangle$.  Description of each field as: $ts$ stands for timestamp which is unique for each transaction, $val$ is the value written by any transaction corresponding to the key, $mark$ is the Boolean variable which can be true or false (if the method corresponding to the key is \npdel{} then the value of $mark$ field will be true, ($T$) and if the method corresponding to the key is \npins{} then the value of $mark$ field will be false, ($F$)), $rvl$ represents $return$-$value$ $list$ which is having all the transactions who has performed \rvmt{} on the same key $k_1$ and $vnext$ is having the information about next available version of the same key $k_1$. The \mvotm system consists of the following main methods: \emph{STM init()}, \emph{STM begin()}, $\npins{}$, $\npluk{}$, $\npdel{}$ and $\nptc{}$.
} 


\vspace{1mm}
\noindent
\textbf{\tins{()}}: This is another optimization done in \emph{\ophmvotm{s}} to identify the early abort which prevents the work done by aborted transactions and saves time. The actual effect of the \tins{()} comes after the successful tryC method. First, t\_insert() searches the key $k$ in the local log, $txLog_i$ of $T_i$ at \Lineref{insert2}. If $k$ does not exist in the $txLog_i$ then it identifies the appropriate location ($pred$ and $curr$) of key $k$ using \bn{} and \rn{} (\Lineref{insert3}) in the \lsl of $B_k$ without acquiring any locks similar to \rvmt{} explained above. 

Next, it acquires the re-entrant locks on all the $pred$ and $curr$ keys in increasing order. After that, all the $pred$ and $curr$ keys are validated by \emph{tryC\_Validation} in \Lineref{insert5} as follows: (1) It does the \emph{rv\_Validation()} as explained above in the \rvmt{}. (2) If key $k$ exists in the $B_k.\lsl$ and let $n$ as a node of $k$. Then algorithm identifies the version of $n$, $ver_j$ which has the timestamp $j$ such that $j$ has the largest timestamp smaller than $i$ (timestamp of $T_i$) at \Lineref{trycv5}. If $max_{rvl}$ of $ver_j$ is greater than timestamp $i$ at \Lineref{trycv6} then it returns $Abort$ in \Lineref{insert6}.

\emph{tryC\_Validation()} in \tins{()} identifies the early abort of invalid transaction. The advantage of doing the early validation to save the significant computation of long running transaction which will abort in the future. Consider \figref{insertadv} where two transaction $T_1$ and $T_2$ working on key $k_5$. In \figref{insertadv} (a), $T_1$ aborts in tryC (delayed validation) because higher timestamp $T_2$ committed. But in \figref{insertadv} (b), $T_1$ validates the t\_insert() instantly by looking into the $max_{rvl}$ of $k_5$ as shown in \figref{insertadv} (c) and save its computation and returns abort. 

\begin{algorithm}
	\scriptsize
	\caption{\emph{t\_insert():} Actual insertion happens in the tryC.} \label{algo:insert} 	
	%\setlength{\multicolsep}{0pt}
	%\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{32}\makeatother
		\Procedure{$t\_insert()$}{}\label{lin:insert1}		
		\If{($k \notin \llog_i$)} \label{lin:insert2}
		\State Search in \lsl to identify the $preds[]$ and $currs[]$ for $k$ using \bn and \rn in bucket $B_k$. \label{lin:insert3}
		\State Acquire the locks on $preds[]$ and $currs[]$ in increasing order. \label{lin:insert4}
		\If{($!tryC\_Validation()$)} \label{lin:insert5}
		\State return $Abort$.\label{lin:insert6} \Comment{Release the locks}
		\EndIf %\label{lin:rvm-end_valid}
		\State Release the locks.
		\Else \label{lin:insert7}
		\State Update the local log.  \label{lin:insert8}
		\EndIf %\label{lin:rvm-end_log}
%		\State return $$. \label{lin:rvm-ret}
		\EndProcedure
	\end{algorithmic}
	%\end{multicols}
\end{algorithm}
%\vspace{-.7cm}


\begin{figure}
	\captionsetup{justification=centering}
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centerline{\scalebox{0.37}{\input{figs/insertadv.pdf_t}}}
	\caption{Advantage of early validation in t\_insert()}
	\label{fig:insertadv}
\end{figure}

\vspace{1mm}
\noindent
\textbf{\upmt{s}}: It can be either $\tins(ht, k, v)$ or $\tdel(ht, k, v)$.
Both the \mth{s} create a version corresponding to the key $k$. The actual effect of \tins{} and \tdel{} in shared memory will take place in \tryc{}. \algoref{mtryc} represents the high level overview of \tryc{}. 

%In the transaction local log, $\llog_i$ consist of \upmt{} only. 
Initially, to avoid deadlocks, the algorithm sorts all the $keys$ in increasing order which are present in the local log, $\llog_i$. In \tryc{}, $\llog_i$ consists of \upmt{s} (\tins{} or \tdel{}) only. For all the \upmt{s} ($opn_i$) it searches the key $k$ in the shared memory corresponding to the bucket $B_k$. It identifies the appropriate location ($pred$ and $curr$) of key $k$ using \bn{} and \rn{} (\Lineref{mtryc3}) in the \lsl of $B_k$ without acquiring any locks similar to \rvmt{} explained above. 


Next, it acquires the re-entrant locks on all the $pred$ and $curr$ keys in increasing order. After that, all the $pred$ and $curr$ keys are validated by \emph{tryC\_Validation} in \Lineref{mtryc5} as explained in t\_insert().

% follows: (1) It does the \emph{rv\_Validation()} as explained above in the \rvmt{}. (2) If key $k$ exists in the $B_k.\lsl$ and let $n$ as a node of $k$. Then algorithm identifies the version of $n$, $ver_j$ which has the timestamp $j$ such that $j$ has the largest timestamp smaller than $i$ (timestamp of $T_i$) at \Lineref{trycv5}. If $max_{rvl}$ of $ver_j$ is greater than timestamp $i$ at \Lineref{trycv6} then algorithm returns $Abort$ in \Lineref{mtryc6}.

\begin{algorithm}
	
	\scriptsize
	\caption{\emph{tryC($T_i$)}: Validate the \upmt{s} of the transaction and then commit.}
	\setlength{\multicolsep}{0pt}
	\label{algo:mtryc}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{44}\makeatother
		\Procedure{$tryC{(T_i)}$}{}
		%\State Get the local log list for corresponding transaction;
		\State /*Operation name ($opn$) which could be either \tins or \tdel*/
		\State /*Sort the $keys$ of $\llog_i$ in increasing order.*/
		\ForAll{($opn_i$ $\in$ $\llog_i$)} \label{lin:mtryc1}
		\If{(($opn_i$ == \tins{}) $||$ ($opn_i$ == \tdel{}))}\label{lin:mtryc2}
		\State Search in $\lsl$ to identify the $preds[]$ and $currs[]$ for $k$ using \bn and \rn in bucket $B_k$. \label{lin:mtryc3}
		\State Acquire the locks on $preds[]$ and $currs[]$ in increasing order. \label{lin:mtryc4}
		\If{($!tryC\_Validation()$)} \label{lin:mtryc5}
		\State return $Abort$.\label{lin:mtryc6} \Comment{Release the locks}
		\EndIf\label{lin:mtryc7}
		\EndIf\label{lin:mtryc8}
		\EndFor\label{lin:mtryc9}
		\ForAll{($opn_i$ $\in$ $\llog_i$)}\label{lin:mtryc10}
		\State $intraTransValidation()$  modifies the $preds[]$ and $currs[]$ of current operation which would have been \blank{.7cm} updated by the previous operation of the same transaction.\label{lin:mtryc11}
		\If{(($opn_i$ == \tins{}) \&\& ($k  ~ \notin ~ B_k.\lsl$))}\label{lin:mtryc12}
		\State Create new node $n$ with $k$ as: $\langle$ \emph{key = k, lock = false, marked = false, vl = ver, nnext = $\phi$} $\rangle$. \label{lin:mtryc13}
		\State Create two versions $ver$ as: $\langle$ \emph{ts=0, val=null, rvl=$\phi$, $max_{rvl}$ = $\phi$, vnext=$i$} $\rangle$ for $T_0$ and $\langle$ \emph{ts=i, val=v, \blank{1.1cm}rvl=$\phi$, $max_{rvl}$ = $\phi$, vnext=$\phi$} $\rangle$ for $T_i$.
		\State Insert node $n$ into $B_k.\lsl$ such that it is accessible via \rn{} as well as \bn{} \Comment{$lock$ sets $true$}.  \label{lin:mmtryc14}
		\ElsIf{($opn_i$ == \tins{})}\label{lin:mtryc14}
		\State Add the version $ver$ as: $\langle$ \emph{ts=i, val=v, rvl=$\phi$, $max_{rvl}$=$\phi$, vnext=$\phi$} $\rangle$ into $B_k.\lsl$ such that it is \blank{1.1cm} accessible via \rn as well as \bn.\label{lin:mtryc15}
		\EndIf\label{lin:mtryc16}
		\If{($opn_i$ == \tdel{})}\label{lin:mtryc17}
		\State Add the version $ver$ as: $\langle$ \emph{ts=i, val=null, rvl=$\phi$, $max_{rvl}$=$\phi$, vnext=$\phi$} $\rangle$ into $B_k.\lsl$ such that \blank{1.1cm}it is accessible only via \rn.\label{lin:mtryc18}
		\EndIf\label{lin:mtryc19}
		\State Update the $preds[]$ and $currs[]$ of $opn_i$ in $\llog_i$.\label{lin:mtryc20}
		
		\EndFor
		%\EndFor
		\State Release the locks; return $Commit$.\label{lin:mtryc21}
		\EndProcedure
	\end{algorithmic}
	%\end{multicols}
\end{algorithm}


If \emph{tryC\_Validation} is successful then each \upmt{s} exist in $\llog_i$ will take the effect in the shared memory after doing the \emph{intraTransValidation()} in \Lineref{mtryc11}. If two $\upmt{s}$ of the same transaction have at least one common shared node among its recorded $pred$ and $curr$ keys, then the previous $\upmt{}$ effect may overwrite if the current $\upmt{}$ of $pred$ and $curr$ keys are not updated according to the updates are done by the previous $\upmt{}$. Thus to solve this we have \emph{intraTransValidation()} that modifies the $pred$ and $curr$ keys of current operation based on the previous operation in \Lineref{mtryc11}.

%\vspace{-.5cm}

%\vspace{-.5cm}
 
Next, we check if \upmt{} is \tins{} and $k$ is in $B_k.\lsl$. If $k$ is not in $B_k$, then create a new node $n$ for $k$ as $\langle key=k, lock=false, marked = false, vl=ver, nnext=\phi \rangle$. This node will have two versions $ver$ as $\langle ts=0, val=null, rvl=\phi, max_{rvl} = \phi, vnext=i \rangle$ for $T_0$ and $\langle ts=i, val=v, rvl=\phi, max_{rvl} = \phi, vnext=\phi \rangle$ for $T_i$. $T_i$ is creating a version with timestamp $0$ to ensure that \rvmt{s} of other transactions will never abort. For second version, $i$ is the timestamp of the transaction $T_i$ invoking this method; $marked$ field sets to false because the node is inserted in the \bn{}. $rvl$, $max_{rvl}$, and $vnext$ are initialized to empty values. We set the $val$ as $v$ and insert $n$ into $B_k.\lsl$ such that it is accessible via \rn{} as well as \bn{} and set the lock field to be $true$ (\linref{mmtryc14}). If $k$ is in $B_k.\lsl$ then, $k$ is the same as $\rc$ or $\bc$ or both. Let $n$ be the node of $k$ in $B_k.\lsl$.
Then, we create the version $ver$ as: $\langle ts=i, val=v, rvl=\phi, max_{rvl}=\phi, vnext=\phi \rangle$ and insert the version into $B_k.\lsl$ such that it is accessible via \rn{} as well as \bn{} (\linref{mtryc15}).

Subsequently, we check if \upmt{} is \tdel{} and $k$ is in $B_k.\lsl$. Let $n$ be the node of $k$ in $B_k.\lsl$.
Then create the version $ver$ as $\langle ts=i, val=null, rvl=\phi, max_{rvl}=\phi, vnext=\phi \rangle$ and insert the version into $B_k.\lsl$ such that it is accessible only via \rn{} (\linref{mtryc18}). 

Finally, at \Lineref{mtryc20} it updates the $pred$ and $curr$ of $opn_i$ in local log, $\llog_i$. At \Lineref{mtryc21} releases the locks on all the $pred$ and $curr$ in increasing order of keys to avoid deadlocks and return $Commit$.  

We illustrate the helping methods of \rvmt{}, t\_insert(), and \upmt{} in detail as follows:

\noindent
\textbf{rv\_Validation():} It is called by the \rvmt{}, t\_insert(), and \upmt{}. It identifies the conflicts among the concurrent methods of different transactions. Consider an example shown in \figref{mvostm9}, where two concurrent conflicting methods of different transactions are working on the same key $k_4$. Initially, at stage $s_1$ in \figref{mvostm9} (c) both the conflicting method optimistically (without acquiring locks) identify the same $pred$ and $curr$ keys for key $k_4$ from $B_k.\lsl$ in \figref{mvostm9} (a). At stage $s_2$ in \figref{mvostm9} (c), method $ins_1(ht, k_4, v_1)$ of transaction $T_1$ acquired the lock on $pred$ and $curr$ keys and inserted the node into $B_k.\lsl$ as shown in \figref{mvostm9} (b). After successful insertion by $T_1$, $pred$ and $curr$ have been changed for $lu_2(ht, k_4)$ at stage $s_3$ in \figref{mvostm9} (c). So, the above modified information is delivered by \emph{rv\_Validation} method at \Lineref{rvv1} when $(\bp.\bn \neq \bc)$ for $lu_2(ht, k_4)$. After that again it will find the new $pred$ and $curr$ for $lu_2(ht, k_4, v_1)$ and eventually it will commit. %Where $\bp$ and $\rp$ are the predecessor nodes in $\bn$ and $\rn$, respectively. $\bc$ and $\rc$ are the successor nodes in $\bn$ and $\rn$ respectively.
%\vspace{-.7cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%rv_validation()%%%%%%%%%%%%%
\begin{algorithm}
	%\label{alg:llsearch} 
	\scriptsize
	\caption{\emph{rv\_Validation()}: Validate against the conflicting method of different transactions.}
	\setlength{\multicolsep}{0pt}
	%\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{72}\makeatother
		\Procedure{$rv\_validation{()}$}{}
		\If{$((\bp.marked) || (\bc.marked) ||(\bp.\bn) \neq \bc || (\rp.\rn) \neq {\rc})$}\label{lin:rvv1}
		\State return $false$. \label{lin:rvv2}
		\Else \label{lin:rvv3}
		\State return $true$. \label{lin:rvv4}
		\EndIf 
		\EndProcedure
	\end{algorithmic}
	%\end{multicols}
\end{algorithm}
%\vspace{-.7cm}
\begin{figure}
	\captionsetup{justification=centering}
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centerline{\scalebox{0.4}{\input{figs/disc1.pdf_t}}}
	\caption{Illustration of rv\_Validation()}
	\label{fig:mvostm9}
\end{figure}
%\vspace{-.7cm}

\begin{figure}[H] 
	\captionsetup{justification=centering}
	%\centering
	%\includegraphics[scale=.5]{figs/fig3.png}
	%\includegraphics[scale=.5]{figs/fig3.pdf_t}
	\centerline{\scalebox{0.45}{\input{figs/disc2.pdf_t}}}
	\caption{Illustration of tryC\_Validation()}
	\label{fig:mvostm12}
\end{figure}

\noindent
\textbf{tryC\_Validation():} It is called by t\_insert(), and \upmt{} in \tryc{}. First, it does the \emph{rv\_Validation()} in \Lineref{trycv1}. If its successful and key $k$ exists in the $B_k.\lsl$ and let $n$ as a node of $k$. Then algorithm identifies the version of $n$, $ver_j$ which has the timestamp $j$ such that $j$ has the largest timestamp smaller than $i$ (timestamp of $T_i$) at \Lineref{trycv5}. If $max_{rvl}$ of $ver_j$ is greater than the timestamp of $i$ then the algorithm returns false (in \Lineref{trycv8}) and eventually, return $Abort$ in \Lineref{insert6} or \Lineref{mtryc6}. Consider an example as shown in \figref{mvostm12} (a), where second method $ins_1(ht, k_5)$ of transaction $T_1$ returns $Abort$ because higher timestamp of transaction $T_2$ is already present in the $max_{rvl}$ of version $T_0$ identified by $T_1$ in \figref{mvostm12} (b).






%If its successful and key $k$ is part of $B_k.\lsl$ then it identifies the version $ver_j$ with $ts=j$ such that $j$ is the largest timestamp smaller than $i$ in \Lineref{trycv5}. From \Lineref{trycv6} to \Lineref{trycv10}, if there exist any higher timestamp transaction in the $ver_j.rvl$ of the $T_j$ return false and eventually return ABORT.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%tryC_validation()%%%%%%%%%%%%%
\begin{algorithm}[H]
	%\label{alg:llsearch} 
	\scriptsize
	\caption{\emph{tryC\_Validation()}: It maintains the order among the transactions.}
	\setlength{\multicolsep}{0pt}
	%\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{79}\makeatother
		\Procedure{$tryC\_validation{()}$}{}
		\If{($!rv\_Validation()$)}\label{lin:trycv1}
		\State Release the locks and retry.\label{lin:trycv2}
		\EndIf\label{lin:trycv3}
		\If{(k $\in$ $B_k.\lsl$)}\label{lin:trycv4}
		\State Identify the version $ver_j$ with $ts=j$ such that $j$ is the largest timestamp smaller than $i$.\label{lin:trycv5}
		\If{($ver_j.max_{rvl}$ $>$ $i$)}\label{lin:trycv6}
%		\ForAll {$T_k$ in $ver_j.rvl$}\label{lin:trycv6}
%		\If{(TS($(T_k)$ $>$ TS($T_i$)))}\label{lin:trycv7}
		\State return $false$.\label{lin:trycv8}
		\EndIf \label{lin:trycv9}
%		\EndFor\label{lin:trycv10}
		\EndIf\label{lin:trycv11}
		\State return $true$.\label{lin:trycv12}
		\EndProcedure
	\end{algorithmic}
	%\end{multicols}
\end{algorithm}
%\vspace{-.7cm}
\begin{algorithm}[H]
	\label{alg:intra} 
	\scriptsize
	\caption{\emph{intraTransValidation()}: Help the upcoming method of the same transaction.}
	\setlength{\multicolsep}{0pt}
	%\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{91}\makeatother
		\Procedure{$intraTransValidation{()}$}{}
		\If{$((\bp.marked) || (\bp.\bn \neq \bc ))$} \label{lin:intra1}
		\If{($opn_k$ == Insert)}\label{lin:intra2}
		\State /*Modify the pred of current transaction $T_i$ with the help of previous transaction $T_k$*/
		\State $\bp_{i}$ = $\bp_{k}$.\bn.\label{lin:intra3} \Comment{Set the $T_i$ \bp{} as $T_k$ \bc{}}
		\Else\label{lin:intra4}
		\State $\bp_{i}$ = $\bp_{k}$.\label{lin:intra5} \Comment{Set the $T_i$ \bp{} as $T_k$ \bp{}}
		\EndIf\label{lin:intra6}
		\EndIf \label{lin:intra9}
		\If{(\rp.\rn $\neq$ \rc)}\label{lin:intra7}
		\State $\rp_{i}$ = $\rp_{k}.\rn$.\label{lin:intra8} \Comment{Set the $T_i$ \rp{} as $T_k$ \rc}
		\EndIf\label{lin:intra10}
		\EndProcedure
	\end{algorithmic}
	%\end{multicols}
\end{algorithm}

\noindent
\textbf{intraTransValidation():} It is called by \upmt{} in \tryc{}. If two $\upmt{s}$ of the same transaction have at least one common shared node among its recorded $pred$ and $curr$ keys, then the previous $\upmt{}$ effect may overwrite if the current $\upmt{}$ of $pred$ and $curr$ keys are not updated according to the updates done by the previous $\upmt{}$. Thus to solve this we have \emph{intraTransValidation()} that modifies the $pred$ and $curr$ keys of current operation based on the previous operation from \Lineref{intra1} to \Lineref{intra10}. Consider an example as shown in \figref{mvostm11}, where two \upmt{s} of transaction $T_1$ are $ins_{11}(ht, k_4, v_1)$ and $ins_{12}(ht, k_6, v_2)$ in \figref{mvostm11} (c). At stage $s_1$ in \figref{mvostm11} (c) both the \upmt{s} identify the same $pred$ and $curr$ from underlying DS as $B_k.\lsl$ shown in \figref{mvostm11} (a). After the successful insertion done by first \upmt{} at stage $s_2$ in \figref{mvostm11} (c), key $k_4$ is part of $B_k.\lsl$ (\figref{mvostm11} (b)). At stage $s_3$ in \figref{mvostm11} (c), $ins_{12}(ht, k_6, v_2)$ identified $(\bp.\bn \neq \bc)$ in \emph{intraTransValidation()} at \Lineref{intra1}. So it updates the $\bp$ in \Lineref{intra3} for correct updation in $B_k.\lsl$. 
%\vspace{-.7cm}

%\vspace{-.7cm}

%if we do not update the $pred$ and $curr$ for $ins_{12}(k_5)$ then it overwrites the previous method updates. To resolve this issue we are doing the intraTransValidation() after each \upmt{} to assign the appropriate $pred$ and $curr$ for the upcoming \upmt{} of same transaction.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%intraTransValidation()%%%%%%%%%%%%%

%\vspace{-.7cm}
\begin{figure}[H]
	\captionsetup{justification=centering}
	%\centering
	%\includegraphics[scale=.5]{figs/fig3.png}
	%\includegraphics[scale=.5]{figs/fig3.pdf_t}
	\centerline{\scalebox{0.43}{\input{figs/disc3.pdf_t}}}
	\caption{Illustration of intraTransValidation()}
	\label{fig:mvostm11}
\end{figure}
%\vspace{-.7cm}


%\todo{remove??}
%Detailed pseudocode and correctness proof are omitted here due to lack of space. For more details please refer the \apnref{appendix} and in the accompanying technical report \cite{Juyal+:MVOSTM:Corr:2017}.
%\noindent
%\textbf{Correctness of \hmvotm:}  




%\todo{}
%\mvpness (explained in \secref{model}) was originally defined for \rwtm{s} \cite{Perel+:2011:SMV:DISC}. When extended to \tab based STM system, \mvpness  implies that no \tlook \mth ever returns abort. \thmref{prog} shows that in \hmvotm with unbounded versions, no \rvmt returns abort. This implies that \tlook will not return abort in a \hmvotm system with unbounded versions. 

\cmnt{
\begin{algorithm}
	%\label{alg:llsearch} 
	\scriptsize
	\caption{\emph{tryC($T_i$)} }
	\setlength{\multicolsep}{0pt}
	%\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{19}\makeatother
		\Procedure{tryC{($T_i$)}}{}
		%\State Get the local log list for corresponding transaction;
		\ForAll{($opn_i$ $\in$ local\_log())} \label{lin:mtryc1}
		\If{(($m_{ij}(k)$ == \npins{}) $||$ ($m_{ij}(k)$ == \npdel{}))}\label{lin:mtryc2}
		\State Search into the $CDS$ to identify the $preds$ and $currs$ for key in \bn{} and \rn.\label{lin:mtryc3}
		\State Acquire the locks in increasing order. \label{lin:mtryc4}
		\If{($!tryC\_Validation()$)} \label{lin:mtryc5}
		\State return $Abort$.\label{lin:mtryc6}
		\EndIf\label{lin:mtryc7}
		\EndIf\label{lin:mtryc8}
		\EndFor\label{lin:mtryc9}
		\ForAll{($opn_i$ $\in$ local\_log())}\label{lin:mtryc10}
		\State $intraTransValidation():$ Modify the preds and currs of consecutive operation which will work on same region.\label{lin:mtryc11}
		\If{(($m_{ij}(k)$ == \npins{}) \&\& (k $\notin$ CDS)}\label{lin:mtryc12}
		\State Create the new node into \bn{} and add the $0^{th}$, $T_i$ versions in it.\label{lin:mtryc13}
		\ElsIf{($m_{ij}(k)$ == \npins{})}\label{lin:mtryc14}
		\State Add the node in \bn{} with $T_i$ version.\label{lin:mtryc15}
		\EndIf\label{lin:mtryc16}
		\If{(($m_{ij}(k)$ == \npdel{})}\label{lin:mtryc17}
		\State Move the node from \bn{} to \rn{} and add the $T_i$ version in it with value NULL.\label{lin:mtryc18}
		\EndIf\label{lin:mtryc19}
		%\State Update the local log;
		\EndFor\label{lin:mtryc20}
		%\EndFor
		\State Release the locks.\label{lin:mtryc21}
		\EndProcedure
	\end{algorithmic}
	%\end{multicols}
\end{algorithm}
%\vspace{-.3cm}
}
 %Otherwise it will perform the above steps for remaining \upmt{s}.
	
%On successful validation of all the \upmt{s}, the actually effect will be taken place. If the \upmt{} is insert and node corresponding to the key is part of underlying DS then it creates the new version tuple and add it in increasing order of version list. Otherwise it will create the node with the help of \nplslins{} and insert the version tuple. If the \upmt{} is delete and node corresponding to the key is part of underlying DS then it creates the new version tuple and set its mark field as TRUE and add it in increasing order of version list. Otherwise it will create the node with the help of \nplslins{} and insert the version tuple with mark field TRUE. After successful completion of each \upmt{} it will release all the locks in the same order of lock acquisition. For more details of each \emph{MV-OSTM} method please refer the \apnref{rpcode}.


\noindent
%This method is called by the \nptc{}. First it will find the $closest\_tuple$ $\langle j,val,mark,rvl,vnext \rangle$ created by the transaction $T_j$ with the largest timestamp smaller than $L\_t\_id$ at \Lineref{checkVersion3}. Then, it checks the version list to identify is there any higher timestamp already present in the $rvl$ of $closest\_tuple$ from \Lineref{checkVersion5} to \Lineref{checkVersion11}. If it presents then it will returns FALSE at \Lineref{checkVersion9} otherwise, TRUE at \Lineref{checkVersion13}. 




%\vspace{-.3cm}


%Version list is playing a vital role to reduce the number of aborts. The size of version list may vary from 1 to $\infty$. Proposed \hmvotm system gives privilege to the programmer to accept the number of versions (say, k) as any integer. If k is 1, it boils down to \otm{}. Currently, we have developed \mvotm with $\infty$ versions. So, we are performing garbage collection method to delete unwanted version. 

%For the \emph{Correctness of MV-OSTM} we can show the acyclicity through graph Characterisation of \emph{MV-OSTM} that all the edges follow the timestamp order.  
   %We have used $\cnt$ as global counter in \tbeg{} to get an unique id for each transaction. 

%\textbf{Execution under \mvotm{}:} \figref{mvostmdesign} a) represents underlying DS of hash table $ht$ with keys $\langle k_1, k_5,k_7,k_8 \rangle$ are in increasing order between the sentinal nodes -$\infty$ and +$\infty$. \figref{mvostmdesign} b) represents the version list of key $k_1$ with $ts$ 0, 15 and 25. We can identify the \upmt{} from mark field of the version. Here transaction $T_0$ has performed delete method whereas transaction $T_{15}$ and $T_{25}$ has inserted versions by insert method. The transaction who has performed \rvmt{} has been added in $return$-$value$ $list$ or $rvl$. Consider transaction $T_{16}$ invoked \npluk{} then its added in the $rvl$ of $T_{15}$. Similarly, we can say about all the transactions added in the $rvl$ of corresponding version. Let say, if any transaction $T_{21}$ wants to create a version but $T_{23}$ with higher timestamp has already been added in the $rvl$ of $T_{15}$ then $T_{21}$ will return ABORT. Otherwise, $T_{21}$ will return COMMIT.


%%%%%%%%%%%%%%%% combine both the pics while removing transactional tree history fig%%%%%%%%%%%%%%%%%%%%%%%
\cmnt{
\section{Pcode of MV-OSTM}
\label{sec:mvdspcode}
The \mvotm system consists of the following methods: $\init()$, $\tbeg()$, $\tlook()$, $\tins()$, $\tdel()$ and $\tryc()$. 
%\vspace{-.3cm}
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STM_init()
\textbf{Pcode convention:} In pcode all the global and local variables are denoted as G\_ and L\_ respectively. We have used $\downarrow$ for input parameters and $\uparrow$ for output parameters (or return value). $\Phi_{lp}$ denotes the linearization point (LP) of corresponding to the each method.   \\
\noindent
\textbf{STM \init():} This method invokes at the start of the STM system. Initialize the global counter ($\cnt$) as 1 at \Lineref{init1} and return it.

\noindent
\textbf{STM \textit{begin()}:} It invoked by a thread to being a new transaction $T_i$. It creates transaction local log and allocate unique id at \Lineref{begin3} and \Lineref{begin5} respectively. %Return the transaction id ($L\_t\_id$) at \Lineref{begin8}.

\noindent
\textbf{STM \textit{insert()}:} Optimistically, actual insertion will happen in the \nptc{} method. First it will identify the node corresponding to the key in local log. If node exist then it just update the local log with useful information like value, operation name and operation status for node corresponding to the key at \Lineref{insert8}, \Lineref{insert9} and \Lineref{insert10} respectively for later use in \nptc{}. Otherwise, it will create a local log and update it.%Transaction id ($L\_t\_id$), object id (L\_obj\_id), node corresponding to the key (L\_key) and value(L\_val) are the inputs of this function.  

\noindent
\textbf{STM \textit{lookup()}:} If \npluk{} is not the first method on a particular key means if its a subsequent method of the same transaction on that key then first it will search into local log from \Lineref{lookup3} to \Lineref{lookup14}. If previous method on the same key of same transaction was insert or lookup (from \Lineref{lookup7} to \Lineref{lookup9}) then \npluk{} will return the value and operation status based on previous operation value and operation status. If previous method on the same key of same transaction was delete (from \Lineref{lookup11} to \Lineref{lookup13}) then \npluk{} will return the value and operation status as NULL and FAIL respectively. 

If \npluk{} is the first method on that key (from \Lineref{lookup16} to \Lineref{lookup22}) then it will identify the location of node corresponding to the key in underlying DS with the help of \nplsls{} inside the \npcld{} method at \Lineref{lookup17}.
\setlength{\textfloatsep}{0pt}
%\vspace{-.3cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------------------------------STM\_LOOKUP-------------------------------------%------
%----
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{spacing}{2}
\begin{algorithm}
%\algsetup{linenosize=\tiny}

	\caption{\tabspace[0.2cm] STM $lookup_{i}()$ %: If the transaction to which this operation belongs has locally done an operation on the same key then returns apt value and status(wrt the previous local operation). Else do the \nplsls{} to find the correct location of the key and validate it.
		%\emph{DESCP}\tabspace: If the Tx has locally done an operation returns apt value and status else does TO \tabspace[2.2cm] and method validation traversal phase in only.\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $obj\_id$, $key$\\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $value$, $op\_status$     
	}
	\scriptsize
\setlength{\multicolsep}{0pt}
\begin{multicols}{2}

	\label{algo:lookup}
%	\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
	
	\begin{algorithmic}[1]
	\makeatletter\setcounter{ALG@line}{0}\makeatother
		\Procedure{STM lookup}{$L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_val \uparrow, L\_op\_status \uparrow$} \label{lin:lookup1}
		%\State $op\_status$ $\gets$ RETRY \label{lin:lookup2};
		\State    /*First identify the node corresponding to the key into local log*/\label{lin:lookup2}
		\If{$($\txlfind$)$} \label{lin:lookup3}
	    \State    /*Getting the previous operation's name*/\label{lin:lookup4}
			\State $L\_opn$ $\gets$ \llgopn{} \label{lin:lookup5}; %\Comment{$\Phi_{lp}$}
			\State    /*If previous operation is insert/lookup then get the value/op\_status based on the previous operations value/op\_status*/\label{lin:lookup6}
			\If{$(($\textup{INSERT} $=$ \textup{$L\_opn$} $)||($ \textup{LOOKUP} $=$ \textup{$L\_opn$}$))$} \label{lin:lookup7}
	
				\State $L\_val$ $\gets$ \llgval{} \label{lin:lookup8};
				\State $L\_op\_status$ $\gets$  $L\_rec.L\_getOpStatus$($L\_obj\_id \downarrow, L\_key \downarrow$) \label{lin:lookup9};
			\State    /*If previous operation is delete then set the value as NULL and op\_status as FAIL*/\label{lin:lookup10}
				\ElsIf{$($\textup{DELETE} $=$ \textup{$L\_opn$}$)$} \label{lin:lookup11}
					\State $L\_val$ $\gets$ NULL \label{lin:lookup12}; 
					\State $L\_op\_status$ $\gets$ FAIL \label{lin:lookup13}; 
				\EndIf \label{lin:lookup14}
		%	\EndIf \label{lin:lookup11}
		\Else \label{lin:lookup15}
	    \State /* Common function for \rvmt{}, if node corresponding to the key is not part of local log*/\label{lin:lookup16}
		\State \cld{};\label{lin:lookup17}
\cmnt{		
            %\State $op\_status $ $\gets$ lslSearch($obj\_id$ $\downarrow$, $key$ $\downarrow$, $preds[]$ $\uparrow$, $currs[]$ $\uparrow$, $value_{BL}$ $\uparrow$, $RV$ $\downarrow$);	
            \State    /*if key is not present in local log then search in underlying DS with the help of list\_lookup*/
			\State \lsls{} \label{lin:lookup13}; 
			%State    /*if list\_lookup return op\_status as ABORT then method will return ABORT*/
			%If{$(op\_status_{ll}$ $=$ \textup{ABORT}$)$} \label{lin:lookup14}
%			\State release all the locks
				%State \handlea{} \label{lin:lookup15}; 
			%Else \label{lin:lookup16}
%			\State    /*check node corresponding to the key is part of underlying DS or not*/	
%			\If{$((G\_curr.key) == L\_key)$} \label{lin:lookup17}
					\State /*From $G\_k.vls$, identify the right $version\_tuple$*/ 
                    \State \find($L\_t\_id \downarrow,L\_key \downarrow, closest\_tuple \uparrow)$;	
                    \State /*Adding $L\_t\_id$ into $j$'s $rvl$*/
                    \State Append $L\_t\_id$ into $rvl$; 
 %                   \State \emph{unlock $x$};
%                    \State return $(v)$; \Comment{v is the value returned}
                \If{$(closest\_tuple.m = TRUE)$}
                    
                    \State $L\_op\_status$ $\gets$ FAIL \label{lin:lookup18};
                    \State $L\_val$ $\gets$ NULL \label{lin:lookup20};
                \Else
                    \State $L\_op\_status$ $\gets$ OK;
                    \State $L\_val$ $\gets$ $closest\_tuple.v$;
                \EndIf    
%            \Else
%                    \State /*Adding $i$ into $0$'s $rvl$*/
%                    \State Append $i$ into $rvl$; 
%                    \State $L\_op\_status$ $\gets$ FAIL;
%                    \State $L\_val$ $\gets$ $NULL$;
					%\EndIf \label{lin:lookup30}
	

			  \State $G\_pred.unlock()$;//$\Phi_{lp}$
                \State $G\_curr.unlock()$;
\State    /*new log entry created to help upcoming method on the same key of the same tx*/
						\State $L\_rec$ $\gets$ Create new $L\_rec\langle L\_obj\_id, L\_key \rangle$\label{lin:lookup31}; 
						%\State ll.setPreds&Currs($obj\_id$ $\downarrow$, $key$ $\downarrow$, $preds[]$ $\downarrow$, $currs[]$ $\downarrow$);
						\State \llsval{$L\_val \downarrow$}
						\State \llspc{} \label{lin:lookup32};
}						  
			
		%\EndIf \label{lin:lookup38}
					
		\EndIf \label{lin:lookup18}
		\State /*Update the local log*/ \label{lin:lookup19}
				\State \llsopn{$LOOKUP \downarrow$} \label{lin:lookup20};
			\State \llsopst{$L\_op\_status \downarrow$} \label{lin:lookup21};
			
			\State return $\langle L\_val, L\_op\_status\rangle$\label{lin:lookup22}; 
				
	\EndProcedure \label{lin:lookup23}
	\end{algorithmic}
	
	\end{multicols}
	
\end{algorithm}
\cmnt{
\begin{figure}
	\centering
	\begin{minipage}[b]{0.49\textwidth}
		\scalebox{.46}{\input{figs/mvostm5.pdf_t}}
		\centering
%		\captionsetup{justification=centering}
		% \vspace{-16cm}
		\caption{History is not opaque}
		\label{fig:mvostm5}
	\end{minipage}
	\hfill
	\begin{minipage}[b]{0.49\textwidth}
		\centering
%		\captionsetup{justification=centering}
		\scalebox{.46}{\input{figs/mvostm6.pdf_t}}
		% \vspace{-16cm}
		\caption{Opaque history}
		\label{fig:mvostm6}
	\end{minipage}   
\end{figure}
}

%\vspace{-.3cm}

%\vspace{-.3cm}
\noindent
\textbf{STM \textit{tryC()}:} The actual effect of \upmt{} (\npins{} and \npdel{}) will take place in \nptc{} method. From \Lineref{tryc5} to \Lineref{tryc15} will identify and validate the $G\_pred$ and $G\_curr$ of each \upmt{} of same transaction. At \Lineref{tryc9} it will validate if there exist any higher timestamp transaction in the $rvl$ of the $closest\_tuple$ of $G\_curr$ then returns ABORT at \Lineref{tryc11}. Otherwise it will perform the above steps for remaining \upmt{s}.

On successful validation of all the \upmt{s}, the actually effect will be taken place from \Lineref{tryc17} to \Lineref{tryc43}. If the \upmt{} is insert and node corresponding to the key is part of underlying DS then it creates the new version tuple and add it in increasing order of version list from \Lineref{tryc22} to \Lineref{tryc24}. Otherwise it will create the node with the help of \nplslins{} and insert the version tuple from \Lineref{tryc25} to \Lineref{tryc29}. 

If the \upmt{} is delete and node corresponding to the key is part of underlying DS then it creates the new version tuple and set its mark field as TRUE and add it in increasing order of version list from \Lineref{tryc31} to \Lineref{tryc34}. Otherwise it will create the node with the help of \nplslins{} and insert the version tuple with mark field TRUE from \Lineref{tryc35} to \Lineref{tryc39}. 
 
After successful completion of each \upmt{}, it will validate the $G\_pred$ and $G\_curr$ of upcoming \upmt{} of the same transaction with the help of \npintv{} at \Lineref{tryc42}. Eventually, it will release all the locks at \Lineref{tryc45} in the same order of lock acquisition.
\vspace{-.3cm}
}


==> Submitted MVOSTM Journal-2019/result.tex <==
%\vspace{-7mm}
\section{Experimental Evaluation}
\label{sec:exp}
%\vspace{1mm}
This section describes the experimental analysis of proposed \emph{\opmvotm{s}} with state-of-the-art STMs. We have three main goals in this section: (1) Analyze the performance benefits of the optimized multi-version object based STMs (or \emph{\opmvotm{s}}) over multi-version object based STMs (or \emph{\mvotm{s}}). (2) Evaluate the benefit of \emph{\opmvotm{s}} over the single-version object based STMs (or \emph{OSTMs}), and (3) Analyze the benefit of \emph{\opmvotm{s}} over  multi-version read-write STMs. We implement hash-table object and list object as \ophmvotm and \oplmvotm described in \secref{pcode}. We also consider the extension of this optimized multi-version object STMs to reduce memory usage. Specifically, we consider a variant that implements garbage collection with unbounded versions and another variant where the number of versions never exceeds a given threshold $K$ for both \emph{\ophmvotm{s}} and \emph{\oplmvotm{s}}. 

%\todo{SK: Remove}
%In this section, we study the performance characteristics of our proposed algorithm hash-table based MVOSTM (HT-MVOSTM) against HT-OSTM \cite{Peri+:OSTM:Netys:2018}, ESTM \cite{Felber+:ElasticTrans:2017:jpdc}, HT-MVTO \cite{Kumar+:MVTO:ICDCN:2014}, HT-MVOSTM with garbage collection (HT-MVOSTM-GC), HT-KOSTM(bounded version OSTM) and HT-RWSTM which is synchronized by basic time-stamp ordering \cite{WeiVoss:TIS:2002:Morg}. We have also compared proposed list-MVOSTM against list-OSTM \cite{Peri+:OSTM:Netys:2018}, list-MVTO \cite{Kumar+:MVTO:ICDCN:2014}, NOrec STM list (NTM) \cite{Dalessandro+:NoRec:PPoPP:2010}, Boosting list (BST) \cite{HerlihyKosk:Boosting:PPoPP:2008}, Lock-free transactional list (LFT) \cite{ZhangDech:LockFreeTW:SPAA:2016}, list-MVOSTM with garbage collection(list-MVOSTM-GC) and list-KOSTM(bounded version OSTM).


%Our experimental goals are : (G1) To study the performance of HT-MVOSTM and list-MVOSTM against the state-of-the-art object and hash-table/list based  STM algorithms over different workloads. (G2) To analyze the number of aborted transactions on both settings. (G3) To analyze the behavior of garbage collection on unbounded OSTM(MVOSTM) against bounded OSTM(KOSTM).
\vspace{1mm}
\noindent
\textbf{Experimental system:} The Experimental system is a large-scale 2-socket Intel(R) Xeon(R) CPU E5-2690 v4 @ 2.60GHz with 14 cores per socket and two hyper-threads (HTs) per core, for a total of 56 threads. Each core has a private 32KB L1 cache and 256 KB L2 cache (which is shared among HTs on that core). All cores on a socket share a 35MB L3 cache. The machine has 32GB of RAM and runs Ubuntu 16.04.2 LTS. All code was compiled with the GNU C++ compiler (G++) 5.4.0 with the build target x86\_64-Linux-gnu and compilation option -std=c++1x -O3.

\vspace{1mm}
\noindent
\textbf{STM implementations:} We have taken the implementation of NOrec-list \cite{Dalessandro+:NoRec:PPoPP:2010}, Boosting-list \cite{HerlihyKosk:Boosting:PPoPP:2008}, Trans-list \cite{ZhangDech:LockFreeTW:SPAA:2016},  ESTM \cite{Felber+:ElasticTrans:2017:jpdc}, and RWSTM directly from the TLDS framework\footnote{https://ucf-cs.github.io/tlds/}. And the implementation of MVOSTM \cite{Juyal+:MVOSTM:SSS:2018}, OSTM \cite{Peri+:OSTM:Netys:2018} and MVTO \cite{Kumar+:MVTO:ICDCN:2014} from our PDCRL library\footnote{https://github.com/PDCRL/}. We implemented our algorithms in C++. Each STM algorithm first creates N-threads, each thread, in turn, spawns a transaction. Each transaction exports \tbeg{}, \tins{}, \tlook{}, \tdel{} and \tryc{} methods as described in \secref{model}.
%Each transaction has two phases, the first phase, i.e., the \emph{return value method execution} followed by the second phase, i.e., the \emph{update method execution} phase defined in detail in \secref{mvdesign}.

\vspace{1mm}
\noindent
\textbf{Methodology:\footnote{Code is available here: https://github.com/PDCRL/MVOSTM/OPT-MVOSTM}} We have considered three types of workloads: ($W1$) Li - Lookup intensive (90\% lookup, 8\% insert, and 2\% delete), ($W2$) Mi - Mid intensive (50\% lookup,  25\% insert, and 25\% delete), and ($W3$) Ui - Update intensive (10\% lookup,  45\% insert, and 45\% delete). The experiments are conducted by varying number of threads from 2 to 64 in power of 2, with 1000 keys randomly chosen. We assume that the \tab{} of \ophmvotm has five buckets and each of the bucket (or list in case of \oplmvotm) can have a maximum size of 1000 keys. Each transaction, in turn, executes 10 operations which include \tlook, \tdel{}, and \tins{} operations. %For accurate results, 
We take an average over 10 results as the final result for each experiment.

\vspace{1mm}
\noindent
\textbf{Results:} \figref{ht-time} represents the performance benefit of all the variants of proposed optimized \mvotm with all variants of \mvotm for hash-table objects. It shows \ophkotm performs best among all the algorithms (OPT-HT-MVOSTM-GC, OPT-HT-MVOSTM, HT-KOSTM, HT-MVOSTM-GC, HT-MVOSTM) by a factor of 1.02, 1.11, 1.05, 1.07, 1.22 for workload W1, 1.06, 1.09, 1.07, 1.08, 1.15 for workload W2, and 1.01, 1.03, 1.02, 1.03, 1.08 for workload W3 respectively. Along with this, \figref{ht-abort} shows the abort count respective algorithms on workload W1, W2, and W3. This represents for less number of threads, the number of aborts are almost same for all the algorithms. But while increasing the number of threads, the number of aborts are least in \ophkotm as compare to others.   So, we compare the performance of \ophkotm with the state-of-the-art STMs as shown in \figref{ht-time-all}. \ophkotm
outperforms all the algorithms (HT-OSTM, ESTM, RWSTM, HT-MVTO, HT-KSTM) by a factor of 3.62, 3.95, 3.44, 2.75, 1.85 for W1,  1.44, 2.36, 4.45, 9.84, 7.42 for W2, and 2.11, 4.05, 7.84, 12.94, 10.70 for W3 respectively. The corresponding number of aborts are represented in \figref{ht-abort-all}. Number of aborts are minimum for \ophkotm as compare to other state-of-the-art STMs. Especially, the number of aborts for \ophkotm is almost negligible as compared to HT-OSTM on lookup-intensive workload (W1) because \ophkotm finds a correct version to looks up as shown in \figref{ht-abort-all} (a). %So, experimental results prove that maintaining multiple version corresponding to each key in \ophkotm gives best speedup for while reducing the number of aborts.   

The observation of optimized list based \mvotm{} is similar as 
optimized hash-table based \mvotm{}. \figref{list-time} represents the performance benefit of all the variants of proposed optimized \mvotm with all variants of \mvotm for list objects. It shows \oplkotm performs best among all the algorithms (OPT-list-MVOSTM-GC, OPT-list-MVOSTM, list-KOSTM, list-MVOSTM-GC, list-MVOSTM) by a factor of 1.14, 1.24, 1.21, 1.20, 1.35 for W1, 1.06, 1.07, 1.12, 1.13, 1.20 for W2, and  1.09, 1.19, 1.11, 1.17, 1.31 for W3 respectively. Along with this, \figref{list-abort} shows the minimum abort count  by \oplkotm as compare to other algorithms on workload W1, W2, and W3. Hence, we choose the best-proposed algorithm \oplkotm and compare with the state-of-the-art list based STMs. 

\begin{figure}[H]
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=12cm]{figs/ht-time.pdf}
	\centering
	\caption{Time comparison among variants of \emph{\ophmvotm{s}} and \emph{\hmvotm{s}} on hash-table}\label{fig:ht-time}
\end{figure}
\vspace{-.5cm}
\begin{figure}[H]
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=12cm]{figs/ht-abort.pdf}
	\centering
	\caption{Abort count among variants of \emph{\ophmvotm{s}} and \emph{\hmvotm{s}} on hash-table}\label{fig:ht-abort}
\end{figure}
\vspace{-.5cm}

\figref{list-time-all} represents \oplkotm
outperforms all the algorithms (list-OSTM, Trans-list, Boosting-list, NOrec-list, list-MVTO, list-KSTM)  by a factor of  2.56, 25.38, 23.57, 27.44, 13.34, 5.99 for W1, 1.51, 20.54, 24.27, 29.45, 24.89, 19.78 for W2, and 2.91, 32.88, 28.45, 40.89, 173.92, 124.89 for W3 respectively. Similarly, \figref{list-abort-all} depicts that \oplkotm obtained the least number of aborts as compare to others on the respective workloads.





\cmnt{
(OPT-HT-MVOSTM-GC, OPT-HT-MVOSTM, HT-KOSTM, HT-MVOSTM-GC, HT-MVOSTM) for W1 1.02, 1.11, 1.05, 1.07, 1.22 for W2 1.06, 1.09, 1.07, 1.08, 1.15 for W3 1.01, 1.03, 1.02, 1.03, 1.08. 

(HT-OSTM, ESTM, RWSTM, HT-MVTO, HT-KSTM) for W1 3.62, 3.21, 3.44, 2.61, 1.85 for W2 1.44, 2.36, 4.45, 9.84, 7.42 for W3 2.11, 4.05, 17.84, 65.94, 56.70.

(OPT-list-MVOSTM-GC, OPT-list-MVOSTM, list-KOSTM, list-MVOSTM-GC, list-MVOSTM) for W1 1.14, 1.24, 1.21, 1.20, 1.35 for W2 1.06, 1.07, 1.12, 1.13, 1.20 for W3 1.09, 1.19, 1.11, 1.17, 1.31.

(list-OSTM, Trans-list, Boosting-list, NOrec-list, list-MVTO, list-KSTM) for W1 2.56, 25.38, 23.57, 27.44, 11.34, 5.99 for W2 1.51, 20.54, 24.27, 29.45, 24.89, 19.78 for W3 1.91, 32.88, 38.45, 43.89, 137.92, 104.89.

(OPT-HT-MVOSTM-GC, OPT-HT-MVOSTM, HT-KOSTM, HT-MVOSTM-GC, HT-MVOSTM) for W1 1.07, 1.16, 1.15, 1.15, 1.21 for W2 1.01, 1.08, 1.06, 1.07, 1.19 for W3 1.01, 1.03, 1.02, 1.03, 1.08.

(OPT-list-MVOSTM-GC, OPT-list-MVOSTM, list-KOSTM, list-MVOSTM-GC, list-MVOSTM) for W1 1.01, 1.05, 1.05, 1.04, 1.11 for W2 1.02, 1.1, 1.1, 1.11 1.19 for W3 1.01, 1.03, 1.05, 1.08, 1.13.
}
\cmnt{
\figref{htw1} shows \hmvotm outperforms all the other algorithms(HT-MVTO, HT-KSTM, RWSTM, ESTM, HT-OSTM) by a factor of 2.6, XXX, 3.1, 3.8, 3.5 for workload type $W1$ and by a factor of 10, YYY, 19, 6, 2 for workload type $W2$ and by a factor of 10.1, ZZZZ, 4.85, 3, 1.4 for workload type $W3$ respectively. As shown in \figref{htw1}, List based MVOSTM (\lmvotm)  performs even better compared with the existing state-of-the-art STMs (list-MVTO, list-KSTM, NOrec-list, Boosting-list, Trans-list, list-OSTM) by a factor of 12, XXX, 24, 22, 20, 2.2 for workload type $W1$ and by a factor of  169, YYY, 35, 24, 28, 2 for workload type $W2$ and by a factor of 26.8, ZZZ, 29.4, 25.9, 20.9, 1.58 for workload type $W3$ respectively.
As shown in \figref{htw2} for both types of workloads, HT-MVOSTM and list-MVOSTM have the least number of aborts.}
%\vspace{1mm}
%\\
%\newpage 


\begin{figure}[H]
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=12cm]{figs/ht-time-all.pdf}
	\centering
	\caption{Time comparison of \ophkotm and State-of-the-art hash-table based STMs}\label{fig:ht-time-all}
\end{figure}
\begin{figure}[H]
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=12cm]{figs/ht-abort-all.pdf}
	\centering
	\caption{Abort count of \ophkotm and State-of-the-art hash-table based STMs}\label{fig:ht-abort-all}
\end{figure}

\begin{figure}[H]
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=12cm]{figs/list-time.pdf}
	\centering
	\caption{Time comparison among variants of \emph{\oplmvotm{s}} and \emph{\lmvotm{s}} on list}\label{fig:list-time}
\end{figure}

\begin{figure}[H]
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=12cm]{figs/list-abort.pdf}
	\centering
	\caption{Abort count among variants of \emph{\oplmvotm{s}} and \emph{\lmvotm{s}} on list}\label{fig:list-abort}
\end{figure}

\begin{figure}[H]
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=12cm]{figs/list-time-all.pdf}
	\centering
	\caption{Time comparison of \oplkotm and State-of-the-art list based STMs}\label{fig:list-time-all}
\end{figure}

\begin{figure}[H]
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=12cm]{figs/list-abort-all.pdf}
	\centering
	\caption{Abort count of \oplkotm and State-of-the-art list based STMs}\label{fig:list-abort-all}
\end{figure}

\begin{figure}[H]
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=12cm]{figs/ht-memory.pdf}
	\centering
	\caption{Memory consumption among variants of \emph{\ophmvotm{s}} and \emph{\hmvotm{s}} on hash-table }\label{fig:ht-memory}
\end{figure}

\begin{figure}[H]
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=12cm]{figs/list-memory.pdf}
	\centering
	\caption{Memory consumption among variants of \emph{\oplmvotm{s}} and \emph{\lmvotm{s}} on list}\label{fig:list-memory}
\end{figure}

\begin{figure}[H]
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=9cm, height=5cm]{figs/optK.pdf}
	\centering
	\caption{Optimal Value of $K$ for \ophkotm and \oplkotm}\label{fig:optK}
\end{figure}

\cmnt{
%\vspace{-1.3cm}
\begin{figure}[H]
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=13cm]{figs/time.pdf}
	\centering
	\caption{Performance of \hmvotm and \lmvotm}\label{fig:htw1}
\end{figure}
%\vspace{-1.8cm}
\begin{figure}[H]
%	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=13.5cm]{figs/aborts.pdf}
	\centering
	\caption{Aborts of \hmvotm and \lmvotm}\label{fig:htw2}
\end{figure}
%\vspace{-1cm}
}

\noindent
\\
As explained in \secref{pcode}, for efficient memory utilization, we develop two variations of \opmvotm.
The first, \opmvotmgc, uses unbounded versions but performs garbage collection. \textbf{This is achieved by deleting non-latest versions whose timestamp is less than the timestamp of  the least live transaction.} \opmvotmgc gave a performance gain of 16\%  over \opmvotm without garbage collection in the best case which is on workload W1 with 64 number of threads. We did one more optimization in \opmvotmgc on the marked node exist in the \rn to make it search efficiently. \textbf{This is achieved by deleting a marked node from \rn whose $max_{rvl}$ of the last version is less than the timestamp of the least live transaction.}  
%as follows: whenever a transaction wants to create a new version of a key, it checks for the least live transaction (LLT) in the system. If current transaction is LLT then it deletes all the previous versions of that key and create one of its own.
%
The second, % technique to efficiently use memory is to restrict the number of versions rather than using unbounded number of versions, without compromising on the benefits of multi-version. 
\opkotm, keeps at most $K$  versions by replacing the oldest version when $(K+1)^{th}$ version is created by a current transaction as explained in \secref{pcode}. \opkotm shows a performance gain of 24\%  over \opmvotm without garbage collection in the best case which is on workload W1 with 64 number of threads. As \opkotm has a limited number of versions while \opmvotmgc can have infinite versions, the memory consumed by \opkotm is also less than \opmvotmgc. We have integrated these variations in both \tab{} based (\ophmvotmgc and \ophkotm) and linked-list based MVOSTMs (\oplmvotmgc and \oplkotm), we observed that these two variations increase the performance, concurrency and reduce the number of aborts as compared to OPT-MVOSTM which does not perform garbage collection.

\textbf{Memory Consumption by OPT-MVOSTM-GC and OPT-KOSTM:} As depicted above \opkotm performs better than \opmvotmgc. Continuing the comparison between the two variations of \opmvotm we chose another parameter as memory consumption. Here we test for the memory consumed by each variation algorithms in creating a version of a key. We count the total versions created, where creating a version increases the counter value by 1 and deleting a version decreases the counter value by 1. % Our experiments, as shown in \figref{memoryC}, under the same contentions $C1$ and $C2$ show that \kotm needs less memory space than \mvotmgc. As \kotm has finite number of versions while \mvotmgc can have infinite versions, the memory consumed by \kotm is 21\% less than \mvotmgc. These experiments are performed for \lmvotm and similar experiments can be performed for \hmvotm. 
\figref{ht-memory} depicts the comparison of memory consumption by all the variants of proposed optimized \mvotm with all variants of \mvotm for hash-table objects. \ophkotm consumes minimum memory among all the algorithms (OPT-HT-MVOSTM-GC, OPT-HT-MVOSTM, HT-KOSTM, HT-MVOSTM-GC, HT-MVOSTM) by a factor of 1.07, 1.16, 1.15, 1.15, 1.21 for W1 , 1.01, 1.08, 1.06, 1.07, 1.19 for W2, and 1.01, 1.03, 1.02, 1.03, 1.08 for W3 respectively. Similarly, \figref{list-memory} depicts the comparison of memory consumption by all the variants of proposed optimized \mvotm with all variants of \mvotm for list objects. \oplkotm consumes minimum memory among all the algorithms
(OPT-list-MVOSTM-GC, OPT-list-MVOSTM, list-KOSTM, list-MVOSTM-GC, list-MVOSTM) by a factor of 1.01, 1.05, 1.05, 1.04, 1.11 for W1, 1.02, 1.1, 1.1, 1.11 1.19 for W2, and 1.01, 1.03, 1.05, 1.08, 1.13 for W3 respectively.






\cmnt{\todo{SK:Remove this paragraph}
one with garbage collection on unbounded MVOSTMs (MVOSTM-GC.\footnote{Implementation details of MVOSTM-GC and KOSTM are give in appendix. ???\label{chirag}}), where each transaction that wants to create a new version of a key checks for the least live transaction (LLT) in the system, if current transaction is LLT then it deletes all the previous versions of that key and create one of its own. Other variation is by using finite limit on the number of versions or bounding the versions in MVOSTMs (KOSTM \footref{chirag}), where oldest versions is overridden by a validated transaction that wishes to create a new version once the limit of version count is reached.} 



%Experiments show that these variations outperform the corresponding MVOSTMs. Between these two variations, \kotm perform better than \mvotmgc as shown in \figref{htw1} and \figref{htw2}. \hkotm helps to achieve a performance speedup of 1.22 and 1.15 for workload type $W1$ and speedup of 1.15 and 1.08 for workload type $W2$ as compared to \hmvotm and \hmvotmgc respectively. Whereas \lkotm (with four versions, i.e., the value of $K$ is four) gives a speedup of 1.1, 1.07 for workload type $W1$ and speedup of 1.25, 1.13 for workload type $W2$ over the \lmvotm and \lmvotmgc respectively. 

%\vspace{1mm}
%\noindent
%\textbf{Mid-Intensive workload:} 
%Similar to Lookup intensive and Update intensive experiments we have conducted experiments for mid intensive workload ($W3$) as well where we have considered 50\% update operations(25\% insert, 25\% delete) and 50\% read operations. Under this setting again \mvotm outperforms all the other algorithms for both \hmvotm and \lmvotm. 
%\figref{pmidI} shows \hmvotm outperforms all the other algorithms(HT-MVTO, RWSTM, ESTM, HT-OSTM) by a factor of 10.1, 4.85, 3, 1.4 for workload type $W3$ respectively. As shown in \figref{pmidI}, list-based MVOSTM (\lmvotm)  performs even better compared with the existing state-of-the-art algorithms (list-MVTO, NOrec-list, Boosting-list, Trans-list, list-OSTM) by a factor of 26.8, 29.4, 25.9, 20.9, 1.58 for workload type $W3$ respectively. Even the abort count for \mvotm is least as compared to all other algorithms for both \hmvotm as well as \lmvotm. \figref{amidI} shows our experimental results for the abort count.
%\vspace{-.7cm}
\cmnt{
\begin{figure}
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=13cm]{figs/mi.pdf}
	\centering
	\caption{Performance of \hmvotm and \lmvotm}\label{fig:pmidI}
\end{figure}
%\vspace{-.7cm}
\begin{figure}
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=13cm]{figs/mi_aborts.pdf}
	\centering
	\caption{Aborts of \hmvotm and \lmvotm}\label{fig:amidI}
\end{figure}
}
%\vspace{-.7cm}

%\vspace{1mm}
%\noindent
%\textbf{Garbage Collection in MVOSTMs (\mvotmgc):} Providing multiple versions to increase the performance of OSTMs in MVOSTMs lead to more space requirements. As many unnecessary versions pertain in the memory a technique to remove these versions or to collect these garbage versions is required. Hence we came up with the idea of garbage collection in MVOSTMs. We have implemented garbage collection for \mvotm for both \tab{} and linked-list based approaches. Each transaction, in the beginning, logs its time stamp in a global list named as ALTL (All live transactions list), which keeps track of all the live transactions in the system. Under the optimistic approach of STM, each transaction performs its updates in the shared memory in \tryc{}. In \tryc{} each transaction performs some validations and if all validations are completed successfully a version of that key is created by that transaction. When a transaction goes to create a version of a key in the shared memory, it checks for the least time stamp live transaction present in the ALTL. If the current transaction is the one with least timestamp present in ALTL, then this transaction deletes all the older versions of the current key and create a version of its own. If current transaction is not the least timestamp live transaction then it doesn't do any garbage collection. In this way, we ensure each transaction performs garbage collection on the keys it is going to create a version on. Once the transaction, changes its state to commit, it removes its entry from the ALTL. As shown in \figref{KHTGC} and \figref{KlistGC} MVOSTM with garbage collection gave a performance gain of 15\% over \mvotm without garbage collection in the best case.
%\vspace{-.7cm}
\cmnt{
\begin{figure}
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=13cm]{figs/KHTGC.pdf}
	\centering
	\caption{Performance comparisons of variations (\hmvotm and \hkotm) of \hmvotm}\label{fig:KHTGC}
\end{figure}
%\vspace{-.7cm}
\begin{figure}
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=13cm]{figs/KlistGC.pdf}
	\centering
	\caption{Performance comparisons of variations (\lmvotm and \lkotm) of \lmvotm}\label{fig:KlistGC}
\end{figure}
%\vspace{-.7cm}
}

\textbf{Finite version \opmvotm (\opkotm):} %Another technique to efficiently use memory is to restrict the number of versions rather than using unbounded number of versions, without compromising on the benefits of multi-version. \opkotm, keeps at most $K$  versions by replacing the oldest version when $(K+1)^{th}$ version is created by a validated transaction, i.e., once a key reaches its maximum number of versions count $K$, no new version is created in a new memory location rather new version overrides the version with the oldest time stamp. 
To find the ideal value of $K$ such that performance as compared to \opmvotmgc does not degrade or can be increased, we perform experiments on all the workloads (W1, W2, and W3) for both (\ophkotm and \oplkotm). %two settings one on high contention high workload ($C1$) and other on low contention low workload ($C2$).
\figref{optK} (a) and (b) shows the best value of $K$ as 5 for \ophkotm and \oplkotm on all the workloads for both hash-table and list objects. %similarly, \figref{optK} (b) represents the best value of $K$ as 5  for  and similar experiments can be performed for \hmvotm.
%\vspace{-.7cm}
\cmnt{
\begin{figure}
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=15cm]{figs/valueofK.pdf}
	\centering
	\caption{Optimal value of K as 4}\label{fig:opmitalK}
\end{figure}
%\vspace{-.7cm}
}
%Under high contention $C1$, each thread spawns over 100  different transactions and each transaction performs 45\% insert, 45\% delete and 10\% lookup operations over 50 random keys. And under low contention $C2$, each thread spawns over one transaction and each transaction performs 45\% insert, 45\% delete and 10\% lookup operations over 1000 random keys. Our experiments as shown in \figref{opmitalK} give the best value of $K$ as 5 under both contention settings. These experiments are performed for \lmvotm and similar experiments can be performed for \hmvotm.
%Between these two variations, \kotm performs better than \mvotmgc as shown in \figref{KHTGC} and \figref{KlistGC}. \hkotm helps to achieve a performance speedup of 1.22 and 1.15 for workload type $W1$ and speedup of 1.15 and 1.08 for workload type $W2$ as compared to \hmvotm and \hmvotmgc respectively. Whereas \lkotm (with four versions) gives a speedup of 1.1, 1.07 for workload type $W1$ and speedup of 1.25, 1.13 for workload type $W2$ over the \lmvotm and \lmvotmgc respectively.  

\vspace{1mm}
\noindent


\cmnt{
\begin{figure}
	\centering
	%\centering
	\captionsetup{justification=centering}
	\includegraphics[width=13cm]{figs/memoryConsumed.pdf}
	\centering
	\caption{Memory Consumption}\label{fig:memoryC}
\end{figure}
}

%For best performance of KOSTM we have considered value of K equals to be 4.\todo{fix macros}


\cmnt{

We have implemented garbage collection for MVOSTM for both hash-based and linked-list based approaches. Each transaction, in the beginning, does its entry in a global list named as ALTL (All live transactions list), which keeps track of all the live transactions. Under the
optimistic approach of STM, each transaction performs its updates in the shared memory in the update execution phase. Each transaction in this phase performs some validations and if all validations are completed successfully a version of that key is created by that transaction. When a transaction goes to create a version of a key in the shared memory, it checks for the least time stamp live transaction present in the ALTL. If the current transaction is the one with least time-stamp present in ALTL, then this transaction deletes all the older versions of the current key and create a version of its own. If current transaction is not the least time-stamp live transaction then it doesn't do any garbage collection. In this way, we ensure each transaction performs garbage collection on the keys it is going to create a version on. Once the transaction, changes its state to commit, it removes its entry from the ALTL. As shown in all the graphs above MVOSTM with garbage collection (HT-MVOSTM-GC and list MVOSTM-GC) performs better than MVOSTM without garbage collection.
}

==> Submitted MVOSTM Journal-2019/sysmodel.tex <==
\vspace{-4mm}
\section{Building System Model}
\label{sec:model}

 Our assumption follows ~\cite{tm-book,Peri+:OSTM:Netys:2018} in which the system consists of a finite set of $p$ processes, $p_1,\ldots,p_n$, accessed by a finite number of $n$ threads in a completely asynchronous fashion and communicates each other using shared keys (or objects). The threads invoke higher level \mth{s} on the shared objects and get corresponding responses. Consequently, we make no assumption about the relative speeds of the threads. We also assume that none of these processors and threads fail or crash abruptly.
 
\vspace{1mm}
\noindent
\textbf{Events and Methods:} We assume that the threads execute atomic \emph{events} and the events by different threads are (1) read/write on shared/local memory objects, (2) \mth{} invocations (or \emph{\inv}) event and responses (or \emph{\rsp}) event on higher level shared memory objects.

Within a transaction, a process can invoke layer-1 \mth{s} (or \op{s}) on a \emph{\tab} \tobj. A \tab{}($ht$) consists of multiple key-value pairs of the form $\langle k, v \rangle$. The keys and values are respectively from sets $\mathcal{K}$ and $\mathcal{V}$. The \mth{s} that a thread can invoke are: (1) $\tbeg_i(){}$: begins a transaction and returns a unique id to the invoking thread. (2) $\tins_i(ht, k, v)$: transaction $T_i$ inserts a value $v$ onto key $k$ in $ht$. (3) $\tdel_i(ht, k, v)$: transaction $T_i$ deletes the key $k$ from the \tab{} $ht$ and returns the current value $v$ for $T_i$. If key $k$ does not exist, it returns $null$. (4) $\tlook_i(ht, k, v)$: returns the current value $v$ for key $k$ in $ht$  for $T_i$. Similar to \tdel, if the key $k$ does not exist then \tlook returns $null$. (5) $\tryc_i()$: which tries to commit all the \op{s} of $T_i$  and (6) $\trya_i()$: aborts $T_i$. We assume that each \mth{} consists of an \inv{} and \rsp{} event.

%The STM system is initialized using init \mth. 

We denote \tins{} and \tdel{} as \emph{update} \mth{s} (or $\upmt{}$ or $up$) since both of these change the underlying data structure. We denote \tdel{} and \tlook{} as \emph{return-value methods (or $\rvmt{}$ or $rvm$)} as these operations return values from $ht$. A \mth{} may return $ok$ if successful or $\mathcal{A}$(abort) if it sees an inconsistent state of $ht$. 

Formally, we denote a \mth{} $m$ by the tuple $\langle \evts{m}, <_m\rangle$. Here, $\evts{m}$ are all the events invoked by $m$ and the $<_m$ a total order among these events.

\vspace{1mm}
\noindent
\textbf{Transactions:} Following the notations used in database multi-level transactions\cite{WeiVoss:TIS:2002:Morg}, we model a transaction as a two-level tree. The \emph{layer-0} consist of read/write events and \emph{layer-1} of the tree consists of \mth{s} invoked by a transaction.
%\begin{figure}[tbph]

Having informally explained a transaction, we formally define a transaction $T$ as the tuple $\langle \evts{T}, <_T\rangle$. Here $\evts{T}$ are all the read/write events at \emph{layer-0} of the transaction. $<_T$ is a total order among all the events of the transaction.
% $\inv(\tlook_1(ht, k_5))~ r_{11}(k_2, o_2) r_{11}(k_5, o_5)~ \rsp(\tlook(ht, k_5, o_5))~ \inv(\tdel_1(ht, k_7))~ r_{11}(k_2, o_2)~ r_{11}(k_5, o_5)~ r_{11}(k_7, o_7)~ w_{11}(k_5, v_i)~ w_{11}(k_7, v_j) \rsp(\tdel(ht, k_7, o_7))$. 

We denote the first and last events of a transaction $T_i$ as $\fevt{T_i}$ and $\levt{T_i}$. Given any other read/write event $rw$ in $T_i$, we assume that $\fevt{T_i} <_{T_i} rw <_{T_i} \levt{T_i}$. All the \mth{s} of $T_i$ are denoted as $\met{T_i}$. We assume that for any method $m$ in $\met{T_i}$, $\evts{m}$ is a subset of $\evts{T_i}$ and $<_m$ is a subset of $<_{T_i}$. We assume that if a transaction has invoked a \mth, then it does not invoke a new \mth{} until it gets the response of the previous one. Thus all the \mth{s} of a transaction can be ordered by $<_{T_i}$. Formally,  $(\forall m_{p}, m_{q} \in \met{T_i}: (m_{p} <_{T_i} m_{q}) \lor (m_{q} <_{T_i} m_{p}))\rangle$, here $m_{p}$ and $m_{q}$ are $p_{th}$ and $q_{th}$ methods of $T_i$ respectively. 

\noindent
\textbf{Histories:} A \emph{history} is a sequence of events belonging to different transactions. The collection of events is denoted as $\evts{H}$. Similar to a transaction, we denote a history $H$ as tuple $\langle \evts{H},<_H \rangle$ where all the events are totally ordered by $<_H$. The set of \mth{s} that are in $H$ is denoted by $\met{H}$. A \mth{} $m$ is \emph{incomplete} if $\inv(m)$ is in $\evts{H}$ but not its corresponding response event. Otherwise, $m$ is \emph{complete} in $H$. 

Coming to transactions in $H$, the set of transactions in $H$ are denoted as $\txns{H}$. The set of committed (resp., aborted) transactions in $H$ is denoted by $\comm{H}$ (resp., $\aborted{H}$). The set of \emph{live} transactions in $H$ are those which are neither committed nor aborted and denoted as $\live{H} =\txns{H}-\comm{H}-\aborted{H}$.  On the other hand, the set of \emph{terminated} transactions are those which have either committed or aborted and is denoted by $\term{H} = \comm{H} \cup \aborted{H}$.

The relation between the events of transactions \& histories is analogous to the relation between \mth{s} \& transactions. We assume that for any transaction $T$ in $\txns{H}$, $\evts{T}$ is a subset of $\evts{H}$ and $<_T$ is a subset of $<_{H}$. Formally, $\langle \forall T \in \txns{H}: (\evts{T} \subseteq \evts{H}) ~ \land (<_T \subseteq <_{H}) \rangle$. 

We denote two histories $H_1, H_2$ as \emph{equivalent} if their events are the same, i.e., $\evts{H_1} = \evts{H_2}$. A history $H$ is qualified to be \emph{well-formed} if: (1) all the \mth{s} of a transaction $T_i$ in $H$ are totally ordered, i.e. a transaction invokes a \mth{} only after it receives a response of the previous \mth{} invoked by it (2) $T_i$ does not invoke any other \mth{} after it received an $\mathcal{A}$ response or after $\tryc(ok)$ \mth. We only consider \emph{well-formed} histories for \opmvotm.

A \mth{} $m_{ij}$ ($j^{th}$ method of a transaction $T_i$) in a history $H$ is said to be \emph{isolated} or \emph{atomic} if for any other event $e_{pqr}$ ($r^{th}$ event of method $m_{pq}$) belonging to some other \mth{} $m_{pq}$ of transaction $T_p$ either $e_{pqr}$ occurs before $\inv(m_{ij})$ or after $\rsp(m_{ij})$. 

\vspace{1mm}
\noindent
\textbf{Sequential Histories:} A history $H$ is said to be \emph{sequential} (term used in \cite{KuznetsovPeri:Non-interference:TCS:2017, KuznetsovRavi:ConcurrencyTM:OPODIS:2011}) if all the methods in it are complete and isolated. From now onwards, most of our discussion would relate to sequential histories. 

Since in sequential histories all the \mth{s} are isolated, we treat each \mth as a whole without referring to its $inv$ and $rsp$ events. For a sequential history $H$, we construct the \emph{completion} of $H$, denoted $\overline{H}$, by inserting $\trya_k(\mathcal{A})$ immediately after the last \mth{} of every transaction $T_k \in \live{H}$. Since all the \mth{s} in a sequential history are complete, this definition only has to take care of completed transactions. 

Consider a sequential history $H$. Let $m_{ij}(ht, k, v/nil)$ be the first \mth of $T_i$ in $H$ operating on the key $k$ as $\fkmth{\langle ht, k \rangle}{T_i}{H}$, where $m_{ij}$ stands for $j^{th}$ method of $i^{th}$ transaction. For a \mth $m_{ix}(ht, k, v)$ which is not the first \mth on $\langle ht, k \rangle$ of $T_i$ in $H$, we denote its previous \mth on $k$ of $T_i$ as $m_{ij}(ht, k, v) = \pkmth{m_{ix}}{T_i}{H}$.

\vspace{1mm}
\noindent
\textbf{Real-time Order and Serial Histories:} Given a history $H$, $<_H$ orders all the events in $H$. For two complete \mth{s} $m_{ij}, m_{pq}$ in $\met{H}$, we denote $m_{ij} \prec_H^{\mr} m_{pq}$ if $\rsp(m_{ij}) <_H \inv(m_{pq})$. Here \mr{} stands for method real-time order. It must be noted that all the \mth{s} of the same transaction are ordered. Similarly, for two transactions $T_{i}, T_{p}$ in $\term{H}$, we denote $(T_{i} \prec_H^{\tr} T_{p})$ if $(\levt{T_{i}} <_H \fevt{T_{p}})$. Here \tr{} stands for transactional real-time order. 

\cmnt{
Thus, $\prec$ partially orders all the \mth{s} and transactions in $H$. It can be seen that if $H$ is sequential, then $\prec_H^{\mr}$ totally orders all the \mth{s} in $H$. Formally, $\langle (H \text{ is seqential}) \implies (\forall m_{ij}, m_{pq} \in \met{H}: (m_{ij} \prec_H^{\mr} m_{pq}) \lor (m_{pq} \prec_H^{\mr} m_{ij}))\rangle$. 
}

We define a history $H$ as \emph{serial} \cite{Papad:1979:JACM} or \emph{t-sequential} \cite{KuznetsovRavi:ConcurrencyTM:OPODIS:2011} if all the transactions in $H$ have terminated and can be totally ordered w.r.t $\prec_{\tr}$, i.e. all the transactions execute one after the other without any interleaving. Intuitively, a history $H$ is serial if all its transactions can be isolated. Formally, $\langle (H \text{ is serial}) \implies (\forall T_{i} \in \txns{H}: (T_i \in \term{H}) \land (\forall T_{i}, T_{p} \in \txns{H}: (T_{i} \prec_H^{\tr} T_{p}) \lor (T_{p} \prec_H^{\tr} T_{i}))\rangle$. Since all the methods within a transaction are ordered, a serial history is also sequential.% Refer \figref{serial} in \apnref{apndx1} to shows a serial history.

\ignore{
\vspace{1mm}
\noindent
\textbf{Real-time Order \& Serial Histories:}  Two \mth{s} $m_{ij}$ and $m_{pq}$ of history $H$ are in real-time order, if $\rsp(m_{ij}) <_H \inv(m_{pq})$. Similarly, two transactions $T_i$ and $T_j$ are in real-time order, if  $(\levt{T_{i}} <_H \fevt{T_{j}})$, where $\levt{T_{i}}$ and $\fevt{T_{j}}$ represents the last method of $T_i$ and first method of $T_j$ respectively. A history $H$ is said to be serial if all the transactions are atomic and totally ordered.

\vspace{1mm}
\noindent
\textbf{\textit{ Valid and Legal Histories:}} A history $H$ is said to valid if all the \rvmt{s} are lookup from previously committed 
}

%\noindent
%To simplify our analysis, we assume that there exists an initial transaction $T_0$ that invokes $\tdel$ \mth on all the keys of the \tab{} used by any transaction. 

\vspace{1mm}
\noindent
\textbf{Valid Histories:} A \rvmt{} (\tdel{} and \tlook{}) $rvm_{ij}$ on key $k$ is valid if it returns the value updated by any of the previously committed transaction that updated key $k$. A history $H$ is said to valid if all the \rvmt{s} of H are valid. 

\vspace{1mm}
\noindent
\textbf{Legal Histories:} %A \rvmt $m_{ij}$ on key $k$ is legal if it returns the value updated the latest committed transaction that updated key $k$. A history $H$ is said to be legal, if all the \rvmt{s} of H are legal. 
We define the \emph{\legality{}} of \rvmt{s} on sequential histories which we use to define correctness criterion as opacity \cite{GuerKap:Opacity:PPoPP:2008}. Consider a sequential history $H$ having a \rvmt{} $\rvm_{ij}(ht, k, v)$ (with $v \neq null$) as $j^{th}$ method belonging to transaction $T_i$. We define this \rvm \mth{} to be \emph{\legal} if: 
\vspace{-1mm}
\begin{enumerate}
	%\setlength\itemsep{-1em}
	%\vspace{-.2cm}
	\item[Rule 1] \label{step:leg-same} If the $\rvm_{ij}$ is not the first \mth of $T_i$ to operate on $\langle ht, k \rangle$ and $m_{ix}$ is the previous \mth of $T_i$ on $\langle ht, k \rangle$. Formally, $\rvm_{ij} \neq \fkmth{\langle ht, k \rangle}{T_i}{H}$ $\land (m_{ix}(ht, k, v') = \pkmth{\langle ht, k \rangle}{T_i}{H})$ (where $v'$ could be null). Then,
	\begin{enumerate}
		\setlength\itemsep{0em}
		%		\item if $m_{ix}(ht, k, v')$ is a \tins{} \mth i.e. $\tins_{ix}(ht, k, v')$ then $v = v'$. 
		%		\item if $m_{ix}(ht, k, v')$ is a \tlook{} \mth i.e. $\tlook_{ix}(ht, k, v')$ then $v = v'$. 
		%		\item if $m_{ix}(ht, k, v')$ is a \tdel{} \mth i.e. $\tdel_{ix}(ht, k, v'/NULL)$ then $v = NULL$. 
		\item If $m_{ix}(ht, k, v')$ is a \tins{} \mth then $v = v'$. 
		\item If $m_{ix}(ht, k, v')$ is a \tlook{} \mth then $v = v'$. 
		\item If $m_{ix}(ht, k, v')$ is a \tdel{} \mth then $v = null$.
	\end{enumerate}
	
	In this case, we denote $m_{ix}$ as the last update \mth{} of $\rvm_{ij}$, i.e., 
	
	 $m_{ix}(ht, k, v') = \lupdt{\rvm_{ij}(ht, k, v)}{H}$. 
	
	\item[Rule 2] \label{step:leg-ins} If $\rvm_{ij}$ is the first \mth{} of $T_i$ to operate on $\langle ht, k \rangle$ and $v$ is not null. Formally, $\rvm_{ij}(ht, k, v) = \fkmth{\langle ht, k \rangle}{T_i}{H} \land (v \neq null)$. Then,
	\begin{enumerate}
		\setlength\itemsep{0em}
		\item There is a \tins{} \mth{} $\tins_{pq}(ht, k, v)$ in $\met{H}$ such that $T_p$ committed before $\rvm_{ij}$. Formally, $\langle \exists \tins_{pq}(ht, k, v) \in \met{H} : \tryc_p \prec_{H}^{\mr} \rvm_{ij} \rangle$. 
		\item There is no other update \mth{} $up_{xy}$ of a transaction $T_x$ operating on $\langle ht, k \rangle$ in $\met{H}$ such that $T_x$ committed after $T_p$ but before $\rvm_{ij}$. Formally, $\langle \nexists up_{xy}(ht, k, v'') \in \met{H} : \tryc_p \prec_{H}^{\mr} \tryc_x \prec_{H}^{\mr} \rvm_{ij} \rangle$. 		
	\end{enumerate}
	
	In this case, we denote $\tryc_{p}$ as the last update \mth{} of $\rvm_{ij}$, i.e.,  $\tryc_{p}(ht, k, v)$= $\lupdt{\rvm_{ij}(ht, k, v)}{H}$.
	
	\item[Rule 3] \label{step:leg-del} If $\rvm_{ij}$ is the first \mth of $T_i$ to operate on $\langle ht, k \rangle$ and $v$ is null. Formally, $\rvm_{ij}(ht, k, v) = \fkmth{\langle ht, k \rangle}{T_i}{H} \land (v = null)$. Then,
	\begin{enumerate}
		\setlength\itemsep{0em}
		\item There is \tdel{} \mth{} $\tdel_{pq}(ht, k, v')$ in $\met{H}$ such that $T_p$ committed before $\rvm_{ij}$. Formally, $\langle \exists \tdel_{pq}\\(ht, k,$ $ v') \in \met{H} : \tryc_p \prec_{H}^{\mr} \rvm_{ij} \rangle$. Here $v'$ could be null. 
		\item There is no other update \mth{} $up_{xy}$ of a transaction $T_x$ operating on $\langle ht, k \rangle$ in $\met{H}$ such that $T_x$ committed after $T_p$ but before $\rvm_{ij}$. Formally, $\langle \nexists up_{xy}(ht, k, v'') \in \met{H} : \tryc_p \prec_{H}^{\mr} \tryc_x \prec_{H}^{\mr} \rvm_{ij} \rangle$. 		
	\end{enumerate}
	In this case, we denote $\tryc_{p}$ as the last update \mth{} of $\rvm_{ij}$, i.e., $\tryc_{p}(ht, k, v)$ $= \lupdt{\rvm_{ij}(ht, k, v)}{H}$. 
\end{enumerate}
%\vspace{-.3cm}
We assume that when a transaction $T_i$ operates on key $k$ of a \tab{} $ht$, the result of this \mth is stored in \emph{local logs} of $T_i$, $\llog_i$ for later \mth{s} to reuse. Thus, only the first \rvmt{} operating on $\langle ht, k \rangle$ of $T_i$ accesses the shared memory. The other \rvmt{s} of $T_i$ operating on $\langle ht, k \rangle$ do not access the shared memory and they see the effect of the previous \mth{} from the \emph{local logs}, $\llog_i$. This idea is utilized in Rule 1. With reference to Rule 2 and Rule 3, it is possible that $T_x$ could have aborted before $\rvm_{ij}$. %For LR3, since we are assuming that transaction $T_0$ has invoked a \tdel{} \mth{} on all the keys used of the \tab{} objects, there exists at least one \tdel{} \mth{} for every \rvmt on $k$ of $ht$. 


%This we also call \emph{conflict inheritance} as the conflict of the later \mth{} of $T_i$ operating on $\langle ht, k \rangle$ can be found using the conflicts of the first \mth{} of $T_i$.

Coming to \tins{} \mth{s}, since a \tins{} \mth{} always returns $ok$ as they overwrite the node if already present therefore they always take effect on the $ht$. Thus, we denote all \tins{} \mth{s} as \legal{} and only give legality definition for \rvmt{}. We denote a sequential history $H$ as \emph{\legal} or \emph{linearized} if all its \rvm \mth{s} are \legal. We formally prove the legality of the proposed \emph{\opmvotm{s}} in \secref{cmvostm}. 

%If $T_j$ invokes \rvmt on key $k_1$ from $T_i$ in $H$, note that in order to this to happen, $T_i$ must have closest committed before $T_j$ i.e. $c_i <_H \rvm_j(k_{1, i})$. %If $T_i$ is having \upmt{} as insert on the same key $k_1$ then $i_i(k_{1, i}, v_{i1}) <_H c_i <_H \rvm_j(k_{1, i}, v_{i1})$. If $T_i$ is having \upmt{} as delete on the same key $k_1$ then $d_i(k_{1, i}, nil_{i1}) <_H c_i <_H \rvm_j(k_{1, i}, nil_{i1})$. Such $\rvm_j$ is considered as legal.

\vspace{1mm}
\noindent
\textbf{Opacity:} It is a \emph{\ccs} for STMs \cite{GuerKap:Opacity:PPoPP:2008}. A sequential history $H$ is said to be \opq{} if there exists a serial history $S$ such that: (1) $S$ is equivalent to $\overline{H}$, i.e., $\evts{\overline{H}} = \evts{S}$ (2) $S$ is \legal{} and (3) $S$ respects the transactional real-time order of $H$, i.e., $\prec_H^{\tr} \subseteq \prec_S^{\tr}$. 

Finally, we show that history generated by \emph{\opmvotm{s}} satisfy correctness criteria as \opq{}.

%\noindent
%\textbf{MV-permissiveness:} It is a progress condition for STMs by Perelman et al.\cite{perel+:2010:MultVer:PODC} which ensures read-only transactions will never return abort while maintaining multi-versions corresponding to each key.

%A valid sequential history $H$ is said to be \opq{} if there exists a serial history $S$ such that: (1) $S$ is equivalent to $\overline{H}$, i.e. , $\evts{\overline{H}} = \evts{S}$ (2) $S$ is \legal{} and (3) $S$ respects the transactional real-time order of $H$, i.e., $\prec_H^{\tr} \subseteq \prec_S^{\tr}$. 


==> citations <==
%%% ====================================================================
%%%  BibTeX-file{
%%%     author          = "Sathya Peri",
%%%     date            = "17 Spet 2009",
%%%     filename        = "citations.bib",
%%%     url             = ""
%%%     www-home        = "http://www.cs.mun.ca/~sathya/",
%%%     address         = "Department of Computer Science,
%%%                        MUN,
%%%                        St John's, CA A1B 3X5,
%%%                        Canada",
%%%     email           = "sathya at mun.ca",
%%%     dates           = {1950--},
%%%     keywords        = "",
%%%     supported       = "yes",
%%%     supported-by    = "Sathya Peri",
%%%     abstract        = "Bibliography for Sathya Peri"
%%%  }
%%% ====================================================================


@String{PROC = {Proceedings of the}}
@String{AMS = {American Mathematical Society}}
@String{AW = {Addison-Wesley}}
@String{TCS = {Theoretical Computer Science}}
@String{JPDC = {Journal of Parallel and Distributed Computing (JPDC)}}
@String{WDAG = {Workshop on Distributed Algorithms (WDAG)}}
@String{WPDD = {ACM/ONR Workshop on Parallel and Distributed Debugging}}
@String{DC = {Distributed Computing (DC)}}
@String{TrCS = {ACM Transactions on Computer Systems}}
@String{SPDP = {IEEE Symposium on Parallel and Distributed Processing (SPDP)}}
@String{ICPP = {International Conference on Parallel Processing}}
@String{Com = {IEEE Computer}}
@String{KAP = {Kluwer Academic Publishers}}
@String{WAD = {International Workshop on Automated Debugging (AADEBUG)}}
@String{CSS = {International Conference on System Sciences}}
@String{Fre = {W. H. Freeman and Company, New York}}
@String{TPDS = {IEEE Transactions on Parallel and Distributed Systems (TPDS)}}
@String{FTCS = {IEEE Fault-Tolerant Computing Symposium (FTCS)}}
@String{JCC = {Journal of Computer Communications}}
@String{WSCT = {International Workshop on Structures in Concurrency Theory (STRICT)}}
@String{MH = {McGraw-Hill}}
@String{CACM = {Communications of the ACM (CACM)}}
@String{ICDCS = {IEEE International Conference on Distributed Computing Systems (ICDCS)}}
@String{PODC = {ACM Symposium on Principles of Distributed Computing (PODC)}}
@String{JS = {Journal of Supercomputing}}
@String{CAV = {International Conference on Computer-Aided Verification (CAV)}}
@String{LNCS = {Lecture Notes in Computer Science (LNCS)}}
@String{WPDS = {Workshop on Parallel and Distributed Simulation}}
@String{DISC = {Symposium on Distributed Computing (DISC)}}
@String{CSE = {Computer Science and Education}}
@String{TMH = {Tata McGraw-Hill Publishing Company Limited}}
@String{ES = {Elsevier Science Publishers B. V. (North-Holland)}}
@String{PDS = {The Parallel and Distributed Systems Laboratory}}
@String{DECE = {Department of Electrical and Computer Engineering}}
@String{DCS = {Department of Computer Science}}
@String{PPL = {Parallel Programming Laboratory}}
@String{UIUC = {University of Illinois at Urbana-Champaign}}
@String{UTA = {The University of Texas at Austin}}
@String{OSU = {The Ohio State University}}
@String{UTD = {The University of Texas at Dallas}}
@String{TC = {IEEE Transactions on Computers}}
@String{IPL = {Information Processing Letters (IPL)}}
@String{AMCSJ = {Applied Mathematics and Computer Science Journal}}
@String{WLCPC = {Workshop on Language and Compilers for Parallel Computing}}
@String{IBMARC = {IBM Almaden Research Center}}
@String{IBMZ = {IBM Research Laboratory, Zurich}}
@String{ICDE = {International Conference on Data Engineering (ICDE)}}
@String{CUP = {Cambridge University Press}}
@String{MVPP = {International Meeting on Vector and Parallel Processing}}
@String{TOPLAS = {ACM Transactions on Programming Languages and Systems (TOPLAS)}}
@String{SPDT = {Symposium on Parallel and Distributed Tools}}
@String{CJ = {The Computer Journal}}
@String{PH = {Prentice Hall}}
@String{MK = {Morgan Kaufmann}}
@String{SIGMOD = {ACM SIGMOD International Conference on Managament of Data}}
@String{SIGACT = {ACM Special Interest Group on Algorithms and Computation Theory (SIGACT)}}
@String{USPATENT = {United States Patent Number}}
@String{INFORMIX = {Informix Software Incorporated}}
@String{SV = {Springer-Verlag}}
@String{PDCS = {ISCA International Conference on Parallel and Distributed Computing Systems (PDCS)}}
@String{MIT = {The MIT Press}}
@String{JHUP = {The Johns Hopkins University Press}}
@String{DAM = {Discrete Applied Mathematics}}
@String{DM = {Discrete Mathematics}}
@String{DS = {Distributed Systems}}
@String{ICSKE = {IEEE International Conference on Software and Knowledge Engineering}}
@String{FSTTCS = {Conference on the Foundations of Software Technology and Theoretical
                  Computer Science (FSTTCS)}}
@String{TSE = {IEEE Transactions on Software Engineering}}
@String{JSS = {The Journal of Systems and Software}}
@String{WGCS = {International Workshop on Graph-Theoretic Concepts in Computer Science (WG)}}
@String{JWS = {John Wiley and Sons Limited}}
@String{JWSUS = {John Wiley and Sons, Incorporated}}
@String{ORDAL = {International Conference on Orders, Algorithms and Applications (ORDAL)}}
@String{AJM = {American Journal of Mathematics}}
@String{SRKU = {Sci. Reports Kanazawa Univ.}}
@String{SIAMJDM = {SIAM Journal on Discrete Mathematics}}
@String{KRUSE = {International KRUSE Symposium: Knowledge Use, Retrieval and Storage for Efficiency}}
@String{SIAMJADM = {SIAM Journal on Algebraic and Discrete Methods}}
@String{SIAMJC = {SIAM Journal on Computing}}
@String{MCT = {Mathematical Center Tracts}}
@String{STOC = {Annual ACM Symposium on Theory of Computing (STOC)}}
@String{OOPSLA = {Conference on Object-Oriented Programming, Systems, Languages, and Applications (OOPSLA)}}
@String{JLMS = {Journal London Mathematics Society}}
@String{AM = {Annals of Mathematics}}
@String{TIT = {IEEE Transactions on Information Theory}}
@String{TR = {IEEE Transactions on Reliability}}
@String{WLP = {Workshop on Logics of Programs}}
@String{ISP = {International Symposium in Programming}}
@String{WSS = {Workshop on Self-Stabilizing Systems (WSS)}}
@String{ICALP = {International Colloquium on Automata, Languages and Systems (ICALP)}}
@String{JA = {Journal of Algorithms}}
@String{KDE = {IEEE Transactions on Knowledge and Data Engineering}}
@String{CS = {ACM Computing Surveys (CSUR)}}
@String{IPDPS = {International Parallel and Distributed Processing Symposium (IPDPS)}}
@String{PDC = {Parallel and Distributed Conference}}
@String{SP = {IEEE Symposium on Security and Privacy}}
@String{USS = {USENIX Security Symposium}}
@String{WNTS = {USENIX Windows NT Symposium}}
@String{UCS = {Computing Systems}}
@String{NCSC = {National Computer Security Conference}}
@String{RV = {Workshop on Runtime Verification (RV)}}
@String{ICPDCS = {IASTED International Conference on Parallel and Distributed Computing and Systems}}
@String{MCDS = {SCS MultiConference on Distributed Simulation}}
@String{SCS = {Society for Computer Simulation}}
@String{BCPC = {The Benjamin Cummings Publishing Company, Incorporated}}
@String{OPODIS = {International Conference on Principles of Distributed Systems (OPODIS)}}
@String{TWSIS = {Texas Workshop on Security of Information Systems (TWSIS)}}
@String{SCISS = {South Central Information Security Symposium (SCISS)}}
@String{CSS = {Computing Systems}}
@String{UCD = {University of California, Davis}}
@String{CSAC = {Annual Computer Security Applications Conference}}
@String{WETICE = {IEEE Workshop on Enabling Technologies: Infrastructure for Collaborative
                  Enterprises (WETICE)}}
@String{TOG = {ACM Transactions on Graphics}}
@String{SCCS = {School of Computer and Communication Sciences}}
@String{EPFL = {{\'E}cole Polytechnique F{\'e}d{\'e}rale de Laussane (EPFL)}}
@String{CORNELL = {Cornell University}}
@String{COMPSAC = {Annual Internation Computer Software and Applications Conference (COMPSAC)}}
@String{JPL = {Journal of Programming Languages}}
@String{PC = {Parallel Computing}}
@String{UWM = {University of Wisconsin, Madison}}
@String{UWTC = {USENIX Winter Technical Conference}}
@String{ICSSE = {Israeli Conference on Computer Systems and Software Engineering}}
@String{IPPS = {International Parallel and Processing Symposium (IPPS)}}
@String{HIS = {Journal of High Integrity Systems}}
@String{HPL = {Hewlett Packard Laboratories}}
@String{ACTA = {Acta Informatica}}
@String{FOCS = {Annual Symposium on Foundations of Computer Science (FOCS)}}
@String{CDS = {IEEE Proceedings---Computers and Digital Techniques}}
@String{JISE = {Journal of Information Science and Engineering}}
@String{ICPADS = {International Conference on Parallel and Distributed Systems (ICPADS)}}
@String{WPPS = {International Workshop on Peer-to-Peer Systems}}
@String{SAC = {IEEE Journal on Selected Areas in Communications}}
@String{TN = {IEEE/ACM Transactions on Networking}}
@String{SNA = {ACM-SIAM Symposium on Discrete Algorithms}}
@String{SIU = {Studia Informatica Universalis}}


@Unpublished{8LGM:1992,
  author =   {8LGM},
  title =    {{[8lgm]-Advisory-5.UNIX.mail.24-Jan-1992}},
  note =     {Available from \texttt{fileserv@bagpuss.demon.co.uk} (January 1992)}
}

@Article{AchBad:1992:IPL,
  author =   {A. Acharya and B. R. Badrinath},
  title =    {{Recording Distributed Snapshots Based on Causal
                   Order of Message Delivery}},
  journal =  IPL,
  volume =   {44},
  number =   {6},
  pages =    {317-321},
  year =     {1992},
  OPTurl =   {http://citeseer.nj.nec.com/acharya92recording.html}
}

@Misc{Adv:1990:SM,
  title =    {{Sendmail Vulnerability}},
  howpublished = {CERT Advisory CA-90:01 available from \textsf{cert.org} via anonymous ftp},
  month =    JAN,
  year =     {1990}
}

@Article{Adv:1992:Mail,
  author =   {8LGM},
  title =    {{[8lgm]-Advisory-5.UNIX.mail.24-Jan-1992}},
  note =     {Available from \texttt{fileserv@bagpuss.demon.co.uk}},
  month =    JAN,
  year =     1992
}

@Article{Adv:1994:Pwd,
  author =   {8LGM},
  title =    {{[8lgm]-Advisory-7.UNIX.passwd.11-May-1994}},
  note =     {Available from \texttt{fileserv@bagpuss.demon.co.uk}},
  month =    MAY,
  year =     1994
}

@Article{AfeBre:1998:TCS,
  author =   {Y. Afek and A. Bremler},
  title =    {{Self-Stabilizing Unidirectional Network Algorithms by Power Supply}},
  journal =      TCS,
  year =     1998,
  volume =   1998,
  number =   3,
  month =    DEC
}

@InProceedings{AfeKut+:1991:WDAG,
  author =       {Y. Afek and S. Kutten and M. Yung},
  title =        {{Memory-Efficient Self-Stabilizing Protocols for General Networks}},
  booktitle =    PROC # " 4th " # WDAG,
  year =         {1991},
  pages =        {15-28},
  address =      {Bari, Italy},
  publisher =    SV,
}

@Manual{AgaGoe+:1996:IBM,
  author =   {A. Agarwal and A. Goel and A. Sood},
  title =    {{Software Design Description for DLFS on Solaris,
                  HP-UX, and AIX}},
  year =     {1996}
}

@InProceedings{AgrBor+:1989:MD,
  author =   {R. Agrawal and A. Borgida and H. V. Jagadish},
  title =    {{Efficient Management of Transitive Relationships in
                  Large Data and Knowledge Bases}},
  booktitle =    PROC # " " # SIGMOD,
  pages =    {253-262},
  year =     1989,
  address =  {Portland, Oregon}
}

@Book{AhoHop:1974:AW,
  author =   {A. V. Aho and J. E. Hopcroft and J. D. Ullman},
  OPTeditor =    {~},
  title =    {{The Design and Analysis of Computer Algorithms}},
  publisher =    AW,
  year =     1974,
  OPTnote =  {pages 384-386}
}

@InProceedings{AlaVen:1993:WAD,
  author =   {S. Alagar and S. Venkatesan},
  title =    {{Hierarchy in Testing Distributed Programs}},
  booktitle =    PROC # " " # WAD,
  pages =    {101-116},
  year =     {1993}
}

@Article{AlaVen:1994:IPL,
  author =   {S. Alagar and S. Venkatesan},
  title =    {{An Optimal Algorithm for Recording Snapshots using Casual
                   Message Delivery}},
  journal =  IPL,
  year =     {1994},
  OPTkey =   {},
  volume =   {50},
  OPTnumber =    {},
  pages =    {311-316},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@InProceedings{AlaVen:1994:PDS,
  author =   {S. Alagar and S. Venkatesan},
  title =    {{Techniques to Tackle State Explosion in Global Predicate Detection}},
  booktitle =    PROC # " " # PDS,
  pages =    {412-417},
  month =    DEC,
  year =     {1994}
}

@Article{AlaVen:2001:TSE,
  author =   {S. Alagar and S. Venkatesan},
  title =    {{Techniques to Tackle State Explosion in Global Predicate Detection}},
  journal =  TSE,
  year =     2001,
  volume =   27,
  number =   8,
  pages =    {704-714},
  month =    AUG
}

@TechReport{AlaVid:1999:TR,
  author =   {K. Alagarsamy and K.Vidyasankar},
  title =    {{Elegant Solutions for Group Mutual Exclusion Problem}},
  institution =  {Department of Computer Science, Memorial University of Newfoundland,
                  St.John's, Newfoundland, Canada},
  year =     {1999},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{AlmBaq+:2002:ICDCS,
  author =   {P. S. Almeida and C. Baquero and V. Fonte},
  title =    {{Version Stamps---Decentralized Version Vectors}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 22nd " # ICDCS,
  pages =    {544-551},
  year =     {2002},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{AlvEln+:1999:FTCS,
  author =   {L. Alvisi and E. N. Elnozahy and S. Rao and
                  S. A. Hussain and A. D. Mel},
  title =    {{An Analysis of Communication-Induced Checkpointing}},
  booktitle =    PROC # " 29th " # FTCS,
  pages =    {242-249},
  year =     1999,
  address =  {Madison, Wisconsin},
  month =    JUN
}

@InProceedings{AlvMar:1995:ICDCS,
  author =   {L. Alvisi and K. Marzullo},
  title =    {{Message Logging: Pessimistic, Optimistic, and Causal}},
  booktitle =    PROC # " 15th " # ICDCS,
  pages =    {229-236},
  year =     1995,
  address =  {Vancouver, Canada},
  month =    JUN
}

@MastersThesis{Ang:2001:Thesis,
  author =   {R. Anguiano},
  title =    {{A Static Analysis Technique for the Detection of
                   TOCTTOU Vulnerabilities}},
  school =   {University of California, Davis},
  year =     {2001},
  OPTkey =   {},
  OPTtype =  {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@Article{AroGou:1994:TC,
  author =   {A. Arora and M. G. Gouda},
  title =    {{Distributed Reset}},
  journal =      TC,
  year =     1994,
  volume =   43,
  number =   9,
  pages =    {1026-1038}
}

@Article{AroSin:1995:HIS,
  author =   {A. Arora and A. Singhai},
  title =    {{Fault-Tolerant Reconfiguration of Trees and Rings in Distributed Systems}},
  journal =      HIS,
  year =     1995,
  volume =   1,
  number =   4,
  pages =    {375-384}
}

@InProceedings{AtrMit+:2003:OPODIS,
  author =   {R. Atreya and N. Mittal and V. K. Garg},
  title =    {{Detecting Locally Stable Predicates without
                   Modifying Application Messages}},
  booktitle =    PROC # " 7th " # OPODIS,
  year =     2003,
  pages =        {20-33},
  address =  {La Martinique, France},
  month =    DEC
}

@Article{BabFro+:1996:JSS,
  author =   {{\"O}. Babao{\v{g}}lu and E. Fromentin and
                  M. Raynal},
  title =    {{A Unified Framework for the Specification and Run-time Detection
                   of Dynamic Properties in Distributed Computations}},
  journal =  JSS,
  volume =   {33},
  number =   {3},
  month =    JUN,
  pages =    {287-298},
  year =     {1996},
  url =      {http://citeseer.nj.nec.com/10396.html}
}

@incollection{BabMar:1993:DS,
  author =   {{\"{O}}. Babao{\v g}lu and K. Marzullo},
  title =    {{Consistent Global States of Distributed Systems: Fundamental Concepts and
                   Mechanisms}},
  booktitle =    DS,
  publisher =    AW,
  editor =   {S. Mullender},
  pages =    {55-96},
  year =     {1993},
  url =
                  {http://citeseer.nj.nec.com/babaoglu93consistent.html}
}

@Article{BabRay:1995:JPDC,
  author =   {{\"{O}}. Babao{\v g}lu and M. Raynal},
  title =    {{Specification and Verification of Dynamic Properties in Distributed Computations}},
  journal =  JPDC,
  year =     1995,
  volume =   28,
  number =   2,
  pages =    {173-185}
}

@Book{Bac:1987:Book,
  author =   {M. J Bach},
  title =    {{The Design of the Unix Operating System}},
  publisher =    PH,
  year =     1987,
  isbn =     0132017997
}

@Book{Bac:1987:PH,
  author =   {M. J. Bach},
  title =    {{The Design of the Unix Operating System}},
  publisher =    PH,
  year =     1987
}

@Manual{BalKan:1999:INFORMIX,
  author =   {I. Balabine and R. Kandasamy},
  title =    {{File System Interface to a Database}},
  note =     USPATENT # " 5937406 granted to " # INFORMIX,
  year =     {1999},
  month =    AUG
}

@InProceedings{BarBra+:1996:ICSSE,
  author =   {A. Barak and A. Braverman and A. Gilderman and O. La'adan},
  title =    {{Performance of PVM with MOSIX Preemptive Process Migration}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 7th " # ICSSE,
  pages =    {38-45},
  year =     {1996},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Herzliya},
  month =    JUN,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{BeaCan+:2003:JISE,
  author =   {J. Beauquier and S. Cantarell and A. K. Datta and F. Petit},
  title =    {{Group Mutual Exclusion in Tree Networks}},
  journal =      JISE,
  year =     {2003},
  OPTkey =   {},
  volume =   {19},
  number =   {3},
  pages =    {415-432},
  month =    MAY,
  OPTnote =      {},
  OPTannote =    {}
}

@Manual{BegDon+:PVM2.0,
  title =    {{H}ence: {A} users' guide - version 2.0. {PVM}
                  {D}esign and {V}isualization},
  author =   {A. Beguelin and J. Dongarra and G. A. Geist and
                  R. Manchek and K. Moore and P. Newton and
                  V. Sunderam}
}

@InProceedings{Bel:1990:MCDS,
  author =   {S. Bellenot},
  title =    {{Global Virtual Time Algorithms}},
  booktitle =    PROC # " " # MCDS,
  pages =    {122-127},
  year =     1990,
  volume =   22,
  number =   1,
  month =    JAN,
  organization = SCS
}

@TechReport{Bis:1995:TR:8,
  author =   {M. Bishop},
  title =    {{Race Conditions, Files, and Security Flaws: or, The
                   Tortoise and the Hare \emph{Redux}}},
  institution =  DCS # ", " # UCD,
  year =     {1995},
  OPTkey =   {},
  OPTtype =  {},
  number =   {95-8},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@Article{BisDil:1996:CSS,
  author =   {M. Bishop and M. Dilger},
  title =    {{Checking for Race Conditions in File Accesses}},
  journal =  CSS,
  year =     2003,
  volume =   9,
  number =   2,
  pages =    {131-152}
}

@Article{BisDil:1996:UCS,
  author =   {M. Bishop and M. Dilger},
  title =    {{Checking for Race Conditions in File
                  Accesses}},
  journal =  UCS,
  year =     1996,
  volume =   9,
  number =   2,
  pages =    {131-152}
}

@Unpublished{BisHol:1978:PR:13,
  author =   {R. Bisbey and D. Hollingsworth},
  title =    {{Protection Analysis Project Final Report}},
  note =     {ISI/RR-78-13, DTIC AD A056816, USC/Information
                  Sciences Institute},
  OPTkey =   {},
  month =    MAY,
  year =     {1978},
  OPTannote =    {}
}

@Article{Bou:1987:TCS,
  author =   {L. Bouge},
  title =    {{Repeated Snapshots in Distributed Systems
                  with Synchronous Communication and their
                  Implementation in CSP}},
  journal =  TCS,
  year =     1987,
  volume =   49,
  pages =    {145-169}
}

@Article{Bre:1966:TIT,
  author =   {M. Breuer},
  title =    {{Coding Vertexes of a Graph}},
  journal =  TIT,
  year =     1966,
  volume =   12,
  pages =    {148-153}
}

@TechReport{BriLit+:1992:CONDOR,
  author =   {A. Bricker and M. Litzkow and M. Livny},
  title =    {{Condor Technical Summary, Version 4.1b}},
  institution =  "Computer Science Department, " # UWM,
  year =     {1992},
  OPTkey =   {},
  OPTtype =      {},
  number =   {CS-TR-92-1069},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{BrzHel+:1993:ICDCS,
  author =   {J. Brzezinski and J.-M. H{\'e}lary and M. Raynal},
  title =    {{Termination Detection in a Very General Distributed
                   Computing Model}},
  booktitle =    PROC # " " # ICDCS,
  pages =    {374-381},
  year =     1993
}

@article{BrzHel+:1995:JPDC,
  author =   {J. Brzezinski and J.-M. H{\'e}lary and M. Raynal and
                  M. Singhal},
  title =    {{Deadlock Models and a General Algorithm for
                   Distributed Deadlock Detection}},
  journal =  JPDC,
  volume =   {31},
  number =   {2},
  pages =    {112-125},
  year =     "1995"
}

@Misc{Bug:2002:RDR,
  title =    {{Recursive Directory Removal Race Condition}},
  howpublished = {http://mail.gnu.org/pipermail/bug-fileutils/2002-March/002433.html},
  month =    MAR,
  year =     2002
}

@Manual{CORBA:1997,
  author =   {Object Management Group},
  title =    {{The Common Object Request Broker: Architecture and Specification}}
}

@InProceedings{CanDat+:2001:ICDCS,
  author =   {S. Cantarell and A. K. Datta and F. Petit and V. Villain},
  title =    {{Token Based Group Mutual Exclusion for Asynchronous Rings}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICDCS,
  pages =    {691-694},
  year =     {2001},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{Cap:1994:ORDAL,
  author =   {C. Capelle},
  title =    {{Representation of an Order as Union of Interval Orders}},
  booktitle =    PROC # " " # ORDAL,
  pages =    {143-161},
  year =     1994,
  number =   831,
  series =   LNCS,
  address =  {Lyon, France},
  month =    JUL,
  publisher =    SV
}

@InProceedings{Cas:1993:OOPSLA,
  author =   {Y. Caseau},
  title =    {{Efficient Handling of Multiple Inheritance Hierarchies}},
  booktitle =    PROC # " " # OOPSLA,
  pages =    {271-287},
  year =     1993
}

@Article{Cas:1995:CSS,
  author =   {J. Casas and R. Konuru and S. W. Otto and R. M. Prouty and J. Walpole},
  title =    {{MPVM---A Migration Transparent Version of PVM}},
  journal =      CSS,
  year =     {1995},
  OPTkey =   {},
  volume =   {8},
  number =   {2},
  pages =    {171-216},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ChaDel+:1995:TOPLAS,
  author =   {B. Charron-Bost and C. Delporte-Gallet and
                  H. Fauconnier},
  title =    {{Local and Temporal Predicates in Distributed Systems}},
  journal =  TOPLAS,
  year =     1995,
  volume =   17,
  number =   1,
  pages =    {157-179}
}

@InProceedings{ChaGar:1995:WDAG,
  author =   {C. Chase and V. K. Garg},
  title =    {{On Techniques and their Limitations for the Global Predicate
                   Detection Problem}},
  booktitle =    PROC # " " # WDAG,
  year =     1995,
  address =  {France},
  month =    SEP,
  pages =    {303-317}
}

@Article{ChaGar:1998:DC,
  author =   {C. Chase and V. K. Garg},
  title =    {{Detection of Global Predicates: Techniques and their Limitations}},
  journal =  DC,
  year =     1998,
  volume =   11,
  number =   4,
  pages =    {191-201}
}

@Article{ChaLam:1985:TrCS,
  author =   {K. M. Chandy and L. Lamport},
  title =    {{Distributed Snapshots: Determining Global States of Distributed Systems}},
  journal =  TrCS,
  year =     1985,
  volume =   3,
  number =   1,
  pages =    {63-75},
  month =    FEB
}

@Article{ChaMis+:1983:TrCS,
  author =   {K. M. Chandy and J. Misra and L. M. Haas},
  title =    {{Distributed Deadlock Detection}},
  journal =      TrCS,
  year =     1983,
  volume =   1,
  number =   2,
  pages =    {144-156},
  month =    MAY
}

@Article{ChaMis:1984:TOPLAS,
  author =   {K. M. Chandy and J. Misra},
  title =    {{The Drinking Philosophers Problem}},
  journal =      TOPLAS,
  year =     {1984},
  OPTkey =   {},
  volume =   {6},
  number =   {4},
  pages =    {632-646},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ChaMis:1986:DC,
  author =   {K. M. Chandy and J. Misra},
  title =    {{How Processes Learn}},
  journal =  DC,
  year =     {1986},
  OPTkey =   {},
  volume =   {1},
  number =   {1},
  pages =    {40-52},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@Book{ChaMis:1988:Book,
  author =   {K. M. Chandy and J. Misra},
  title =    {{Parallel Program Design: A Foundation}},
  publisher =    AW,
  year =     1988
}

@Article{ChaTou:1996:JACM,
  author =   {T. D. Chandra and S. Toueg},
  title =    {{Unreliable Failure Detectors for Reliable Distributed Systems}},
  journal =  JACM,
  year =     {1996},
  volume =   {43},
  number =   {2},
  pages =    {225-267}
}

@Article{ChaVen:1990:JPDC,
  author =   {S. Chandrasekaran and S. Venkatesan},
  title =    {{A Message-Optimal Algorithm for Distributed
                  Termination Detection}},
  journal =  JPDC,
  year =     {1990},
  OPTkey =   {},
  volume =   {8},
  number =   {3},
  pages =    {245-252},
  month =    MAR,
  OPTnote =  {},
  OPTannote =    {}
}

@Article{Charron-Bost:size,
  author =   {B. Charron-Bost},
  title =    {{Concerning the Size of Logical Clocks in Distributed Systems}},
  journal =  IPL,
  year =     1991,
  month =    JUL,
  volume =   {39},
  pages =    {11-16},
}

@InProceedings{Che:1993:WAD,
  author =   {J. Cheng},
  title =    {{Slicing Concurrent Programs---A Graph-Theoretical Approach}},
  booktitle =    PROC # " " # WAD,
  pages =    {223-240},
  year =     1993
}

@Article{ChoMil+:1991:TOPLAS,
  author =   {J. Choi and B. P. Miller and R. Netzer},
  title =    {{Techniques for Debugging Parallel Programs with Flowback Analysis}},
  journal =  TOPLAS,
  year =     1991,
  volume =   13,
  number =   4,
  pages =    {491-530},
  month =    OCT
}

@InProceedings{ClaEme:1981:WLP,
  author =   {E. M. Clarke and E. A. Emerson},
  title =    {{Design and Synthesis of Synchronization Skeletons using
                   Branching Time Temporal Logic}},
  booktitle =    PROC # " " # WLP,
  address =  {Yorktown Heights, New York},
  month =    MAY,
  series =   LNCS,
  volume =   131,
  year =     1981
}

@InProceedings{CohLeh:1982:PODC,
  author =   {S. Cohen and D. Lehmann},
  title =    {{Dynamic Systems and their Distributed Termination}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 1st " # PODC,
  pages =    {29-33},
  year =     {1982},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Ottawa},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ColDol:1994:IPL,
  author =   {Z. Collin and S. Dolev},
  title =    {{Self-Stabilizing Depth-First Search}},
  journal =      IPL,
  year =     1994,
  volume =   49,
  number =   6,
  pages =    {297-301}
}

@InProceedings{CooMar:1991:WPDD,
  author =   {R. Cooper and K. Marzullo},
  title =    {{Consistent Detection of Global Predicates}},
  booktitle =    PROC # " " # WPDD,
  pages =    {163-173},
  year =     1991,
  address =  {Santa Cruz, California}
}

@Book{CorLei+:1991:MIT,
  author =   {T. H. Cormen and C. E. Leiserson and R. L. Rivest},
  title =    {{Introduction to Algorithms}},
  publisher =    MIT,
  address =  {Cambridge, Massachusetts},
  year =     {1991},
}

@InProceedings{CowBea+:2001:USS,
  author =   {C. Cowan and S. Beattie and C. Wright and
                  G. Korah-Hartman},
  title =    {{RaceGuard: Kernel Protection from Temporary File
                   Race Vulnerabilities}},
  booktitle =    PROC # " 10th " # USS,
  pages =    {165-172},
  year =     2001,
  month =    AUG
}

@Book{CoxGoo:1994:PH,
  author =   {J. Cox and B. Goodheart},
  title =    {{The Magic Garden Explained: The Internals of Unix
                   System V Release 4: An Open Systems Design}},
  publisher =    PH,
  year =     1994
}

@InProceedings{CypLeu:1995:SPDP,
  author =   {R. Cypher and E. Leu},
  title =    {{Efficient Race Detection for Message-Passing
                   Programs with Nonblocking Sends and Receives}},
  booktitle =    PROC # " " # SPDP,
  pages =    {534-541},
  year =     1995
}

@Manual{DB2SQL:1999:IBM,
  title =    {DB2 UDB SQL Reference},
  organization = {IBM},
  edition =  {V6.1},
  year =     1999
}

@Article{DarMay:2003:JPDC,
  author =   {D. Darling and J. Mayo},
  title =    {{Stable Predicate Detection in Dynamic Systems}},
  journal =      "Submitted to the " # JPDC,
  OPTpages =     {},
  year =     {2003},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Manual{Dav:1999:IBM,
  title =    {{DataLinks: Managing External Data with DB2
                   Universal Database}},
  organization = {IBM Corporation},
  month =    FEB,
  year =     {1999},
  note =     {White paper prepared by J. R. Davis}
}

@Book{DavPri:1990:CUP,
  author =   {B. A. Davey and H. A. Priestley},
  title =    {{Introduction to Lattices and Order}},
  publisher =    CUP,
  address =  {Cambridge, UK},
  year =     {1990},
}

@TechReport{DemAro:2000:TR:05,
  author =   {M. Demirbas and A. Arora},
  title =    {{An Optimal Termination Detection Algorithm for
                   Rings}},
  institution =  OSU,
  year =     2000,
  number =   {OSU-CISRC-2/00-TR05},
  month =    FEB
}

@Article{Den:1987:TSE,
  author =   {D. Denning},
  title =    {{An Intrusion Detection Model}},
  journal =  TSE,
  volume =   {13},
  number =   {2},
  month =    FEB,
  year =     {1987},
  pages =    {222-232}
}

@Article{DhaIye+:1997:PC,
  author =   {D. M. Dhamdhere and S. R. Iyer and E. K. K. Reddy},
  title =    {{Distributed Termination Detection for Dynamic Systems}},
  journal =      PC,
  year =     {1997},
  OPTkey =   {},
  volume =   {22},
  OPTnumber =    {},
  pages =    {2025-2045},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Dij:1965:CACM,
  author =   {E. W. Dijkstra},
  title =    {{Solution of a Problem in Concurrent Programming
                   Control}},
  journal =  CACM,
  pages =    569,
  year =     1965,
  volume =   8,
  number =   9,
  organization = {ACM}
}

@Article{Dij:1971:ACTA,
  author =   {E. W. Dijkstra},
  title =    {{Hierarchical Ordering of Sequential Processes}},
  journal =      ACTA,
  year =     1971,
  volume =   1,
  number =   2,
  pages =    {115-138},
  month =    OCT
}

@Article{Dij:1974:CACM,
  author =   {E. W. Dijkstra},
  title =    {{Self-Stabilizing Systems in spite of Distributed Control}},
  journal =  CACM,
  year =     {1974},
  volume =   {17},
  number =   {11},
  pages =    {643-644}
}

@InCollection{Dij:1985:SV,
  author =   {E. W. Dijsktra},
  title =    {{The Distributed Snapshot of K. M. Chandy and L. Lamport}},
  booktitle =    {Control Flow and Data Flow: Concepts of Distributed
                  Programming},
  OPTcrossref =  {},
  OPTkey =   {},
  OPTpages =     {},
  publisher =    SV,
  year =     {1985},
  editor =   {M. Broy},
  volume =   {F14},
  OPTnumber =    {},
  series =   {NATO ASI},
  OPTtype =  {},
  OPTchapter =   {},
  address =  {New York, NY},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =  {},
  OPTannote =    {}
}

@Article{Dij:1986:DC,
  author =   {E. W. Dijkstra},
  title =    {{A Belated Proof of Self-Stabilization}},
  journal =  DC,
  year =     {1986},
  volume =   {1},
  pages =    {5-6}
}

@Article{DijFei+:1983:IPL,
  author =   {E. W. Dijkstra and W. H. J. Feijen and A. J. M. van
                  Gasteren},
  title =    {{Derivation of a Termination Detection Algorithm for
                   Distributed Computations}},
  journal =  IPL,
  volume =   {16},
  pages =    {217-219},
  OPTkey =   {},
  OPTmonth =     {},
  year =     {1983},
  OPTannote =    {}
}

@Article{DijSch:1980:IPL,
  author =   {E. W. Dijkstra and C. S. Scholten},
  title =    {{Termination Detection for Diffusing Computations}},
  journal =  IPL,
  year =     1980,
  volume =   11,
  number =   1,
  pages =    {1-4}
}

@Article{Dil:1950:AM,
  author =   {R. P. Dilworth},
  title =    {{A Decomposition Theorem for Partially Ordered Sets}},
  journal =  AM,
  year =     1950,
  volume =   51,
  pages =    {161-166}
}

@Article{DolIsr+:1993:DC,
  author =   {S. Dolev and A. Israeli and S. Moran},
  title =    {{Self-Stabilization of Dynamic Systems Assuming Only Read/Write Atomicity}},
  journal =      DC,
  year =     1993,
  volume =   7,
  number =   1,
  pages =    {3-16}
}

@InProceedings{DueGup+:1992:WLCPC,
  author =   {E. Duesterwald and R. Gupta and M. L. Soffa},
  title =    {{Distributed Slicing and Partial Re-execution for Distributed Programs}},
  booktitle =    PROC # " 5th " # WLCPC,
  pages =    {329-337},
  year =     1992
}

@Article{DusMil:1941:AJM,
  author =   {B. Dushnik and E. W. Miller},
  title =    {{Partially Ordered Sets}},
  journal =  AJM,
  year =     1941,
  volume =   63,
  pages =    {600-610}
}

@PhdThesis{Ell:1995:PhD,
  author =   {G. Ellis},
  title =    {{Managing Complex Objects}},
  school =   {University of Queensland},
  year =     1995
}

@Article{ElnAlv+:2002:CS,
  author =   {E. N. Elnozahy and L. Alvisi and Y.-M. Wang and
                  D. B. Johnson},
  title =    {{A Survey of Rollback-Recovery Protocols in
                   Message-Passing Systems}},
  journal =  CS,
  volume =   {34},
  number =   {3},
  year =     {2002},
  pages =    {373-408},
}

@Article{FelHab+:1994:SIAMJDM,
  author =   {S. Felsner and M. Habib and R. H. M{\"o}hring},
  title =    {{On the Interplay of Interval Dimension and Dimension}},
  journal =  SIAMJDM,
  volume =   7,
  pages =    {32-40},
  year =     1994,
  OPTurl =       {http://www.inf.fu-berlin.de/{\symbol{126}}felsner/Paper/Idim-dim.ps.gz},
}

@Article{FelTro:1994:DM,
  author =   {S. Felsner and W. T. Trotter},
  title =    {{On the Fractional Dimension of Partially Ordered Sets}},
  journal =  DM,
  volume =   136,
  pages =    {101-117},
  year =     1994,
  OPTurl =       {http://www.inf.fu-berlin.de/{\symbol{126}}felsner/Paper/fdim.ps.gz},
}

@Article{Fid:1991:Com,
  author =   {C. Fidge},
  title =    {{Logical Time in Distributed Computing Systems}},
  journal =  Com,
  year =     1991,
  volume =   24,
  number =   8,
  pages =    {28-33},
  month =    AUG
}

@InProceedings{FisLyn+:1979:FCS,
  author =   {M. J. Fischer and N. A. Lynch and  J. E. Burns and A. Borodin},
  title =    {{Resource Allocation with Immunity to Limited Process Failure
                   (preliminary report)}},
  booktitle =    PROC # " 20th " # FOCS,
  pages =    {234-254},
  year =     1979,
  month =    OCT
}

@Article{Fra:1980:TOPLAS,
  author =   {N. Francez},
  title =    {{Distributed Termination}},
  journal =  TOPLAS,
  year =     1980,
  volume =   2,
  number =   1,
  pages =    {42-55},
  month =    JAN
}

@InProceedings{FroRay+:1994:ICPP,
  author =   {E. Fromentin and M. Raynal and V. K. Garg and
                  A. I. Tomlinson},
  title =    {{On the Fly Testing of Regular Patterns in Distributed Computations}},
  booktitle =    PROC # " 23rd " # ICPP,
  pages =    {73-76},
  year =     1994,
  number =   2,
  address =  {Chicago, Illinois},
  month =    AUG
}

@InProceedings{FroRay:1994:SPDP,
  author =   {E. Fromentin and M. Raynal},
  title =    {{Inevitable Global States: A Concept to Detect
                   Unstable Properties of Distributed Computations in
                   an Observer Independent Way}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 6th " # SPDP,
  pages =    {242-248},
  year =     {1994},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization ={},
  OPTpublisher = {},
  OPTnote =  {},
  OPTannote =    {}
}

@Misc{GDB,
  OPTkey =   {},
  OPTauthor =    {},
  title =    {{GDB: The GNU Project Debugger}},
  OPThowpublished = {},
  OPTmonth =     {},
  OPTyear =      {},
  note =     {Available at
                  \texttt{http://www.gnu.org/software/gdb/gdb.html}},
  OPTannote =    {}
}

@TechReport{Gae:2003:TR:38,
  author =   {F. C. G{\"a}rtner},
  title =    {{A Survey of Self-Stabilizing Spanning-Tree Construction Algorithms}},
  institution =  SCCS # ", " # EPFL,
  address =      {Lausanne, Switzerland},
  year =     2003,
  number =   {IC 2003/38}
}

@InProceedings{GaeKlo:2000:SRDS,
  author =   {F. C. G{\"a}rtner and S. Kloppenburg},
  title =    {{Consistent Detection of Global Predicates under a Weak Fault Assumption}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # ", " # SRDS,
  pages =    {94-103},
  year =     {2000},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {N{\"u}rnberg, Germany},
  month =    OCT,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{GaePle:2001:DISC,
  author =   {F. C. G{\"a}rtner and S. Pleisch},
  title =    {{(Im)Possibilities of Predicate Detection in
                  Crash-Affected Systems using
                  Interrupt-Style Failure Detectors (Brief Announcement)}},
  booktitle =    PROC # " " # DISC,
  year =     2001,
  address =  {Lisbon, Portugal},
  month =    {October}
}
@TechReport{GaePle:2001:TR,
  author =   {F. C. G{\"a}rtner and S. Pleisch},
  title =    {{(Im)Possibilities of Predicate Detection in Crash-Affected Systems}},
  institution =  IBMZ,
  year =     2001,
  number =   {RZ 3361 (\# 93407)},
  month =    AUG
}
@InProceedings{GaePle:2001:WSS,
  author =   {F. C. G{\"a}rtner and S. Pleisch},
  title =    {{(Im)Possibilities of Predicate Detection in Crash-Affected Systems}},
  booktitle =    PROC # " 5th " # WSS,
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {98-113},
  year =     {2001},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   LNCS # " 2194",
  address =  {Lisbon, Portugal},
  month =    {October},
  OPTorganization ={},
  publisher =    SV,
  OPTnote =  {},
  OPTannote =    {}
}
@InProceedings{GaePle:2002:DISC,
  author =   {F. C. G{\"a}rtner and S. Pleisch},
  title =    {{Failure Detection Sequencers: Necessary and Sufficient
                  Information about Failures to Solve Predicate Detection}},
  booktitle =    PROC # " 16th " #  DISC,
  pages =    {280-294},
  year =     2002,
  number =   2508,
  series =   LNCS,
  publisher =    SV
}
@InProceedings{GamNes+:1987:ICALP,
  author =   {G. Gambosi and J. Ne\v{s}et\v{r}il and M. Talamo},
  title =    {{Posets, Boolean Representations and Quick
                   Path Searching}},
  booktitle =    PROC # " 14th " # ICALP,
  year =     1987,
  pages =    {404-424},
  number =   267,
  series =   LNCS
}
@Article{GamNes+:1990:TCS,
  author =   {G. Gambosi and J. Ne\v{s}et\v{r}il and M. Talamo},
  title =    {{On Locally Presented Posets}},
  journal =  TCS,
  year =     {1990},
  OPTkey =   {},
  volume =   {70},
  number =   {2},
  pages =    {251-260},
  month =    JAN,
  OPTnote =  {},
  OPTannote =    {}
}
@InProceedings{Gar:1996:ICSKE,
  author =   {V. K. Garg},
  title =    {{Observation of Global Properties in Distributed Systems}},
  booktitle =    ICSKE,
  pages =    {418-425},
  year =     1996,
  address =  {Lake Tahoe, Nevada},
  month =    JUN
}
@Book{Gar:1996:KAP,
  author =   {V. K. Garg},
  OPTeditor =    {~},
  title =    {{Principle of Distributed Systems}},
  publisher =    KAP,
  year =     1996
}
@InProceedings{Gar:1997:WAD,
  author =   {V. K. Garg},
  title =    {{Observation and Control for Debugging
                   Distributed Computations}},
  booktitle =    PROC # " " # WAD,
  pages =    {1-12},
  year =     1997,
  address =  {Link{\"o}ping, Sweden},
  note =     {Keynote Presentation}
}
@Book{Gar:2002:Book,
  author =   {V. K. Garg},
  title =    {{Elements of Distributed Computing}},
  publisher =    JWSUS,
  address =  {New York, NY},
  year =     {2002},
}
@InProceedings{Gar:2002:FSTTCS,
  author =   {V. K. Garg},
  title =    {{Algorithmic Combinatorics based on Slicing Posets}},
  booktitle =    PROC # " 22nd " # FSTTCS,
  year =     2002,
  address =  {Kanpur, India},
  month =    {December}
}
@Article{GarBar:1985:ACM,
  author =   {H. Garcia-Molina and D. Barbar},
  title =    {{How to Assign Votes in a Distributed System}},
  journal =  JACM,
  year =     {1985},
  volume =   {32},
  number =   {4},
  pages =    {841-860},
  month =    OCT
}
@InProceedings{GarCha+:1995:CSS,
  author =   {V. K. Garg and C. Chase and R. Kilgore and
                  J. R. Mitchell},
  title =    {{Detecting Conjunctive Channel Predicates in
                   a Distributed Programming Environment}},
  booktitle =    PROC # " " # CSS,
  pages =    {232-241},
  year =     1995,
  volume =   2,
  address =  {Maui, Hawaii},
  month =    JAN
}
@Article{GarCha+:1997:JPDC,
  author =   {V. K. Garg and C. Chase and R. Kilgore and
                  J. R. Mitchell},
  title =    {{Efficient Detection of Channel Predicates in
                   Distributed Systems}},
  journal =  JPDC,
  year =     {1997},
  volume =   {45},
  number =   {2},
  pages =    {134-147},
  month =    SEP
}
@InProceedings{GarCha:1995:ICDCS,
  author =   {V. K. Garg and C. Chase},
  title =    {{Distributed Algorithms for Detecting
                   Conjunctive Predicates}},
  booktitle =    PROC # " " # ICDCS,
  pages =    {423-430},
  year =     1995,
  address =  {Vancouver, Canada},
  month =    JUN
}

@Book{GarJoh:1991:Fre,
  author =   {M. R. Garey and D. S. Johnson},
  OPTeditor =    {Victor Klee},
  title =    {{Computer and Intractability: A Guide to the
                   Theory of \mbox{NP-Completeness}}},
  publisher =    Fre,
  year =     1991
}
@InProceedings{GarLun:1991:NCSC,
  author =   {T. D. Garvey and T. F. Lunt},
  title =    {{Model-Based Intrusion Detection}},
  booktitle =    PROC # " 14th " # NCSC,
  pages =    {372-385},
  year =     1991
}
@Article{GarMit+:2003:SIGACT,
  author =   {V. K. Garg and N. Mittal and A. Sen},
  title =    {{Applications of Lattice Theory to Distributed
                  Computing}},
  journal =  SIGACT # " News Distributed Computing Column",
  year =     2003,
  OPTpublisher = {ACM Press},
  editor =   {Sergio Rajsbaum},
  volume =   34,
  number =   3,
  pages =    {40-61},
  month =    SEP
}
@InProceedings{GarMit:1998:FSTTCS,
  author =   {V. K. Garg and J. R. Mitchell},
  title =    {{Implementable Failure Detectors in
                   Asynchronous Systems}},
  booktitle =    PROC # " " # FSTTCS,
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {158-169},
  year =     {1998},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =  {Chennai, India},
  OPTmonth =     {},
  OPTorganization ={},
  OPTpublisher = {},
  OPTnote =  {},
  OPTannote =    {}
}
@InProceedings{GarMit:1998:ICDCS,
  author =   {V. K. Garg and J. R. Mitchell},
  title =    {{Distributed Predicate Detection in a Faulty
                   Environment}},
  booktitle =    PROC # " " # ICDCS,
  pages =    {416-423},
  year =     {1998},
  address =  {Amsterdam, The Netherlands},
  month =    MAY
}
@InProceedings{GarMit:2001:ICDCS,
  author =   {V. K. Garg and N. Mittal},
  title =    {{On Slicing a Distributed Computation}},
  booktitle =    PROC # " 21st " # ICDCS,
  pages =    {322-329},
  year =     2001,
  address =  {Phoenix, Arizona},
  month =    APR,
  OPTnote =  {Available at \texttt{http://www.cs.utexas.edu/users/neerajm/research.html}}
}
@InProceedings{GarSka:2001:PODC,
  author =   {V. K. Garg and C. Skawratananond},
  title =    {{String Realizers of Posets with Applications
                   to Distributed Computing}},
  booktitle =    PROC # " 20th " # PODC,
  year =     2001,
  address =  {Newport, Rhode Island},
  month =    AUG,
  pages =    {72-80}
}
@InProceedings{GarTom+:1995:SPDP,
  author =   {V. K. Garg and A. I. Tomlinson and E. Fromentin and
                  Michel Raynal},
  title =    {{E}xpressing and {D}etecting {G}eneral {C}ontrol
                  {F}low {P}roperties of {D}istributed {C}omputations},
  booktitle =    PROC # " 7th " # SPDP,
  pages =    {432-438},
  year =     1995,
  address =  {San Antonio, Texas},
  month =    OCT
}
@InProceedings{GarWal:1991:WPDD,
  author =   {V. K. Garg and B. Waldecker},
  title =    {{D}etection of {U}nstable {P}redicates},
  booktitle =    PROC # " " # WPDD,
  address =  {Santa Cruz, California},
  month =    MAY,
  year =     {1991},
  OPTorganization ={ACM/ONR},
}
@InProceedings{GarWal:1992:FSTTCS,
  author =   {V. K. Garg and B. Waldecker},
  title =    {{D}etection of {U}nstable {P}redicates in
                  {D}istributed {P}rograms},
  booktitle =    PROC # " 12th " # FSTTCS,
  OPTcrossref =  {},
  OPTkey =   {},
  pages =    {253-264},
  year =     {1992},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  series =   LNCS,
  address =  {New Delhi, India},
  OPTmonth =     {},
  OPTorganization ={},
  OPTpublisher = {},
  OPTnote =  {},
  OPTannote =    {}
}
@Article{GarWal:1994:TPDS,
  author =   {V. K. Garg and B. Waldecker},
  title =    {{Detection of Weak Unstable Predicates in Distributed Programs}},
  journal =  TPDS,
  year =     1994,
  volume =   5,
  number =   3,
  pages =    {299-307},
  month =    MAR
}
@Article{GarWal:1996:TPDS,
  author =   {V. K. Garg and B. Waldecker},
  title =    {{Detection of Strong Unstable Predicates in Distributed Programs}},
  journal =  TPDS,
  year =     1996,
  volume =   7,
  number =   12,
  pages =    {1323-1333},
  month =    DEC
}
@Article{GhoGup+:1996:JCI,
  author =   {S. Ghosh and A. Gupta and S. V. Pemmaraju},
  title =    {{A Fault-containing Self-stabilizing Spanning Tree Algorithm}},
  journal =      JCI,
  year =     1996,
  volume =   2,
  number =   1,
  pages =    {322-328}
}
@Book{God:1996:SV,
  author =   {P. Godefroid},
  ALTeditor =    {},
  title =    {{P}artial-{O}rder {M}ethods for the {V}erification of
                  {C}oncurrent {S}ystems},
  publisher =    SV,
  year =     {1996},
  volume =   {1032},
  series =   {Lecture Notes in Computer Science}
}
@Book{GodCox:1993:PH,
  author =   {B. Goodheart and J. Cox},
  title =    {The Magic Garden Explained: The Internals of Unix
                  System V Release 4},
  publisher =    PH,
  year =     {1993}
}
@Misc{GoySit+:2003:SCISS,
  author =   {B. Goyal and S. Sitaraman and N. Mittal and S. Venkatesan},
  title =    {{A Partial Order Approach to Detect Race Condition Attacks}},
  howpublished = "Abstract published in " # SCISS ,
  month =    APR,
  year =     2003
}
@TechReport{GoySit+:2003:TR:03,
  author =       {B. Goyal and S. Sitaraman and S. Venkatesan},
  title =        {{A Unified Approach to Detect Binding Based Race Condition Attacks}},
  number =       {UTDCS-02-03},
  year =         2003,
  institution =  DCS # ", " # UTD # ", " # "\textsf{http://www.utdallas.edu/{\textasciitilde}venky/publications/race.pdf}"
}
@InProceedings{GoySri+:2003:TWSIS,
  author =   {B. Goyal and S. Sitaraman and N. Mittal and S. Venkatesan},
  title =    {{Methods To Tackle Vulnerabilities Caused by Lack of Mutual Exclusion}},
  booktitle =    PROC # " " # TWSIS,
  year =     2003,
  pages =        {17-21},
  address =      {College Station, Texas},
  month =    APR
}
@Book{GraReu:1993:MK,
  author =   {J. Gray and A. Reuter},
  title =    {Transaction Processing: Concepts and Techniques},
  publisher =    MK,
  year =     {1993}
}
@InProceedings{GraVol:1993:MVPP,
  author =   {S. Grabner and J. Volkert},
  title =    {{Debugging Parallel Programs Using Event Graph Manipulation}},
  booktitle =    PROC # " " # MVPP,
  pages =    {443-450},
  year =     1993,
  month =    OCT
}
@Book{Gratzer,
  author =       {G. Gratzer},
  title =        {{General Lattice Theory}},
  publisher =    {Academic Press},
  address =      {New York, NY},
  year =         1978
}
@InProceedings{HabHuc+:1995:KRUSE,
  author =   {M. Habib and M. Huchard and L. Nourine},
  title =    {{Embedding Partially Ordered Sets into Chain-Products}},
  booktitle =    PROC # " " # KRUSE,
  pages =    {147-161},
  year =     1995,
  address =      {University of California, Santa Cruz},
  month =    AUG
}
@InProceedings{HabNou:1994:ORDAL,
  author =   {M. Habib and L. Nourine},
  title =    {{Bit-Vector Encoding for Partially Ordered Sets}},
  booktitle =    PROC # " " # ORDAL,
  pages =    {1-12},
  year =     1994,
  number =   831,
  series =   LNCS,
  address =      {Lyon, France},
  month =    JUL,
  publisher = SV
}


@inproceedings{KuznetsovRavi:ConcurrencyTM:OPODIS:2011,
  author    = {Petr Kuznetsov and
               Srivatsan Ravi},
  title     = {On the Cost of Concurrency in Transactional Memory},
  booktitle = {Principles of Distributed Systems - 15th International Conference,
               {OPODIS} 2011, Toulouse, France, December 13-16, 2011. Proceedings},
  pages     = {112--127},
  year      = {2011},
  url       = {https://doi.org/10.1007/978-3-642-25873-2\_9},
  doi       = {10.1007/978-3-642-25873-2\_9},
  timestamp = {Wed, 17 May 2017 14:24:33 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/opodis/KuznetsovR11},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@InProceedings{Had:2001:PODC,
  author =   {V. Hadzilacos},
  title =    {{A Note on Group Mutual Exclusion}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 20th " # PODC,
  OPTpages =     {},
  year =     {2001},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    AUG,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@article{Hadzilacos:1988:JACM,
 author = {Hadzilacos, Vassos},
 title = {A theory of reliability in database systems},
 journal = {J. ACM},
 issue_date = {Jan. 1988},
 volume = {35},
 number = {1},
 month = jan,
 year = {1988},
 issn = {0004-5411},
 pages = {121--145},
 numpages = {25}
} 


@InProceedings{HelJar+:1987:PODC,
  author =       {J.-M. H{\'e}lary and C. Jard and N. Plouzeau and M. Raynal},
  title =        {{Detection of Stable Properties in Distributed Applications}},
  booktitle =    PROC # " " # PODC,
  pages =        {125-136},
  year =         {1987}
}
@article{HelRay:1994:DC,

  author =       {J.-M. H{\'e}lary and M. Raynal},
  title =        {{Towards the Construction of Distributed Detection Programs, with
                   an Application to Distributed Termination}},
  journal =      DC,
  volume =       {7},
  number =       {3},
  pages =        {137-147},
  year =         "1994"
}
@Article{Hir:1951:SRKU,
  author =   {T. Hiraguchi},
  title =    {{On the Dimension of Partially Ordered Sets}},
  journal =      SRKU,
  year =     1951,
  volume =   1,
  pages =    {77-94}
}
@Article{Hir:1955:SRKU,
  author =   {T. Hiraguchi},
  title =    {{O}n the {D}imension of {O}rders},
  journal =      SRKU,
  year =     1955,
  volume =   4,
  pages =    {1-20}
}
@Article{HoRam:1982:TSE,
  author =   {G. S. Ho and C. V. Ramamoorthy},
  title =    {{Protocols for Deadlock Detection in Distributed Database Systems}},
  journal =      TSE,
  year =     {1982},
  OPTkey =   {},
  volume =   {8},
  number =   {6},
  pages =    {554-557},
  month =    NOV,
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Hol:1997:TSE,
  author =   {G. Holzmann},
  title =    {{The Model Checker SPIN}},
  journal =      TSE,
  year =     1997,
  OPTkey =   {},
  volume =   23,
  number =   5,
  pages =    {279-295},
  month =    MAY,
  OPTnote =      {},
  OPTannote =    {}
}
@TechReport{HsiMit:2000:TC,
  author =   {H. Hsiao and N. Mittal},
  title =    {{Database Managed External File Update}},
  institution =  IBMARC,
  year =     2000,
  number =   {RJ10183},
  address =  {San Jose, California, 95120}
}
@Manual{HsiNar:1999:IBMARC,
  author =   {H. Hsiao and I. Narang},
  title =    {{Update In-Place Support with DataLinks}},
  organization = IBMARC,
  year =     {1999},
  note =     {Internal Document}
}
@InProceedings{HsiNar:2000:SIGMOD,
  author =   {H. Hsiao and I. Narang},
  title =    {{DLFM: A Transactional Resource Manager}},
  booktitle =    PROC # " 19th " # SIGMOD,
  pages =    {518-528},
  year =     2000,
  address =  {Dallas, Texas},
  month =    MAY
}
@InProceedings{Hua:1989:ICDCS,
  author =   {S.-T. Huang},
  title =    {{Detecting Termination of Distributed Computations by External Agents}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICDCS,
  pages =    {79-84},
  year =     {1989},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Hua:1989:IPL,
  author =   {S.-T. Huang},
  title =    {{Termination Detection by using Distributed Snapshots}},
  journal =      IPL,
  year =     {1989},
  OPTkey =   {},
  volume =   {32},
  OPTnumber =    {},
  pages =    {113-119},
  month =    AUG,
  OPTnote =      {},
  OPTannote =    {}
}
@Article{HuaChe:1992:IPL,
  author =   {S.-T. Huang and N.-S. Chen},
  title =    {{A Self-Stabilizing Algorithm for Constructing Breadth-First Trees}},
  journal =      IPL,
  year =     1992,
  volume =   41,
  number =   2,
  pages =    {109-117},
  month =    FEB
}
@InProceedings{HuaKin:1993:FTCS,
  author =   {Y. Huang and C. Kintala},
  title =    {{S}oftware {I}mplemented {F}ault {T}olerance:
                  {T}echnologies and {E}xperience},
  booktitle =    PROC # " " # FTCS,
  pages =    {138-144},
  year =     1993,
  month =    JUN
}
@InProceedings{HurMiz+:1996:SPDP,
  author =   {M. Hurfin and M. Mizuno and M. Raynal and
                  M. Singhal},
  title =    {{Efficient Distributed Detection of Conjunctions of Local Predicates in
                   Asynchronous Computations}},
  booktitle =    PROC # " 8th " # SPDP,
  pages =    {588-594},
  year =     1996,
  address =  {New Orleans},
  month =    OCT
}
@Article{HurPlo+:1993:JCC,
  author =   {M. Hurfin and N. Plouzeau and M. Raynal},
  title =    {{A Debugging Tool for Distributed Estelle Programs}},
  journal =  JCC,
  year =     1993,
  volume =   16,
  number =   5,
  pages =    {328-333},
  month =    MAY
}
@InProceedings{HurPlo+:1993:WPDD,
  author =   {M. Hurfin and N. Plouzeau and M. Raynal},
  title =    {{D}etecting {A}tomic {S}equences of {P}redicates in
                  {D}istributed {C}omputations},
  booktitle =    PROC # " " # WPDD,
  pages =    {32-42},
  year =     1993
}
@InProceedings{HurRay:1996:WGCS,
  author =   {M. Hurfin and M. Raynal},
  title =    {{D}etecting {D}iamond {N}ecklaces in {L}abeled {D}ags
                  ({A} {P}roblem from {D}istributed  {D}ebugging},
  booktitle =    PROC # " " # WGCS,
  pages =    {211-223},
  year =     1996,
  series =   LNCS,
  publisher =    SV
}
@Manual{ISO:1993,
  author =       {ISO},
  title =        {{S}pecification of the {A}synchronous {T}ransfer {M}ode
                  {R}ing {(ATMR)} {P}rotocol},
  month =        JAN,
  year =         1993,
}
@InProceedings{JarJer+:1994:ICDCS,
  author =       {C. Jard and T. J{\'e}ron and G.-V. Jourdan and J.-X. Rampon},
  title =        {{A} {G}eneral {A}pproach to {T}race-{C}hecking in
                  {D}istributed {C}omputing {S}ystems},
  booktitle =    PROC # " " # ICDCS,
  pages =        {396-403},
  year =         {1994},
  url =          {http://citeseer.nj.nec.com/jard94general.html}
}
@InProceedings{JegMed+:1995:WSCT,
  author =   {R. Jegou and R. Medina and L. Nourine},
  title =    {{L}inear {S}pace {A}lgorithm for {O}n-line
                  {D}etection of {G}lobal {P}redicates},
  booktitle =    PROC # " " # WSCT,
  pages =        {175-189},
  year =     1995,
  editor =   {J. Desel},
  publisher =    SV
}
@InProceedings{JohZwa:1988:PODC,
  author =   {D. B. Johnson and W. Zwaenepoel},
  title =    {{R}ecovery in {D}istributed {S}ystems {U}sing
                  {O}ptimistic {M}essage {L}ogging and
                  {C}heckpointing},
  booktitle =    PROC # " 6th " # PODC,
  pages =    {171-181},
  year =     1988,
  month =    AUG
}
@Article{JohZwa:1990:JA,
  author =       {D. B. Johnson and W. Zwaenepoel},
  title =        {{R}ecovery in {D}istributed {S}ystems using {O}ptimistic {M}essage {L}ogging
                 and {C}heckpointing},
  journal =      JA,
  volume =       {11},
  number =       {3},
  month =        SEP,
  year =         {1990},
  pages =        {462-491},
}
@Article{Jou:2000:DC,
  author =       {Y.-J. Joung},
  title =        {{A}synchronous {G}roup {M}utual {E}xclusion},
  journal =      DC,
  volume =       {13},
  number =       {4},
  pages =        {189-206},
  year =         {2000},
}
@Article{Jou:2002:DC,
  author =       {Y.-J. Joung},
  title =        {{T}he {C}ongenial {T}alking {P}hilosophers {P}roblem in {C}omputer
                  {N}etworks},
  journal =       DC,
  pages =        {155-175},
  year =         {2002},
}
@Article{Jou:2003:TPDS,
  author =       {Y.-J. Joung},
  title =        {{Q}uorum-{B}ased {A}lgorithms for {G}roup {M}utual {E}xclusion},
  journal =      TPDS,
  pages =        {463-475},
  year =         {2003},
  volume =       {14},
  number =       {5},
  month =        MAY
}
@Article{KaeMoh:1978:SIAM,
  author =   {R. Kaerkes and R. H. M{\"o}hring},
  title =    {{V}orlesungen u{\"b}er {O}rdnungen und {N}etzplantheorie},
  journal =      {Schriften zur Informatik und Angewandten Mathematik 45, RWTH Aachen},
  year =     1978
}
@InProceedings{KanNao+:1988:STOC,
  author =   {S. Kannan and M. Naor and S. Rudich},
  title =    {{I}mplicit {R}epresentation of {G}raphs},
  booktitle =    PROC # " 20th " # STOC,
  pages =    {334-343},
  year =     1988,
  address =      {Chicago},
  month =    MAY
}
@Article{KanNao+:1992:SIAMJDM,
  author =   {S. Kannan and M. Naor and S. Rudich},
  title =    {{I}mplicit {R}epresentation of {G}raphs},
  journal =      SIAMJDM,
  year =     1992,
  volume =   5,
  number =   4,
  pages =    {596-603},
  month =    NOV
}
@InProceedings{KanWil+:2003:ICDCS,
  author =   {B. B. H. Kang and R. Wilensky and J, Kubiatowicz},
  title =    {{The Hash History Approach for Reconciling Mutual Inconsistency}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 23rd " # ICDCS,
  pages =    {670-677},
  year =     {2003},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Providence, Rhode Island},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{KeaMoi:1999:PODC,
  author =   {P. Keane and M. Moir},
  title =    {{A} {S}imple {L}ocal-{S}pin {G}roup {M}utual {E}xclusion {A}lgorithm},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PODC,
  pages =    {23-32},
  year =     {1999},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{KhoHam+:2003:JPDC,
  author =   {A. A. Khokhar and S. E. Hambrusch and E. Kocalar},
  title =    {{Termination Detection in Data-Driven Parallel Computations/Applications}},
  journal =      JPDC,
  year =     2003,
  volume =   63,
  number =   3,
  pages =    {312-326},
  month =    MAR
}
@Article{KilCha:1997:CJ,
  author =   {R. Kilgore and C. Chase},
  title =    {{T}esting {D}istributed {P}rograms {C}ontaining
                  {R}acing {M}essages},
  journal =  CJ,
  year =     1997,
  volume =   40,
  number =   8,
  pages =    {489-498},
  month =    NOV
}
@InProceedings{KilCha:1997:CSS,
  author =   {R. Kilgore and C. Chase},
  title =    {{R}e-execution of {D}istributed {P}rograms to
                  {D}etect {B}ugs {H}idden by {R}acing {M}essages},
  booktitle =    PROC # " " # CSS,
  pages =        {423-432},
  year =     1997,
  address =  {Hawaii},
  month =    JAN
}
@PhdThesis{KoChe:1996:Thesis,
  author =       {C. Ko and W. Cheuk},
  title =        {{Execution Monitoring Of Security Critical Programs in a Distributed
                   System: A Specification Based Approach}},
  year =         1996,
  school =       UCD
},
  month =        {August},
  year =         1997
}
@InProceedings{KoRed:2002:SP,
  author =   {C. Ko and T. Redmond},
  title =    {{Noninterference and Intrusion Detection}},
  year =     2002,
  booktitle =    PROC # " " # SP,
  pages =        {177-187},
  address =      {Berkeley, California},
  month =    MAY
}
@InProceedings{KocKho+:1999:PDC,
  author =   {E. Kocalar and A. A. Khokhar and S. E. Hambrusch},
  title =    {{T}ermination {D}etection: {M}odels and {A}lgorithms for {SPMD}
                  {C}omputing {P}aradigms},
  booktitle =    PROC # " " # PDC,
  year =     1999
}
@Book{Koh:1978:MH,
  author =   {Z. Kohavi},
  OPTeditor =    {~},
  title =    {{S}witching and {F}inite {A}utomata {T}heory},
  publisher =    MH,
  year =     1978,
  edition =  {2nd}
}
@Misc{KohGei:1995,
  OPTkey =   {},
  author =   {J. A. Kohl and G. A. Geist},
  title =    {{T}he {PVM 3.4} {T}racing {F}acility and {XPVM 1.1}},
  howpublished = {Computer Science and Mathematics Divison, Oak Ridge National Laboratory, TN, USA},
  OPTmonth =     {},
  year =     {1995},
  note =     {},
  OPTannote =    {}
}
@Article{KorFer:1992:AMCSJ,
  author =   {B. Korel and R. Ferguson},
  title =    {{Dynamic Slicing of Distributed Programs}},
  journal =  AMCSJ,
  year =     1992,
  volume =   2,
  number =   2,
  pages =    {199-215}
}
@Article{KorLas:1988:IPL,
  author =   {B. Korel and J. Laski},
  title =    {{Dynamic Program Slicing}},
  journal =  IPL,
  year =     1988,
  volume =   29,
  number =   3,
  pages =    {155-163}
}
@InProceedings{KorRil:1997:WAD,
  author =   {B. Korel and J. Rilling},
  title =    {{Application of Dynamic Slicing in Program Debugging}},
  booktitle =    PROC # " 3rd " # WAD,
  pages =    {43-57},
  year =     1997,
  editor =   {Mariam Kamkar},
  address =  {Link{\" o}ping, Sweden},
  month =    MAY
}
@Article{Ksh:1998:TCS,
  author =   {A. D. Kshemkalyani},
  title =    {{A Framework for Viewing Atomic Events in Distributed Computations}},
  journal =      TCS,
  year =     {1998},
  OPTkey =   {},
  volume =   {196},
  number =   {1-2},
  pages =    {45-70},
  month =    APR,
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{KshSin:1990:SPDP,
  author =       {A. D. Kshemkalyani and M. Singhal},
  title =        {{Correct Two-phase and One-phase Deadlock Detection
                   Algorithms for Distributed Systems}},
  booktitle =    PROC # " " # SPDP,
  pages =        {126-129},
  month =        DEC,
  year =         {1990}
}
@Article{KunBla+:1997:CJ,
  author =   {T. Kunz and J. P. Black and D. J. Taylor and T. Basten},
  title =    {{POET}: {T}arget-{S}ystem {I}ndependent {V}isualizations of {C}omplex
                  {D}istributed-{A}pplications {E}xecutions},
  journal =      CJ,
  year =     {1997},
  OPTkey =   {},
  volume =   {40},
  number =   {8},
  OPTpages =     {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Lai:1986:JPDC,
  author =   {T. H. Lai},
  title =    {{Termination Detection for Dynamic Distributed Systems with
                  Non-First-In-First-Out Communication}},
  journal =      JPDC,
  year =     {1986},
  OPTkey =   {},
  volume =   {3},
  OPTnumber =    {},
  pages =    {577-599},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{LaiTse+:1992:IPPS,
  author =       {T.-H. Lai and Y.-C. Tseng and X. Dong},
  title =        {{A More Efficient Message-Optimal Algorithm for
                  Distributed Termination Detection}},
  booktitle =    PROC # " 6th " # IPPS,
  year =         {1992},
  pages =        {646--649},
  publisher = {IEEE Computer Society},
}
@Article{LaiWu:1995:TPDS,
  author =   {T.-H. Lai and L.-F. Wu},
  title =    {{An $(N -1)$-Resilient Algorithm for Distributed Termination Detection}},
  journal =      TPDS,
  year =     1995,
  volume =   6,
  number =   1,
  pages =    {63-78}
}
@Article{LaiYan:1987:IPL,
  author =   {T.-H. Lai and T. H. Yang},
  title =    {{On Distributed Snapshots}},
  journal =      IPL,
  year =     {1987},
  OPTkey =   {},
  volume =   {25},
  number =   {3},
  pages =    {153-158},
  month =    MAY,
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Lam:1974:CACM,
  author =   {L. Lamport},
  title =    {{A New Solution of Dijkstra's Concurrent Programming Problem}},
  journal =      CACM,
  year =     {1974},
  OPTkey =   {},
  volume =   {18},
  number =   {8},
  pages =    {453-455},
  month =    AUG,
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Lam:1978:CACM,
  author =   {L. Lamport},
  title =    {{T}ime, {C}locks, and the {O}rdering of {E}vents in
                  a {D}istributed {S}ystem},
  journal =  CACM,
  year =     1978,
  volume =   21,
  number =   7,
  pages =    {558-565},
  month =    JUL
}
@Article{LanBul+:1994:CS,
  author =   {C. E. Landwehr and A. R. Bull and J. P. McDermott and W. S. Choi},
  title =    {{A} {T}axonomy of {C}omputer {P}rogram {S}ecurity {F}laws},
  journal =      CS,
  year =     1994,
  volume =   26,
  number =   3,
  pages =    {211-254},
  issn =         {0360-0300}
}
@Article{Law:1976:MCT,
  author =   {E. L. Lawler},
  title =    {{G}raphical {A}lgorithms and their {C}omplexity},
  journal =      MCT,
  year =     1976,
  volume =   81,
  pages =    {3-32}
}
@Article{LebMel:1987:TC,
  author =   {T. J. LeBlanc and J. M. Mellor-Crummey},
  title =    {{D}ebugging {P}rograms with {I}nstant {R}eplay},
  journal =  TC,
  year =     1987,
  volume =   {C-36},
  number =   4,
  pages =    {471-482},
  month =    APR
}
@Article{MadWes:1991:DM,
  author =   {T. Madej and D. B. West},
  title =    {{T}he {I}nterval {I}nclusion {N}umber of a {P}artially {O}rdered {S}et},
  journal =      DM,
  year =     1991,
  volume =   88,
  pages =    {259-277},
  note =     ES
}
@Article{Mae:1985:TrCS,
  author =       {M. Maekawa},
  title =        {{A}lgorithm for {M}utual {E}xclusion in {D}ecentralized {S}ystem},
  journal =      TrCS,
  pages =        {145-159},
  year =         {1985},
  volume =       {3},
  number =       {2},
  month =        MAY,
  OPTorganization = {ACM}
}
@Book{Mae:1987:Book,
  author =   {M. Maekawa and A. E. Oldehoft and R. R. Oldehoft},
  OPTeditor =    {},
  title =    {{Operating Systems Advanced Concepts}},
  publisher =    BCPC,
  year =     {1987},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Menlo Park, California},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Book{MaeOld+:1987:Book,
  author =   {M. Maekawa and A. E. Oldehoft and R. R. Oldehoft},
  title =    {{O}perating {S}ystems {A}dvanced {C}oncepts},
  publisher =    BCPC,
  year =     1987,
  address =      {Menlo Park, California}
}
@Article{MagWel+:1981:TCS,
  author =   {A. Maggiolo-Schettini and H. Welde and J. Winkowski},
  title =    {{M}odeling a {S}olution for a {C}ontrol {P}roblem in
                  {D}istributed {S}ystems by {R}estrictions},
  journal =  TCS,
  year =     1981,
  volume =   13,
  number =   1,
  pages =    {61-83},
  month =    JAN
}
@Unpublished{MahDut:2004:JPDC,
  author =   {N. R. Mahapatra and S. Dutt},
  title =    {{An Efficient Delay-Optimal Distributed Termination Detection Algorithm}},
  note =     "To Appear in " # JPDC,
  OPTkey =   {},
  OPTmonth =     {},
  year =     {2004},
  OPTannote =    {}
}
@Misc{Man:Rdist,
   title =      {{Man pages: Rdist - Remote File Distribution Program}},
   organization = {Sun Microsystems}
}
@article{ManIma:1992:JPDC,
  author =       {Y. Manabe and M. Imase},
  title =        {{G}lobal {C}onditions in {D}ebugging {D}istributed {P}rograms},
  journal =      JPDC,
  volume =       {15},
  number =       {1},
  pages =        {62-69},
  year =         {1992}
}
@InProceedings{MarNei:1991:WDAG,
  author =       {K. Marzullo and G. Neiger},
  title =        {{D}etection of {G}lobal {S}tate {P}redicates},
  booktitle =    PROC # " " # WDAG,
  pages =        {254-272},
  year =         {1991}
}
@Article{MarSab:1994:DC,
  author = {K. Marzullo and L. Sabel},
  title = {{E}fficient {D}etection of a {C}lass of {S}table {P}roperties},
  journal = DC,
  volume = {8},
  number = {2},
  pages = {81-91},
  year = {1994},
  url = "citeseer.nj.nec.com/marzullo94efficient.html"
}
@Article{Mat:1987:DC,
  author =   {F. Mattern},
  title =    {{Algorithms for Distributed Termination Detection}},
  journal =      DC,
  year =     {1987},
  OPTkey =   {},
  volume =   {2},
  number =   {3},
  pages =    {161-175},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{Mat:1989:IPL,
  author =   {F. Mattern},
  title =    {{Global Quiescence Detection based on Credit Distribution
                   and Recovery}},
  journal =      IPL,
  year =     {1989},
  OPTkey =   {},
  volume =   {30},
  number =   {4},
  pages =    {195-200},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{Mat:1989:WDAG,
  author =   {F. Mattern},
  title =    {{Virtual Time and Global States of Distributed Systems}},
  booktitle =    "Parallel and Distributed Algorithms: " # PROC # " "
                  # WDAG,
  pages =    {215-226},
  year =     1989,
  publisher =    ES
}
@Article{Mat:1993:JPDC,
  author =       {F. Mattern},
  title =        {{E}fficient {A}lgorithms for {D}istributed {S}napshots and {G}lobal
                  {V}irtual {T}ime {A}pproximation},
  journal =      JPDC,
  volume =       {18},
  number =       {4},
  pages =        {423-434},
  year =         {1993},
  url =          {http://citeseer.nj.nec.com/mattern93efficient.html}
}
@Article{MatCap:1999:JSS,
  author =   {J. Matocha and T. Camp},
  title =    {{A Taxonomy of Distributed Termination Detection Algorithms}},
  journal =      JSS,
  year =     1999,
  volume =   43,
  number =   3,
  pages =    {207-221},
  month =    NOV
}
@Techreport{MatMeh+:1991:TR:32,
  author =       {F. Mattern and H. Mehl and A. Schoone and G. Tel},
  title =        {{Global Virtual Time Approximation with Distributed
                  Termination Detection Algorithms}},
  institution =  {University of Utrecht, The Netherlands},
  number =       {RUU-CS-91-32},
  year =         {1991},
  url =          {http://citeseer.nj.nec.com/mattern91global.html}
}
@Manual{MatMel+:1997:ISO,
  author =   {N. Mattos and J. Melton and J. Richey},
  title =    {Database Language SQL - Part 9: Management of
                  External Data (SQL/MED)},
  organization = {ISO working draft},
  month =    JUN,
  year =     1997
}
@InProceedings{McMLi:1993:COMPSAC,
  author =   {P. Li and B. McMillin},
  title =    {{Fault-Tolerant Distributed Deadlock Detection/Resolution}},
  booktitle =    PROC # " 17th " # COMPSAC,
  pages =    {224-230},
  year =     1993,
  month =    NOV
}
@InProceedings{MilCho:1988:ICDCS,
  author =   {B. P. Miller and J. Choi},
  title =    {{B}reakpoints and {H}alting in {D}istributed
                  {P}rograms},
  booktitle =    PROC # " 8th " # ICDCS,
  pages =    {316-323},
  year =     1988
}
@InProceedings{Mis:1983:PODC,
  author =   {J. Misra},
  title =    {{Detecting Termination of Distributed Computations using Markers}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # PODC,
  pages =    {290-294},
  year =     {1983},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@PhdThesis{Mit:2002:Thesis,
  author =       {N. Mittal},
  title =        {{T}echniques for {A}nalyzing {D}istributed {C}omputations},
  school =       UTA,
  year =         2002,
  month =        MAY,
  note =         {Available at \texttt{http://www.utdallas.edu/{\symbol{126}}neerajm}}
}
@InProceedings{MitGar:1998:ICDCS,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Consistency Conditions for Multi-Object Distributed Operations}},
  booktitle =    PROC # " 18th " # ICDCS,
  pages =    {582-589},
  year =     {1998},
  address =      {Amsterdam, The Netherlands},
  month =    MAY
}
@TechReport{MitGar:1998:TR:005,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Consistency Conditions for Multi-Object Distributed Operations}},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     1998,
  number =   {TR-PDS-1998-005},
  address =      {Austin, TX 78712}
}
@InProceedings{MitGar:2000:PODC,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Debugging Distributed Programs using Controlled Re-execution}},
  booktitle =    PROC # " 19th " # PODC,
  pages =    {239-248},
  year =     2000,
  address =  {Portland, Oregon},
  month =    JUL
}
@TechReport{MitGar:2000:TR:002,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Debugging Distributed Programs using Controlled Re-execution}},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     2000,
  number =   {TR-PDS-2000-002},
  address =  {Austin, TX 78712},
  month =    MAY
}
@InProceedings{MitGar:2001:DISC,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Computation Slicing: Techniques and Theory}},
  booktitle =    PROC # " " # DISC,
  pages =    {78-92},
  year =     2001,
  address =      {Lisbon, Portugal},
  month =    OCT
}
@InProceedings{MitGar:2001:ICDCS,
  author =   {N. Mittal and V. K. Garg},
  title =    {{On Detecting Global Predicates in Distributed Computations}},
  booktitle =    PROC # " 21st " # ICDCS,
  pages =    {3-10},
  year =     2001,
  address =      {Phoenix, Arizona},
  month =    APR,
  OPTnote =  {Available at
                  \texttt{http://www.cs.utexas.edu/users/neerajm/research.html}}
}
@TechReport{MitGar:2001:TR:002,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Computation Slicing: Techniques and Theory}},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     2001,
  number =   {TR-PDS-2001-002},
  OPTaddress =   {Austin, TX 78712},
  month =    APR,
  note =         {Available at \texttt{http://www.cs.utexas.edu/users/neerajm}}
}
@TechReport{MitGar:2001:TR:005,
  author =   {N. Mittal and V. K. Garg},
  title =    {{A Rigorous Proof of $O(n^2)$ Bound on the Number of Moves
                  for Stabilization of Dijkstra's 3-State Algorithm}},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     {2001},
  OPTkey =   {},
  OPTtype =      {},
  number =   {TR-PDS-2001-005},
  address =      {Austin, TX 78712},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{MitGar:2003:ICDCS,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Software Fault Tolerance of Distributed Programs using Computation Slicing}},
  booktitle =    PROC # " 23rd " # ICDCS,
  pages =    {105-113},
  year =     2003,
  address =  {Providence, Rhode Island},
  month =    MAY
}
@TechReport{MitGar:2003:TR:15,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Techniques and Applications of Computation Slicing}},
  institution =  DCS # ", " # UTD,
  year =     2003,
  number =   {UTDCS-15-03},
  OPTaddress =   {Richardson, TX 75083},
  month =    APR
}
@Article{MitGar:2004:DC,
  author =   {N. Mittal and V. K. Garg},
  title =    {{Finding Missing Synchronization in a Distributed Computation using
                  Controlled Re-execution}},
  journal =      DC,
  year =     {2004},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTpages =     {},
  month =    MAR,
  note =     {Online First},
  OPTannote =    {}
}
@InProceedings{MitHsi:2000:ICDE,
  author =   {N. Mittal and H. Hsiao},
  title =    {{D}atabase {M}anaged {E}xternal {F}ile {U}pdate},
  booktitle =    PROC # " 17th " # ICDE,
  pages =    {557-564},
  year =     2001,
  address =  {Heidelberg, Germany},
  month =    APR
}
@InProceedings{MitSen+:2004:IPDPS,
  author =   {N. Mittal and A. Sen and V. K. Garg and R. Atreya},
  title =    {{Finding Satisfying Global States: All for One and One for All}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # IPDPS,
  OPTpages =     {},
  year =     {2004},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    APR,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{MitVen+:2004:DISC,
  author =   {N. Mittal and S. Venkatesan and S. Peri},
  title =    {{Message-Optimal and Latency-Optimal Termination Detection
                  Algorithms for Arbitrary Topologies}},
  booktitle =    PROC # " " # DISC,
  pages =        {290-304},
  year =     2004,
  address =      {Amsterdam, The Netherlands},
  month =    OCT
}
@TechReport{MitVen+:2004:TR,
  author =   {N. Mittal and S. Venkatesan and S. Peri},
  title =    {{Message-Optimal and Latency-Optimal Termination Detection
                  Algorithms for Arbitrary Topologies}},
  institution =  UTD,
  number =       {UTDCS-08-04},
  month =        FEB,
  year =     2004,
  note =     {Available at
                  \texttt{http://www.utdallas.edu/{\textasciitilde}neerajm/}}
}
@InProceedings{MurGar:1997:ICDCS,
  author =   {V. V. Murty and V. K. Garg},
  title =    {{C}haracterization of {M}essage {O}rdering
                  {S}pecifications and {P}rotocols},
  booktitle =    PROC # " 17th " # ICDCS,
  year =     1997,
  month =    MAY
}
@Article{Nas:1961:JLMS,
  author =   {C. Nash-Williams},
  title =    {{E}dge-{D}isjoint {S}panning {T}rees of {F}inite {G}raphs},
  journal =      JLMS,
  year =     1961,
  volume =   36,
  pages =    {445-450}
}
@InProceedings{NetBre+:1996:SPDT,
  author =   {R. Netzer and T. Brennan and S. Damodaran-Kamal},
  title =    {{D}ebugging {R}ace {C}onditions in
                  {M}essage-{P}assing {P}rograms},
  booktitle =    PROC # " " # SPDT,
  pages =    {31-40},
  year =     1996,
  month =    MAY
}
@Article{NetMil:1995:JS,
  author =   {R. H. B. Netzer and B. P. Miller},
  title =    {{O}ptimal {T}racing and {R}eplay for {D}ebugging
                  {M}essage-{P}assing {P}rograms},
  journal =  JS,
  year =     1995,
  volume =   8,
  number =   4,
  pages =    {371-388}
}
@Article{NetXu:1995:TPDS,
  author =   {R. H. B. Netzer and J. Xu},
  title =    {{N}ecessary and {S}ufficient {C}onditions for {C}onsistent
                  {G}lobal {S}napshots},
  journal =      TPDS,
  year =     1995,
  volume =   6,
  number =   2,
  pages =    {165-169},
  month =    FEB
}
@Unpublished{POTAwebsite,
  author =   {A. Sen and V. K. Garg},
  title =    {{P}artial {O}rder {T}race {A}nalyzer {(POTA)}},
  note =     {http://maple.ece.utexas.edu/{\textasciitilde}sen/POTA.html},
  OPTkey =   {},
  OPTmonth =     {},
  OPTyear =      {},
  OPTannote =    {}
}
@Article{PapWas+:1999:SIGMOD,
  author =   {M. Papiani and J. Wason and A. Dunlop and D. Nicole},
  title =    {{A} {D}istributed {S}cientific {A}rchive {U}sing the
                  {W}eb, {XML} and {SQL}/{MED}},
  journal =  {SIGMOD Record},
  volume =   {28},
  number =   {3},
  pages =    {56-62},
  month =    SEP,
  year =     {1999}
}
@Article{ParPop+:1983:TSE,
  author =   {D. S. Parker and G. J. Popek and G. Rudisin and A. Stoughton
                  and B. J. Walker and E. Walton and J. M. Chow and D. A. Edwards
                  and S. Kiser and C. S. Kline},
  title =    {{Detection of Mutual Inconsistency in Distributed Systems}},
  journal =      TSE,
  year =     {1983},
  OPTkey =   {},
  volume =   {9},
  number =   {3},
  pages =    {240-247},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{PerMit:2004:PDCS,
  author =   {S. Peri and N. Mittal},
  title =    {{On Termination Detection in an Asynchronous Distributed System}},
  booktitle =    PROC # " " # PDCS,
  pages =        {209-215},
  year =     2004,
  address =      {San Francisco, California},
  month =    SEP
}
@TechReport{PerMit:2004:TR,
  author =   {S. Peri and N. Mittal},
  title =    {{An Efficient Snapshot Protocol for a Dynamic System}},
  institution =  DCS # ", " # UTD,
  year =     {2004},
  OPTkey =   {},
  OPTtype =      {},
  OPTnumber =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@TechReport{PerMit:2004:TR:15,
  author =   {S. Peri and N. Mittal},
  title =    {{On Termination Detection in an Asynchronous Distributed System}},
  institution =  DCS # ", " # UTD,
  year =     {2004},
  OPTkey =   {},
  OPTtype =      {},
  number =   {UTDCS-15-04},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{PlaBec+:1995:UWTC,
  author =   {J. S. Plank and M. Beck and G. Kingsley},
  title =    {{Libckpt: Transparent Checkpointing under UNIX}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # UWTC,
  pages =    {213-223},
  year =     {1995},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {New Orleans, Louisiana},
  month =    JAN,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}
@Misc{Pom:2000:TUT,
  OPTkey =   {},
  author =   {W. Torres-Pomales},
  title =    {{S}oftware {F}ault {T}olerance: {A} {T}utorial},
  OPThowpublished = {},
  OPTmonth =     {},
  year =     {2000},
  note =     {NASA Langley Research Center},
  OPTannote =    {}
}
@InProceedings{PraSin:1994:SPDP,
  author =   {R. Prakash and M. Singhal},
  title =    {{Maximal Global Snapshot with Concurrent Initiators}},
  booktitle =    PROC # " 6th " # SPDP,
  pages =    {344-351},
  year =     1994,
  address =      {Dallas, Texas},
  month =    OCT
}
@InProceedings{QueSif:1982:ISP,
  author =       {J. P. Queille and J. Sifakis},
  title =        {{S}pecification and {V}erification of {C}oncurrent {S}ystems in {CESAR}},
  address =      {New York},
  booktitle =    PROC # " 5th " # ISP,
  pages =        {337-351},
  publisher =    SV,
  series =       LNCS,
  volume =       137,
  year =         1982
}
@Article{Ran:1983:IPL,
  author =   {S. P. Rana},
  title =    {{A Distributed Solution of the Distributed Termination
                   Problem}},
  journal =      IPL,
  year =     {1983},
  OPTkey =   {},
  volume =   {17},
  number =   {1},
  pages =    {43-46},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{RaoAlv+:2000:KDE,
  author =       {S. Rao and L. Alvisi and H. Vin},
  title =        {{T}he {C}ost of {R}ecovery in {M}essage {L}ogging {P}rotocols},
  journal =      KDE,
  volume =       {12},
  number =       {2},
  year =         {2000},
  pages =        {160-173},
}
@Book{Ray:1988:JWS,
  author =       {M. Raynal},
  title =        {{D}istributed {A}lgorithms and {P}rotocols},
  publisher =    JWS,
  year =         {1988}
}
@Article{Ray:1989:TrCS,
  author =   {K. Raymond},
  title =    {{A} {T}ree based {A}lgorithm for {D}istributed {M}utual {E}xclusion},
  journal =      TrCS,
  year =     1989,
  volume =   7,
  number =   1,
  pages =    {61-77}
}
@Article{RicAgr:1981:CACM,
  author =       {G. Ricart and A. K. Agrawala},
  title =        {{An Optimal Algorithm for Mutual Exclusion in Computer Networks}},
  journal =      CACM,
  volume =       {24},
  number =       {1},
  year =         {1981},
  pages =        {9-17},
  publisher =    {ACM Press},
  month =        JAN,
}
@Article{Riv:1974:AMS,
  author =   {I. Rival},
  title =    {{M}aximal {S}ublattices of {F}inite {D}istributive {L}attices {II}},
  journal =      PROC # " " # AMS,
  year =     1974,
  volume =   44,
  number =   2,
  pages =    {263-268}
}
@Book{STA,
  author =       {R. Stanley},
  title =        {{E}numerative {C}ombinatorics {V}olume 1},
  publisher =    {Wadsworth and Brookes/Cole},
  address =      {Monterey, California},
  year =         1986
}
@Unpublished{SafDij:1987:998,
  author =   {E. W. Dijkstra},
  title =    {{Shmuel Safra's Version of Termination Detection}},
  note =     {EWD Manuscript 998. Available at \texttt{http://www.cs.utexas.edu/users/EWD}},
  OPTkey =   {},
  OPTmonth =     {},
  year =     {1987},
  OPTannote =    {}
}
@TechReport{Sai:2002:TR:51,
  author =   {Y. Saito},
  title =    {{Unilateral Version Vector Pruning using Loosely Synchronized Clocks}},
  institution =  HPL,
  year =     {2002},
  OPTkey =   {},
  OPTtype =      {},
  number =   {HPL-2002-51},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@Article{SchGet:1987:TOG,
  author =       {R.W. Scheifler and J. Gettys},
  title =        {{The X Window System}},
  journal =      TOG,
  month =        APR,
  year =         1987,
  volume =       5,
  number =       2,
  pages =        {79-109}
}
@Article{SchMat:1994:DC,
  author =   {R. Schwartz and F. Mattern},
  title =    {{D}etecting {C}ausal {R}elationships in {D}istributed  {C}omputations:
                  {I}n {S}earch of the {H}oly {G}rail},
  journal =      DC,
  year =     1994,
  volume =   7,
  number =   3,
  pages =    {149-174}
}
@InProceedings{SchWyl:1991:SOSP,
  author =   {F. Schmuck and J. Wyllie},
  title =    {{Experience with Transactions in QuickSilver}},
  booktitle =    PROC # " 13th " # SOSP,
  pages =    {239-253},
  year =     1991,
  month =    OCT
}
@InProceedings{SenGar:2002:IPDPS,
  author =   {A. Sen and V. K. Garg},
  title =    {{D}etecting {T}emporal {L}ogic {P}redicates in the {H}appened-{B}efore {M}odel},
  booktitle =    PROC # " " # IPDPS,
  year =     2002,
  address =      {Florida},
  month =    APR
}
@TechReport{SenGar:2002:TR:001,
  author =   {A. Sen and V. K. Garg},
  title =    {{A}utomatic {G}eneration of {C}omputation {S}lices for
                  {D}etecting {T}emporal {L}ogic {P}redicates},
  institution =  PDS # ", " # DECE # ", " # UTA,
  year =     {2003},
  OPTkey =   {},
  OPTtype =      {},
  number =   {TR-PDS-2003-001},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}
@InProceedings{SenGar:2003:OPODIS,
  author =       {A. Sen and V. K. Garg},
  title =        {{Detecting Temporal Logic Predicates in Distributed
                   Programs using Computation Slicing}},
  booktitle =    PROC # " " # OPODIS,
  OPTpages =     {},
  month =        DEC,
  year =         {2003}
}
@InProceedings{SenGar:2003:RV,
  author =       {A. Sen and V. K. Garg},
  title =        {{P}artial {O}rder {T}race {A}nalyzer ({POTA}) for
                  {D}istributed {P}rograms},
  booktitle =    PROC # " Third " # RV,
  OPTseries =    {Electronic Notes in Theoretical Computer Science},
  volume =       {89},
  issue =        {2},
  publisher =    {Elsevier},
  year =         {2003}
}


@InProceedings{ShaFra:1986:ICALP,
  author =   {N. Shavit and N. Francez},
  title =    {{A New Approach to Detection of Locally Indicative Stability}},
  booktitle =    PROC # " " # ICALP,
  pages =    {344-358},
  year =     1986,
  address =      {Rennes, France}
}


@TechReport{ShaTou:1984:TR:624,
  author =   {A. Shah and S. Toueg},
  title =    {{Distributed Snapshots in spite of Failures}},
  institution =  DCS # ", " # CORNELL,
  year =     1984,
  number =   {TR84-624},
  address =      {Ithaca, NY},
  month =    JUL,
  note =     {(Revised February 1985)}
}


@InProceedings{SheDea:2002:WETICE,
  author =       {J. S. Sherif and T. G. Dearmond},
  title =        {{Intrusion Detection: Systems and Models}},
  booktitle =    PROC # " " # WETICE,
  pages =        {115-136},
  month =        JUN,
  year =         {2002},
  address =      {Pittsburgh, Pennsylvania}
}


@Book{SinShi:1994:Book,
  author =       {M. Singhal and N. G. Shivaratri},
  title =        {{Advanced Concepts in Operating Systems}},
  publisher =    MH # " and " # MIT,
  year =         {1994},
  ISBN =         {0-07-057572-X}
}

@InProceedings{SkaMit+:1999:PDCS,
  author =   {C. Skawratananond and N. Mittal and V. K. Garg},
  title =    {{A} {L}ightweight {A}lgorithm for {C}ausal {M}essage
                  {O}rdering in {M}obile {C}omputing {S}ystems},
  booktitle =    PROC # " 12th " # PDCS,
  pages =    {245-250},
  year =     {1999},
  address =      {Florida}
}


@Unpublished{SolDes,
  author =   {Solar Designer},
  title =    {{Root Programs and Links}},
  note =     {Available at \texttt{http://www.openwall.com/linux/}},
  OPTkey =   {},
  OPTmonth =     {},
  OPTyear =      {},
  OPTannote =    {}
}


@Unpublished{SolDes:OP,
  author =   {Openwall Project},
  title =    {{Linux Kernel Patch}},
  note =     {\textsf{http://www.openwall.com/linux}},
  OPTkey =   {},
  OPTmonth =     {},
  OPTyear =      {},
  OPTannote =    {}
}


@InProceedings{SpeKea:1986:ICDCS,
  author =   {M. Spezialetti and P. Kearns},
  title =    {{Efficient Distributed Snapshots}},
  booktitle =    PROC # " 6th " # ICDCS,
  pages =    {382-388},
  year =     1986
}


@Article{SpiBra:1987:DAM,
  author =   {J. Spinrad and A. Brandstadt and L. Stewart},
  title =    {{Bipartite Permutation Graphs}},
  journal =      DAM,
  year =     1987,
  volume =   18,
  pages =    {279-292}
}



@InProceedings{SriSiv:2002:ICPDCS,
  author =   {N. Sridhar and P. A. G. Sivilotti},
  title =    {{L}azy {S}napshots},
  booktitle =    PROC # " 14th " # ICPDCS,
  pages =    {96-101},
  year =     {2002},
  OPTeditor =    {S.G. Akl and T.Gonzalez},
  address =      {Cambridge, MA},
  month =    NOV,
  OPTorganization = {IASTED},
  OPTpublisher =    {ACTA Press},
  OPTurl =          {http://citeseer.nj.nec.com/sridhar02lazy.html}
}



@InProceedings{SroSch+:1998:WNTS,
  author =   {J. Srouji and P. Schuster and M. Bach and Y. Kuzmin},
  title =    {{A Transparent Checkpoint Facility on NT}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 2nd " # WNTS,
  OPTpages =     {},
  year =     {1998},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Seattle, Washington},
  month =    {August},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@Book{Sta:2001:PH,
  author =   {W. Stallings},
  title =    {{O}perating {S}ystems: {I}nternals and {D}esign {P}rinciples},
  publisher =    PH,
  year =     2001
}




@InCollection{StoLiu:1998:CAV,
  author =   {S. D. Stoller and Y. A. Liu},
  title =    {{E}fficient {S}ymbolic {D}etection of {G}lobal
                  {P}roperties in {D}istributed {S}ystems},
  booktitle =    PROC # " 10th " # CAV,
  pages =    {357-368},
  publisher =    {Springer-Verlag},
  year =     1998,
  editor =   {Alan J. Hu and Moshe Y. Vardi},
  volume =   1427,
  series =   LNCS
}



@InProceedings{StoSch:1995:WDAG,
  author =   {S. D. Stoller and F. Schneider},
  title =    {{F}aster {P}ossibility {D}etection by {C}ombining
                  {T}wo {A}pproaches},
  booktitle =    PROC # " " # WDAG,
  pages =        {318-332},
  year =     1995,
  volume =       {972},
  series =       LNCS,
  address =  {France},
  month =    SEP
}


@InProceedings{StoUnn+:2000:CAV,
  author =   {S. D. Stoller and L. Unnikrishnan and Y. A. Liu},
  title =    {{Efficient Detection of Global Properties in
                  Distributed Systems Using Partial-Order Methods}},
  booktitle =    PROC # " 12th " # CAV,
  pages =    {264-279},
  year =     2000,
  volume =   1855,
  series =   LNCS,
  month =    JUL,
  publisher =    {Springer-Verlag}
}



@InProceedings{Stu:2002:DISC,
  author =   {G. Stupp},
  title =    {{Stateless Termination Detection}},
  booktitle =    PROC # " 16th " # DISC,
  pages =    {163-172},
  year =     2002,
  address =      {Toulouse, France}
}


@InProceedings{Tai:1997:ICDCS,
  author =   {K. Tai},
  title =    {{R}ace {A}nalysis of {T}races of {A}synchronous
                  {M}essage-{P}assing {P}rograms},
  booktitle =    PROC # " 17th " # ICDCS,
  pages =    {261-268},
  year =     1997
}



@PhdThesis{Tar:2000:Thesis,
  author =   {A. Tarafdar},
  title =    {{S}oftware {F}ault {T}olerance in {D}istributed {S}ystems
                  {U}sing {C}ontrolled {R}e-execution},
  school =   {The University of Texas at Austin},
  year =     2000,
  month =    AUG
}


@InProceedings{TarGar:1998:ICDCS,
  author =   {A. Tarafdar and V. K. Garg},
  title =    {{A}ddressing {F}alse {C}ausality while {D}etecting
                  {P}redicates in {D}istributed {P}rograms},
  booktitle =    PROC # " 9th " # ICDCS,
  pages =    {94-101},
  year =     1998,
  address =  {Amsterdam, The Netherlands},
  month =    MAY
}

@InProceedings{TarGar:1998:SPDP,
  author =   {A. Tarafdar and V. K. Garg},
  title =    {{P}redicate {C}ontrol for {A}ctive {D}ebugging of
                  {D}istributed {P}rograms},
  booktitle =    PROC # " 9th " # SPDP,
  pages =        {763-769},
  year =     1998,
  address =  {Orlando}
}

@InProceedings{TarGar:1999:DISC,
  author =   {A. Tarafdar and V. K. Garg},
  title =    {{S}oftware {F}ault {T}olerance of {C}oncurrent
                  {P}rograms {U}sing {C}ontrolled {R}e-execution},
  booktitle =    PROC # " 13th " # DISC,
  pages =    {210-224},
  year =     1999,
  address =  {Bratislava, Slovak Republic},
  month =    SEP
}


@Book{Tel:2000:CUP,
  author =   {G. Tel},
  title =    {{Introduction to Distributed Algorithms}},
  publisher =    CUP # "~(US Server)",
  year =     2000,
  edition =      {Second},
  month =    SEP
}

@Article{TelMat:1993:TOPLAS,
  author =   {G. Tel and F. Mattern},
  title =    {{The Derivation of Distributed Termination Detection Algorithms from Garbage Collection Schemes}},
  journal =      TOPLAS,
  year =     1993,
  volume =   15,
  number =   1,
  pages =    {1-35},
  month =    JAN
}



@Article{Tip:1995:JPL,
  author =   {F. Tip},
  title =    {{A Survey of Program Slicing Techniques}},
  journal =      JPL,
  year =     1995,
  volume =   3,
  number =   3,
  pages =    {121-189}
}

@InProceedings{TomGar:1993:WPDS,
  author =   {A. I. Tomlinson and V. K. Garg},
  title =    {{An Algorithm for Minimally Latent Global Virtual Time}},
  booktitle =    PROC # " 7th " # WPDS,
  pages =        {35-42},
  year =     1993,
  address =  {San Diego, California},
  month =    MAY
}


@InProceedings{TomGar:1994:CSE,
  author =   {A. I. Tomlinson and V. K. Garg},
  title =    {{Maintaining Global Assertions in Distributed Systems}},
  booktitle =    CSE,
  pages =    {257-272},
  year =     1994,
  publisher =    TMH
}


@Article{TomGar:1994:JPDC,
  author =   {A. I. Tomlinson and V. K. Garg},
  title =    {{M}onitoring {F}unctions on {G}lobal {S}tates of
                  {D}istributed {P}rograms},
  journal =  JPDC,
  year =     1997,
  volume =       {41},
  number =       {},
  pages  =       {173-189},
  month =        MAR,
  OPTnote =  "A revised version of ``Detecting Relational Global
                  Predicates in Distributed Systems'', In " # PROC #
                  " " # WPDD # ", San Diego, California, " # MAY # "
                  1993, pages 21-31"
}


@InProceedings{TomGar:1995:FSTTCS,
  author =       {A. I. Tomlinson and V. K. Garg},
  title =        {{Observation of Software for Distributed Systems with RCL}},
  booktitle =    PROC # " 15th " # FSTTCS,
  pages =        {195-209},
  year =         {1995},
  url =          {http://citeseer.nj.nec.com/tomlinson95observation.html}
}

@Article{TomGar:1997:JPDC,
  author =   {A. I. Tomlinson and V. K. Garg},
  title =    {{M}onitoring {F}unctions on {G}lobal {S}tates of
                  {D}istributed {P}rograms},
  journal =  JPDC,
  year =     1997,
  volume =       {41},
  number =       {2},
  pages  =       {173-189},
  month =        MAR,
  OPTnote =  "A revised version of ``Detecting Relational Global
                  Predicates in Distributed Systems'', In " # PROC #
                  " " # WPDD # ", San Diego, California, " # MAY # "
                  1993, pages 21-31"
}


@Book{Tro:1992:JHUP,
  author =   {W. T. Trotter},
  title =    {{C}ombinatorics and {P}artially {O}rdered {S}ets: {D}imension {T}heory},
  publisher =    JHUP,
  year =     1992,
  address =      {Baltimore, MD}
}

@article{Tse:1995:JPDC,
  author =       {Y.-C. Tseng},
  title =        {{Detecting Termination by Weight-Throwing in a Faulty Distributed System}},
  journal =      JPDC,
  volume =       {25},
  number =       {1},
  pages =        {7-15},
  year =         "1995",
  OPTnote =      "previous label was Tse:1992:JPDC"
}

@Article{TseTan:2001:TPDS,
  author =       {Y.-C. Tseng and C.-C. Tan},
  title =        {{On Termination Detection Protocols in a Mobile Distributed
                   Computing Environment}},
  journal =      TPDS,
  year =         2001,
  volume =       12,
  number =       6,
  pages =        {558-566}
}


@InProceedings{TsyYee:2003:USS,
  author =   {E. Tsyrklevich and B. Yee},
  title =    {{Dynamic Detection and Prevention of Race Conditions in File Accesses}},
  booktitle =    PROC # " 12th " # USS,
  pages =    {243-255},
  year =     2003,
  month =    AUG
}

@Article{Tur:1984:DAM,
  author =   {G. Turan},
  title =    {{Succinct Representations of Graphs}},
  journal =      DAM,
  year =     1984,
  volume =   8,
  pages =    {289-294}
}

@Book{Vah:1996:PH,
  author =   {U. Vahalia},
  title =    {Unix Internals: The New Frontiers},
  publisher =    PH,
  year =     1996,
  month =    JAN
}

@Article{ValTar+:1982:SIAMJC,
  author =   {J. Valdes and R. E. Tarjan and E. L. Lawler},
  title =    {{T}he {R}ecognition of {S}eries-{P}arallel {D}igraphs},
  journal =      SIAMJC,
  year =     1982,
  volume =   11,
  pages =    {298-314}
}

@Article{Ven:1989:TR,
  author =   {S. Venkatesan},
  title =    {{Reliable Protocols for Distributed Termination Detection}},
  journal =      TR,
  year =     1989,
  volume =   38,
  number =   1,
  pages =    {103-110},
  month =    APR
}




@Article{Ven:1995:TOPLAS,
  author =   {G. Venkatesh},
  title =    {{Experimental Results from Dynamic Slicing of C Programs}},
  journal =      TOPLAS,
  year =     1995,
  volume =   17,
  number =   2,
  pages =    {197-216}
}







@Article{SuzKas:1985:TrCS,
  author =   {I. Suzuki and T. Kasami},
  title =    {{A Distributed Mutual Exclusion Algorithm}},
  journal =      TrCS,
  year =     1985,
  volume =   3,
  number =   4,
  pages =    {344-349}
}



@Article{VenDat:1995:TSE,
  author =   {S. Venkatesan and B. Dathan},
  title =    {{T}esting and {D}ebugging {D}istributed {P}rograms {U}sing
                  {G}lobal {P}redicates},
  journal =      TSE,
  year =     1995,
  volume =   21,
  number =   2,
  pages =    {163-177},
  month =    FEB
}


@InProceedings{VieBlo+:2000:CSAC,
  author =   {J. Viega, J. Bloch, T. Kohno and G. McGraw},
  title =    {{ITS4: A Static Vulnerability Scanner for C and C++ Code}},
  booktitle =    PROC # " " # CSAC,
  year =     2000,
  month =    DEC
}


@InProceedings{WalGar:1991:WPDD,
  author =       {B. Waldecker and V. K. Garg },
  title =        {{U}nstable {P}redicate {D}etection in {D}istributed
                  {P}rogram {D}ebugging},
  booktitle =    PROC # " " # WPDD,
  address =  {Santa Cruz, California},
  pages =        {276-278},
  month =    MAY,
  year =     1991
}

@Article{Wan:1997:TC,
  author =   {Y.-M. Wang},
  title =    {{C}onsistent {G}lobal {C}heckpoints that {C}ontain a
                  {G}iven {S}et of {L}ocal {C}heckpoints},
  journal =      TC,
  year =     1997,
  volume =   46,
  number =   4,
  pages =    {456-468},
  month =    APR
}


@InProceedings{WanDam+:1997:ICDCS,
  author =       {Y. M. Wang and O. P. Damani and V. K. Garg},
  title =        {{D}istributed {R}ecovery with {K}-{O}ptimistic Logging},
  pages =        {60-67},
  booktitle =    PROC # " 17th " # ICDCS,
  address =      {Baltimore, Maryland},
  month =        JUN,
  publisher =    {IEEE},
  address =  {Washington - Brussels - Tokyo},
  year =         1997,
}



@Article{WanHua+:1997:TC,
  author =   {Y.-M. Wang and Y. Huang and W. K. Fuchs and
                  C. Kintala and G. Suri},
  title =    {{P}rogressive {R}etry for {S}oftware {F}ailure
                  {R}ecovery in {M}essage-{P}assing {A}pplications},
  journal =  TC,
  year =     1997,
  volume =   46,
  number =   10,
  pages =    {1137-1141},
  month =    OCT
}



@InProceedings{WanMay:2004:IPDPS,
  author =   {X. Wang and J. Mayo},
  title =    {{A General Model for Detecting Termination in Dynamic Systems}},
  booktitle =    PROC # " 18th " # IPDPS,
  year =     2004,
  address =      {Santa Fe, New Mexico},
  month =    APR
}


@Article{Wei:1982:CACM,
  author =   {M. Weiser},
  title =    {{P}rogrammers {U}se {S}lices when {D}ebugging},
  journal =  CACM,
  year =     1982,
  volume =   25,
  number =   7,
  pages =    {446-452}
}

@Article{WuJou:2000:CDS,
  author =   {K.-P. Wu and Y.-J. Joung},
  title =    {{Asynchronous Group Mutual Exclusion in Ring Networks}},
  OPTcrossref =  {},
  OPTkey =   {},
  journal =      CDS,
  pages =    {1-8},
  year =     {2000},
  OPTeditor =    {},
  volume =   {147},
  number =   {1}
}



@Article{Yan:1982:SIAMHADM,
  author =   {M. Yannakakis},
  title =    {{T}he {C}omplexity of the {P}artial {O}rder {D}imension {P}roblem},
  journal =      SIAMJADM,
  year =     1982,
  volume =   3,
  pages =    {351-358}
}




@InProceedings{ZibGil:1997:OOPSLA,
  author =   {Y. Zibin and Y. Gil},
  title =    {{E}fficient {S}ubtyping {T}ests with {PQ}-{E}ncoding},
  booktitle =    PROC # " 16th Annual " # OOPSLA,
  pages =    {96-107},
  year =     1997,
  address =      {Tampa Bay, Florida},
  month =    OCT
}

@Manual{iFS:1999,
  author =   {Oracle},
  title =    {iFS: Oracle Internet File System},
  note =     {\\ {\sf
                  http://www.oracle.com/database/options/ifs.html}},
  year =     1999
}

@InProceedings{WuLai+:1992:ICPADS,
  author =   {L.-F. Wu and T.-H. Lai and Y.-C. Tseng},
  title =    {{Consensus and Termination Detection in the Presence of Faulty Processes}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICPADS,
  pages =    {267-274},
  year =     {1992},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {Hsinchu, Taiwan},
  month =    DEC,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{DwoLyn+:1988:JACM,
  author =       {C. Dwork and N. Lynch and L. Stockmeyer},
  title =        {{Consensus in the presence of partial synchrony}},
  OPTcrossref =  "",
  OPTkey =       "",
  journal =      JACM,
  year =         "1988",
  volume =       "35",
  number =       "2",
  pages =        {288-323},
  month =        APR,
  OPTnote =      "",
  annote =       "The authors study practically motivated models of
                  synchrony that lie between fully asynchronous and
                  fully synchronous systems in which consensus shall
                  be achieved. The models of partial synchrony studied
                  include: (1) upper bounds on processor speeds and
                  message latency exist but are unknown, and (2) upper
                  bounds exists and are known, but only hold after
                  some unknown time (eventually). In both cases
                  consensus with different resiliency can be achieved."
}


@InProceedings{DelFau+:2004:PODC,
  author =   {C. Delporte-Gallet and H. Fauconnier and R. Guerraoui and
                  V. Hadzilacos and P. Kouznetsov and S. Toueg},
  title =    {{The Weakest Failure Detector to Solve Certain Fundamental Problems
                   in Distributed Computing}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # PODC,
  OPTpages =     {},
  year =     {2004},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  address =      {St. Johns, Newfoundland, Canada},
  month =    JUL,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{MitGae+:2004:TR:37,
  author =   {N. Mittal and F. G{\"a}rtner and S. Venkatesan and L. D. Penso},
  title =    {{ Detecting Termination in a Crash-Prone Distributed System}},
  institution =  DCS # ", " # UTD,
  year =     {2004},
  OPTkey =   {},
  OPTtype =      {},
  number =   {UTDCS-37-04},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{HurMiz+:1998:TSE,
  author =       {M. Hurfin and M. Mizuno and M. Singhal and M. Raynal},
  title =        {Efficient Distributed Detection of Conjunctions of Local Predicates},
  journal =      TSE,
  volume =       {24},
  number =       {8},
  year =         {1998},
  issn =         {0098-5589},
  pages =        {664--677},
  doi =          {http://dx.doi.org/10.1109/32.707701},
  publisher =    {IEEE Press},
}

@Book{Lyn:1996:MK,
  author =   {N. Lynch},
  OPTeditor =    {},
  title =    {{Distributed Algorithms}},
  publisher =    MK,
  year =     {1996},
  OPTkey =   {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTedition =   {},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{Awe:1987:STOC,
  author =       {B. Awerbuch},
  title =        {{Optimal Distributed Algorithms for Minimum Weight Spanning Tree, Counting,
                   Leader Election, and Related Problems}},
  booktitle =    PROC # " 19th " # STOC,
  year =         {1987},
  pages =        {230-240},
  address =      {New York, New York, United States},
  publisher =    {ACM Press},
}

@Article{SchSan:1994:DC,
  author =   {A. Schiper and A. Sandoz},
  title =    {{Strong Stable Properties in Distributed Systems}},
  journal =      DC,
  year =     {1994},
  OPTkey =   {},
  volume =   {8},
  number =   {2},
  pages =    {93-103},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@TechReport{SinKal+:1993:TR:93-11,
  author =   {A. Sinha and L. Kal{\'e} and B. Ramkumar},
  title =    {{A Dynamic and Adaptive Quiescence Detection Algorithm}},
  institution =  PPL # ", " #  DCS # ", "  # UIUC,
  year =     {1993},
  OPTkey =   {},
  OPTtype =      {},
  number =   {93-11},
  OPTaddress =   {Urbana-Champaign, IL 61801},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ChaMis:1986:TOPLAS,
  author =   {K. M. Chandy and J. Misra},
  title =    {{An Example of Stepwise Refinement of Distributed Programs: Quiescence Detection}},
  journal =      TOPLAS,
  year =     {1986},
  OPTkey =   {},
  volume =   {8},
  number =   {3},
  pages =    {326-343},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{KshSin:1994:TSE,
  author =   {A. D. Kshemkalyani and M. Singhal},
  title =    {{Efficient Detection and Resolution of Generalized Distributed Deadlocks}},
  journal =      TSE,
  year =     {1994},
  OPTkey =   {},
  volume =   {20},
  number =   {1},
  pages =    {43-54},
  month =    JAN,
  OPTnote =      {},
  OPTannote =    {}
}



@Article{BraTou:1987:DC,
  author =   {G. Bracha and S. Toueg},
  title =    {{Distributed Deadlock Detection}},
  journal =      DC,
  year =     {1987},
  OPTkey =   {},
  volume =   {2},
  number =   {3},
  pages =    {127-138},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Kna:1987:CS,
  author =   {E. Knapp},
  title =    {{Deadlock Detection in Distributed Databases}},
  journal =      CS,
  year =     {1987},
  OPTkey =   {},
  volume =   {19},
  number =   {4},
  pages =    {303-328},
  month =    DEC,
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{LynMal+:2002:WPPS,
  author =   {N. Lynch and D. Malkhi and D. Ratajczak},
  title =    {{Atomic Data Access in Content Addressable Networks}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 1st " # WPPS,
  pages =    {295-305},
  year =     {2002},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    MAR,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{LiMis+:2004:DISC,
  author =   {X. Li and J. Misra and C. G. Plaxton},
  title =    {{Active and Concurrent Topology Maintenance}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # DISC,
  OPTpages =     {},
  year =     {2004},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{ZhaHua+:2003:SAC,
  author =   {B. Y. Zhao and L. Huang and J. Stribling and S. C. Rhea and A. D. Joseph and J. Kubiatowicz},
  title =    {{Tapestry: A Resilient Global-Scale Overlay for Service Deployment}},
  journal =      SAC,
  year =     {2003},
  OPTkey =   {},
  volume =   {22},
  number =   {1},
  pages =    {41-53},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{StoMor+:2003:TN,
  author =   {I. Stoica and R. Morris and D. Liben-Nowell and D. R. Karger and M. F. Kaashoek
                  and F. Dabek and H. Balakrishnan},
  title =    {{Chord: A Scalable Peer-to-Peer Lookup Service for Internet Applications}},
  journal =      TN,
  year =     {2003},
  OPTkey =   {},
  volume =   {11},
  number =   {1},
  pages =    {17-32},
  month =    FEB,
  OPTnote =      {},
  OPTannote =    {}
}

@InProceedings{AspSha:2003:SDA,
  author =   {J. Aspnes and G. Shah},
  title =    {{Skip Graphs}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " 14th Annual " # SDA,
  pages =    {384-393},
  year =     {2003},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    JAN,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{BanMay:2004:SIU,
  author =   {S. Bansod and J. Mayo},
  title =    {{A Distributed Algorithm for Unstable Global Predicate Evaluation with Approximately Synchronized Clocks}},
  journal =      SIU,
  year =     {2004},
  OPTkey =   {},
  volume =   {3},
  number =   {2},
  pages =    {151-168},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Unpublished{AgaGar:2004:TR,
  author =   {A. Agarwal and V. K. Garg},
  title =    {{Chain Clock: Efficient Causality Tracking for Shared Memory Systems}},
  note =     "Submitted to the " # ICDCS,
  OPTkey =   {},
  month =    JUN,
  year =     {2005},
  OPTannote =    {}
}



@Article{Lee:2004:TSE,
  author =   {S. Lee},
  title =    {{Fast, Centralized Detection and Resolution of Distributed Deadlocks in the
                   Generalized Model}},
  journal =      TSE,
  year =     {2004},
  OPTkey =   {},
  volume =   {30},
  number =   {9},
  pages =    {561-573},
  month =    SEP,
  OPTnote =      {},
  OPTannote =    {}
}


@Article{BouTro:1998:TPDS,
  author =   {A. Boukerche and C. Tropper},
  title =    {{A Distributed Graph Algorithm for the Detection of Local Cycles and Knots}},
  journal =      TPDS,
  year =     {1998},
  OPTkey =   {},
  volume =   {9},
  number =   {8},
  pages =    {748-757},
  month =    AUG,
  OPTnote =      {},
  OPTannote =    {}
}



@InProceedings{CheDen+:1996:ICDCS,
  author =   {S. Chen and Y. Deng and P. C. Attie and W. Sun},
  title =    {{Optimal Deadlock Detection in Distributed Systems based on
                   Locally Constructed Wait-For Graphs}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICDCS,
  pages =    {613-619},
  year =     {1996},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  month =    MAY,
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}



@Article{Hol:1972:CS,
  author =   {R. C. Holt},
  title =    {{Some Deadlock Properties of Computer Systems}},
  journal =      CS,
  year =     {1972},
  OPTkey =   {},
  volume =   {4},
  OPTnumber =    {},
  pages =    {179-195},
  month =    SEP,
  OPTnote =      {},
  OPTannote =    {}
}


@Article{KshSin:1999:KDE,
  author =   {A. D. Kshemkalyani and M. Singhal},
  title =    {{A One-Phase Algorithm to Detect Distributed Deadlocks in
                   Replicated Databases}},
  journal =      KDE,
  year =     {1999},
  OPTkey =   {},
  volume =   {11},
  number =   {6},
  pages =    {880-895},
  month =    NOV,
  OPTnote =      {},
  OPTannote =    {}
}


@InProceedings{ManSin:2002:ICPP,
  author =   {D. Manivannan and M. Singhal},
  title =    {{A Distributed Algorithm for Knot Detection in a Distributed Graph}},
  OPTcrossref =  {},
  OPTkey =   {},
  booktitle =    PROC # " " # ICPP,
  OPTpages =     {},
  year =     {2002},
  OPTeditor =    {},
  OPTvolume =    {},
  OPTnumber =    {},
  OPTseries =    {},
  OPTaddress =   {},
  OPTmonth =     {},
  OPTorganization = {},
  OPTpublisher = {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{ManSin:2003:TPDS,
  author =   {D. Manivannan and M. Singhal},
  title =    {{An Efficient Distributed Algorithm for Detecting Knots and
                   Cycles in a Distributed Graph}},
  journal =      TPDS,
  year =     {2003},
  OPTkey =   {},
  volume =   {14},
  OPTnumber =    {10},
  pages =    {961-972},
  month =    OCT,
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Sin:1989:Com,
  author =   {M. Singhal},
  title =    {{Deadlock Detection in Distributed Systems}},
  journal =      Com,
  year =     {1989},
  OPTkey =   {},
  volume =   {22},
  OPTnumber =    {},
  pages =    {37-48},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}


@Article{KshSin:1994:JPDC,
  author =   {A. D. Kshemkalyani and M. Singhal},
  title =    {{On Characterization and Correctness of Distributed Deadlock Detection}},
  journal =      JPDC,
  year =     {1994},
  OPTkey =   {},
  volume =   {22},
  number =   {1},
  pages =    {44-59},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@Article{JagVas:1983:TSE,
  author =   {J. R. Jagannathan and R. Vasudevan},
  title =    {{Comments on ``Protocols for Deadlock Detection in
                  Distributed Database Systems''}},
  journal =      TSE,
  year =     {1983},
  OPTkey =   {},
  volume =   {9},
  number =   {3},
  pages =    {371},
  month =    MAY,
  OPTnote =      {},
  OPTannote =    {}
}

@Article{Awe:1985:JACM,
  author =   {B. Awerbuch},
  title =    {{Complexity of Network Synchronization}},
  journal =      JACM,
  year =     {1985},
  OPTkey =   {},
  volume =   {32},
  number =   {4},
  pages =    {804-823},
  OPTmonth =     {},
  OPTnote =      {},
  OPTannote =    {}
}

@inproceedings{XiaPlax:2002:POMC,
 author = {Xiaozhou Li and C. Greg Plaxton},
 title = {On name resolution in peer-to-peer networks},
 booktitle = {POMC '02: Proceedings of the second ACM international workshop on Principles of mobile computing},
 year = {2002},
 isbn = {1-58113-511-4},
 pages = {82--89},
 location = {Toulouse, France},
 doi = {http://doi.acm.org/10.1145/584490.584507},
 publisher = {ACM Press},
 address = {New York, NY, USA},
 }

@URL{dist,
  author =       {},
  title =        "www.distributed.net/rc5",
  howpublished = {},
  year =         "2002",
  month =        "Dec",
  note =         {},
  abstract =     {},
  keywords =     {},
  source =       {},
  file = F
}

@CONFERENCE{SatNeer:2005:FSTTCS,
  author =       {Sathya Peri and Neeraj Mittal},
  title =        {Monitoring Stable Properties in Dynamic Peer-to-Peer Distributed Systems},
  booktitle =    PROC # " 25th " # FSTTCS,
  year =         {2005},
  pages  =       {420-431},
  address =      {Hyderabad, India},
  month =        {December},
  note =         {},
  key =          {},
  crossref =     {},
  annote =       {},
}

@TECHREPORT{BalHelPier:2004:TR,
  AUTHOR =       {R. Baldoni and J. Helary and S. Tucci Piergiovanni},
  TITLE =        {Maintaining group connectivity in dynamic asynchronous distributed systems},
  INSTITUTION =  {``Dipartimento di Informatica e Sistemistica, A.Ruberti, Universit?? di Roma la Sapienza"},
  YEAR =         {2004},
  doi=           {"http://www.dis.uniroma1.it/~midlab"},
}

@article{PageJacChen:1993:TPDS,
 author = {I. Page and T. Jacob and E. Chern},
 title = {Fast Algorithms for Distributed Resource Allocation},
 journal = {IEEE Trans. Parallel Distrib. Syst.},
 volume = {4},
 number = {2},
 year = {1993},
 issn = {1045-9219},
 pages = {188--197},
 doi = {http://dx.doi.org/10.1109/71.207594},
 publisher = {IEEE Press},
 address = {Piscataway, NJ, USA},
}

@article{ChoiSing:1995:TOPLAS,
 author = {Manhoi Choy and Ambuj K. Singh},
 title = {Efficient fault-tolerant algorithms for distributed resource allocation},
 journal = {ACM Trans. Program. Lang. Syst.},
 volume = {17},
 number = {3},
 year = {1995},
 issn = {0164-0925},
 pages = {535--559},
 doi = {http://doi.acm.org/10.1145/203095.203101},
 publisher = {ACM Press},
 address = {New York, NY, USA},
 }

@TECHREPORT{SatNeer:2006:TR,
  AUTHOR =       {Sathya Peri and Neeraj Mittal},
  TITLE =        {Lower bounds on Departures for Dynamic Asynchronous Peer-to-Peer systems},
  INSTITUTION =  {University of Texas at Dallas},
  YEAR =         {2006},
}

@INPROCEEDINGS{WeidPagPerv:1991:SPDP,
  AUTHOR =       {Weidman.E.B and Page.I.P and Pervin.W.J},
  TITLE =        {{Explicit dynamic exclusion algorithm}},
  BOOKTITLE =    {Proceedings of the Third IEEE Symposium on Parallel and Distributed Processing},
  YEAR =         {1991},
  pages =        {142-149},
  month =        {DEC},
  organization = {IEEE},
}

@INPROCEEDINGS{LynMalRata:2002:IPTPS,
  AUTHOR =       {N. Lynch and D. Malkhi and D. Ratajczak},
  TITLE =        {{Atomic Data Access in Content Addressable Networks}},
  BOOKTITLE =    {Proceedings for the 1st International Workshop on Peer-to-Peer Systems (IPTPS '02)},
  YEAR =         {2002},
  month =        {Mar},
  publisher =    {Springer-Verlag},
}
%% Citations included by Sat in the area of STMs

@article{HerlMoss:1993:SigArch,
 author = {Maurice Herlihy and J. Eliot B.Moss },
 title = {{Transactional memory: {A}rchitectural {S}upport for {L}ock-{F}ree {D}ata {S}tructures}},
 journal = {SIGARCH Comput. Archit. News},
 volume = {21},
 number = {2},
 year = {1993},
 issn = {0163-5964},
 pages = {289--300},
 doi = {},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{ShavTou:1995:PODC,
 author = {Shavit, Nir and Touitou, Dan},
 title = {{{S}oftware {T}ransactional {M}emory}},
 booktitle = {PODC},
 year = {1995},
 isbn = {0-89791-710-3},
 pages = {204--213},
 location = {Ottowa, Ontario, Canada},
 doi = {},
 publisher = {},
 address = {},
 }

@inproceedings{Harretal:2005:PPoPP,
 author = {Tim Harris and Simon Marlow and Simon Peyton-Jones and Maurice Herlihy},
 title = {{Composable memory transactions}},
 booktitle = {PPoPP},
 year = {2005},
 isbn = {1-59593-080-9},
 pages = {48--60},
 location = {Chicago, IL, USA},
 doi = {},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{Yangetal:2007:PPoPP,
 author = {Ni, Yang and Menon, Vijay S. and Adl-Tabatabai, Ali-Reza and Hosking, Antony L. and Hudson, Richard L. and Moss, J. Eliot B. and Saha, Bratin and Shpeisman, Tatiana},
 title = {{Open nesting in software transactional memory}},
 booktitle = {PPoPP},
 year = {2007},
 isbn = {978-1-59593-602-8},
 pages = {68--78},
 location = {San Jose, California, USA},
 doi = {http://doi.acm.org/10.1145/1229428.1229442},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{AgarLeiSukh:2006:MSPC,
 author = {Agrawal, Kunal and Leiserson, Charles E. and Sukha, Jim},
 title = {{Memory models for open-nested transactions}},
 booktitle = {MSPC '06: Proceedings of the 2006 workshop on Memory system performance and correctness},
 year = {2006},
 isbn = {1-59593-578-9},
 pages = {70--81},
 location = {San Jose, California},
 doi = {http://doi.acm.org/10.1145/1178597.1178610},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@article{MossAnt:2006:SCP,
 author = {Moss, J. Eliot B. and Hosking, Antony L.},
 title = {{Nested transactional memory: model and architecture sketches}},
 journal = {Sci. Comput. Program.},
 volume = {63},
 number = {2},
 year = {2006},
 issn = {0167-6423},
 pages = {186--201},
 doi = {http://dx.doi.org/10.1016/j.scico.2006.05.010},
 publisher = {Elsevier North-Holland, Inc.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 }

@inproceedings{AgarFinSukh:2008:PPoPP,
 author = {Agrawal, Kunal and Fineman, Jeremy T. and Sukha, Jim},
 title = {{Nested parallelism in transactional memory}},
 booktitle = {PPoPP '08: Proceedings of the 13th ACM SIGPLAN Symposium on Principles and practice of parallel programming},
 year = {2008},
 isbn = {978-1-59593-795-7},
 pages = {163--174},
 location = {Salt Lake City, UT, USA},
 doi = {http://doi.acm.org/10.1145/1345206.1345232},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{Moretal:2006:ASPLOS,
 author = {Moravan, Michelle J. and Bobba, Jayaram and Moore, Kevin E. and Yen, Luke and Hill, Mark D. and Liblit, Ben and Swift, Michael M. and Wood, David A.},
 title = {{Supporting nested transactional memory in logTM}},
 booktitle = {ASPLOS-XII: Proceedings of the 12th international conference on Architectural support for programming languages and operating systems},
 year = {2006},
 isbn = {1-59593-451-0},
 pages = {359--370},
 location = {San Jose, California, USA},
 doi = {http://doi.acm.org/10.1145/1168857.1168902},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@Article{Moss:2006:MPI,
	author = {J.E.B.Moss},
	journal = {In Workshop on Memory Performance Issues},
	year = {2006},
	title = {{Open Nested Transactions: Semantics and Support}}
}


@inproceedings{GuerKap:Opacity:PPoPP:2008,
 author = {Guerraoui, Rachid and Kapalka, Michal},
 title = {On the Correctness of Transactional Memory},
 booktitle = {Proceedings of the 13th ACM SIGPLAN Symposium on Principles and Practice of Parallel Programming},
 series = {PPoPP '08},
 year = {2008},
 isbn = {978-1-59593-795-7},
 location = {Salt Lake City, UT, USA},
 pages = {175--184},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1345206.1345233},
 doi = {10.1145/1345206.1345233},
 acmid = {1345233},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {correctness, lower bound, model, transactional memory},
}

@inproceedings{ImbsRay:LockSTM:OPODIS:2008,
 author = {Imbs, Damien and Raynal, Michel},
 title = {{A Lock-Based STM Protocol That Satisfies Opacity and Progressiveness}},
 booktitle = {OPODIS '08: Proceedings of the 12th International Conference on Principles of Distributed Systems},
 year = {2008},
 isbn = {978-3-540-92220-9},
 pages = {226--245},
 location = {Luxor, Egypt},
 doi = {http://dx.doi.org/10.1007/978-3-540-92221-6_16},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
 }

@article{Herlihy+:Linearizability:TPLS:1990,
 author = {Herlihy, Maurice P. and Wing, Jeannette M.},
 title = {{Linearizability: a correctness condition for concurrent objects}},
 journal = {ACM Trans. Program. Lang. Syst.},
 volume = {12},
 number = {3},
 year = {1990},
 issn = {0164-0925},
 pages = {463--492},
 doi = {},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

 @article{Papad:1979:JACM,
 author = {Papadimitriou, Christos H.},
 title = {The Serializability of Concurrent Database Updates},
 journal = {J. ACM},
 issue_date = {Oct. 1979},
 volume = {26},
 number = {4},
 month = oct,
 year = {1979},
 issn = {0004-5411},
 pages = {631--653},
 numpages = {23},
 url = {http://doi.acm.org/10.1145/322154.322158},
 doi = {10.1145/322154.322158},
 acmid = {322158},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@BOOK{tm-book,
  author    = {Rachid Guerraoui and
               Michal Kapalka},
  title     = {Principles of Transactional Memory},
  series    = {Synthesis Lectures on Distributed Computing Theory},
  publisher = {Morgan {\&} Claypool Publishers},
  year      = {2010},
  url       = {https://doi.org/10.2200/S00253ED1V01Y201009DCT004},
  doi       = {10.2200/S00253ED1V01Y201009DCT004},
  timestamp = {Tue, 16 May 2017 01:00:00 +0200},
  biburl    = {https://dblp.org/rec/bib/series/synthesis/2010Guerraoui},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Vidya:1987:AINF,
 author = {Vidyasankar, K.},
 title = {{Generalized theory of serializability}},
 journal = {Acta Inf.},
 volume = {24},
 number = {1},
 year = {1987},
 issn = {0001-5903},
 pages = {105--109},
 doi = {http://dx.doi.org/10.1007/BF00290709},
 publisher = {Springer-Verlag New York, Inc.},
 address = {Secaucus, NJ, USA},
 }

@article{RenAbba:1994:IPL,
 author = {Resende, R. F. and El Abbadi, A.},
 title = {{On the serializability theorem for nested transactions}},
 journal = {Inf. Process. Lett.},
 volume = {50},
 number = {4},
 year = {1994},
 issn = {0020-0190},
 pages = {177--183},
 doi = {http://dx.doi.org/10.1016/0020-0190(94)00033-6},
 publisher = {Elsevier North-Holland, Inc.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 }

@book{WeiVoss:TIS:2002:Morg,
  author    = {Gerhard Weikum and
               Gottfried Vossen},
  title     = {{Transactional Information Systems: Theory, Algorithms, and
               the Practice of Concurrency Control and Recovery}},
  publisher = {Morgan Kaufmann},
  year      = {2002},
  isbn      = {1-55860-508-8},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{Imbs+:2009:PODC,
 author = {Imbs, Damien and de Mendivil, Jos\'{e} Ramon and Raynal, Michel},
 title = {{Brief announcement: virtual world consistency: a new condition for STM systems}},
 booktitle = {PODC '09: Proceedings of the 28th ACM symposium on Principles of distributed computing},
 year = {2009},
 isbn = {978-1-60558-396-9},
 pages = {280--281},
 location = {Calgary, AB, Canada},
 doi = {http://doi.acm.org/10.1145/1582716.1582764},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

@inproceedings{ImbsRay:2009:SIROCCO,
 author = {Imbs, Damien and Raynal, Michel},
 title = {{A versatile {STM} protocol with invisible read operations that satisfies the virtual world consistency condition}},
 booktitle = {Proceedings of the 16th international conference on Structural Information and Communication Complexity},
 series = {SIROCCO'09},
 year = {2010},
 isbn = {3-642-11475-X, 978-3-642-11475-5},
 location = {Piran, Slovenia},
 pages = {266--280},
 numpages = {15},
 url = {http://dx.doi.org/10.1007/978-3-642-11476-2_21},
 doi = {10.1007/978-3-642-11476-2_21},
 acmid = {2174448},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
 keywords = {atomic object, causal past, commit/abort, concurrency control, consistency condition, consistent global state, lock, read-from relation, regular read/write object, serializability, shared memory, software transactional memory, transaction, vector clock},
} 

@inproceedings{CIR11,
  author    = {Tyler Crain and
               Damien Imbs and
               Michel Raynal},
  title     = {{Read Invisibility, Virtual World Consistency and Probabilistic
               Permissiveness are Compatible}},
  booktitle = {ICA3PP (1)},
  year      = {2011},
  pages     = {244-257}
}

@inproceedings{israeli-disjoint,
 author = {Israeli, Amos and Rappoport, Lihu},
 title = {{Disjoint-access-parallel implementations of strong shared memory primitives}},
 booktitle = {Proceedings of the thirteenth annual ACM symposium on Principles of distributed computing},
 series = {PODC '94},
 year = {1994},
 isbn = {0-89791-654-9},
 location = {Los Angeles, California, United States},
 pages = {151--160},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/197917.198079},
 doi = {http://doi.acm.org/10.1145/197917.198079},
 acmid = {198079},
 publisher = {ACM},
 address = {New York, NY, USA},
} 


@inproceedings{AHM09,
 author = {Attiya, Hagit and Hillel, Eshcar and Milani, Alessia},
 title = {{Inherent limitations on disjoint-access parallel implementations of transactional memory}},
 booktitle = {Proceedings of the twenty-first annual symposium on Parallelism in algorithms and architectures},
 series = {SPAA '09},
 year = {2009},
 isbn = {978-1-60558-606-9},
 location = {Calgary, AB, Canada},
 pages = {69--78},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1583991.1584015},
 doi = {http://doi.acm.org/10.1145/1583991.1584015},
 acmid = {1584015},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {disjoint-access parallelism, impossibility result, lower bound, partial snapshots, transactional memory},
} 

@InProceedings{Doherty+:2009:REFINE,
	booktitle = {REFINE},
	year = {2009},
	author = {Simon Doherty and Lindsay Groves and Victor Luchangco and Mark Moir},
	title = {{Towards Formally Specifying and Verifying Transactional Memory}}
}

@TechReport{SatVid:2010:TR,
	author = {Sathya Peri and K.Vidyasankar},
	institution = {Memorial University of Newfoundland},
	title = {{Correctness of Concurrent Executions of Closed Nested Transactions in Transactional Memory Systems}},
	year = {July, 2011}
}

@inproceedings{SatVid:2011:ICDCN,
 author = {Sathya Peri and K.Vidyasankar},
 title = {{Correctness of Concurrent Executions of Closed Nested Transactions in Transactional Memory Systems}},
 booktitle = {12th International Conference on Distributed Computing and Networking},
 pages = {95--106},
 year = {2011},
 location = {Bangalore, Canada},
 }

@inproceedings{SatVid:2012:ICDCN,
 author = {Sathya Peri and K.Vidyasankar},
 title = {{An efficient scheduler for closed nested transactions that satisfies all-read-consistency and non-interference}},
 booktitle = {13th International Conference on Distributed Computing and Networking},
 year = {2012},
 location = {Bangalore, Canada},
 }

@inproceedings{Guer+:disc:2008,
  author	= {Guerraoui, Rachid and Henzinger, Thomas and Singh, Vasu},
  title		= {{Permissiveness in {T}ransactional {M}emories}},
  booktitle	= {DISC~'08: Proc. 22nd International Symposium on Distributed Computing},
  note		= {Springer-Verlag Lecture Notes in Computer Science volume 5218},
  urlpage	= {http://dx.doi.org/10.1007/978-3-540-87779-0_21},
  pdf		= {http://infoscience.epfl.ch/record/125702/files/main.pdf},
  pages		= {305--319},
  year		= {2008},
  month		= {sep},
}

@InProceedings{Baretto+:PPoPP:2010,
   address     = { },
   affiliation = {EPFL},
   author      = {Baretto, Joao and Dragojevic, Aleksandar and Ferreira,
                 Paulo and Guerraoui, Rachid and Kapalka, Michal},
   booktitle   = {Proceedings of the 15th {ACM} {SIGPLAN} symposium on
                 {P}rinciples and {P}ractice of {P}arallel {C}omputing},
   details     = {http://infoscience.epfl.ch/record/144050},
   documenturl = {http://infoscience.epfl.ch/getfile.py?recid=144050&mode=best},
   doi         = {10.1145/1693453.1693466},
   keywords    = {Nested parallel programs; Fork-join; Work-stealing; Transactional memory},
   location    = {Bangalore, India},
   pages       = {91--100},
   publisher   = {ACM},
   review      = {REVIEWED},
   series      = { },
   status      = {PUBLISHED},
   title       = {{Leveraging {P}arallel {N}esting in {T}ransactional {M}emory}},
   unit        = {LPD},
   url         = { },
   year        = 2010
}

@InProceedings{RanVid:Tran:2011,
	author = {Ranjeet Kumar and Krishnamurthy Vidyasankar},
	booktitle = {TRANSACT 2011},
	title = {{HParSTM: A Hierarchy-based STM Protocol for Supporting Nested Parallelism}},
	month = {June},
	year = {2011}
}

@Article{RaviSat:IJCCT:2012,
	title = {{A Correctness Criterion for Eager Approach Validation for Transactional Memory System}},
	year = {2012},
	pages = {43-49},
	author = {Ravi Kumar and Sathya Peri},
	volume = {3},
	journal = {International Journal of Computer and Communication Technology (IJCCT)},
	number = {2}
}

@article{KuzSat:Corr:2012,
  author    = {Petr Kuznetsov and
               Sathya Peri},
  title     = {{On Non-Interference of Transactions}},
  journal   = {CoRR},
  volume    = {abs/1211.6315},
  year      = {2012},
  ee        = {http://arxiv.org/abs/1211.6315},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{Bernstein+:MCC:TDS:1983,
 author = {Bernstein, Philip A. and Goodman, Nathan},
 title = {{{M}ultiversion {C}oncurrency {C}ontrol: {T}heory and {A}lgorithms}},
 journal = {ACM Trans. Database Syst.},
 issue_date = {Dec. 1983},
 volume = {8},
 number = {4},
 month = dec,
 year = {1983},
 issn = {0362-5915},
 pages = {465--483},
 numpages = {19},
 url = {http://doi.acm.org/10.1145/319996.319998},
 doi = {10.1145/319996.319998},
 acmid = {319998},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {transaction processing},
}
 
@Article{CachRito:2006:CP,
	title = {{{V}ersioned {B}oxes as the basis for {M}emory {T}ransactions}},
	year = {2006},
	number = {2},
	author = {J. Cachopo and A. Rito-Silva},
	pages = {172--185},
	journal = {Science of Computer Programming},
	volume = {63}
}

@inproceedings{AydAbd:2008:Serial:transact,
  author	= {Aydonat, Utku and Abdelrahman, Tarek},
  title		= {{Serializability of {T}ransactions in {S}oftware {T}ransactional {M}emory}},
  booktitle	= {TRANSACT~'08: 3rd Workshop on Transactional Computing},
  pdf		= {http://www.unine.ch/transact08/papers/Aydonat-Serializability.pdf},
  year		= {2008},
  month		= {feb},
}

@article{PapadKanel:1984:MultVer:TDS,
 author = {Papadimitriou, Christos H. and Kanellakis, Paris C.},
 title = {{On Concurrency Control by Multiple Versions}},
 journal = {ACM Trans. Database Syst.},
 issue_date = {March 1984},
 volume = {9},
 number = {1},
 month = mar,
 year = {1984},
 issn = {0362-5915},
 pages = {89--99},
 numpages = {11},
 url = {http://doi.acm.org/10.1145/348.318588},
 doi = {10.1145/348.318588},
 acmid = {318588},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{Perel+:2011:SMV:DISC,
  author    = {Dmitri Perelman and
               Anton Byshevsky and
               Oleg Litmanovich and
               Idit Keidar},
  title     = {{SMV}: {S}elective {M}ulti-{V}ersioning {STM}},
  booktitle = {DISC},
  year      = {2011},
  pages     = {125-140},
  ee        = {http://dx.doi.org/10.1007/978-3-642-24100-0_9},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{herlihy+:2003:stm-dynamic:podc,
  author	= {Herlihy, Maurice and Luchangco, Victor and Moir, Mark and {William N. Scherer}, III},
  title		= {{Software Transactional Memory for Dynamic-Sized Data Structures}},
  booktitle	= {PODC~'03: Proc. 22nd ACM Symposium on Principles of Distributed Computing},
  pages		= {92--101},
  month		= {Jul},
  urlpage	= {http://doi.acm.org/10.1145/872035.872048},
  year		= {2003},
}

@inproceedings{dice:2006:tl2:disc,
  author	= {Dice, Dave and Shalev, Ori and Shavit, Nir},
  title		= {{Transactional Locking II}},
  booktitle	= {DISC~'06: Proc. 20th International Symposium on Distributed Computing},
  note		= {Springer-Verlag Lecture Notes in Computer Science volume 4167},
  pages		= {194--208},
  year		= {2006},
  month		= {sep},
}

@inproceedings{perel+:2010:MultVer:PODC,
 author = {Perelman, Dmitri and Fan, Rui and Keidar, Idit},
 title = {On Maintaining Multiple Versions in STM},
 booktitle = {Proceedings of the 29th ACM SIGACT-SIGOPS Symposium on Principles of Distributed Computing},
 series = {PODC '10},
 year = {2010},
 isbn = {978-1-60558-888-9},
 location = {Zurich, Switzerland},
 pages = {16--25},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1835698.1835704},
 doi = {10.1145/1835698.1835704},
 acmid = {1835704},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {transactional memory},
} 

@incollection{riegel+:2006:LSA:DISC,
  author	= {Riegel, Torvald and Felber, Pascal and Fetzer, Christof},
  editor	= {},
  title		= {{A {L}azy {S}napshot {A}lgorithm with {E}ager {V}alidation}},
  booktitle	= {Proceedings of the 20th International Symposium on Distributed Computing, {DISC} 2006},
  publisher	= {Springer},
  month		= {Sep},
  year		= {2006},
  volume	= {4167},
  isbn		= {3-540-44624-9},
  pages		= {284--298},
  series	= {Lecture Notes in Computer Science},
  urlpage	= {http://dx.doi.org/10.1007/11864219_20}
}

@inproceedings{riegel+:sistm:transact:2006,
  author	= {Riegel, Torvald and Fetzer, Christof and Felber, Pascal},
  booktitle	= {Proceedings of the First ACM SIGPLAN Workshop on Languages, Compilers, and Hardware Support for Transactional Computing},
  month		= {Jun},
  title		= {{Snapshot Isolation for Software Transactional Memory }},
  year		= {2006}
}

@article{attiyaHill:sinmvperm:tcs:2012,
  author    = {Hagit Attiya and
               Eshcar Hillel},
  title     = {{A {S}ingle-{V}ersion {STM} that is {M}ulti-{V}ersioned {P}ermissive}},
  journal   = {Theory Comput. Syst.},
  volume    = {51},
  number    = {4},
  year      = {2012},
  pages     = {425-446},
  ee        = {http://dx.doi.org/10.1007/s00224-012-9406-3},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{prisat:mvto:corr:2013,
  author    = {Priyanka Kumar and
               Sathya Peri},
  title     = {{A TimeStamp based Multi-version STM Protocol that satisfies
               Opacity}},
  journal   = {CoRR},
  volume    = {abs/1305.6624},
  year      = {2013},
  ee        = {http://arxiv.org/abs/1305.6624},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{Fern+:LSMVSTM:PPoPP:2011,
 author = {Fernandes, S{\'e}rgio Miguel and Cachopo, Joao},
 title = {{Lock-free and {S}calable {M}ulti-version {S}oftware {T}ransactional {M}emory}},
 booktitle = {Proceedings of the 16th ACM symposium on Principles and practice of parallel programming},
 series = {PPoPP '11},
 year = {2011},
 isbn = {978-1-4503-0119-0},
 location = {San Antonio, TX, USA},
 pages = {179--188},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1941553.1941579},
 doi = {10.1145/1941553.1941579},
 acmid = {1941579},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {garbage collection, lock-free synchronization, multi-version concurrency control, transactional memory},
} 

@Article{LuScott:UMV:Transact:2012,
	journal = {Transact},
	title = {{Unmanaged Multiversion STM}},
	year = {2012},
	author = {Li Lu and Michael L. Scott}
}

@inproceedings{SinhaMalik:RuntimeSee:IPDPS:2010,
  author    = {Arnab Sinha and
               Sharad Malik},
  title     = {{Runtime checking of serializability in software transactional
               memory}},
  booktitle = {IPDPS},
  year      = {2010},
  pages     = {1-12},
  ee        = {http://dx.doi.org/10.1109/IPDPS.2010.5470389},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{HadzPapad:AAMVCC:PODS:1985,
 author = {Hadzilacos, Thanasis and Papadimitriou, Christos H.},
 title = {{Algorithmic aspects of multiversion concurrency control}},
 booktitle = {Proceedings of the fourth ACM SIGACT-SIGMOD symposium on Principles of database systems},
 series = {PODS '85},
 year = {1985},
 isbn = {0-89791-153-9},
 location = {Portland, Oregon, USA},
 pages = {96--104},
 numpages = {9},
 url = {http://doi.acm.org/10.1145/325405.325417},
 doi = {10.1145/325405.325417},
 acmid = {325417},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@article{KuznetsovPeri:Non-interference:TCS:2017,
  author    = {Petr Kuznetsov and
               Sathya Peri},
  title     = {Non-interference and local correctness in transactional memory},
  journal   = {Theor. Comput. Sci.},
  volume    = {688},
  pages     = {103--116},
  year      = {2017},
  url       = {https://doi.org/10.1016/j.tcs.2016.06.021},
  doi       = {10.1016/j.tcs.2016.06.021},
  timestamp = {Thu, 28 Dec 2017 00:00:00 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/tcs/KuznetsovP17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Kumar+:MVTO:ICDCN:2014,
 author = {Kumar, Priyanka and Peri, Sathya and Vidyasankar, K.},
 title = {A TimeStamp Based Multi-version STM Algorithm},
 booktitle = {Proceedings of the 15th International Conference on Distributed Computing and Networking - Volume 8314},
 series = {ICDCN 2014},
 year = {2014},
 isbn = {978-3-642-45248-2},
 location = {Coimbatore, India},
 pages = {212--226},
 numpages = {15},
 url = {http://dx.doi.org/10.1007/978-3-642-45249-9_14},
 doi = {10.1007/978-3-642-45249-9_14},
 acmid = {2741924},
 publisher = {Springer-Verlag New York, Inc.},
 address = {New York, NY, USA},
} 



@book{Har+:TMBook:2010,
  author    = {Tim Harris and
               James R. Larus and
               Ravi Rajwar},
  title     = {{Transactional Memory, 2nd edition}},
  booktitle = {Transactional Memory (2.ed.)},
  publisher = {Morgan {\&} Claypool Publishers},
  series    = {Synthesis Lectures on Computer Architecture},
  year      = {2010},
  ee        = {http://dx.doi.org/10.2200/S00272ED1V01Y201006CAC011},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{OluHamm:MicroBook:Queue:2005,
 author = {Olukotun, Kunle and Hammond, Lance},
 title = {{The Future of Microprocessors}},
 journal = {Queue},
 issue_date = {September 2005},
 volume = {3},
 number = {7},
 month = sep,
 year = {2005},
 issn = {1542-7730},
 pages = {26--29},
 numpages = {4},
 url = {http://doi.acm.org/10.1145/1095408.1095418},
 doi = {10.1145/1095408.1095418},
 acmid = {1095418},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@book{Herlihy:ArtBook:2012,
  title={{The Art of Multiprocessor Programming}},
  author={Herlihy, M. and Shavit, N.},
  isbn={9780080569581},
  url={},
  year={2012},
  publisher={Elsevier Science}
}

@inproceedings{Harris:NBList:DISC:2001,
 author = {Harris, Timothy L.},
 title = {A Pragmatic Implementation of Non-blocking Linked-Lists},
 booktitle = {Proceedings of the 15th International Conference on Distributed Computing},
 series = {DISC '01},
 year = {2001},
 isbn = {3-540-42605-1},
 pages = {300--314},
 numpages = {15},
 url = {http://dl.acm.org/citation.cfm?id=645958.676105},
 acmid = {676105},
 publisher = {Springer-Verlag},
 address = {London, UK, UK},
}

@article{Herlihy:WaitFree:1991,
  title={{Wait-free synchronization}},
  author={Herlihy, Maurice},
  journal={ACM Transactions on Programming Languages and Systems (TOPLAS)},
  volume={13},
  number={1},
  pages={124--149},
  year={1991},
  publisher={ACM}
}

@INPROCEEDINGS{Attiya+:DUOp:ICDCS:2013,
author={Attiya, H. and Hans, S. and Kuznetsov, P. and Ravi, S.},
booktitle={Distributed Computing Systems (ICDCS), 2013 IEEE 33rd International Conference on},
title={{Safety of Deferred Update in Transactional Memory}},
year={2013},
month={July},
pages={601-610},
keywords={concurrency control;transaction processing;committed transactions;deferred update safety;deferred-update semantics;opacityc riterion;prefix serializations;sequential execution;sequential order;speculative transactions;transactional memory;unique-write assumption;History;Law;Real-time systems;Safety;Semantics;Silicon;Limit-closure;Safety;Transactional Memory},
doi={10.1109/ICDCS.2013.57},
ISSN={1063-6927},}

@article{PriSat:MVC:Corr:2015,
  author    = {Priyanka Kumar and
               Sathya Peri},
  title     = {{Multi-Version Conflict Notion}},
  journal   = {CoRR},
  volume    = {abs/1307.8256},
  year      = {2013},
  url       = {http://arxiv.org/abs/1307.8256},
  timestamp = {Thu, 15 Aug 2013 15:30:58 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/KumarP13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Attiya+:TMS:DISC:2014,
  author    = {Hagit Attiya and
               Alexey Gotsman and
               Sandeep Hans and
               Noam Rinetzky},
  title     = {{Safety of Live Transactions in Transactional Memory: {TMS} is Necessary
               and Sufficient}},
  booktitle = {Distributed Computing - 28th International Symposium, {DISC} 2014,
               Austin, TX, USA, October 12-15, 2014. Proceedings},
  pages     = {376--390},
  year      = {2014},
  crossref  = {DBLP:conf/wdag/2014},
  url       = {http://dx.doi.org/10.1007/978-3-662-45174-8_26},
  doi       = {10.1007/978-3-662-45174-8_26},
  timestamp = {Tue, 30 Sep 2014 10:44:00 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/wdag/AttiyaGHR14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{Herlihy:WFS:TPLS:1991,
 author = {Herlihy, Maurice},
 title = {{Wait-free Synchronization}},
 journal = {ACM Trans. Program. Lang. Syst.},
 issue_date = {Jan. 1991},
 volume = {13},
 number = {1},
 month = jan,
 year = {1991},
 issn = {0164-0925},
 pages = {124--149},
 numpages = {26},
 url = {http://doi.acm.org/10.1145/114005.102808},
 doi = {10.1145/114005.102808},
 acmid = {102808},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {linearization, wait-free synchronization},
} 

@book{HerlihyShavit:AMP:Book:2012,
 author = {Herlihy, Maurice and Shavit, Nir},
 title = {{The Art of Multiprocessor Programming, Revised Reprint}},
 year = {2012},
 isbn = {9780123973375, 9780123977953},
 edition = {1st},
 publisher = {Morgan Kaufmann Publishers Inc.},
 address = {San Francisco, CA, USA},
} 

@inproceedings{LuScott:GMV:DISC:2013,
  author    = {Li Lu and
               Michael L. Scott},
  title     = {{Generic Multiversion {STM}}},
  booktitle = {Distributed Computing - 27th International Symposium, {DISC} 2013,
               Jerusalem, Israel, October 14-18, 2013. Proceedings},
  pages     = {134--148},
  year      = {2013},
  crossref  = {DBLP:conf/wdag/2013},
  url       = {http://dx.doi.org/10.1007/978-3-642-41527-2_10},
  doi       = {10.1007/978-3-642-41527-2_10},
  timestamp = {Mon, 28 Oct 2013 18:03:50 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/wdag/LuS13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{CachAnt:VBoxes:SCOOL:2005,
  author	= {Cachopo, Joao and Rito-Silva, Antonio},
  title		= {{Versioned Boxes as the Basis for Memory Transactions}},
  booktitle	= {OOPSLA 2005 Workshop on Synchronization and Concurrency in Object-Oriented Languages (SCOOL)},
  urlpage	= {http://hdl.handle.net/1802/2101},
  year		= {2005},
  month		= {oct},
}

@article{Thomas:TWR:TDS:1979,
 author = {Thomas, Robert H.},
 title = {{A Majority Consensus Approach to Concurrency Control for Multiple Copy Databases}},
 journal = {ACM Trans. Database Syst.},
 issue_date = {June 1979},
 volume = {4},
 number = {2},
 month = jun,
 year = {1979},
 issn = {0362-5915},
 pages = {180--209},
 numpages = {30},
 url = {http://doi.acm.org/10.1145/320071.320076},
 doi = {10.1145/320071.320076},
 acmid = {320076},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {clock synchronization, computer networks, concurrency control, distributed computation, distributed control, distributed databases, multiprocess systems, update synchronization},
} 

@inproceedings{Gramoli+:OptListSet:DISC-BA:2015,
  TITLE = {{Brief Announcement: A Concurrency-Optimal List-Based Set}},
  AUTHOR = {Gramoli, Vincent and Kuznetsov, Petr and Ravi, Srivatsan and Shang, Di},
  URL = {https://hal.archives-ouvertes.fr/hal-01207872},
  BOOKTITLE = {{DISC 2015}},
  ADDRESS = {Tokyo, Japan},
  ORGANIZATION = {{Toshimitsu Masuzawa and Koichi Wada}},
  EDITOR = {Yoram Moses and Matthieu Roy},
  PUBLISHER = {{Springer-Verlag Berlin Heidelberg}},
  SERIES = {29th International Symposium on Distributed Computing},
  VOLUME = {LNCS 9363},
  YEAR = {2015},
  MONTH = Oct,
  PDF = {https://hal.archives-ouvertes.fr/hal-01207872/file/37-BA.pdf},
  HAL_ID = {hal-01207872},
  HAL_VERSION = {v1},
}

@article{Gramoli+:OptListSet:CoRR:2015,
  author    = {Vincent Gramoli and
               Petr Kuznetsov and
               Srivatsan Ravi and
               Di Shang},
  title     = {{A Concurrency-Optimal List-Based Set}},
  journal   = {CoRR},
  volume    = {abs/1502.01633},
  year      = {2015},
  url       = {http://arxiv.org/abs/1502.01633},
  timestamp = {Mon, 02 Mar 2015 14:17:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/GramoliKRS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Heller+:LazyList:PPL:2007,
  author    = {Steve Heller and
               Maurice Herlihy and
               Victor Luchangco and
               Mark Moir and
               William N. Scherer III and
               Nir Shavit},
  title     = {{A Lazy Concurrent List-Based Set Algorithm}},
  journal   = {Parallel Processing Letters},
  volume    = {17},
  number    = {4},
  pages     = {411-424},
  year      = {2007},
  url       = {},
  doi       = {},
  timestamp = {Mon, 23 Jun 2008 13:43:26 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/ppl/HellerHLMSS07},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Ziv+:Composing:POPL:2015,
  title={{Composing Concurrency Control}},
  author={Ziv, Ofri and Aiken, Alex and Golan-Gueta, Guy and Ramalingam, G and Sagiv, Mooly},
  booktitle={Proceedings of the 36th ACM SIGPLAN Conference on Programming Language Design and Implementation},
  pages={240--249},
  year={2015},
  organization={ACM}
}

@article{marathe2004qualitative,
  title={{A qualitative survey of modern software transactional memory systems}},
  author={Marathe, Virendra J and Scott, Michael L},
  journal={University of Rochester Computer Science Dept., Tech. Rep},
  year={2004}
}

@inproceedings{Vafeiadis:2006:PCH:1122971.1122992,
 author = {Vafeiadis, Viktor and Herlihy, Maurice and Hoare, Tony and Shapiro, Marc},
 title = {{Proving Correctness of Highly-concurrent Linearisable Objects}},
 booktitle = {PPoPP},
 series = {},
 year = {2006},
 isbn = {1-59593-189-9},
 location = {},
 pages = {129--136},
 numpages = {8},
 url = {},
 doi = {},
 acmid = {1122992},
 publisher = {},
 address = {},
 keywords = {concurrent programming, formal verification, linearisability, rely-guarantee reasoning, shared-memory concurrency},
}


@techreport{marathe:stm-survey:urcs-tr:2004,
  author	= {Marathe, Virendra J. and Scott, Michael L.},
  title		= {{A Qualitative Survey of Modern Software Transactional Memory Systems}},
  number	= {TR 839},
  institution	= {University of Rochester Computer Science Dept.},
  month		= {Jun},
  year		= {2004},
  pdf		= {http://www.cs.rochester.edu/u/scott/papers/2004_TR839.pdf}
}

@phdthesis{Fraser:PracticalLF:2004,
  title={{Practical lock-freedom}},
  author={Fraser, Keir},
  year={2004},
  school={University of Cambridge}
}

@inproceedings{Herlihy+:STM-DynamicSize:PODC:2003,
  title={{Software transactional memory for dynamic-sized data structures}},
  author={Herlihy, Maurice and Luchangco, Victor and Moir, Mark and Scherer III, William N},
  booktitle={Proceedings of the twenty-second annual symposium on Principles of distributed computing},
  pages={92--101},
  year={2003},
  organization={ACM}
}
@inproceedings{Marathe+:STM-Tradeoff:LCRS:2004,
  title={{Design tradeoffs in modern software transactional memory systems}},
  author={Marathe, Virendra J and Scherer, William N and Scott, Michael L},
  booktitle={Proceedings of the 7th workshop on Workshop on languages, compilers, and run-time support for scalable systems},
  pages={1--7},
  year={2004},
  organization={ACM}
}

@article{Barghouti:1991:CCA:116873.116875,
 author = {Barghouti, Naser S. and Kaiser, Gail E.},
 title = {{Concurrency Control in Advanced Database Applications}},
 journal = {ACM Comput. Surv.},
 issue_date = {Sept. 1991},
 volume = {23},
 number = {3},
 month = sep,
 year = {1991},
 issn = {0360-0300},
 pages = {269--317},
 numpages = {49},
 url = {http://doi.acm.org/10.1145/116873.116875},
 doi = {10.1145/116873.116875},
 acmid = {116875},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {advanced database applications, concurrency control, cooperative transactions, design environments, extended transaction models, long transactions, object-oriented databases, relaxing serializability},
}

@article{Beeri+:Nested:JACM:1989,
 author = {Beeri, Catriel and Bernstein, Philip A. and Goodman, Nathan},
 title = {{A Model for Concurrency in Nested Transactions Systems}},
 journal = {J. ACM},
 issue_date = {April 1989},
 volume = {36},
 number = {2},
 month = apr,
 year = {1989},
 issn = {0004-5411},
 pages = {230--269},
 numpages = {40},
 url = {http://doi.acm.org/10.1145/62044.62046},
 doi = {10.1145/62044.62046},
 acmid = {62046},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{HerlihyKosk:Boosting:PPoPP:2008,
	author    = {Maurice Herlihy and
	Eric Koskinen},
	title     = {Transactional boosting: a methodology for highly-concurrent transactional
	objects},
	booktitle = {Proceedings of the 13th {ACM} {SIGPLAN} Symposium on Principles and
	Practice of Parallel Programming, {PPOPP} 2008, Salt Lake City, UT,
	USA, February 20-23, 2008},
	pages     = {207--216},
	year      = {2008},
	url       = {http://doi.acm.org/10.1145/1345206.1345237},
	doi       = {10.1145/1345206.1345237},
	timestamp = {Tue, 22 May 2012 15:24:56 +0200},
	biburl    = {https://dblp.org/rec/bib/conf/ppopp/HerlihyK08},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{Hassan+:OptBoost:PPoPP:2014,
 author = {Hassan, Ahmed and Palmieri, Roberto and Ravindran, Binoy},
 title = {Optimistic Transactional Boosting},
 booktitle = {Proceedings of the 19th ACM SIGPLAN Symposium on Principles and Practice of Parallel Programming},
 series = {PPoPP '14},
 year = {2014},
 isbn = {978-1-4503-2656-8},
 location = {Orlando, Florida, USA},
 pages = {387--388},
 numpages = {2},
 url = {http://doi.acm.org/10.1145/2555243.2555283},
 doi = {10.1145/2555243.2555283},
 acmid = {2555283},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {STM, transactional boosting, transactional data structures},
} 


@inproceedings{Hassan:OptTransLazy:Opodis:2014,
	title={{On developing optimistic transactional lazy set}},
	author={Hassan, Ahmed and Palmieri, Roberto and Ravindran, Binoy},
	booktitle={OPODIS},
	pages={437--452},
	year={2014},
	organization={Springer}
}

@inproceedings{Spiegelman+:TransDS:PLDI:2016,
	title={{Transactional data structure libraries}},
	author={Spiegelman, Alexander and Golan-Gueta, Guy and Keidar, Idit},
	booktitle={PLDI},
	pages={682--696},
	year={2016},
	organization={ACM}
}

@article{Anand+:CaPRa:Corr:2015,
  author    = {Anshu S. Anand and
               R. K. Shyamasundar and
               Sathya Peri},
  title     = {{Opacity Proof for CaPR+ Algorithm}},
  journal   = {CoRR},
  volume    = {abs/1510.06967},
  year      = {2015},
  url       = {http://arxiv.org/abs/1510.06967},
  timestamp = {Sun, 01 Nov 2015 17:30:45 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/AnandSP15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Lev-Ari+:OnCorrectness:DISC:2014,
	author    = {Kfir Lev{-}Ari and
	Gregory V. Chockler and
	Idit Keidar},
	title     = {{On Correctness of Data Structures under Reads-Write Concurrency}},
	booktitle = {DISC},
	pages     = {273--287},
	year      = {2014},
	crossref  = {DBLP:conf/wdag/2014},
	url       = {},
	doi       = {},
	timestamp = {Fri, 19 May 2017 01:25:17 +0200},
	biburl    = {http://dblp.uni-trier.de/rec/bib/conf/wdag/Lev-AriCK14},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Lev-Ari+:ConsApproachLinz:DISC:2015,
	author = {Lev-Ari, Kfir and Chockler, Gregory V and Keidar, Idit},
	booktitle = {DISC},
	doi = {},
	editor = {Moses, Yoram},
	isbn = {978-3-662-48652-8},
	pages = {356--370},
	publisher = {Springer},
	series = {},
	title = {{A Constructive Approach for Proving Data Structures' Linearizability}},
	url = {},
	volume = {},
	year = {2015}
}

@article{zhang2016high,
  title={{High-Performance Composable Transactional Data Structures}},
  author={Zhang, Deli},
  year={2016}
}

@techreport{zhang2010composability,
  author={Zhang, Rui and Budimli{\'c}, Zoran and Scherer III, William N},
  title={{Composability for application-specific transactional optimizations}},
  institution={Department of Computer Science, Rice University},
  year={2010}
}

@article{DBLP:journals/corr/abs-0910-0366,
  author    = {Daniel Cederman and
               Philippas Tsigas},
  title     = {{Supporting Lock-Free Composition of Concurrent Data Objects}},
  journal   = {CoRR},
  volume    = {abs/0910.0366},
  year      = {2009},
  url       = {},
  timestamp = {Wed, 07 Jun 2017 14:40:49 +0200},
  biburl    = {http://dblp.dagstuhl.de/rec/bib/journals/corr/abs-0910-0366},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Hassan2015,
author = {Hassan, Ahmed and Wang, Chao and Broadwater, Robert P},
mendeley-groups = {PhD Thesis},
title = {{Designing , Modeling , and Optimizing Transactional Data Structures}},
year = {2015}
}

@article{harris2007abstract,
	title={{Abstract nested transactions}},
	author={Harris, Tim and others},
	year={2007},
	publisher={Citeseer}
}

@article{Peri+:OSTM:Corr:2017,
	author    = {Sathya Peri and
	Ajay Singh and
	Archit Somani},
	title     = {{Efficient means of Achieving Composability using Transactional Memory}},
	journal   = {CoRR},
	volume    = {abs/1709.00681},
	year      = {2017},
	url       = {http://arxiv.org/abs/1709.00681},
	archivePrefix = {arXiv},
	eprint    = {1709.00681},
	timestamp = {Thu, 05 Oct 2017 09:42:55 +0200},
	biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1709-00681},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Peri+:OSTM:Netys:2018,
  author    = {Sathya Peri and
               Ajay Singh and
               Archit Somani},
  title     = {Efficient Means of Achieving Composability Using Object Based Semantics
               in Transactional Memory Systems},
  booktitle = {Networked Systems - 6th International Conference, {NETYS} 2018, Essaouira,
               Morocco, May 9-11, 2018, Revised Selected Papers},
  pages     = {157--174},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-05529-5\_11},
  doi       = {10.1007/978-3-030-05529-5\_11},
  timestamp = {Tue, 08 Jan 2019 16:57:19 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/netys/PeriSS18},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Felber+:ElasticTrans:2017:jpdc,
 author = {Felber, Pascal and Gramoli, Vincent and Guerraoui, Rachid},
 title = {{Elastic Transactions}},
 journal = {J. Parallel Distrib. Comput.},
 issue_date = {February 2017},
 volume = {100},
 number = {C},
 month = feb,
 year = {2017},
 issn = {0743-7315},
 pages = {103--127},
 numpages = {25},
 url = {https://doi.org/10.1016/j.jpdc.2016.10.010},
 doi = {10.1016/j.jpdc.2016.10.010},
 acmid = {3066828},
 publisher = {Academic Press, Inc.},
 address = {Orlando, FL, USA},
 keywords = {Concurrent data structures, Transactional memory},
} 


@inproceedings{ZhangDech:LockFreeTW:SPAA:2016,
 author = {Zhang, Deli and Dechev, Damian},
 title = {Lock-free Transactions Without Rollbacks for Linked Data Structures},
 booktitle = {Proceedings of the 28th ACM Symposium on Parallelism in Algorithms and Architectures},
 series = {SPAA '16},
 year = {2016},
 isbn = {978-1-4503-4210-0},
 location = {Pacific Grove, California, USA},
 pages = {325--336},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/2935764.2935780},
 doi = {10.1145/2935764.2935780},
 acmid = {2935780},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {lock-free, transactional boosting, transactional data structure, transactional memory},
} 

@inproceedings{Dalessandro+:NoRec:PPoPP:2010,
  added-at = {2010-01-19T00:00:00.000+0100},
  author = {Dalessandro, Luke and Spear, Michael F. and Scott, Michael L.},
  biburl = {https://www.bibsonomy.org/bibtex/2bb4ff560750c574e33fceb87457d3cce/dblp},
  booktitle = {PPOPP},
  editor = {Govindarajan, R. and Padua, David A. and Hall, Mary W.},
  ee = {http://doi.acm.org/10.1145/1693453.1693464},
  interhash = {65ad98c6f111ce3b454219b4fd45ebb8},
  intrahash = {bb4ff560750c574e33fceb87457d3cce},
  isbn = {978-1-60558-877-3},
  keywords = {dblp},
  pages = {67-78},
  publisher = {ACM},
  timestamp = {2012-05-23T11:41:17.000+0200},
  title = {{NOrec: Streamlining STM by Abolishing Ownership Records}},
  url = {http://dblp.uni-trier.de/db/conf/ppopp/ppopp2010.html#DalessandroSS10},
  year = 2010
}


@inproceedings{Juyal+:MVOSTM:SSS:2018,
  author    = {Chirag Juyal and
               Sandeep S. Kulkarni and
               Sweta Kumari and
               Sathya Peri and
               Archit Somani},
  title     = {An Innovative Approach to Achieve Compositionality Efficiently Using
               Multi-version Object Based Transactional Systems},
  booktitle = {Stabilization, Safety, and Security of Distributed Systems - 20th
               International Symposium, {SSS} 2018, Tokyo, Japan, November 4-7, 2018,
               Proceedings},
  pages     = {284--300},
  year      = {2018},
  url       = {https://doi.org/10.1007/978-3-030-03232-6\_19},
  doi       = {10.1007/978-3-030-03232-6\_19},
  timestamp = {Thu, 06 Dec 2018 00:00:00 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/sss/JuyalKKPS18},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


==> dpcode.tex <==
\section{Detailed Pcode of MVOSTM}
\label{apn:rpcode}
%\vspace{-.3cm}


\subsection{Global DS}
\begin{lstlisting}{language = C++}
struct G_node{
int G_key;
struct G_vl;
G_lock;			
node G_knext;    
};
\end{lstlisting}

\begin{lstlisting}{language = C++}
struct G_vl{
int G_ts;
int G_val;
bool G_mark; 	
/*rvl stands for return value list*/
int G_rvl[];			
vl G_vnext;    
};
\end{lstlisting}

\subsection{Local DS}

\begin{lstlisting}{language = C++}
class L_txlog{
int L_t_id;			
STATUS L_tx_status;
vector <L_rec> L_list;
find();
getList();
};
\end{lstlisting}

\begin{lstlisting}{language = C++}
class L_rec{
int L_obj_id;
int L_key; 
int L_val;		
node* L_knext, G_pred, G_curr, node;
STATUS L_op_status;		
OP_NAME L_opn;
getOpn();	getPreds&Currs();  getOpStatus();
getKey&Objid();	getVal();	   getAptCurr();
setVal();	setPreds&Currs();  setOpStatus();   setOpn();
};
enum OP_NAME = {INSERT, DELETE, LOOKUP}
enum STATUS = {ABORT = 0, OK, FAIL, COMMIT}
\end{lstlisting}

\begin{table}[H]
	\centering
	\begin{tabular}{ || m{8em} | m{9cm}|| } 
		\hline
		\textbf{Functions} & \textbf{Description} \\ 
		\hline 		\hline
		setOpn() & set method name into transaction local log\\ 
		\hline
		setVal() & set value of the key into transaction local log\\ 
		\hline
		setOpStatus() & set status of method into transaction local log\\ 
		\hline
		setPred\&Curr() & set location of $G\_pred$ and $G\_curr$ according to the node corresponding to the key into transaction local log\\ 
		\hline
		getOpn() & get method name from transaction local log\\ 
		\hline
		getVal() & get value of the key from transaction local log\\ 
		\hline
		getOpStatus() & get status of the method from transaction local log\\ 
		\hline
		getKey\&Objid() & get key and obj\_id corresponding to the method from transaction local log\\ 
		\hline
		getPred\&Curr() & get location of $G\_preds$ and $G\_currs$ according to the node corresponding to the key from transaction local log \\ 
		\hline		
	\end{tabular}
	\caption{Description of accessing transaction local log methods}
	\label{tabel:1}
\end{table}


\begin{table}[H]
	\centering
	\begin{tabular}{ || m{2.3cm} | m{2.3cm} | m{2.3cm} | m{2.3cm} | m{2.3cm}|| } 
		\hline
		\textbf{p/q} & \textbf{\npins{}} & \textbf{\npdel{}} & \textbf{\npluk{}} & \textbf{\nptc} \\ 
		\hline 		
		\textbf{\npins{}} & + & + & + & +\\
		\hline
		\textbf{\npdel{}} & + & + & + & -\\
		\hline
		\textbf{\npluk{}} & + & + & + & -\\
		\hline
		\textbf{\nptc{}} & + & - & - & -\\
		\hline
	\end{tabular}
	\caption{Commutative table}
	\label{tabel:2}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STM_init()
 %Return the transaction id ($L\_t\_id$) at \Lineref{begin8}.

%Transaction id ($L\_t\_id$), object id (L\_obj\_id), node corresponding to the key (L\_key) and value(L\_val) are the inputs of this function.  

\cmnt{
\setlength{\textfloatsep}{0pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%rv_method()%%%%%%%%%%%%%
\begin{algorithm} [H]
%\label{alg:llsearch} 
\scriptsize
\caption{\emph{\rvmt()} }
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{0}\makeatother
\Procedure{\rvmt{()}}{}
\If{(($m_{ij}(k)$ == \npluk{}) $||$ ($m_{ij}(k)$ == \npdel{}))}
\If{(k $\in$ local\_log(key))}
\State Update the local log \& return;
\Else
\State Search into the $CDS$ to identify the $preds$ \& $currs$ for key in \bn{} \& \rn.
\State Acquire the locks in increasing order.
\If{($!rv\_Validation()$)}
\State Release the locks and retry;
\ElsIf{(k $\notin$ $CDS$)} 
\State Create the new node in \rn{} and add the $T_0$ version in it. 
\EndIf
\State $find\_lts():$ Identify the version with largest TS as $T_j$ but less then TS($T_i$);
\State Add TS($T_i$) into $rvl$ of $T_j$;
\State Release the locks and update the local log;
\EndIf
\EndIf
\EndProcedure
\end{algorithmic}
%\end{multicols}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%rv_validation()%%%%%%%%%%%%%
\begin{algorithm} [H]
%\label{alg:llsearch} 
\scriptsize
\caption{\emph{rv\_Validation()} }
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{0}\makeatother
\Procedure{rv\_validation{()}}{}
\If{$((\bp.marked) || (\bc.marked) ||(\bp.\bn) \neq \bc || (\rp.\rn) \neq {\rc})$}
\State return $false$;
\Else 
\State return $true$;
\EndIf 
\EndProcedure
\end{algorithmic}
%\end{multicols}
\end{algorithm}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%try_C()%%%%%%%%%%%%%
\begin{algorithm} [H]
%\label{alg:llsearch} 
\scriptsize
\caption{\emph{tryC()} }
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{0}\makeatother
\Procedure{tryC{()}}{}
\State Get the local log list for corresponding transaction;
\ForAll{(opn $\in$ local\_log\_list)}
\If{(($m_{ij}(k)$ == \npins{}) $||$ ($m_{ij}(k)$ == \npdel{}))}
\State Search into the $CDS$ to identify the $preds$ \& $currs$ for key in \bn{} \& \rn;
\State Acquire the locks in increasing order;
\If{($!rv\_Validation()$)}
\State Release the locks and retry;
\EndIf
\State $find\_lts():$ If (k $\in$ $CDS$) then identify the version with largest TS as $T_j$ but less then TS($T_i$);
\If{($!tryC\_Validation()$)}
\State return $Abort$;
\EndIf
\EndIf
\EndFor
\ForAll{(opn $\in$ local\_log\_list)}
\If{(($m_{ij}(k)$ == \npins{}) $||$ ($m_{ij}(k)$ == \npdel{}))}
\State $intraTransValidation():$ Update the preds and currs of consecutive operation working on same region.
\If{(k $\notin$ CDS)}
\State Create the new node in \rn{}, \bn{} and add the $T_0$ version in it;
\EndIf
\State $find\_lts():$ Identify the version with largest TS as $T_j$ but less then TS($T_i$);
\State Add TS($T_i$) into $rvl$ of $T_j$;
\State Update the local log;
\EndIf
\EndFor
%\EndFor
\State Release the locks;
\EndProcedure
\end{algorithmic}
%\end{multicols}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%tryC_validation()%%%%%%%%%%%%%
\begin{algorithm} [H]
%\label{alg:llsearch} 
\scriptsize
\caption{\emph{tryC\_Validation()} }
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{0}\makeatother
\Procedure{tryC\_validation{()}}{}
\ForAll {$T_k$ in $rvl$ of $T_j$}
\If{(TS($(T_k)$ $>$ TS($T_i$)))}
\State return $false$;
\EndIf 
\EndFor
\EndProcedure
\end{algorithmic}
%\end{multicols}
\end{algorithm}

 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Local Log Search()%%%%%%%%%%%%%
\begin{algorithm} [H]
\label{alg:llsearch} 
\scriptsize
\caption{\emph{MV-OSTM} Algorithm}
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{0}\makeatother
%\Procedure{STM local log search}{key} \label{lin:ll1}
\If{($G\_key$ $\in$ local\_log($L\_key$))} \label{lin:ll2}\Comment{Search into local log}
\If{$(($\textup{INSERT} $=$ \textup{$L\_opn$} $)||($ \textup{LOOKUP} $=$ \textup{$L\_opn$}$))$} \label{lin:ll3};
\State $L\_val$ $\gets$ $L\_getVal(L\_opn,L\_key)$ \label{lin:ll4};
\State $L\_op\_status$ $\gets$  $L\_getOpStatus$(L\_opn, L\_key) \label{lin:ll5};
%\State Update the local log.\label{lin:ll6}
			\ElsIf{$($\textup{DELETE} $=$ \textup{$L\_opn$}$)$} \label{lin:ll7}
			\State $L\_val$ $\gets$ NULL \label{lin:ll8}; 
			\State $L\_op\_status$ $\gets$ FAIL \label{lin:ll9}; 
\EndIf
\State Update the local log.
\State return $\langle L\_val$, $L\_op\_status \rangle$.\label{lin:ll10}
\EndIf

\State \Comment{Traversal phase}
\State $\bp$ $\gets$ $G\_head$ \label{lin:ltraversal2}; 
\State $\bc$ $\gets$ $\bp.\bn$ \label{lin:ltraversal3};
\While{$((\bc.key) < L\_key)$} \label{lin:ltraversal4};
\State $\bp$ $\gets$ $\bc$ \label{lin:ltraversal5};
\State $\bc$ $\gets$ $\bc.\bn$ \label{lin:ltraversal6};
\EndWhile \label{lin:ltraversal12}
\State $\rp$ $\gets$ $\bp$ \label{lin:ltraversal7}; 
\State $\rc$ $\gets$ $\rp.\rn$ \label{lin:ltraversal8};
\While{$((\rc.key) < L\_key)$} \label{lin:ltraversal9}
\State $\rp$ $\gets$ $\rc$ \label{lin:ltraversal10};
\State $\rc$ $\gets$ $\rc.\rn$ \label{lin:ltraversal11};
\EndWhile \label{lin:ltraversal14}
\State Update the \preds{} and \currs{} into local log.
\State \Comment{Validation phase}
\If{(($\bp$.marked) || ($\bc$.marked) ||($\bp.\bn$) $\neq$ $\bc$ || ($\rp.\rn$) $\neq$ {$\rc$})}\Comment{Validation}
\State return $\langle RETRY \rangle$;
\Else
\State return $\langle OK \rangle$;
\EndIf
\State /*Find the largest time-stamp but less then itself($T_i$).*/
\State $find\_lts$(max(closest\_tuple(TS($T_j$))) $<$ TS($T_i$))
\ForAll {($T_k$ $\in$ rvl($T_i$))}
\If{(TS($T_i$) < TS($T_k$))}
\State return $\langle ABORT \rangle$;
\Else
\State return $\langle OK \rangle$;
\end{algorithmic}
%\end{multicols}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------------------------------TryCommit----------------------------------%---------
%----
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[H]
\scriptsize
	\caption{\tabspace[0.2cm] STM $tryC()$ }
	\label{algo:trycommit}
	\setlength{\multicolsep}{0pt}
		%\begin{multicols}{2}
	\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{33}\makeatother
		\Procedure{STM tryC}{($L\_t\_id$)} \label{lin:tryc1}
    \State $L\_list$ $\gets$ $getList$($L\_t\_id$) \label{lin:tryc3};
		\While{$(\textbf{$L\_rec_{i} \gets \textup{next}(L\_list$}))$} \label{lin:tryc5}
		\State ($L\_key, L\_obj\_id$) $\gets$ \llgkeyobj{} \label{lin:tryc6};
		\State \lsls{$COMMIT \downarrow$} \label{lin:tryc8};
			
		\If {$((\bc.key = L\_key) \& (\checkv(L\_t\_id \downarrow,\bc \downarrow) = FALSE))$}\label{lin:tryc9}
\State Unlock all the variables;\label{lin:tryc10}
\State return $ABORT$;\label{lin:tryc11}
\ElsIf {$((\rc.key = L\_key) \& (\checkv(L\_t\_id \downarrow,\rc \downarrow) = FALSE))$}\label{lin:stryc9}
\State Unlock all the variables;\label{lin:stryc10}
\State return $ABORT$;\label{lin:stryc11}

\EndIf;\label{lin:tryc12}
		\State \llspc{} \label{lin:tryc14};
		\EndWhile \label{lin:tryc15}
	\While{$(\textbf{$L\_rec_{i} \gets \textup{next}(L\_list$}))$} \label{lin:tryc17}
		\State ($L\_key, L\_obj\_id$) $\gets$ \llgkeyobj{} \label{lin:tryc18};
		\State $L\_opn$ $\gets$ $(L\_rec)_{i}$.$L\_opn$ \label{lin:tryc20};
		\State intraTransValdation($L\_rec_{i} \downarrow$, $\preds \uparrow$, $\currs \uparrow$) \label{lin:tryc42};
		\If{$($\textup{INSERT} $=$ \textup{$L\_opn$}$)$} \label{lin:tryc22}
		\If{$(\bc.key) = L\_key)$} \label{lin:tryc23}
	\State insert $v\_tuple \langle L\_t\_id,val,F,NULL,NULL \rangle$ into $G\_curr.vl$ in the increasing order;	\label{lin:tryc24}
	
	\ElsIf{$(\rc.key) = L\_key)$} \label{lin:stryc23}
	\State \lslins{$RL\_BL \downarrow$} \label{lin:stryc24}
	\State insert $v\_tuple \langle L\_t\_id,val,F,NULL,NULL \rangle$ into $G\_curr.vl$ in the increasing order;	\label{lin:stryc25}
	
		\Else \label{lin:tryc25}
		\State \lslins{$BL \downarrow$} \label{lin:tryc27};
		\State insert $v\_tuple \langle L\_t\_id,val,F,NULL,NULL \rangle$ into $node.vl$ in the increasing order;	\label{lin:tryc28}
	\EndIf \label{lin:tryc29}
\ElsIf{$($\textup{DELETE} $=$ $L\_opn)$} \label{lin:tryc31}
	\If{$(\bc.key) = L\_key)$} \label{lin:tryc33}
		\State insert $v\_tuple \langle L\_t\_id,NULL,T,NULL,NULL \rangle$ into $G\_curr.vl$ in the increasing order;	\label{lin:tryc34}
			\State \lsldel{} \label{lin:stryc35};
		\EndIf \label{lin:tryc39}
	
		\EndIf \label{lin:tryc40}
		\EndWhile \label{lin:tryc43}
        \State \rlsol{} \label{lin:tryc45};  
        \State $L\_tx\_status$ $\gets$ OK \label{lin:tryc47};
		\State return $\langle L\_tx\_status\rangle$\label{lin:tryc48};
		\EndProcedure \label{lin:tryc49}
	\end{algorithmic}
	%	\end{multicols}
\end{algorithm}

}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STM_init()

\begin{algorithm} 
\label{alg:init} 
\scriptsize

\caption{STM $\init()$: This method invokes at the start of the STM system. Initialize the global counter ($\cnt$) as 1 at \Lineref{init1} and return it.}
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{52}\makeatother	
\Procedure{STM init}{$\cnt \uparrow$}
\cmnts{Initializing the global counter}
\State $\cnt$ $\gets$ 1; \label{lin:init1}
\cmnt{
\ForAll {key $G\_k$ used by the STM System}
%\State /* $T_0$ is initializing key $k$ */
\State /*$T_0$ is initializing key $k$*/
\State add $\langle 0, 0, T, NULL, NULL \rangle$ to $G\_k.vl$;  \label{lin:init} %\Comment{Implies that $T_0$ has initialized $x$}
\EndFor;
}
\State return $\langle \cnt \rangle$; 
\EndProcedure
\end{algorithmic}
	
%	\end{multicols}
\end{algorithm}




\cmnt{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Traversal Phase%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[H]
\scriptsize
	\caption{list\_traversal() : It finds the location of the node corresponding to the key in underlying DS. First it identifies the node in \bn{} then in \rn{}. After finding the appropriate $\preds$ and $\currs$ corresponding to the key, it acquires the locks and validate it.}
	\label{algo:traversal}
	\setlength{\multicolsep}{0pt}
		%\begin{multicols}{2}
	\begin{algorithmic}[1]
	\makeatletter\setcounter{ALG@line}{166}\makeatother	
	\Procedure{list\_traversal}{$L\_Bucket\_id, L\_key$} \label{lin:ltraversal1}

%\cmnts{By default setting the $L\_op\_status$ as RETRY}\label{lin:lslsearch2}
	    %\State STATUS $L\_op\_status$ $\gets$ RETRY; \label{lin:lslsearch3}
	 %\cmnts{Identify the \preds and \currs for node corresponding to the key if $L\_op\_status$ is RETRY}\label{lin:lslsearch4}   
		%\While{($L\_op\_status$ = \textup{RETRY})} \label{lin:lslsearch5}
	%	\cmnts{Get the head of the bucket in chaining hash-table with the help of $L\_obj\_id$ and $L\_key$}\label{lin:lslsearch6}
		%\State $G\_head$ $\gets$ \glslhead \label{lin:lslsearch7};
	%	\cmnts{Initialize $\bp$ to head}\label{lin:lslsearch8}
		\State $\bp$ $\gets$ $G\_head$ \label{lin:ltraversal2}; 
	%	\cmnts{Initialize $\bc$ to $\bp.\bn$}\label{lin:lslsearch10}
		\State $\bc$ $\gets$ $\bp.\bn$ \label{lin:ltraversal3};
	%	\cmnts{Searching node corresponding to the key into \bn}
		\While{$((\bc.key) < L\_key)$} \label{lin:ltraversal4};
		\State $\bp$ $\gets$ $\bc$ \label{lin:ltraversal5};
				
		\State $\bc$ $\gets$ $\bc.\bn$ \label{lin:ltraversal6};
			
	%\EndWhile \label{lin:lslsearch15}
		
%		\cmnts{Initialize $\rp$ to head}\label{lin:slslsearch8}
		\State $\rp$ $\gets$ $\bp$ \label{lin:ltraversal7}; 
%		\cmnts{Initialize $\rc$ to $\rp.\rn$}\label{lin:slslsearch10}
		\State $\rc$ $\gets$ $\rp.\rn$ \label{lin:ltraversal8};
	%	\cmnts{Searching node corresponding to the key into \rn}
		\While{$((\rc.key) < L\_key)$} \label{lin:ltraversal9}
		\State $\rp$ $\gets$ $\rc$ \label{lin:ltraversal10};
				
		\State $\rc$ $\gets$ $\rc.\rn$ \label{lin:ltraversal11};
			
		\EndWhile \label{lin:ltraversal12}
		
		
		%\State    /*get the value*/
		%\State $L\_val$ $\gets$ $G\_curr.value$
		%\cmnts{Acquire the locks on increasing order of keys}\label{lin:lslsearch16}
	    \State acquirePred\&CurrLocks($ \preds$, $ \currs$); \label{lin:ltraversal13}
%\cmnts{Method validation to identify the changes done by concurrent conflicting method}\label{lin:lslsearch19}
		%\State methodValidation($\preds$ $\downarrow$, $\currs$ $\downarrow$, $L\_op\_status \uparrow$)\label{lin:lslsearch20};	
		%\State $op\_status$ $\gets$ \validation \label{lin:lslsearch21};
%\cmnts{If $L\_op\_status$ is RETRY then release all the locks}		\label{lin:lslsearch21}
	%	\If{(($L\_op\_status$ = \textup{RETRY}))} \label{lin:lslsearch22}
	   % \State releasePred\&CurrLocks($ \preds \downarrow$, $ \currs \downarrow$);
	    %\EndIf \label{lin:lslsearch25}
			
		\EndWhile \label{lin:ltraversal14}
		
		\State return $\langle G\_preds[], G\_currs[]\rangle$ \label{lin:ltraversal15};
	
	\EndProcedure \label{lin:ltraversal16}
	
	\end{algorithmic}
	%	\end{multicols}
\end{algorithm}
%\end{spacing}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STM_begin()
\begin{algorithm} 
\label{alg:begin} 
\scriptsize
\caption{STM $begin()$: It invoked by a thread to being a new transaction $T_i$. It creates transaction local log and allocate unique id at \Lineref{begin3} and \Lineref{begin5} respectively.}
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{88}\makeatother
\Procedure{STM begin}{$\cnt \downarrow$, $L\_t\_id \uparrow$} \label{lin:begin1}
\cmnts{Creating a local log for each transaction}\label{lin:begin2}
\State \txll $\gets$ create new \txllf;  \label{lin:begin3}
%\State /*Acquiring lock on live set of transaction*/
%\State $\livetx.lock()$;  
\cmnts{Getting transaction id ($L\_t\_id$) from $\cnt$}\label{lin:begin4}
\State \txll.$L\_t\_id$ $\gets$ $\cnt$;  \label{lin:begin5}
\cmnts{Incremented global counter atomically $\cnt$}\label{lin:begin6}
\State $\cnt$ $\gets$ \gi; //$\Phi_{lp}(Linearization Point)$ \label{lin:begin7}
%\State add $t\_id$ to $\livetx$; 
%\State /*Release lock on live set of transaction*/
%\State $\livetx.unlock()$; 
\State return $\langle L\_t\_id \rangle$; \label{lin:begin8}
\EndProcedure\label{lin:begin9}
\end{algorithmic}
%\end{multicols}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STM_ Insert()

\begin{algorithm}[H]

	\caption{STM $insert():$ Optimistically, the actual insertion will happen in the \nptc{} method. First, it will identify the node corresponding to the key in local log. If the node exists then it just update the local log with useful information like value, operation name and status for the node corresponding to the key at \Lineref{insert8}, \Lineref{insert9} and \Lineref{insert10} respectively for later use in \nptc{}. Otherwise, it will create a local log and update it.}
    \scriptsize
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
	\label{algo:insert}
	\begin{algorithmic}[1]
	\makeatletter\setcounter{ALG@line}{97}\makeatother
	\Procedure{STM insert}{$L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_val \downarrow$}\label{lin:insert1}
	\cmnts{First identify the node corresponding to the key into local log using $find()$ funciton}\label{lin:insert2}
		\If{$(!$\txlfind$)$}\label{lin:insert3}
		\cmnts{Create local log record and append it into increasing order of keys} \label{lin:insert4}
		\State $L\_rec$ $\gets$ create new $L\_rec \langle L\_obj\_id, L\_key \rangle$; \label{lin:insert5}
		\EndIf \label{lin:insert6}
		\cmnts{Updating the local log} \label{lin:insert7}		\State \llsval{$L\_val \downarrow$};//$\Phi_{lp} (Linearization Point)$ \label{lin:insert8}
		\State \llsopn{$INSERT \downarrow$}; \label{lin:insert9}
		\State \llsopst{$OK \downarrow$}; \label{lin:insert10}
		\State return $\langle void \rangle$; \label{lin:insert11} 
    	%\State loclog.setOpStatus$(obj\_id \downarrow, key \downarrow, OK \downarrow)$;
    \EndProcedure	\label{lin:insert12}
	\end{algorithmic}
%\end{multicols}	
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------------------------------STM\_LOOKUP-------------------------------------%------
%----
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{spacing}{2}
\begin{algorithm}[H]
	%\algsetup{linenosize=\tiny}
	
	\caption{\tabspace[0.2cm] STM $lookup_{i}()$: If \npluk{} is not the first method on a particular key means if its a subsequent method of the same transaction on that key then first it will search into the local log from \Lineref{lookup3} to \Lineref{lookup14}. If the previous method on the same key of same transaction was insert or lookup (from \Lineref{lookup7} to \Lineref{lookup9}) then \npluk{} will return the value and operation status based on previous operation value and status. If the previous method on the same key of same transaction was delete (from \Lineref{lookup11} to \Lineref{lookup13}) then \npluk{} will return the value and operation status as NULL and FAIL respectively. If \npluk{} is the first method on that key (from \Lineref{lookup16} to \Lineref{lookup22}) then it will identify the location of node corresponding to the key in underlying DS with the help of \nplsls{} inside the \npcld{} method at \Lineref{lookup17}.} %: If the transaction to which this operation belongs has locally done an operation on the same key then returns apt value and status(wrt the previous local operation). Else do the \nplsls{} to find the correct location of the key and validate it.
		%\emph{DESCP}\tabspace: If the Tx has locally done an operation returns apt value and status else does TO \tabspace[2.2cm] and method validation traversal phase in only.\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $obj\_id$, $key$\\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $value$, $op\_status$     }
	\scriptsize
	\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
		
		\label{algo:lookup}
		%	\setlength{\multicolsep}{0pt}
		%	\begin{multicols}{2}
		
		\begin{algorithmic}[1]
			\makeatletter\setcounter{ALG@line}{109}\makeatother
			\Procedure{STM lookup}{$L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_val \uparrow, L\_op\_status \uparrow$} \label{lin:lookup1}
			%\State $op\_status$ $\gets$ RETRY \label{lin:lookup2};
			\cmnts{First identify the node corresponding to the key into local log}\label{lin:lookup2}
			\If{$($\txlfind$)$} \label{lin:lookup3}
			\cmnts{Getting the previous operation's name}\label{lin:lookup4}
			\State $L\_opn$ $\gets$ \llgopn{} \label{lin:lookup5}; %\Comment{$\Phi_{lp}$}
			\cmnts{If previous operation is insert/lookup then get the value/op\_status based on the previous operations value/op\_status}\label{lin:lookup6}
			\If{$(($\textup{INSERT} $=$ \textup{$L\_opn$} $)||($ \textup{LOOKUP} $=$ \textup{$L\_opn$}$))$} \label{lin:lookup7}
			
			\State $L\_val$ $\gets$ \llgval{} \label{lin:lookup8};
			\State $L\_op\_status$ $\gets$  $L\_rec.L\_getOpStatus$($L\_obj\_id \downarrow, L\_key \downarrow$) \label{lin:lookup9};
			\cmnts{If previous operation is delete then set the value as NULL and op\_status as FAIL}\label{lin:lookup10}
			\ElsIf{$($\textup{DELETE} $=$ \textup{$L\_opn$}$)$} \label{lin:lookup11}
			\State $L\_val$ $\gets$ NULL \label{lin:lookup12}; 
			\State $L\_op\_status$ $\gets$ FAIL \label{lin:lookup13}; 
			\EndIf \label{lin:lookup14}
			%	\EndIf \label{lin:lookup11}
			\Else \label{lin:lookup15}
			\cmnts{ Common function for \rvmt{}, if node corresponding to the key is not part of local log}\label{lin:lookup16}
			\State \cld{};\label{lin:lookup17}
			\cmnt{		
				%\State $op\_status $ $\gets$ lslSearch($obj\_id$ $\downarrow$, $key$ $\downarrow$, $preds[]$ $\uparrow$, $currs[]$ $\uparrow$, $value_{BL}$ $\uparrow$, $RV$ $\downarrow$);	
				\State    /*if key is not present in local log then search in underlying DS with the help of list\_lookup*/
				\State \lsls{} \label{lin:lookup13}; 
				%State    /*if list\_lookup return op\_status as ABORT then method will return ABORT*/
				%If{$(op\_status_{ll}$ $=$ \textup{ABORT}$)$} \label{lin:lookup14}
				%			\State release all the locks
				%State \handlea{} \label{lin:lookup15}; 
				%Else \label{lin:lookup16}
				%			\State    /*check node corresponding to the key is part of underlying DS or not*/	
				%			\If{$((G\_curr.key) == L\_key)$} \label{lin:lookup17}
				\State /*From $G\_k.vls$, identify the right $version\_tuple$*/ 
				\State \find($L\_t\_id \downarrow,L\_key \downarrow, closest\_tuple \uparrow)$;	
				\State /*Adding $L\_t\_id$ into $j$'s $rvl$*/
				\State Append $L\_t\_id$ into $rvl$; 
				%                   \State \emph{unlock $x$};
				%                    \State return $(v)$; \Comment{v is the value returned}
				\If{$(closest\_tuple.m = TRUE)$}
				
				\State $L\_op\_status$ $\gets$ FAIL \label{lin:lookup18};
				\State $L\_val$ $\gets$ NULL \label{lin:lookup20};
				\Else
				\State $L\_op\_status$ $\gets$ OK;
				\State $L\_val$ $\gets$ $closest\_tuple.v$;
				\EndIf    
				%            \Else
				%                    \State /*Adding $i$ into $0$'s $rvl$*/
				%                    \State Append $i$ into $rvl$; 
				%                    \State $L\_op\_status$ $\gets$ FAIL;
				%                    \State $L\_val$ $\gets$ $NULL$;
				%\EndIf \label{lin:lookup30}
				
				
				\State $G\_pred.unlock()$;//$\Phi_{lp}$
				\State $G\_curr.unlock()$;
				\State    /*new log entry created to help upcoming method on the same key of the same tx*/
				\State $L\_rec$ $\gets$ Create new $L\_rec\langle L\_obj\_id, L\_key \rangle$\label{lin:lookup31}; 
				%\State ll.setPreds&Currs($obj\_id$ $\downarrow$, $key$ $\downarrow$, $preds[]$ $\downarrow$, $currs[]$ $\downarrow$);
				\State \llsval{$L\_val \downarrow$}
				\State \llspc{} \label{lin:lookup32};
			}						  
			
			%\EndIf \label{lin:lookup38}
			
			\EndIf \label{lin:lookup18}
			\cmnts{Update the local log} \label{lin:lookup19}
			\State \llsopn{$LOOKUP \downarrow$} \label{lin:lookup20};
			\State \llsopst{$L\_op\_status \downarrow$} \label{lin:lookup21};
			
			\State return $\langle L\_val, L\_op\_status\rangle$\label{lin:lookup22}; 
			
			\EndProcedure \label{lin:lookup23}
		\end{algorithmic}
		
%	\end{multicols}
	
\end{algorithm}



%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------------------------------STM\_DELETE-------------------------------------%------
%----
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{spacing}{2}
\begin{algorithm}[H]
%\algsetup{linenosize=\tiny}
\scriptsize
	\caption{\tabspace[0.2cm] STM $delete_{i}()$ : It will work same as a \npluk{}. If it is not the first method on a particular key means if its a subsequent method of the same transaction on that key then first it will search into the local log from \Lineref{delete3} to \Lineref{delete23}. If the previous method on the same key of same transaction was insert (from \Lineref{delete77} to \Lineref{delete10}) then \npdel{} will return the value based on previous operation value and status as OK and set the value and operation as NULL and DELETE respectively. 
    If previous method on the same key of same transaction was delete (from \Lineref{delete12} to \Lineref{delete15}) then \npdel{} will return the value and operation status as NULL and FAIL respectively.
    If previous method on the same key of same transaction was lookup (from \Lineref{delete16} to \Lineref{delete21}) then \npdel{} will return the value and operation status based on the previous operation value and status. If \npdel{} is the first method on that key (from \Lineref{delete24} to \Lineref{delete30}) then it will identify the location of node corresponding to the key in underlying DS with the help of \nplsls{} inside the \npcld{} method at \Lineref{delete25}.}
		%\emph{DESCP}\tabspace: If the Tx has locally done an operation returns apt value and status else does TO \tabspace[2.2cm] and method validation traversal phase in only.\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $obj\_id$, $key$\\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $value$, $op\_status$     }
	\label{algo:delete}
	\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
	
	\begin{algorithmic}[1]
	\makeatletter\setcounter{ALG@line}{132}\makeatother
		\Procedure{STM delete}{$L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_val \uparrow, L\_op\_status \uparrow$} \label{lin:delete1}
		%\State $op\_status$ $\gets$ RETRY \label{lin:lookup2};
			\cmnts{First identify the node corresponding to the key into local log}\label{lin:delete2}
		\If{$($\txlfind$)$} \label{lin:delete3}
	    \cmnts{Getting the previous operation's name}\label{lin:delete4}
			\State $L\_opn$ $\gets$ \llgopn{} ;\label{lin:delete5} %\Comment{$\Phi_{lp}$}
		\cmnts{If previous operation is insert then get the value based on the previous operations value and set the value and operation name as NULL and DELETE respectively}\label{lin:delete6}
		\If{$($\textup{INSERT} $=$ \textup{$L\_opn$}$)$} \label{lin:delete77}
		\State $L\_val$ $\gets$ \llgval{} \label{lin:delete7};
		
		\State \llsval{NULL $\downarrow$} \label{lin:delete8};

		\State \llsopn{DELETE $\downarrow$} \label{lin:delete9};
		
		\State $L\_op\_status$ $\gets$ OK \label{lin:delete10};
		\cmnts{If previous operation is delete then set the value as NULL}\label{lin:delete11}
		\ElsIf{$($\textup{DELETE} $=$ \textup{$L\_opn$}$)$} \label{lin:delete12}
		\State \llsval{NULL $\downarrow$} \label{lin:delete13};
		\State $L\_val$ $\gets$ NULL \label{lin:delete14}; 
		\State $L\_op\_status$ $\gets$ FAIL \label{lin:delete15}; 
		\Else \label{lin:delete16}
		
		\cmnts{If previous operation is lookup then get the value based on the previous operations value and set the value and operation name as NULL and DELETE respectively}\label{lin:delete17}
		\State $L\_val$ $\gets$ \llgval{} \label{lin:delete18}; 
		
		\State \llsval{NULL$ \downarrow$} \label{lin:delete19};
		
		
		\State \llsopn{DELETE $\downarrow$} \label{lin:delete20};
		\State $L\_op\_status$ $\gets$  $L\_rec.getOpStatus$($L\_obj\_id \downarrow$, $L\_key \downarrow$) \label{lin:delete21};
		
		\EndIf \label{lin:delete22}
		
		\Else \label{lin:delete23}
						  
					
	%	\EndIf 
		    \cmnts{Common function for \rvmt{}, if node corresponding to the key is not part of local log}\label{lin:delete24}
			\State \cld{};		\label{lin:delete25}
		\EndIf \label{lin:delete26}
		\cmnts{Update the local log}\label{lin:delete27}
		\State \llsopn{$DELETE \downarrow$} ;\label{lin:delete28}
			\State \llsopst{$L\_op\_status \downarrow$} ;\label{lin:delete29}
			
			\State return $\langle L\_val, L\_op\_status\rangle$; \label{lin:delete30}
				
	\EndProcedure\label{lin:delete31}
	\end{algorithmic}
	
%	\end{multicols}
	
\end{algorithm}
\cmnt{
\begin{figure}[H]
	\captionsetup{justification=centering}
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centerline{\scalebox{0.38}{\input{figs/pnetys5.pdf_t}}}
	\caption{Need of inserting $0^{th}$ version by \rvmt{} to satisfy opacity}
	\label{fig:mvostm8}
\end{figure}	
}
\begin{figure}[H]
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centerline{\scalebox{0.35}{\input{figs/mvostm8.pdf_t}}}
	\caption{Need of inserting $0^{th}$ version by \rvmt{} to satisfy opacity}
	\label{fig:mvostm8}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------------------------------commonLu\&Del-------------------------------------%------
%----
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{spacing}{2}
\begin{algorithm}[H]
%\algsetup{linenosize=\tiny}
%\scriptsize
	\caption{\tabspace[0.2cm] $commonLu\&Del()$ : This method is invoked by a \rvmt{} (\npluk{} and \npdel{}$)$, if node corresponding to the key is not part of local log. At \Lineref{com3} it identify the $\preds$ and $\currs$ for the node corresponding to the key in underlying DS with the help of \nplsls{}. If node corresponding to the key is in \bn{} of underlying DS then (from \Lineref{com5} to \Lineref{com17}) it finds the version tuple corresponding to the key which is having the largest timestamp less than itself as $closest\_tuple$ at \Lineref{com7}. After that, it will add itself into $closest\_tuple.rvl$ at \Lineref{com9}. If identified version mark field is TRUE then it will set the $L\_op\_status$ and $L\_val$ as FAIL and NULL otherwise, OK and value of identified tuple from \Lineref{com11} to \Lineref{com17} respectively. If node corresponding to the key is in \rn{} of underlying DS then (from \Lineref{scom5} to \Lineref{scom17}) it finds the version tuple corresponding to the key which is having the largest timestamp less than itself as $closest\_tuple$ at \Lineref{scom7}. After that, it will add itself into $closest\_tuple.rvl$ at \Lineref{scom9}. If identified version mark field is TRUE then it will set the $L\_op\_status$ and $L\_val$ as FAIL and NULL otherwise, OK and value of identified tuple from \Lineref{scom11} to \Lineref{scom17} respectively. 
	If node corresponding to the key is not part of underlying DS then (from \Lineref{com19} to \Lineref{com27}) it will create the new node corresponding to the key and add it into \rn{} of underlying DS with the help of \nplslins{} at \Lineref{com20}. After that it creates the $0^{th}$ version (at \Lineref{com22}) and add itself into $0^{th}.rvl$ at \Lineref{com23}. Then, it will set the $L\_op\_status$ and $L\_val$ as FAIL and NULL respectively at \Lineref{com25} and \Lineref{com26}. Finally, it will release the lock which is acquired in \nplsls{} at \Lineref{com3} and update the local log to help the upcoming method of the same transaction on the same key. \textbf{Why do we need to create a $0^{th}$ version by \rvmt{} in \rn{}?} This will be clear by the \figref{mvostm8}, where we have two concurrent transactions $T_1$ and $T_2$. History in the \figref{mvostm8}.a) is not opaque because we can't come up with any serial order. To make it serial (or opaque) first method $lu_2(ht, k_3, NULL)$ of transaction $T_2$ have to create the $0^{th}$ version in \rn{} if its not present in the underlying DS and add itself into $0^{th}.rvl$. So in future if any lower timestamp transaction less than $T_2$ will come then that lower transaction will ABORT (in this case transaction $T_1$ is aborting in (\figref{mvostm8}.b))) because higher timestamp already present in the $rvl$ (\figref{mvostm8}.c)) of the same version. After aborting $T_1$ we will get the serial history.}
	\scriptsize
\setlength{\multicolsep}{0pt}
%\begin{multicols}{2}
	
	\label{algo:commonlu&del}
%	\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
	
	\begin{algorithmic}[1]
	\makeatletter\setcounter{ALG@line}{164}\makeatother
		\Procedure{commonLu\&Del}{$L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_val \uparrow, L\_op\_status \uparrow$} \label{lin:com1} %\label{lin:commonlu&del}
		%\State $op\_status$ $\gets$ RETRY \label{lin:lookup2};
    \cmnts{If node corresponding to the key is not present in local log then search into underlying DS with the help of list\_lookup} \label{lin:com2}
			\State \lsls{}\label{lin:com3};
			\cmnts{ If node corresponding to the key is part of \bn{}}\label{lin:com4}
			\If{$(\bc.key = L\_key)$}\label{lin:com5}
						\cmnts{From $\bc.vls$, identify the right $version\_tuple$} \label{lin:com6}
                    \State \find($L\_t\_id \downarrow,\bc \downarrow, closest\_tuple \uparrow)$;\label{lin:com7}
                    
                    \cmnts{ Closest\_tuple is $\langle j,val,mark,rvl,vnext \rangle$} \label{lin:com8}

                    \State Adding $L\_t\_id$ into $j$'s $rvl$; \label{lin:com9}
                    %\State Append $L\_t\_id$ into $rvl$; 
 %                   \State \emph{unlock $x$};
%                    \State return $(v)$; \Comment{v is the value returned}
\cmnts{If the $closest\_tuple$ mark field is TRUE then $L\_op\_status$ and $L\_val$ set as FAIL and NULL otherwise set OK and value of $closest\_tuple$ respectively}\label{lin:com10}
                \If{$(closest\_tuple.mark = TRUE)$}\label{lin:com11}
                    
                    \State $L\_op\_status$ $\gets$ FAIL \label{lin:com12};
                    \State $L\_val$ $\gets$ NULL \label{lin:com13};
                \Else\label{lin:com14}
                    \State $L\_op\_status$ $\gets$ OK;\label{lin:com15}
                    \State $L\_val$ $\gets$ $closest\_tuple.val$; \label{lin:com16}
                \EndIf    \label{lin:com17}
        \cmnts{If node corresponding to the the key is part of \rn }
			\ElsIf{$(\rc.key = L\_key)$}\label{lin:scom5}
						\cmnts{From $\rc.vls$, identify the right $version\_tuple$} \label{lin:scom6}
                    \State \find($L\_t\_id \downarrow,\rc \downarrow, closest\_tuple \uparrow)$;\label{lin:scom7}
                    
                    \cmnts{Closest\_tuple is $\langle j,val,mark,rvl,vnext \rangle$} \label{lin:scom8}
\algstore{myalg}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}                     
	\begin{algorithmic} [1]                   % enter the algorithmic environment
			\scriptsize
		\algrestore{myalg}
                    \State Adding $L\_t\_id$ into $j$'s $rvl$; \label{lin:scom9}
                    %\State Append $L\_t\_id$ into $rvl$; 
 %                   \State \emph{unlock $x$};
%                    \State return $(v)$; \Comment{v is the value returned}
\cmnts{If the $closest\_tuple$ mark field is TRUE then $L\_op\_status$ and $L\_val$ set as FAIL and NULL otherwise set OK and value of $closest\_tuple$ respectively}\label{lin:scom10}
                \If{$(closest\_tuple.mark = TRUE)$}\label{lin:scom11}
                    
                    \State $L\_op\_status$ $\gets$ FAIL \label{lin:scom12};
                    \State $L\_val$ $\gets$ NULL \label{lin:scom13};
                \Else\label{lin:scom14}
                    \State $L\_op\_status$ $\gets$ OK;\label{lin:scom15}
                    \State $L\_val$ $\gets$ $closest\_tuple.val$; \label{lin:scom16}
                \EndIf    \label{lin:scom17}
 
        
        
                
        \Else\label{lin:com18}
        		\cmnts{If node corresponding to the key is not part of \rn as well as \bn then create the node into \rn with the help of list\_Ins()}\label{lin:com19}
		        \State \lslins{$RL \downarrow$};\label{lin:com20}
		        \cmnts{Insert the $0^{th}$ version tuple} \label{lin:com21}
		        \State insert $v\_tuple \langle 0,NULL,T,NULL,NULL \rangle$ into $node.vl$ in the increasing order;	 \label{lin:com22}
                  \State Adding $L\_t\_id$ into $0^{th}.rvl$;\label{lin:com23}
                    %\State Append $L\_t\_id$ into $rvl$;
                \cmnts{Setting $L\_op\_status$ and $L\_val$ as FAIL and NULL because its reading from the marked version, which is TRUE}\label{lin:com24}    
                \State    $L\_op\_status$ $\gets$ FAIL ;\label{lin:com25}
                    \State $L\_val$ $\gets$ NULL ;\label{lin:com26}
			\EndIf\label{lin:com27}
			\cmnts{Releasing the locks in increasing order}\label{lin:com28}
			  	    \State releasePred\&CurrLocks($ \preds \downarrow$, $ \currs \downarrow$);
\cmnts{Create local log record and append it into increasing order of keys}\label{lin:com31}						\State $L\_rec$ $\gets$ Create new $L\_rec\langle L\_obj\_id, L\_key \rangle$\label{lin:com32}; 
						%\State ll.setPreds&Currs($obj\_id$ $\downarrow$, $key$ $\downarrow$, $preds[]$ $\downarrow$, $currs[]$ $\downarrow$);
						\State \llsval{$L\_val \downarrow$} \label{lin:com33}
						\State \llspc{} ;
						  
			
			\State return $\langle L\_val, L\_op\_status\rangle$;\label{lin:com34}
				
	\EndProcedure 
	\end{algorithmic}
	
%	\end{multicols}
	
\end{algorithm}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------------------------------TryCommit----------------------------------%---------
%----
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[H]
\scriptsize
	\caption{\tabspace[0.2cm] STM $tryC()$ : The actual effect of \upmt{s} (\npins{} and \npdel{}) will take place in \nptc{} method. From \Lineref{tryc5} to \Lineref{tryc15} will identify and validate the $\preds$ and $\currs$ of each \upmt{} of same transaction. At \Lineref{tryc9} it will validate if there exist any higher timestamp transaction in the $rvl$ of the $closest\_tuple$ of $\bc$ then returns ABORT at \Lineref{tryc11}. Same as at \Lineref{stryc9} it will validate if there exist any higher timestamp transaction in the $rvl$ of the $closest\_tuple$ of $\rc$ then returns ABORT at \Lineref{stryc11}. Otherwise it will perform the above steps for remaining \upmt{s}. On successful validation of all the \upmt{s}, the actually effect will be taken place from \Lineref{tryc17} to \Lineref{tryc43}. If the \upmt{} is insert and node corresponding to the key is part of \bn{} then it creates the new version tuple and add it in increasing order of version list from \Lineref{tryc22} to \Lineref{tryc24}. If node corresponding to the key is part of \rn{} then it adds the same node in the \bn{} as well with the help of \nplslins{} at \Lineref{stryc24} and creates the new version tuple and add it in increasing order of version list from \Lineref{stryc23} to \Lineref{stryc25}. Otherwise it will create the node and insert it into \bn{} with the help of \nplslins{} and insert the version tuple from \Lineref{tryc25} to \Lineref{tryc29}. If the \upmt{} is delete and node corresponding to the key is part of \bn{} then it creates the new version tuple and set its mark field as TRUE and add it in increasing order of version list from \Lineref{tryc31} to \Lineref{stryc35}. After successful completion of each \upmt{}, it will validate the $\preds$ and $\currs$ of upcoming \upmt{} of the same transaction with the help of \npintv{} at \Lineref{tryc42}. Eventually, it will release all the locks at \Lineref{tryc45} in the same order of lock acquisition.} %: All update methods will takes effect in underlying data-structure atomically if the validation will succeed. 
		%\emph{DESCP}\tabspace: All update methods of the transaction take ordered locks, validate and update underlying \tabspace[2.2cm]  data-structure atomically. \\
		%\emph{IN}\tabspace \tabspace[0.72cm]: \\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $txstatus$     }
	\label{algo:trycommit}
	\setlength{\multicolsep}{0pt}
%		\begin{multicols}{2}
	\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{213}\makeatother
		\Procedure{STM tryC}{$L\_t\_id \downarrow, L\_tx\_status \uparrow$} \label{lin:tryc1}

%\State    /*get the tx id*/
%		\State $L\_t\_id$ $\gets$ getTS($t_i \downarrow$) \label{lin:tryc2};
		\cmnts{Get the local log list corresponding to each transaction which is in increasing order of keys}\label{lin:tryc2}
		\State $L\_list$ $\gets$ $L\_txlog.getList$($L\_t\_id \downarrow$) \label{lin:tryc3};
%		\State    /*sort the local log in increasing order of keys and copy into ordered list*/
%		\State $L\_ordered$ $\gets$ \llsort{} \label{lin:tryc4};
\cmnts{Identify the new $\preds$ and $\currs$ for all update methods of a transaction and validate it}\label{lin:tryc4}
		\While{$(\textbf{$L\_rec_{i} \gets \textup{next}(L\_list$}))$} \label{lin:tryc5}
		\State ($L\_key, L\_obj\_id$) $\gets$ \llgkeyobj{} \label{lin:tryc6};
		\cmnts{Identify the new $G\_pred$ and $G\_curr$ location with the help of list\_lookup()}\label{lin:tryc7}
		\State \lsls{$COMMIT \downarrow$} \label{lin:tryc8};
			
		\If {$((\bc.key = L\_key) \& (\checkv(L\_t\_id \downarrow,\bc \downarrow) = FALSE))$}\label{lin:tryc9}
%\State $\remid(i)$;
\State Unlock all the variables;\label{lin:tryc10}
\State return $ABORT$;\label{lin:tryc11}
\ElsIf {$((\rc.key = L\_key) \& (\checkv(L\_t\_id \downarrow,\rc \downarrow) = FALSE))$}\label{lin:stryc9}
%\State $\remid(i)$;
\State Unlock all the variables;\label{lin:stryc10}
\State return $ABORT$;\label{lin:stryc11}

\EndIf;\label{lin:tryc12}

					%State    /*if list\_lookup return op\_status as ABORT then method will return ABORT*/
		%If{$(op\_status_{ll}$ $=$ \textup{ABORT}$)$} \label{lin:tryc8}
%		\State release all the locks
		%State \handlea{} \label{lin:tryc9};
		
		%\State return \label{lin:tryc10};
		
		%EndIf \label{lin:tryc11}
			\cmnts{Update the log entry} \label{lin:tryc13}

		\State \llspc{} \label{lin:tryc14};
		\EndWhile \label{lin:tryc15}
	\cmnts{Get each update method one by one and take effect in underlying DS}\label{lin:tryc16}
		\While{$(\textbf{$L\_rec_{i} \gets \textup{next}(L\_list$}))$} \label{lin:tryc17}
		\State ($L\_key, L\_obj\_id$) $\gets$ \llgkeyobj{} \label{lin:tryc18};
		\cmnts{Get the operation name from local log record}\label{lin:tryc19}
		\State $L\_opn$ $\gets$ $(L\_rec)_{i}$.$L\_opn$ \label{lin:tryc20};
		
					\cmnts{Modify the $\preds$ and $\currs$ for the consecutive update methods which are working on overlapping zone in lazy-list}\label{lin:tryc41}
		\State intraTransValdation($L\_rec_{i} \downarrow$, $\preds \uparrow$, $\currs \uparrow$) \label{lin:tryc42};
\cmnts{If operation is insert then after successful completion of it node corresponding to the key should be part of \bn}\label{lin:tryc21}
\algstore{myalg}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}                     
	\begin{algorithmic} [1]                   % enter the algorithmic environment
			\scriptsize
		\algrestore{myalg}
		\If{$($\textup{INSERT} $=$ \textup{$L\_opn$}$)$} \label{lin:tryc22}
	%\State    /*if node corresponding to the key is part of \bn*/
		\If{$(\bc.key) = L\_key)$} \label{lin:tryc23}
	\State insert $v\_tuple \langle L\_t\_id,val,F,NULL,NULL \rangle$ into $G\_curr.vl$ in the increasing order;	\label{lin:tryc24}
	
	\ElsIf{$(\rc.key) = L\_key)$} \label{lin:stryc23}
	\State \lslins{$RL\_BL \downarrow$} \label{lin:stryc24}
	\State insert $v\_tuple \langle L\_t\_id,val,F,NULL,NULL \rangle$ into $G\_curr.vl$ in the increasing order;	\label{lin:stryc25}
	
		\Else \label{lin:tryc25}
		\cmnts{If node corresponding to the key is not part underlying DS then create the node with the help of list\_Ins() and insert it into \bn}\label{lin:tryc26}
		\State \lslins{$BL \downarrow$} \label{lin:tryc27};
		\State insert $v\_tuple \langle L\_t\_id,val,F,NULL,NULL \rangle$ into $node.vl$ in the increasing order;	\label{lin:tryc28}
%	\State    /*set the op\_status as OK in local log*/
%		\State \llsopst{$OK \downarrow$} \label{lin:tryc30};
	%\State    /*update the max\_ts of insert for node corresponding to the key into underlying DS*/		
	%	\State $\texttt{write}$(node.max\_ts.insert, TS($t_i$)) \label{lin:tryc31};
		\EndIf \label{lin:tryc29}
		\cmnts{If operation is delete then after successful completion of it node corresponding to the key should part of \rn only}\label{lin:tryc30}
		\ElsIf{$($\textup{DELETE} $=$ $L\_opn)$} \label{lin:tryc31}
	\cmnts{If node corresponding to the key is part of \bn}\label{lin:tryc32}
	

	
		\If{$(\bc.key) = L\_key)$} \label{lin:tryc33}
	%\State    /*delete the node corresponding to the key from the \bn with the help of lslDel()*/	
			\State insert $v\_tuple \langle L\_t\_id,NULL,T,NULL,NULL \rangle$ into $G\_curr.vl$ in the increasing order;	\label{lin:tryc34}
			\State \lsldel{} \label{lin:stryc35};
%		\State    /*set the op\_status as OK in local log*/
%		\State \llsopst{$OK \downarrow$} \label{lin:tryc36};
		%\State    /*update the max\_ts of delete for node corresponding to the key into underlying DS*/	
		%\State $\texttt{write}$(\textcolor{blue}{$currs[1]$}.max\_ts.delete, TS($t_i$)) \label{lin:tryc37};
\cmnt{
		\Else \label{lin:tryc35}
		\State    /*If node corresponding to the key is not part underlying DS then create the node with the help of list\_Ins() */\label{lin:tryc36}
		\State \lslins{$RL \downarrow$};\label{lin:tryc37}
		
		\State insert $v\_tuple \langle L\_t\_id,NULL,T,NULL,NULL \rangle$ into $node.vl$ in the increasing order;	\label{lin:tryc38}
		%\State \llsopst{$FAIL \downarrow$} \label{lin:tryc39};
		
		%\State $write$(\textcolor{red}{$currs[0]$}.max\_ts.delete, TS($t_i$)) \label{lin:tryc40};
}	
		\EndIf \label{lin:tryc39}
	
		\EndIf \label{lin:tryc40}
		

			
		\EndWhile \label{lin:tryc43}
		\cmnts{Release all the locks in increasing order}\label{lin:tryc44}
		\State \rlsol{} \label{lin:tryc45};  
		\cmnts{Set the transaction status as OK}\label{lin:tryc46}
		\State $L\_tx\_status$ $\gets$ OK \label{lin:tryc47};
%		
%		\State \txsetst{} \label{lin:tryc46};
		\State return $\langle L\_tx\_status\rangle$\label{lin:tryc48};
		\EndProcedure \label{lin:tryc49}
	\end{algorithmic}
%		\end{multicols}
\end{algorithm}


	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%------------------- lazyrblist-delete -----------------------
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\begin{algorithm}[H]
		\scriptsize
		\caption{\tabspace[0.2cm] \dell() : Delete a node from blue link in underlying hash table at location corresponding to $\preds$ \& $\currs$.}
			%\emph{DESCP}\tabspace: Deletes a node from blue list in underlying hash table at location corresponding to \tabspace[2.2cm] preds[] \& currs[].\\
			%\emph{IN}\tabspace \tabspace[0.72cm]: $preds[], currs[]$  \\
			%\emph{OUT}\tabspace \tabspace[0.37cm]:  }
		\label{algo:lsldelete}
		\setlength{\multicolsep}{0pt}
%		\begin{multicols}{2}
			\begin{algorithmic}[1]
				\makeatletter\setcounter{ALG@line}{265}\makeatother
				\Function{list\_del}{$\preds \downarrow, \currs \downarrow$} \label{lin:lsldel1}
				
				%\cmnts{mark the node$ \langle obj\_id, key \rangle$ for deletion}
				%\State $\texttt{write}$($\bc$.marked, True) \label{lin:lsldel2};
				\cmnts{Update the blue links}
				\State $\bp$.\bn $\gets$ $\bc$.\bn \label{lin:lsldel3};
				\State return $\langle void \rangle$;
				\EndFunction \label{lin:lsldel4}
			\end{algorithmic}
			
%		\end{multicols}
	\end{algorithm}
	



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%----------------- List lookup() ---------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{spacing}{0.8}
\begin{algorithm}[H]
\scriptsize
%lslSearch($obj\_id \downarrow, key \downarrow, preds[] \uparrow, currs[] \uparrow, value \uparrow, val\_type \downarrow$)
	\caption{list\_lookup() : This method is called by \rvmt{} and \upmt{}. It finds the location of the node corresponding to the key in underlying DS from \Lineref{lslsearch5} to \Lineref{slslsearch15}. First it identifies the node in \bn{} (from \Lineref{lslsearch5} to \Lineref{lslsearch15}) then in \rn{} (from \Lineref{slslsearch9} to \Lineref{slslsearch15}). After finding the appropriate location of the node corresponding to the key in the form of $\preds$ and $\currs$, it will acquire the locks on it at \Lineref{lslsearch17} and validate it at \Lineref{lslsearch20}.}
		%\emph{DESCP}\tabspace: Finds location of the corresponding $\left\langle obj\_id, key  \right\rangle$ in underlying hash table. color of preds[] \tabspace[2.2cm] \& currs[] depicts the red or blue node.\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $\left\langle obj\_id, key  \right\rangle$, $val\_type$  \\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $preds[], currs[], value$     }
	\label{algo:lslsearch}
	\setlength{\multicolsep}{0pt}
%		\begin{multicols}{2}
	\begin{algorithmic}[1]
	\makeatletter\setcounter{ALG@line}{270}\makeatother	
		\Procedure{list\_lookup}{$L\_obj\_id \downarrow, L\_key \downarrow, G\_preds[] \uparrow, G\_currs[] \uparrow$} \label{lin:lslsearch1}

	\cmnts{By default setting the $L\_op\_status$ as RETRY}\label{lin:lslsearch2}
	    \State STATUS $L\_op\_status$ $\gets$ RETRY; \label{lin:lslsearch3}
	 \cmnts{Identify the \preds and \currs for node corresponding to the key if $L\_op\_status$ is RETRY}\label{lin:lslsearch4}   
		\While{($L\_op\_status$ = \textup{RETRY})} \label{lin:lslsearch5}
		\cmnts{Get the head of the bucket in chaining hash-table with the help of $L\_obj\_id$ and $L\_key$}\label{lin:lslsearch6}
		\State $G\_head$ $\gets$ \glslhead \label{lin:lslsearch7};
		\cmnts{Initialize $\bp$ to head}\label{lin:lslsearch8}
		\State $\bp$ $\gets$ $G\_head$ \label{lin:lslsearch9}; 
		\cmnts{Initialize $\bc$ to $\bp.\bn$}\label{lin:lslsearch10}
		\State $\bc$ $\gets$ $\bp.\bn$ \label{lin:lslsearch11};
		\cmnts{Searching node corresponding to the key into \bn}
		\While{$((\bc.key) < L\_key)$} \label{lin:lslsearch12}
		\State $\bp$ $\gets$ $\bc$ \label{lin:lslsearch13};
				
		\State $\bc$ $\gets$ $\bc.\bn$ \label{lin:lslsearch14};
			
		\EndWhile \label{lin:lslsearch15}
		
		\cmnts{Initialize $\rp$ to head}\label{lin:slslsearch8}
		\State $\rp$ $\gets$ $\bp$ \label{lin:slslsearch9}; 
		\cmnts{Initialize $\rc$ to $\rp.\rn$}\label{lin:slslsearch10}
		\State $\rc$ $\gets$ $\rp.\rn$ \label{lin:slslsearch11};
		\cmnts{Searching node corresponding to the key into \rn}
		\While{$((\rc.key) < L\_key)$} \label{lin:slslsearch12}
		\State $\rp$ $\gets$ $\rc$ \label{lin:slslsearch13};
				
		\State $\rc$ $\gets$ $\rc.\rn$ \label{lin:slslsearch14};
			
		\EndWhile \label{lin:slslsearch15}
		
		
		%\State    /*get the value*/
		%\State $L\_val$ $\gets$ $G\_curr.value$
		\cmnts{Acquire the locks on increasing order of keys}\label{lin:lslsearch16}
	    \State acquirePred\&CurrLocks($ \preds \downarrow$, $ \currs \downarrow$); \label{lin:lslsearch17}
\cmnts{Method validation to identify the changes done by concurrent conflicting method}\label{lin:lslsearch19}
		\State methodValidation($\preds$ $\downarrow$, $\currs$ $\downarrow$, $L\_op\_status \uparrow$)\label{lin:lslsearch20};	
		%\State $op\_status$ $\gets$ \validation \label{lin:lslsearch21};
\cmnts{If $L\_op\_status$ is RETRY then release all the locks}		\label{lin:lslsearch21}
		\If{(($L\_op\_status$ = \textup{RETRY}))} \label{lin:lslsearch22}
	    \State releasePred\&CurrLocks($ \preds \downarrow$, $ \currs \downarrow$);
	    \EndIf \label{lin:lslsearch25}
			
		\EndWhile \label{lin:lslsearch26}
		
		\State return $\langle G\_preds[], G\_currs[]\rangle$ \label{lin:lslsearch27};
	
	\EndProcedure \label{lin:lslsearch28}
	\end{algorithmic}
%		\end{multicols}
\end{algorithm}
%\end{spacing}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%------------------- acquirepreds&currs -----------------------
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\begin{algorithm}[H]
		\scriptsize
		\caption{\tabspace[0.2cm] acquirePred\&CurrLocks() : acquire all locks taken during \nplsls{}.}
			%\emph{DESCP}\tabspace: releases all locks taken during tryCommit\\
			%\emph{IN}\tabspace \tabspace[0.72cm]: $ordered\_ll\_list$\\
			%\emph{OUT}\tabspace \tabspace[0.37cm]:   }
		\label{algo:acquirepreds&currs}
		\setlength{\multicolsep}{0pt}
%		\begin{multicols}{2}
			\begin{algorithmic}[1]
				\makeatletter\setcounter{ALG@line}{306}\makeatother
				\Function{acquirePred\&CurrLocks}{$ \preds \downarrow$, $ \currs \downarrow$}
				\State $\bp$.$\texttt{lock()}$;
				\State $\rp$.$\texttt{lock()}$;
				\State $\rc$.$\texttt{lock()}$;
				\State $\bc$.$\texttt{lock()}$;
				\State return $\langle void \rangle$;        
				\EndFunction
			\end{algorithmic}
			
%		\end{multicols}
	\end{algorithm}
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%------------------- releasepreds&currs -----------------------
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\begin{algorithm}[H]
		\scriptsize
		\caption{\tabspace[0.2cm] releasePred\&CurrLocks() : Release all locks taken during \nplsls{}.}
			%\emph{DESCP}\tabspace: releases all locks taken during tryCommit\\
			%\emph{IN}\tabspace \tabspace[0.72cm]: $ordered\_ll\_list$\\
			%\emph{OUT}\tabspace \tabspace[0.37cm]:    }
		\label{algo:releasepreds&currs}
		\setlength{\multicolsep}{0pt}
%		\begin{multicols}{2}
			\begin{algorithmic}[1]
				\makeatletter\setcounter{ALG@line}{313}\makeatother
				\Function{releasePred\&CurrLocks}{$ \preds \downarrow$, $ \currs \downarrow$}
				\State $\bp$.$\texttt{unlock()}$\label{lin:rpandc};//$\Phi_{lp}$ 
				\State $\rp$.$\texttt{unlock()}$;
				\State $\rc$.$\texttt{unlock()}$;
				\State $\bc$.$\texttt{unlock()}$;
				\State return $\langle void \rangle$;        
				\EndFunction
			\end{algorithmic}
			
%		\end{multicols}
	\end{algorithm}
	%\end{multicols}
	

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%----------------------------list-insert --------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\vspace{-.5cm}
\begin{algorithm}[H]
\scriptsize
	\caption{\tabspace[0.2cm] list\_Ins(): This method is called by the \rvmt{} and \upmt{}. Color of preds \& currs depicts the red or blue node.}
		%\emph{DESCP}\tabspace: Inserts or overwrites a node in underlying hash table at location corresponding to \tabspace[2.2cm] preds[] \& currs[]. Color of preds[] \& currs[] depicts the red or blue node.\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $preds[], currs[], list\_type$  \\
		%\emph{OUT}\tabspace \tabspace[0.37cm]:     }
	\label{algo:lslins}
		\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
	\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{320}\makeatother
		\Procedure{list\_Ins}{$\preds \downarrow, \currs \downarrow, list\_type \downarrow, node \uparrow$} \label{lin:lslins1}


\cmnts{Inserting the node from redlist to bluelist}
				\If{$((list\_type)$ $=$ $($\textcolor{black}{$RL$}$\_$\textcolor{black}{$BL$}$))$} \label{lin:lslins2}
				
				%\State $\texttt{write}$($\rc$.marked, false) \label{lin:lslins3}; 
				\State $\rc$.\bn $\gets$ $\bc$ \label{lin:lslins4};
				\State $\bp$.\bn $\gets$ $\rc$ \label{lin:lslins5};
				\cmnts{Inserting the node into redlist only}
				\ElsIf{$((list\_type$) $=$ \textcolor{black}{$RL$}$)$} \label{lin:lslins6}
				\State node = Create new node()
				\label{lin:lslins7};
						\cmnts{After created the node acquiring the lock on it}\label{lin:lslins4}
		\State node.lock();\label{lin:lslins5}
		
				\State node.\rn $\gets$ $\rc$ \label{lin:lslins9};
				\State $\rp$.\rn $\gets$ node \label{lin:lslins10};
				
				\Else \label{lin:lslins11}
				\cmnts{Inserting the node into red as well as blue list}
				\State node = new node() \label{lin:lslins12}; %\Comment{default locked state for thread validation}
				\cmnts{After creating the node acquiring the lock on it}
				\State node.lock();
				\State node.\rn $\gets$ $\rc$ \label{lin:lslins13};
				\State node.\bn $\gets$ $\bc$ \label{lin:lslins14};
				
				\State $\rp$.\rn $\gets$ node \label{lin:lslins15};
				
				\State $\bp$.\bn $\gets$ node \label{lin:lslins16};
				\EndIf \label{lin:lslins17}
				\State return $\langle node \rangle$;
			
\cmnt{

        \State    /*Inserting the new node corresponding to the key into Underlying DS/\label{lin:lslins2}
		\State node = Create new node() \label{lin:lslins3}; %\Comment{default locked state for thread validation}
		\State    /*After created the node acquiring the lock on it*/\label{lin:lslins4}
		\State node.lock();\label{lin:lslins5}
		\State /*Adding the new node at appropriate location (in increasing order of the keys) with the help of $G\_pred$ and $G\_curr$*/\label{lin:lslins6}
		\State node.knext $\gets$ $G\_curr$ \label{lin:lslins7};
		\State $G\_pred$.knext $\gets$ node \label{lin:lslins8};
		\State return $\langle node \rangle$;\label{lin:lslins9}}
		\EndProcedure \label{lin:lslins10}
	\end{algorithmic}
%	\end{multicols}
\end{algorithm}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% find_lts(largest timestamp but less then itself)   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}  
\scriptsize
\label{alg:select}
\caption{$\find()$: This method is called by \rvmt{} and \upmt{} to identify a  $closest\_tuple$ $\langle j,val,mark,rvl,vnext \rangle$ created by the transaction $T_j$ with the largest timestamp smaller than $L\_t\_id$ from \Lineref{findlts5} to \Lineref{findlts10}.}
		\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{344}\makeatother
\Procedure{find\_lts}{$L\_t\_id \downarrow, \currs \downarrow, closest\_tuple \uparrow$} \label{lin:findlts1}
\cmnts{Initialize $closest\_tuple$} \label{lin:findlts2}
\State $closest\_tuple = \langle 0,NULL,F,NULL,NULL \rangle$;\label{lin:findlts3}
\cmnts{For all the version of $\currs$ identify the largest timestamp less than $L\_t\_id$} \label{lin:findlts4}
\ForAll {$\langle p,val,mark,rvl,vnext \rangle \in \currs.vl$} \label{lin:findlts5}
\If {$(p < L\_t\_id)$ and $(closest\_tuple.ts < p)$} \label{lin:findlts6}
\cmnts{Assign closest tuple as $\langle p,val,mark,rvl,vnext \rangle$, if any version tuple is having largest timestamp less then L\_t\_id exist} \label{lin:findlts7}
\State $closest\_tuple = \langle p,val,mark,rvl,vnext \rangle$; \label{lin:findlts8}
\EndIf\label{lin:findlts9}
\EndFor\label{lin:findlts10}
\State return $\langle closest\_tuple\rangle$; \label{lin:findlts11}
\EndProcedure\label{lin:findlts12}
\end{algorithmic}
%\end{multicols}
\end{algorithm}

\begin{figure} [tbph]
	\captionsetup{justification=centering}
	%\centering
	%\includegraphics[scale=.5]{figs/fig3.png}
	%\includegraphics[scale=.5]{figs/fig3.pdf_t}
	\centerline{\scalebox{0.5}{\input{figs/disc2.pdf_t}}}
	\caption{Validation by $check\_version$}
	\label{fig:mvostmm12}
\end{figure}


\cmnt{
\begin{figure} [tbph]
	%\centering
	%\includegraphics[scale=.5]{figs/fig3.png}
	%\includegraphics[scale=.5]{figs/fig3.pdf_t}
	\centerline{\scalebox{0.5}{\input{figs/mvostm12.pdf_t}}}
	\caption{Validation by $check\_version$}
	\label{fig:mvostm12}
\end{figure}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%---------------------------------Check Version -------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{algorithm}  
\scriptsize
\label{alg:checkVersion} 
\caption{$\checkv()$: This method is called by the \nptc{}. First it will find the $closest\_tuple$ $\langle j,val,mark,rvl,vnext \rangle$ created by the transaction $T_j$ with the largest timestamp smaller than $L\_t\_id$ at \Lineref{checkVersion3}. Then, it checks the version list to identify is there any higher timestamp already present in the $rvl$ of $closest\_tuple$ from \Lineref{checkVersion5} to \Lineref{checkVersion11}. If it presents then it will returns FALSE at \Lineref{checkVersion9} otherwise, TRUE at \Lineref{checkVersion13}. It will be more clear by the \figref{mvostmm12}.a) where second method $ins_1(ht, k_3, ABORT)$ of transaction $T_1$ will ABORT because higher transaction $T_2$ timestamp is already present in the $rvl$ of $closest\_tuple$ as $0^{th}$ version in \figref{mvostmm12}.b).}
		\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{356}\makeatother
\Procedure{check\_versions}{$L\_t\_id \downarrow,\currs \downarrow$} \label{lin:checkVersion1}
\cmnts{From $\currs.vls$, identify the correct $version\_tuple$ means identfy the tuple which is having higher time-stamp but less then it} \label{lin:checkVersion2}
\State $\find(L\_t\_id \downarrow, \currs \downarrow, closest\_tuple \uparrow)$;\label{lin:checkVersion3}	
\cmnts{Got the closest\_tuple as $\langle j,val,mark,rvl,vnext \rangle$}\label{lin:checkVersion4}
%\ForAll {$v\_tuples \langle j,v,rl \rangle $ in $x \cdot vl$}
\ForAll {$T_k$ in $rvl$ of $closest\_tuple.j$}\label{lin:checkVersion5}
\cmnts{$T_k$ has already read the version created by $T_j$}\label{lin:checkVersion6}
\If {$(L\_t\_id < k)$}   \label{lin:checkVersion7}
\cmnts{If in $rvl$ of $closest\_tuple.j$, any higher time-stamp exists then $L\_t\_id$ then return $FALSE$}\label{lin:checkVersion8}
\State return $\langle FALSE\rangle$;  \label{lin:checkVersion9}
\EndIf\label{lin:checkVersion10}
\EndFor\label{lin:checkVersion11}
%\EndFor;
\cmnts{If in $rvl$ of $closest\_tuple.j$, there is no higher time-stamp exists then $L\_t\_id$ then return $TRUE$}\label{lin:checkVersion12}
\State return $\langle TRUE\rangle$;\label{lin:checkVersion13}
\EndProcedure\label{lin:checkVersion14}
\end{algorithmic}
%\end{multicols}
\end{algorithm}

\begin{figure}[tbph]
	\captionsetup{justification=centering}
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centerline{\scalebox{0.47}{\input{figs/disc1.pdf_t}}}
	\caption{Method validation}
	\label{fig:mvostm9}
\end{figure}
\cmnt{
\begin{figure}[tbph]
	%\includegraphics[scale=0.7]{figs/ex1.pdf_t}
	%\centerline{\scalebox{0.7}{\input{ex1.pstex_t}}}
	\centerline{\scalebox{0.5}{\input{figs/mvostm9.pdf_t}}}
	\caption{Method validation}
	\label{fig:mvostm9}
\end{figure}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%---------------------------------methodValidation -------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[H]
\scriptsize
	\caption{\tabspace[0.2cm] methodValidation() : This method is called by the \rvmt{} and \upmt{}. It will identify the conflicts among the concurrent methods of different transactions at \Lineref{iv2}. It will be more clear by the \figref{mvostm9}, where two concurrent conflicting methods of different transactions are working on the same key $k_3$. Initially, at stage $s_1$ in \figref{mvostm9}.c) both the conflicting method optimistically (without acquiring locks) identify the same $\preds$ and $\currs$ for key $k_3$ from underlying DS in \figref{mvostm9}.a). At stage $s_2$ in \figref{mvostm9}.c), method $ins_1(k_3)$ of transaction $T_1$ acquired the lock on $\preds$ and $\currs$ and inserted the node into it (\figref{mvostm9}.b)). After successful insertion by $T_1$, $\preds$ and $\currs$ will change for $lu_2(k_3)$ at stage $s_3$ in \figref{mvostm9}.c). It will caught via method validation function at \Lineref{iv2} when $(\preds.\bn \neq G\_curr)$ for $lu_2(k_3)$. After that again it will find the new $\preds$ and $\currs$ for $lu_2(k_3)$ with the help of \nplsls{} method and eventually it will commit.}
		%\emph{DESCP}\tabspace: method validation for conflicting concurrent operations.\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $preds[]$, $currs[]$\\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $RETRY$, $OK$     }
	\label{algo:interferenceValidation}
			\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
	\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{370}\makeatother	
		\Procedure{methodValidation}{$\preds \downarrow, \currs \downarrow, L\_op\_status \uparrow$} \label{lin:iv1}
	    \cmnts{Validating $\preds$ and $\currs$}
		\If{$((\bp.marked) || (\bc.marked) ||(\bp.\bn) \neq \bc || (\rp.\rn) \neq {\rc})$}  \label{lin:iv2}
		\cmnts{If validation fail then $L\_op\_status$ set as $RETRY$}
        \State $L\_op\_status$ $\gets$ RETRY

		\Else \label{lin:iv4}
		
	    \State $L\_op\_status$ $\gets$ OK

		\EndIf \label{lin:iv6}
				\State return $\langle L\_op\_status\rangle$ \label{lin:iv5};
	
		\EndProcedure \label{lin:iv7}
	\end{algorithmic}
%\end{multicols}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%------------------- find -----------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{algorithm}[H]
\scriptsize
	\caption{\tabspace[0.2cm] $L\_find()$ : This method is called by \npins{}, \rvmt{} and \upmt{}. It will check whether any method corresponding to $\left\langle L\_obj\_id, L\_key  \right\rangle$ is present in local log from \Lineref{findll4} to \Lineref{findll8}.}
		%\emph{DESCP}\tabspace: Checks weather any operation corresponding to $\left\langle obj\_id, key  \right\rangle$ is present in ll\_list.\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $\left\langle obj\_id, key  \right\rangle$  \\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $true, false$     }
	\label{algo:findInLL}
				\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
	\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{380}\makeatother		
		\Procedure{L\_find}{$L\_t\_id \downarrow, L\_obj\_id \downarrow, L\_key \downarrow, L\_rec \uparrow$} \label{lin:findll1}
		
		%\State    /*get the tx id*/
		%\State $L\_t\_id$ $\gets$ getTS($t_i$) \label{lin:findll2};
		
		\State $L\_list$ $\gets$ \txgllist{} \label{lin:findll3}; 
	\cmnts{Every method first identify the node corresponding to the key into local log}
		\While{$(L\_rec_{i} \gets next(L\_list))$} \label{lin:findll4}
		\cmnts{Taking one by one $L\_obj\_id$ and $L\_key$ form $L\_rec$}
		\If{$((L\_rec_{i}.first = L\_obj\_id) \& (L\_rec_{i}.sec = L\_key))$} \label{lin:findll5}

		\State return $\langle TRUE, L\_rec \rangle$ \label{lin:findll6};
		\EndIf \label{lin:findll7}
		\EndWhile \label{lin:findll8}
		\State return $\langle FALSE, NULL \rangle$ \label{lin:findll9};
		\EndProcedure \label{lin:findll10}
	\end{algorithmic}
%	\end{multicols}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%------------------- releaseorderedlocks -----------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[H]
\scriptsize
	\caption{\tabspace[0.2cm] releaseOrderedLocks(): Release all locks in increasing order of their keys from \Lineref{rlock2} to \Lineref{rlock7}.}
		%\emph{DESCP}\tabspace: releases all locks taken during tryCommit\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $ordered\_ll\_list$\\
		%\emph{OUT}\tabspace \tabspace[0.37cm]:    }
	\label{algo:releaseorderedlocks}
			\setlength{\multicolsep}{0pt}
%	\begin{multicols}{2}
	\begin{algorithmic}[1]
	\makeatletter\setcounter{ALG@line}{391}\makeatother
		\Procedure{releaseOrderedLocks}{$L\_list \downarrow$} \label{lin:rlock1}
	\State    /*Releasing all the locks in increasing order of the keys */
		\While{($\textbf{$L\_rec_{i} \gets next(L\_list$})$)} \label{lin:rlock2}
		
		\State $L\_rec_{i}$.$\preds$.$\texttt{unlock()}$ \label{lin:rlock3};//$\Phi_{lp}$ 
		\State $L\_rec_{i}$.$\currs$.$\texttt{unlock()}$ \label{lin:rlock4};
		
		%\State $ll\_entry_i$.\textcolor{red}{$currs[0]$}.$\texttt{unlock()}$ \label{lin:rlock5};
		%\State $ll\_entry_i$.\textcolor{blue}{$currs[1]$}.$\texttt{unlock()}$ \label{lin:rlock6}; 
		\EndWhile \label{lin:rlock7}
		\State return $\langle void \rangle$;
		\EndProcedure \label{lin:rlock8}
	\end{algorithmic}
			
%	\end{multicols}
\end{algorithm}
%\end{multicols}

\begin{figure} [H]
	\captionsetup{justification=centering}
	%\centering
	%\includegraphics[scale=.5]{figs/fig3.png}
	%\includegraphics[scale=.5]{figs/fig3.pdf_t}
	\centerline{\scalebox{0.45}{\input{figs/disc3.pdf_t}}}
	\caption{Intra transaction validation}
	\label{fig:mvostmm11}
\end{figure}

\cmnt{
\begin{figure} [H]
	%\centering
	%\includegraphics[scale=.5]{figs/fig3.png}
	%\includegraphics[scale=.5]{figs/fig3.pdf_t}
	\centerline{\scalebox{0.5}{\input{figs/mvostm11.pdf_t}}}
	\caption{Intra transaction validation}
	\label{fig:mvostm11}
\end{figure}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%intraTransValidation%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[H]
\scriptsize
	\caption{\tabspace[0.2cm] intraTransValidation() : This method is called by \nptc{} only. If two $\upmt{s}$ within same transaction have at least one shared node among its recorded $\preds$ and $\currs$, in this case the previous $\upmt{}$ effect might be overwritten if the next $\upmt{}$ $\preds$ and $\currs$ are not updated according to the updates done by the previous $\upmt{}$. Thus to solve this we have intraTransValidation() after each $\upmt{}$ in $\nptc$. This will be more clear by the \figref{mvostmm11}, where two \upmt{s} of same transaction $T_1$ are $ins_{11}(k_3)$ and $ins_{12}(k_5)$ (\figref{mvostmm11}.c)). At stage $s_1$ in \figref{mvostmm11}.c) both the \upmt{s} identify the same $\preds$ and $\currs$ from underlying DS (\figref{mvostmm11}.a)). After the successful insertion done by first \upmt{} at stage $s_2$ in \figref{mvostmm11}.c), key $k_3$ is part of underlying DS (\figref{mvostmm11}.b)). At stage $s_3$ in \figref{mvostmm11}.c) if we will not update the $\preds$ and $\currs$ for $ins_{12}(k_5)$ then it will overwrite the previous method updates. To resolve this issue we are doing the intraTransValidation() after each \upmt{} to assign the appropriate $\preds$ and $\currs$ for the upcoming \upmt{} of same transaction.}
		%\emph{DESCP}\tabspace: program order validation\\
		%\emph{IN}\tabspace \tabspace[0.72cm]: $ll\_entry_i$  \\
		%\emph{OUT}\tabspace \tabspace[0.37cm]: $preds[], currs[]$}
	\label{algo:povalidation}
	\setlength{\multicolsep}{0pt}
%		\begin{multicols}{2}
	\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{399}\makeatother		
		\Procedure{intraTransValidation}{$L\_rec_{i} \downarrow, \preds \uparrow, \currs \uparrow$} \label{lin:threadv1}

	\State $L\_rec.getAllPreds\&Currs(L\_rec$ $\downarrow$, $\preds$ $\uparrow$, $\currs$ $\uparrow$) \label{lin:threadv2};	
				%\State \llgallpc{} \label{lin:threadv2};
				\cmnts{if $\bp$ is marked or $\bc$ is not reachable from $\bp.\bn$ then modify the next consecutive \upmt{} $\bp$ based on previous \upmt{}}
				\If{$(($$\bp$.\textup{marked}$) ||$ $($ $\bp$.\textup{\bn}$)$ != $\bc$$))$} \label{lin:threadv3}
				\cmnts{find $k$ < $i$; such that $le_k$ contains previous update method on same bucket }
				\If{$(($$L\_rec_{k}$.\textup{opn}$)$ $=$ INSERT$)$} \label{lin:threadv4}
				
				\State $L\_rec_{i}$.$\bp$.$\texttt{unlock()}$ \label{lin:thredv4-5};
				\State $\bp$ $\gets$ ($L\_rec_{k}.\bp.\bn)$ \label{lin:threadv5};
				\State $L\_rec_{i}$.$\bp$.$\texttt{lock()}$ \label{lin:thredv5-5};		
				\Else \label{lin:threadv6}
				\cmnts{\upmt{} method $\bp$ will be previous method $\bp$}
				\State $L\_rec_{i}$.$\bp$.$\texttt{unlock()}$ \label{lin:thredv6-5};
				\State $\bp$ $\gets$ ($L\_rec_{k}$.$\bp$) \label{lin:threadv7};
				
				\State $L\_rec_{i}$.$\bp$.$\texttt{lock()}$ \label{lin:thredv7-5};
				\EndIf \label{lin:threadv8}
				
				\EndIf \label{lin:threadv9}
				\cmnts{if $\rc$ \& $\rp$ is modified by prev operation then update them also}
				\If{$($$\rp$.\textup{\rn} != $\rc$$)$} \label{lin:threadv10}
				\State $L\_rec_{i}$.$\rp$.$\texttt{unlock()}$
				\State $\rp$ $\gets$ ($L\_rec_{k}$.$\rp.\rn$)  \label{lin:threadv11}; 
				\State $L\_rec_{i}$.$\rp$.$\texttt{lock()}$
				\EndIf \label{lin:threadv12}
				\State return $\langle \preds, \currs\rangle$;
	\cmnt{		


	
	
	
	        \State $L\_rec.getAllPreds\&Currs(L\_rec_{i}$ $\downarrow$, $G\_pred$ $\uparrow$, $G\_curr$ $\uparrow$) \label{lin:threadv2};	
		%\State \llgallpc{} \label{lin:threadv2};
	%\State    /*if $\bp$ is marked or $\bc$ is not reachable from $\bp.\bn$ then modify the next consecutive \upmt{} $\bp$ based on previous \upmt{}*/
		\If{$(G\_pred.knext \neq G\_curr)$} \label{lin:threadv3}
		\State    /*Find $k$ $>$ $i$; such that $L\_rec_{k}$ contains next update method on same bucket */
		\If{$((($$L\_rec_{k}$.\textup{L\_opn}$)$ $=$ INSERT$)$ $||$ $(($$L\_rec_{k}$.\textup{L\_opn}$)$ $=$ DELETE$))$} \label{lin:threadv4}
		
	\State $L\_rec_{k}$.$G\_pred$.$\texttt{unlock()}$ \label{lin:thredv4-5};
		\State $G\_pred$ $\gets$ ($L\_rec_{i}.G\_pred.knext)$ \label{lin:threadv5};
	\State $L\_rec_{k}$.$G\_pred$.$\texttt{lock()}$ \label{lin:thredv5-5};		
		%\Else \label{lin:threadv6}
	%\State    /*\upmt{} method $\bp$ will be previous method $\bp$*/
	%\State $L\_rec_{i}$.$G\_pred$.$\texttt{unlock()}$ \label{lin:thredv6-5};
	%	\State $G\_pred$ $\gets$ ($L\_rec_{i}$.$G\_pred$) \label{lin:threadv7};
		
	%		\State $L\_rec_{i}$.$G\_pred$.$\texttt{lock()}$ \label{lin:thredv7-5};
		\EndIf \label{lin:threadv8}
		
		\EndIf \label{lin:threadv9}
	\State return $\langle G\_pred, G\_curr\rangle$;
	}
	\EndProcedure	
	\end{algorithmic}
%		\end{multicols}
\end{algorithm}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%% Garbage Collection 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Garbage Collection}
\label{sec:gc}
We have performed garbage collection method to delete the unwanted version of keys i.e. if the particular version corresponding to any key is not going to use in future then we can delete that version. For the better understanding of it please consider \figref{mvostm4}. Here, we are having 3 versions of key $k_1$ with timestamp 0, 15 and 25 respectively. Each version is having 5 fields described in \secref{mvdesign}. Now, consider the version 15, there exist the next version 25 and all the transactions between 15 to 25 has been terminated (either commit or abort) then we are deleting version 15. Similarly, we can delete other versions corresponding to each key as well and optimize the memory. 

\begin{figure} [H]
	%\centering
	%\includegraphics[scale=.5]{figs/fig3.png}
	%\includegraphics[scale=.5]{figs/fig3.pdf_t}
	\centerline{\scalebox{0.35}{\input{figs/mvostm4.pdf_t}}}
	\caption{Data Structures for Garbage Collection}
	\label{fig:mvostm4}
\end{figure}

\begin{algorithm}[H] 
\scriptsize
\label{alg:begin1} 
\caption{STM $begin()$: Invoked by a thread to being a new transaction $T_i$}
	\setlength{\multicolsep}{0pt}
	%	\begin{multicols}{2}
\begin{algorithmic}[1]
%\State lock $\tcntr$;
\makeatletter\setcounter{ALG@line}{423}\makeatother
\Procedure{STM begin}{$L\_t\_id \uparrow$}
\State /*Creating a local log for each transaction*/
\State \txll $\gets$ create new \txllf;  
%\State /*Acquiring lock on live set of transaction*/
%\State $\livetx.lock()$;  
\State /*Get $t\_id$ from $\cnt$*/
\State \txll.$L\_t\_id$ $\gets$ $\cnt$;  
\State /*Incremented $\cnt$*/
\State $\cnt$ $\gets$ \gi;  
%\State add $t\_id$ to $\livetx$; 
%\State /*Release lock on live set of transaction*/
%\State $\livetx.unlock()$;
\State $\livel.lock()$; \label{lin:beginit}
\State add $L\_t\_id$ to $\livel$; 
\State $\livel.unlock()$;
\State return $\langle L\_t\_id \rangle$; 
\EndProcedure
%\State unlock $\tcntr$;
%\State return $i$; \label{lin:begfin}
%\EndFunction{$\begtrans${}}
\end{algorithmic}
%\end{multicols}
\end{algorithm}


\begin{algorithm}[H]  
\scriptsize
\label{alg:instuple}
\caption{$\instup()$: Inserts the version tuple for $(L\_t\_id,v)$ created by the transaction $T_i$ into the version list of $L\_key$}
	\setlength{\multicolsep}{0pt}
%		\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{435}\makeatother
\Procedure{ins\_tuple}{$L\_key \downarrow, L\_t\_id\downarrow, v\downarrow, NULL\downarrow, NULL\downarrow$}
\State /*Initialize $cur\_tuple$*/
\State $cur\_tuple = \langle L\_t\_id, val, F, NULL, NULL \rangle$; 
\State /* Finds the tuple with the largest timestamp smaller than i */
\State $\find(L\_t\_id \downarrow, L\_key \downarrow, prev\_tuple \uparrow)$; \label{lin:prevtup}
\State /*$prev\_tuple$ is $\langle ts, val, mark, rvl, nts\rangle$*/
\State $cur\_tuple.nts = prev\_tuple.nts$;
\State $prev\_tuple.nts = L\_t\_id$;
\State insert $cur\_tuple$ into $L\_key.vl$ in the increasing order of timestamps;  
\State /* $\lvert L\_key.vl \lvert$ denotes number of versions of $L\_key$ created and threshold is a predefined value. */
\If {($\lvert L\_key.vl \lvert > threshold$)} 
\State /*If number of created versions for $L\_key$ crossed the threshold value then calling the Garbage Collection*/ 
\State $gc(L\_key)$;
\EndIf 
\State return $\langle void \rangle$
\EndProcedure
\end{algorithmic}
%\end{multicols}
\end{algorithm}




\begin{algorithm}[H]
\scriptsize
\caption{STM $\gc()$: Unused version of a \tobj{} $L\_key$ will deleted from $L\_key.vl$}
	\setlength{\multicolsep}{0pt}
%		\begin{multicols}{2}
\begin{algorithmic}[1]
\makeatletter\setcounter{ALG@line}{451}\makeatother
\Procedure{gc}{$L\_key \downarrow$}
\State $\livel.lock()$;
\State /*\tobj{} $L\_key$ is already locked*/
\ForAll {$(cur\_tuple \in L\_key.vl)$} 
\If {$(cur\_tuple.nts == NULL)$}
\State /* If $nts$ is NULL, check the next tuple in the version list */
\State continue; 
\EndIf
\State $j = cur\_tuple.ts + 1$;
\State /*Check for all ids $j$ in the range $j < nts$*/
\While {$(j < cur\_tuple.nts)$} 
\If {$(j \in \livel)$}
\State /* If any tuples with timestamp $j$, such that  $i< j < nts$ have not terminated (means exist in $liveList$) then $cur\_tuple$ can't be deleted*/

\State break;
\EndIf
\EndWhile
\State /* If all the tuples with timestamp $j$, such that  $i< j < nts$ have terminated then $cur\_tuple$ can be deleted*/
\State delete $cur\_tuple$;
\EndFor 
\State /* $\livel$ is not unlocked when this function returns */
%\State unlock $\livel$;
\State return $\langle void \rangle$
\EndProcedure
\end{algorithmic}
%\end{multicols}
\end{algorithm}

